Dynamic Pricing Provides Robust Equilibria in Stochastic Ridesharing Networks

Ridesharing markets are complex: drivers are strategic, rider demand and driver availability are stochastic, and complex city-scale phenomena like weather induce large scale correlation across space and time. At the same time, past work has focused on a subset of these challenges. We propose a model of ridesharing networks with strategic drivers, spatiotemporal dynamics, and stochasticity. Supporting both computational tractability and better modeling flexibility than classical fluid limits, we use a two-level stochastic model that allows correlated shocks caused by weather or large public events. Using this model, we propose a novel pricing mechanism: stochastic spatiotemporal pricing (SSP). We show that the SSP mechanism is asymptotically incentive-compatible and that all (approximate) equilibria of the resulting game are asymptotically welfare-maximizing when the market is large enough. The SSP mechanism iteratively recomputes prices based on realized demand and supply, and in this sense prices dynamically. We show that this is critical: while a static variant of the SSP mechanism (whose prices vary with the market-level stochastic scenario but not individual rider and driver decisions) has a sequence of asymptotically welfare-optimal approximate equilibria, we demonstrate that it also has other equilibria producing extremely low social welfare. Thus, we argue that dynamic pricing is important for ensuring robustness in stochastic ride-sharing networks.

==> approx_eqlbm/establishing_approx_eqlbm.tex <==
\subsection{Establishing $(\bar{\bff},\bar{\bfg},\bar{\bfx})$ is an Approximate Fluid Equilibrium}
From the definition of appproximate fluid equilibrium, stated in Definition \ref{def:exact_fluid_eqlbm}, there are two properties
we need to establish: 
\begin{enumerate}
\item Approximate incentive compatibility.  Specifically, no driver should be able to deviate from their action 
and achieve more than a negligible improvement to their expected utility.
\item Compatibility of the dispatch trips and the acceptance thresholds.  The dispatch vector $\bar{\bfg}$ and the
acceptance threshold vector $\bar{\bfx}$ must be compatible with each other, in the sense that the implied volume of drivers
who receive a dispatch towards each destination does not exceed the volume of available driver supply.
\end{enumerate}

We start by establishing approximate incentive compatibility.
Let $\bar{\calQ}$ be the Q-values associated with the fluid strategy $(\bar{\bff}, \bar{\bfg}, \bar{\bfx})$. Recall the Q-values
specify the expected utility to go values of the different actions drivers take under the specified strategy.  For relocation
trip actions $(\ell,d,0)$ the Q-value is defined by
\begin{equation}
    \bar{\calQ}(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), d\right)\right],
\end{equation}
where $\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), d\right)$ is the fluid utility-to-go for drivers positioned at $d$,
under the time $t+1$ scenario $\omega_{t+1}$ and the supply-location vector $\bar{\bfS}_{\omega_{t+1}}( \bar{\bff})$.
For relocation trip actions $(\ell,d,1)$ the Q-value is defined by 
\begin{equation}
    \bar{\calQ}(\ell,d,1, X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}
where $X\in [0,\bar{x}_{(\ell,d)}]$ is any add-passenger disutility value smaller than the common acceptance threshold $\bar{x}_{(\ell,d)}$,
and $P_{(\ell,d)}$ is the price set by the platform for trips from $\ell$ to $d$.

A key challenge we need to address for establishing approximate incentive compatibility is to bound the difference between
the value of future locations in the fluid model and in the two-level model.  In the fluid model, the expected value of
being positioned at a destination location $\ell$ is given by 
$$
\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), \ell\right),
$$
where $\bar{\bfS}_{\omega_{t+1}}( \bar{\bff})$ is the expected supply-location vector at time $t+1$ given the time $t$ trips $\bar{\bff}$ and the
time $t+1$ scenario $\omega_{t+1}$, and Lemma \mccomment{ref} establishes the equivalence between utility-to-go in the fluid model and
partial derivatives of the fluid optimization function:
\begin{equation}
\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), \ell\right) = \frac{\partial}{\partial S_\ell} \Phi_{\omega_{t+1}}(\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})).
\end{equation}
  Notice that $\bar{\bfS}_{\omega_{t+1}}( \bar{\bff})$ is deterministic given the scenario $\omega_{t+1}$ and
trips $\bar{\bff}$: indeed, the $\ell$th component $\bar{S}_{\omega_{t+1},\ell}$ is specified by
\begin{equation}
\bar{S}_{\omega_{t+1},\ell} = \bar{M}_{\omega_{t+1},\ell} + \sum_{o\in\calL}\bar{f}_{(o,\ell)},
\end{equation}
where $\bar{M}_{\omega_{t+1},\ell}$ is the expected volume of drivers who join the market positioned at location $\ell$ under the scenario $\omega_{t+1}$.

In contrast, a driver's value of being at a particular location $\ell$ at the next time period in the two-level model is
given by
$$
\bbE\left[U_i^{t+1}\mid (\omega_{t+1},\bfS_{\omega_{t+1}}(\bff)), \ell_i=\ell\right],
$$
which depends on the scenario $\omega_{t+1}$ as well as the microscopic randomness that governs the realized volume of trips in time period
$t$ (i.e. the randomness inherent to $\bff$) as well as the microscopic randomness that governs the volume of drivers who join at each
location in the next time period. Both of these sources of randomness are captured by the random supply-location vector $\bfS_{\omega_{t+1}}(\bff)$, where 
each component $S_{\omega_{t+1},\ell}$ is defined by
\begin{equation}
S_{\omega_{t+1},\ell} = M_{\omega_{t+1},\ell} + \sum_{o\in\calL}f_{(o,\ell)}.
\end{equation}
Our backwards induction assumption \ref{assn:backwards_induction} states that the value for being positioned at $\ell$ is approximately
equal to the partial derivative of the fluid optimization function, i.e. if $(\omega_{t+1}, \bfS_{t+1})\in\calS_{t+1}$ is a good time $t+1$ state
then the following holds with probability $1$:
\mccomment{I am going to change notation from $\bbE\left[U_i^{t+1}\mid (\omega_{t+1},\bfS_{\omega_{t+1}}), \ell_i=\ell\right]$ to 
$\bbE\left[U_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff),\ell)\right]$ for expected time $t+1$ utility of being positioned at $\ell$, under $\omega_{t+1}$,
in the two level model}
\begin{equation}
\left|U_{\omega_{t+1}}(\bfS_{\omega_{t+1}}) - \frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{t+1})\right|\leq \epsilon_{t+1},
\end{equation}
where $\epsilon_{t+1}$ is an error term coming from Assumption \ref{assn:backwards_induction}.
Taking expectations,  we obtain the bound
\begin{align*}
\bbE\left[\left|U_{\omega_{t+1}}(\bfS_{\omega_{t+1}}) - \frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{t+1})\right|\right]
& \leq \epsilon_{t+1} q_{t+1} + C_{t+1}(1- q_{t+1}),
\end{align*}
where $C_{t+1}$ is a uniform upper bound on the time $t+1$ utility, and $q_{t+1}$ is defined by 
$$
q_{t+1} = \bbP\left((\omega_{t+1},\bfS_{t+1})\notin \calS_{t+1}\mid (\omega_t,\bfS_t)\right),
$$
which corresponds to the probability of landing in a good time $t+1$ state given the current state $(\omega_t,\bfS_t)$.

This almost puts the expected time $t+1$ value from the two-level model on the same footing as the expected time $t+1$ value from the fluid model.  
Indeed, for any location $\ell$ we have the following:
\begin{align*}
& \bbE\left[ \left|U_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff),\ell) - \calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), \ell\right)\right|\right] \\
=\ \  & \bbE\left[ \left|U_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff),\ell) - \frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff})\right) \right|\right]\\
\leq\ \  & \epsilon_{t+1} q_{t+1} + C_{t+1}(1-q_{t+1}) + 
\bbE\left[\left|\frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
\frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}\right)\right|\mid (\omega_{t+1},\bfS_{t+1})\in\calS_{t+1}\right].
\end{align*}


==> approx_eqlbm/good_state_discussion.tex <==

\subsection{Discussion of ``Good'' States $\calS_t$ and Desired Concentration Properties}
The current definition of approximate equilibrium in the two level model is parameterized by a sequence of probabilities $p_1,\dots,p_T$,
and a corresponding set of ``good'' states $\calS_t$, where $p_t$ is the probability of the time $t$ state being ``good'', and the approximate-incentive
compatibility guarantees only hold when the state is good.

The problem is: we can't provide incentive guarantees at locations where the volume of drivers is very small. When the volume of drivers is very small,
the variance for the actions that the drivers take is large, which means we can't accurately approximate the two-level model dynamics with the
fluid model dynamics.

I'm not sure what exactly is the right definition for the set of good states $\calS_t$.

One potential definition of $\calS_t$ is that it contains states $(\omega_t,\bfS_t)$ where each component of the supply-location
vector $\bfS_t$ is either $0$ or strictly bounded away from $0$, i.e. choose a constant $C_t>0$
$$
\calS_t = \left\{(\omega_t,\bfS_t)\in\Omega_t\times\bbR^\calL_+ : (\bfS_t)_\ell = 0\mbox{ or }(\bfS_t)_\ell \geq C_t\right\}.
$$

Another option is that we do away with the explicit set of good states, and instead we somehow ``ignore'' locations where the volume
of drivers is too small. 

And maybe the proper way of ignoring these low-volume locations is to go back to allowing an $\epsilon$ fraction of drivers to take arbitrarily
bad actions.

But I digress, and I'm not thinking clearly about the problem right now.
The reason we need these concentration properties is the following. Let $(\bff,\bfg)$ be the (stochastic) trip volumes
that arise from some state $(\omega_t,\bfS_t)$. 

We can think of the dispatch trips as a collection of $|\calL|$ different dispatch trip vectors $\bfg=(\bfg_\ell : \ell\in\calL)$,
where each $\bfg_\ell = (g_{(\ell,d)} : d\in\calL)$ specifies the dispatch trips originating from $\bfg$.  
Each vector $\bfg_\ell$ comes from the matching process that runs for location $\ell$.

The relocation trips, which correspond to $\bff - \bfg$, comes from driver's relocation decisions.
It might also be useful to think of $\bff$ as a collection of vectors $\bff_\ell$ for $\ell\in\calL$ where $\bff_\ell=(f_{(\ell,d)} : d\in\calL)$
corresponds to total trip volumes originating from $\ell$.

When we try to establish that $\bar{\bff},\bar{\bfg}, \bar{\bfx}$ is an approximate equilibrium, we need to compare the following two
quantities:
$$
\bbE\left[\calU_{\omega_{t+1}}(\ell,\bfS_{\omega_{t+1}}(\bff))\right],
$$
which is the expected utility-to-go from location $\ell$ with respect to scenario $\omega_{t+1}$ and the (stochastic!) supply-location vector
$\bfS_{\omega_{t+1}}(\bff)$.

\textbf{Important Point 1:} We need $\bfS_{\omega_{t+1}}(\bff)$ to be a ``good state'' in order to apply the induction hypothesis
$$
\bbE\left[\calU_{\omega_{t+1}}(\ell,\bfS_{\omega_{t+1}}(\bff))\right]
\approx \bbE\left[\frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))\right].
$$

\textbf{Important Point 2:} In order to conclude the expected partial derivative of $\Phi_{\omega_{t+1}}(\cdot)$ with respect to the stochastic supply location
vector $\bfS_{\omega_{t+1}}(\bff)$ is close to the partial derivative w.r.t. the expected supply location vector $\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})$, i.e.
in order to have
\begin{equation}
    \label{eq:desired_approximation}
\bbE\left[\frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))\right] \approx 
\bbE\left[\frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bar{\bfS}_{\omega_{t+1}}(\bar{\bff}))\right],
\end{equation}
where the expectation on the left is over $\bfS_{\omega_{t+1}}(\bff)$ as well as the scenario $\omega_{t+1}$ and the expectation on the right is only over the
scenario $\omega_{t+1}$,
we need $\bfS_{\omega_{t+1}}(\bff)$ to be close to its mean, $\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})$ with high probability.
The reason we want this property to hold is so that we can derive approximate incentive-compatibility of $\bar{\bff},\bar{\bfg}$ in the fluid model
from approximate incentive-compatibility conditions on $\Pi$ in the two-level model.

\textbf{Question:} Can we reframe the incentive-compatibility conditions in the two-level model so that achieving the approximation (\ref{eq:desired_approximation}) is simpler?
E.g. if the incentive-compatibility conditions held (with high probability) for each realization of $(\bff,\bfg)$ then we could show that each realization $(\bff,\bfg,\bfx)$
is an approximate equilibrium, and not have to worry about explicitly establishing (\ref{eq:desired_approximation}).  But this feels like a much stronger assumption than
assuming that incentive-compatibility only need hold in expectation.

\textbf{Followup Question:} Actually, does high-probability incentive compatibility follow from the expected incentive-compatibility definition we currently have?  

Observe the components for each $\ell$ are equal to
$$
\left(\bfS_{\omega_{t+1}}(\bff)\right)_\ell = M_{\omega_{t+1},\ell} + \sum_{o\in\calL} f_{(o,\ell)},\ \ \ \ \ \ \ \ 
\left(\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})\right)_\ell = \bar{M}_{\omega_{t+1},\ell} + \sum_{o\in\calL} \bar{f}_{(o,\ell)}.
$$

By assumption we have that $M_{\omega_{t+1},\ell}$ (which corresponds to stochastic volume of new drivers at $\ell$ under $\omega_{t+1}$)
is close to its mean $\bar{M}_{\omega_{t+1},\ell}$ with high probability when $k$ is large. 
So in order for $\bfS_{\omega_{t+1}}(\bff)$ to be close to $\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})$ we need $\bff$ to be close to $\bar{\bff}$.

\subsubsection{How do we characterize the concentration of $\bff$ towards $\bar{\bff}$?}

It makes sense to think about concentration of dispatch trips $\bfg$ and relocation trips $\bff-\bfg$ separately.
Relocation trips are the easier case: since drivers essentially all use the same acceptance threshold in an equilibrium,
the driver labels of drivers who take relocation trips are essentially uniform across all drivers at the same origin location.

The concentration of $\bfg$ towards $\bar{\bfg}$ depends on the matching process.  Concentration properties of the matching process can
be established through something like hoeffding's inequality for sampling without replacement.  The problem is, concentration depends on 
the total number of ``trials'' in the balls-and-bins description of the process, i.e. the total number of drivers at that location.

But our saving grace might be that we don't need per-location concentration!  

\textbf{Important Point 3:} As long as $\|\bfS_{\omega_{t+1}}(\bff) - \bar{\bfS}_{\omega_{t+1}}(\bar{\bff})\|_1$
is small with high probability, we don't care if the (relative) error in one or two locations is large.

At least, this saving grace helps us deal with the $\calS_t$ definition problem: we could just set $\calS_t$ to include $(\omega_t,\bfS_t)$ 
where $\|\bfS_t\|_1$ is larger than a constant.

Concentration of $\bfg$ also depends on $\bar{\bfr}$, which is the expected dispatch request volume under the prices set by the platform, and 
$\bfx$, the threshold vector used by the drivers.

I think/hope a similar phenomenon will work here: If $\bar{\bfr}$ and $\bfx$ are too small, then we don't get (relative) concentration, but the
overall error to $\|\bff - \bar{\bff}\|_1$ should be small.

For tomorrow: try to work out, at a high level, bounds on $\|\bfS_t\|_1$, $\bar{\bfr}$, $\bfx$, assuming some functional form for the concentration
of $\bfg$ towards $\bar{\bfg}$.

It is now tomorrow: I'm returning to properties about the matching process, and thinking about its concentration properties at a high level.
Concenetration properties of the matching process are discussed below.  This text is also included in Section \ref{subsubsec:matching_concentration}.
\subsubsection*{Matching Process Concentration}
\input{approx_eqlbm/matching_process_concentration.tex}



==> approx_eqlbm/lemmas.tex <==
\subsection{Additional Lemmas}
Our next Lemma states a useful generic property about the gap between $\bbE[F(X)]$ and $F(\bbE[X])$, for a continuous
function $F$ and a random variable $X$.
\begin{lemma}
\label{lem:expected_value_lipschitz_bound}
    Suppose $F$ is a Lipschitz continuous function taking values between $0$ and $C$ with Lipschitz constant $L$,
    and suppose $X$ is a random variable which satisfies the property $\bbP(|X - \bbE[X]| \leq \epsilon_0) \geq 1-\epsilon_1$,
    for error parameters $\epsilon_0$ and $\epsilon_1$. Then
    \begin{equation}
        \bbE\left[F(X)\right] - F(\bbE[X]) \leq L\epsilon_0 + C\epsilon_1.
    \end{equation}
\end{lemma}


==> approx_eqlbm/main_section_text.tex <==


Our main result in this paper concerns the welfare achieved by approximate-equilibrium strategy profiles.
Before stating the result, let us revisit welfare in our model and describe expected welfare as a function of the strategy profile.

Let $W_i^t$ denote the welfare generated in the action driver by $i$ at time $t$.  The welfare $W_i^t$
differs from the driver reward $R_i^t$ when driver $i$ fulfils a dispatch in time $t$; in this case, the rider collects utility
equal to the difference between their value for the trip and the trip price.  Let $V_i^t$ be the value held by the rider whose dispatch
driver $i$ fulfils in time $t$, if any such rider exists.  The welfare term $W_i^t$ is defined as follows:
\begin{equation}
    W_i^t=\begin{cases}
    R_i^t + (V_i^t - P_{(\ell,d)}^t) & \mbox{if }a_i^t=(\ell,d,1),\\
        R_i^t & \mbox{otherwise.}
    \end{cases}
\end{equation}

The total welfare generated by the marketplace is then the sum over welfare terms $W_i^t$ for all drivers $i$ and time periods $t$.
In the context of the two-level model, where the number of riders and drivers scales with the population-size parameter $k$, we
normalize the expected welfare by dividing by $k$, so that expected welfare terms are comparable across different population sizes.

Let $W_{\omega_t}(\bfS_t;\Pi)$ be the expected welfare-to-go given a strategy profile $\Pi$, a population size $k$, as a function
of the market state $(\omega_t,\bfS_t)$:
\begin{equation}
    W_{\omega_t}(\bfS_t;\Pi) = \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM}\sum_{\tau=t}^T W_i^\tau \mid (\omega_t,\bfS_t)\right].
\end{equation}
Notice the expected welfare term $ \Phi_{\omega_t}(\bfS_t;\Pi) $ implicitly depends on the population size parameter $k$, but we
omit this dependence from the notation for convenience.

Recall that $\Phi_{\omega_t}(\bfS_t)$ denotes the optimal value of the state-dependent optimization problem given the state $(\omega_t,\bfS_t)$,
which corresponds to the optimal welfare achievable given the state $(\omega_t,\bfS_t)$ in the stochastic fluid model.
The following Lemma states that the optimal fluid welfare is always an upper bound on the expected welfare in the two-level model.
\begin{lemma}
    Let $\Pi$ be any strategy profile and consider any time $t$ with state $(\omega_t,\bfS_t)$.
    The optimal welfare from the state $(\omega_t,\bfS_t)$ in the fluid model is always larger than the expected welfare generated by $\Pi$ in the
    two-level model, i.e.
    \begin{equation}
        \label{eq:fluid_welfare_ub}
    \Phi_{\omega_t}(\bfS_t) \geq W_{\omega_t}(\bfS_t;\Pi)
    \end{equation}
    always holds.
\end{lemma}

Our main result in this subsection is to show that the bound (\ref{eq:fluid_welfare_ub}) is nearly tight whenever $\Pi$ is an approximate
equilibrium.
\begin{theorem}
    \label{thm:two_level_robustness}
    Let $\Pi$ be an $(p_{1:T}, \epsilon_{1:T})$-approximate equilibrium.
    Let $\calS_t$ be the set of good time $t$ states with respect to the error term $\epsilon_t$.
    Assume that the probability terms satisfy the bound $$\bbP((\omega_t,\bfS_t)\in\calS_t) \geq p_t \geq 1- \dots,$$
    and assume the error terms satisfy the bound $$\epsilon_t\leq \dots$$
    Then for each $t$ there exists an error term $\gamma_t = \dots$ such that
    \begin{equation}
    W_{\omega_t}(\bfS_t;\Pi) \geq \Phi_{\omega_t}(\bfS_t) - \gamma_t
    \end{equation}
    holds for all good states $(\omega_t,\bfS_t)\in\calS_t$. \mccomment{The statement of this theorem might need to change because there are low-probability
    states $(\omega_t,\bfS_t)$ for which it is hard to provide a bound}
\end{theorem}

%\input{approx_eqlbm/good_state_discussion.tex}

\subsection{Proof of Theorem \ref{thm:two_level_robustness}}

We prove Theorem \ref{thm:two_level_robustness} by backwards induction on the time period. Our backwards induction assumption
states that the utility-to-go of drivers at a location $\ell$ is (approximately) equal to the partial derivative of the
state-dependent optimization function, with respect to the volume of drivers at $\ell$.
Specifically, we consider an arbitrary time period $t$, and a good time $t$ state $(\omega_t,\bfS_t)\in\calS_t$.
\mccomment{Fill in details about what we mean by ``good'' states $\calS_t$, and give precise definitions for $\calS_t$}
We assume, via backwards induction, that the following properties have already been established for the future time
period $t+1$.

\begin{assumption}
    \label{assn:backwards_induction}
    Assume the time period $t$ is smaller than the final time period $T$ (otherwise there is no assumption needed).
    For any future market state $(\omega_{t+1},\bfS_{t+1})$ satisfying the condition \mccomment{insert condition on $\sum_\ell S_\ell \leq C$, if necessary}, 
    assume that the conclusion of Theorem \ref{thm:two_level_robustness}
    holds with respect to the error term $\gamma_{t+1}=\dots$, that is
    $$
    W_{\omega_{t+1}}(\bfS_{t+1};\Pi) \geq \Phi_{\omega_{t+1}}(\bfS_{t+1}) - \gamma_{t+1}.
    $$
    Additionally, for each location $\ell$
    assume that the utility-to-go of each driver positioned at $\ell$ is within $\epsilon$ of the
    partial derivative of the state dependent optimization function for the location $\ell$. That is,
    \begin{equation}
    \left|U_i^{t+1} - \frac{\partial}{\partial S_\ell} \Phi_{\omega_{t+1}}(\bfS_{t+1})\right| \leq \epsilon
    \end{equation}
    where $i\in\calM_{\ell,t+1}$ is any driver positioned at $\ell$, and the error term $\epsilon$
    satisfies $$\epsilon\leq\dots$$
\end{assumption}


Our path to proving the inductive step for Theorem \ref{thm:two_level_robustness} will be to construct a deterministic
solution $(\bar{\bff},\bar{\bfg})$ for the fluid optimization problem which approximately corresponds to the actions specified by $\Pi$.
Our first step is to establish that, for an approximate equilibrium strategy profile $\Pi$, at the cost of a small error term we can assume
that all drivers use the same acceptance thresholds.
\begin{lemma}
    \label{lem:common_threshold}
    Let $\bfx_i=(x_i^d : d\in\calL)$ be the disutility acceptance threshold used by each driver $i$ in time period $t$ under
    the strategy profile $\Pi$. Then for each location $\ell$ there exists a disutility threshold vector 
    $\bfx_\ell = (x_{(\ell,d)} : d\in\calL)$ and an error term $\epsilon$ \mccomment{TODO: fill in $\epsilon_\ell$ details} 
    such that every driver positioned at $\ell$ uses a disutility threshold that is at most $\epsilon$ distance from
    $\bfx_\ell$, i.e.
    \begin{equation}
        \max_{d\in\calL}|x_i^d - x_{(\ell,d)}|_ \leq \epsilon , \ \ \ \ \forall i\in\calM_{t,\ell}.
    \end{equation}
    The error term $\epsilon$ is equal to
    \begin{equation}
    \epsilon = 2\delta + 4\epsilon^{BI} + \frac{CL}{k},
    \end{equation}
    where $\delta$ is the approximation error in the strategy profile $\Pi$, $\epsilon^{BI}$ is the error term from
    the backwards induction assumption Assumption \ref{assn:backwards_induction}\mccomment{$\epsilon^{BI}$ is an error term
    that needs to work for every $\bfS_{t+1}$}, $C$ is a constant, $L$ is the lipschitz
    constant for the state-dependent optimization problem partial derivative, and $k$ is the population-size parameter.
\end{lemma}

We defer the proof of Lemma \ref{lem:common_threshold} to Section \ref{subsec:common_threshold_proof}.
The important takeaway from Lemma \ref{lem:common_threshold} is that, since $\Pi$ is an approximate equilibrium,
we can find an acceptance-threshold vector $\bar{\bfx}$ such that whenever a driver $i$ is allocated a dispatch from $\ell$ to $d$,
the acceptance threshold $x_i^d$ on which driver $i$ bases their decision to accept or reject the dispatch is within
$\epsilon$ of $\bar{x}_{(\ell,d)}$.


Let $\bar{\bfx}$ be the common disutility threshold vector established in Lemma \ref{lem:common_threshold},
    and let $\tilde{\Pi}$ be the same as the strategy profile $\Pi$, with the modification that all drivers use exactly the
    threshold $\bar{\bfx}$.

\begin{lemma}
    \label{lem:exact_common_threshold}
    $\tilde{\Pi}$ remains an approximate equilibrium, and the welfare under $\tilde{\Pi}$ is approximately the
    same as the welfare under $\Pi$:
    \begin{equation}
    W_{\omega_t}(\bfS_t;\tilde{\Pi}) \geq W_{\omega_t}(\bfS_t;\Pi) - \epsilon.
    \end{equation}
    \mccomment{TODO: fill in details and write proof}
\end{lemma}

Now, we construct the deterministic flow vectors $(\bar{\bff},\bar{\bfg})$ by considering the output of the fluid matching process
with respect to the disutility thresholds $\bar{\bfx}$ and the relocation distribution used by the drivers under the strategy profile $\tilde{\Pi}$.
For each origin location $\ell$, the relocation distribution is a vector $\bfh_\ell\in\Delta(\calL)$, where the probability $h_{(\ell,d)}$ of taking a relocation
trip from $\ell$ towards a destination $d$ is given by
$$
h_{(\ell,d)} = \frac{1}{|\calM_{t,\ell}|}\sum_{i\in\calM_{t,\ell}} \bfone\{r_i=d\},
$$
where $r_i\in \calL$ is the relocation destination selected by driver $i$.


For each pair of locations $(\ell,d)$ let $\bar{g}_{(\ell,d)}$ be volume of dispatches that get served from $\ell$ to $d$,
and let $\bar{f}_{(\ell,d)}$ be the total trip volume from $\ell$ to $d$,
under the fluid matching process with respect to the acceptance thresholds $\bar{\bfx}$ and the relocation probability $h_{(\ell,d)}$.
Recall the fluid matching process
is described in Section \ref{subsec:fluid_matching_process}. The fluid dispatch volumes $\bar{\bfg}$ are defined in equation (\ref{eq:fluid_dispatch_volume})
and the fluid total trip volumes $\bar{\bff}$ are defined in equation (\ref{eq:fluid_total_trip_volume}).

We now show that the trips specified by $(\bar{\bff},\bar{\bfg})$ constitute an approximate equilibrium for the fluid model.
Let $\bar{\calQ}$ denote the Q-values associated with the trips specified by $(\bar{\bff},\bar{\bfg})$ and the acceptance thresholds $\bar{\bfx}$.
For relocation
trip actions $(\ell,d,0)$ the Q-value is defined by
\begin{equation}
    \bar{\calQ}(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), d\right)\right],
\end{equation}
where $\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), d\right)$ is the fluid utility-to-go for drivers positioned at $d$,
under the time $t+1$ scenario $\omega_{t+1}$ and the supply-location vector $\bar{\bfS}_{\omega_{t+1}}( \bar{\bff})$.
For relocation trip actions $(\ell,d,1)$ the Q-value is defined by 
\begin{equation}
    \bar{\calQ}(\ell,d,1, X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}
where $X\in [0,\bar{x}_{(\ell,d)}]$ is any add-passenger disutility value smaller than the common acceptance threshold $\bar{x}_{(\ell,d)}$,
and $P_{(\ell,d)}$ is the price set by the platform for trips from $\ell$ to $d$.
Assume that drivers play according to an equilibrium at all future time periods, so we have the equality
\begin{equation}
\calV_{\omega_{t+1}}\left(\bar{\bfS}_{\omega_{t+1}}( \bar{\bff}), \ell\right) = \frac{\partial}{\partial S_\ell} \Phi_{\omega_{t+1}}(\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})).
\end{equation}

We show that $(\bar{\bff},\bar{\bfg},\bar{\bfx})$ constitutes an approximate equilibrium for the fluid model by relating the
incentive compatibility conditions on $\Pi$ to the Q-values defined above.

Let $(\bff,\bfg)$ encode the stochastic trips that occur under $\tilde{\Pi}$ in the two-level model. 
Recall that $a_i^t$ is a random variable which corresponds to the action that each active driver $i\in\calM_t$ takes
in time period $t$.
Define $g_{(\ell,d)}$ by 
\begin{equation}
    \label{eq:two_level_g}
     g_{(\ell,d)} = \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,1)\right\},\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
and $f_{(\ell,d)}$ by
\begin{equation}
    \label{eq:two_level_f}
    f_{(\ell,d)} = g_{(\ell,d)} + \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,0)\right\}.\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
Note that $(\bff,\bfg)$
are random variables that depend on stochastic dispatch demand, stochastic add-passenger disutilities, as well as the randomness inherent
to the matching process.  

\begin{lemma}
    As the population-size parameter $k$ increases, the probability that the stochastic trip volumes $(\bff,\bfg)$ are significantly
    different from the fluid trip volumes $(\bar{\bff},\bar{\bfg})$ approaches $0$. That is, there is an error function $\epsilon(k)=o(k)$
    and a probability function $q(k)=o(k)$ such that the following is true:
    \begin{equation}
        \bbP\left(\|\bfg - \bar{\bfg}\|_1 + \|\bff - \bar{\bff}\|_1 \geq \epsilon(k)\right) \leq q(k).
    \end{equation}
\end{lemma}

\begin{lemma}
    $(\bar{\bff},\bar{\bfg},\bar{\bfx})$ is an approximate equilibrium. This means that, except for a negligible $o(k)$ fraction of drivers, the most
    utility that a driver can gain by deviating from $(\bar{\bff},\bar{\bfg},\bar{\bfx})$ is at most $o(k)$.
\end{lemma}





==> approx_eqlbm/matching_process.tex <==
We now describe the matching process that the platform uses to allocate dispatch requests to drivers.
Let $\calR_t$ be an index set of riders who request a dispatch in the current time period.
For each rider $j\in\calR_t$ let $(\ell_j,d_j)\in\calL^2$ denote the origin and destination associated with rider $j$'s
dispatch request.  The volume of riders who request a trip for each route $(\ell,d)$ is stochastic and depends on the price $P_{(\ell,d)}$ 
that the SSPM mechanism sets along that route.  Our assumptions regarding stochastic rider dispatch requests are summarized in Section
\mccomment{insert reference}.

The matching process refers to our mathematical model for how dispatch requests are allocated to drivers.
Since our ridesharing model assumes that dispatch requests can only be served by drivers already positioned at
the origin location, our matching model operates independently for each location $\ell$.
Let $\calR_{t,\ell}\subseteq \calR$ be the set of riders whose origin location is $\ell$, and let
$\calM_{t,\ell}\subseteq\calM_t$ be the set of drivers who are positioned at $\ell$.

\mccomment{Here is one possible definition for how the matching process can work}
We assume the matching process operates by taking the following steps for each location $\ell$.
Let $N_\ell = |\calM_{t,\ell}|$ be the number of active drivers at $\ell$.  Define $\calM_1 = \calM_{t,\ell}$,
define $\calR_1 = \calR_{t,\ell}$, and for each $n=1,2,\dots,N$, take the following steps:
\begin{enumerate}
\item Independently sample a driver $i_n\sim \mathrm{Uniform}(\calM_n)$.
\item If $\calR_n$ is not empty, i.e. if there are riders that remain to be dispatched, independently sample a rider $j_n\sim \mathrm{Uniform}(\calR_n)$.
If $\calR_n$ is empty, go to step \ref{item:R_n_empty}.
\item Try to match rider $j_n$ to driver $i_n$.  Let $\delta_n\in\{0,1\}$ indicate the result of the match ($\delta_n=1$ indicates
the match was accepted, $\delta_n=0$ indicates the match was rejected).
\begin{itemize}
\item The driver $i_n$ makes a decision about whether or not to accept the match based on their add-passenger disutility $X_{i_n}$
and the destination $d_{j_n}$ requested by the rider $j_n$.
\item Recall driver $i_n$ uses a policy $\pi_{i_n}$ that produces a vector of thresholds $(x^{i_n}_{d} : d\in\calL)$ for each location $d$.
\item Driver $i_n$ accepts the dispatch if $X_{i_n}\leq x^{i_n}_{d_{j_n}}$.
\end{itemize}
\item \label{item:R_n_empty} If $\calR_n$ is empty, i.e. if there are no more riders requesting a dispatch, set $j_n=\emptyset$ to be the
``empty rider'' and indicate that driver $i_n$ did not get a dispatch by setting $\delta_n=0$. 
\item Remove driver $i_n$ from the list of drivers. Set $\calM_{n+1}\coloneqq \calM_n \setminus \{i_n\}$.
\item If the dispatch is accepted, i.e. if $\delta_n=1$, remove $j_n$ from the list of drivers by setting $\calR_{n+1}\coloneqq \calR_n \setminus \{j_n\}$.
If the dispatch is not accepted, i.e. if $\delta_n=0$, set $\calR_{n+1}\coloneqq\calR_n$.
\end{enumerate}

The above procedure produces a sequence of matches $M=((i_n,j_n,\delta_n):n=1,2,\dots,|\calM_{t,\ell}|)$ which has exactly one entry 
for each driver positioned at $\ell$.
Notice that the trip taken by each driver $i\in\calM_{t,\ell}$ is fully determined by the information in $M$.  Indeed, for each driver $i$,
we have
\begin{equation}
a_i^t = \begin{cases}
(\ell,d_{j_{n(i)}},1) & \mbox{if }\delta_{n(i)}=1,\\
(\ell,r_i,0) & \mbox{else}.
\end{cases}
\end{equation}
In the above, we use
 $n(i)\in \{1,2,\dots,|\calM_{t,\ell}|\}$ to be the position in the sequence $M$ of each driver $i\in\calM_{t,\ell}$,
and $r_i\in\calL$ is driver $i$'s relocation destination if they do not accept a match ($r_i$ is determined by driver $i$'s policy $\pi_i$).

An important property about the matching process as we've defined it is that the action of any one driver
does not have a significant effect on the global distribution of actions taken by other drivers.
Let us introduce some notation to formally state this property.  
Let $\calA_\ell = \{(\ell,d,0) : d\in\calL\}\cup\{(\ell,d,1) : d\in\calL\}$ be the set of all possible trips that a
driver positioned at $\ell$ can take, and let $\bfh=(h_a : a\in\calA_\ell)$ be a vector counting the volume of drivers who take each
trip type:
\begin{equation}
h_a = \frac{1}{k}\sum_{i\in\calM_{\ell,t}} \bfone\{a_i^t=a\}.
\end{equation}
Since $\bfh$ is a deterministic function of the realized actions $\{a_i^t : i\in\calM_{\ell,t}$, and since the realized actions are a deterministic function
of the matching sequence $M$, we can think of the vector $\bfh$ as a deterministic function of the matching sequence $M$.
We write 
\begin{equation}
\bfh(M)\equiv \mbox{trip-volume vector arising from the matching sequence }M.
\end{equation}
We refer to $\bfh=\bfh(M)$ as the matching vector.

\Xomit{
The important property we alluded to above states that the distribution of $\bfh$ does not change very much if we condition on any one match
being contained in $M$.
Suppose we want to condition on observing a matching sequence $M$ if we know that a particular rider $j\in\calR_{t,\ell}$ was matched to a particular driver $i\in\calM_{t,\ell}$
and we know the driver's response to the match $\delta\in\{0,1\}$.  By ``condition on observing the match'' we mean to condition on the event that the tuple $(i,j,\delta)$
is contained in the sequence $M$, i.e. $(i,j,\delta)\in M$.

Let $\calP_\ell$ denote the distribution over matching sequences $M$ without any additional information, and let $\calP(\cdot\mid (i,j,\delta)\in\calM)$ denote
the distribution over matching sequences $M$ which contain the match $(i,j,\delta)$.

\begin{lemma}
\label{lem:matching_coupling}
Fix a location $\ell$, let $\calM_{t,\ell}$ denote the set of drivers positioned at $\ell$, and let $\calR_{t,\ell}$ denote the set of riders who request
a rider originating from $\ell$. Let $(i,j,\delta)$ be any match specifying a driver $i$, a rider $j$, and an outcome $\delta$. Then there exists a coupling $(\bfh_1,\bfh_2)$ with the
following properties:
\begin{enumerate}
\item The marginal distribution of $\bfh_1$ is the same as $\bfh(M)$ where $M\sim \calP$.
\item The marginal distribution of $\bfh_2$ is the same as $\bfh(M)$ where $M\sim \calP(\cdot|(i,j,\delta)\in M)$.
\item With probability $1$, the difference between $\bfh_1$ and $\bfh_2$ is at most $\frac{2}{k}$, i.e. $\bbP(\|\bfh_1-\bfh_2\|\leq \frac{2}{k})=1$.
\mccomment{$\frac{2}{k}$ bound may not be correct}.
\end{enumerate}
\end{lemma}

\subsubsection{Brainstorming how to obtain the coupling}
It is not immediately clear to me how to construct the coupling claimed to exist by Lemma \ref{lem:matching_coupling}.
At a high level, what we'd like is to find a function $F(\cdot)$ which takes arbitraty matching sequences $M$ as input,
produces new matching sequences $M'=F(M)$ which satisfy $(i,j,\delta)\in M'$ as output, and such that the distribution of 
vectors $\bfh(M')$, where $M'\sim F(M)$ and $M\sim \calP$,
is the same as the distribution $\bfh(M')$ where $M'\sim \calP(\cdot|(i,j,\delta)\in M)$.

\subsubsection{The ``swap'' idea}
In this section we'll construct one transformation $F$, that takes arbitrary matching sequences $M$ and produces new matching
sequences $M'=F(M)$ which satisfy our desired condition.
Let $(i_0,j_0,\delta_0)$ denote the match we want to condition on, so the new matching sequences $M'$ should always satisfy $(i_0,j_0,\delta_0)\in M'$.
}

\subsubsection{A balls-in-a-bag description of the matching process}
Here is an alternative description of the distribution for the matching vector $\bfh$, in terms of a more general sampling-balls-from-a-bag problem description.
Consider a bag with $R$ balls.  There are $L$ distinct ball colours, and $R_\ell$ balls of each colour $\ell=1,2,\dots,L$,
with $\sum_{\ell=1}^L R_\ell=R$.  For each colour $\ell$, associate an acceptance probability $p_\ell\in [0,1]$.

The $R$ balls correspond to riders.  The ball colours correspond to rider destinations.  The acceptance probability $p_\ell$ is 
the probability any given driver accepts a dispatch towards the destination $\ell$.  For this version of the problem description,
I am going to assume that all drivers at the same location use the same disutility-acceptance thresholds, i.e. for now I will ignore the
small differences between distinct drivers acceptance thresholds.

Consider a sequence of $M$ trials.  On the $i$th trial there are $R^i$ balls in total, and $R^i_\ell$ balls of colour $\ell$.  Initialize $R^1=R$
and $R^1_\ell=R_\ell$ for each $\ell$. 

On the $i$th trial we first check if the bag is empty: if $\sum_\ell R^i_\ell = 0$, then we set $\ell_i=\emptyset$ to indicate a ``failed trial''. 
Otherwise we sample a colour $\ell_i$ from the current bag:
$$
\ell_i\sim \mathrm{Multinomial}\left(\frac{R^i_\ell}{R^i} : \ell=1,2,\dots,L\right).
$$
After sampling the colour $\ell_i$, we sample an accept/reject decision based on the threshold $p_{\ell_i}$:
$$
\delta_i\sim\mathrm{Bernoulli}(p_{\ell_i}).
$$
If $\delta_i=1$ indicates an ``accepted ball'' then we leave $\ell_i$ unchanged.  If $\delta_i=0$ then we set $\ell_i=\emptyset$ to indicate a failed trial.

Another way to describe the above sampling step, which might be simpler to think about, is on each step $i$ we construct a distribution $q_i$ over $L+1$ ``colours``.
The distribution $q_i$ has mass proportional to $\frac{p_\ell R^i_\ell}{R^i}$ for each of the first $\ell=1,2,\dots,L$ colours, and the final 
``colour'' $\ell=L+1$, which corresponds to a rejected dispatch, has the remaining mass.
Then we just sample $\ell_i\sim \mathrm{Multinomial}(q_i)$.
At the end of each trial, we subtract $1$ from $R^i_\ell$ if $\ell\leq L$ is one of the ball colours.  If $\ell=L+1$ indicates a rejected dispatch, we
don't change the number of balls in the bag.


After the $M$ trials we use a vector $\bfh\in \bbR^{L+1}$ to record our samples.  For each $\ell=1,2,\dots,L,L+1$ we have
$$
h_\ell = \frac{1}{k}\sum_{i=1}^M \bfone\left\{\ell_i=\ell\right\},
$$
where $k$ is the population-size parameter, which we can think of as proportional to the number of drivers (trials) $M$, or the number
of riders $R$.

We want to compare the distribution of the random vector $\bfh$, to the distribution of $\bfh$ conditioned on one of the components $h_\ell$ being
at least one.
\Xomit{
\begin{lemma}
\label{lem:balls_in_bag_coupling}
Fix any colour $\ell=1,2,\dots,L+1$.
There exists a random variable $(\bfh_1,\bfh_2)$ with the following properties:
\begin{enumerate}
\item The marginal distribution of $\bfh_1$ is the same as the distribution of $\bfh$.
\item The marginal distribution of $\bfh_2$ is the same as the distribution of $\bfh\mid h_\ell \geq \frac{1}{k}$.
\item With probability $1$ the difference between $\bfh_1$ and $\bfh_2$ is at most $C$, i.e. $\bbP\left(\|\bfh_1 - \bfh_2\|_1\leq C\right) = 1$.
\end{enumerate}
\end{lemma}

\mccomment{I thought I could construct this coupling by letting $\bfh_1$ and $\bfh_2$ have the same distribution except for potentially 
on the last trial, where we check if the condition $h_\ell\geq 1$ is violated and if so we set the last sample for $\bfh_2$ to be $\ell$
and proceed as normal with $\bfh_1$.  But it's not so simple: this modification always produces a sample $\bfh_2$ which satisfies $h_{2,\ell}\geq 1$, but it
does not have the same distribution as sampling from $\bfh\mid h_\ell\geq \frac{1}{k}$.}

\subsubsection{Analyzing the Probability Mass Functions}
In this subsection we take a different approach to analyzing the conditional distribution $\bfh\mid h_\ell\geq \frac{1}{k}$, where instead of trying to
explicitly construct a coupling,}

We directly compare the probability mass function of the conditional distribution to the unconditional distribution.
Notice that the random variable $\bfh$ has discrete support.  Let $\calH$ be the support of $\bfh$, and let $P:\calH\to [0,1]$ be the unconditional
probability mass function for $\bfh$, defined by 
$$
P(\bfh_0) \coloneqq \bbP(\bfh=\bfh_0)
$$
for any $\bfh_0\in\calH$. Fix a location $\ell$ and let $Q:\calH\to [0,1]$ be the conditional probability mass function for $\bfh$ given $h_\ell \geq \frac{1}{k}$,
defined by
$$
Q(\bfh_0)\coloneqq \bbP\left(\bfh = \bfh_0 \mid h_\ell \geq \frac{1}{k}\right).
$$
Conditional probability gives us the relationship
$$
\bbP\left(\bfh = \bfh_0 \mid h_\ell \geq \frac{1}{k}\right) = \frac{\bbP\left(\bfh=\bfh_0\right)}{\bbP\left(h_\ell \geq \frac{1}{k}\right)}\bfone\left\{h_{0,\ell}\geq \frac{1}{k}\right\}.
$$
In other words, we have the relationship
$$
Q(\bfh_0) = \frac{P(\bfh_0)}{q_\ell}\delta(\bfh_0),
$$
where $q_\ell=\bbP(h_\ell\geq \frac{1}{k})$ and $\delta(\bfh_0)$ is an indicator variable specifying whether the $\ell$th component of $\bfh_0$ exceeds $\frac{1}{k}$.
The following Lemma shows that $q_\ell$ is close to $1$ for large population sizes.
\begin{lemma}
Fix a location $\ell$.  Let $R_0 = \frac{R}{k}$ be the normalized number of riders, let $M_0=\frac{M}{k}$ be the normalized number of drivers, and let
$R_{0,\ell}=\frac{R_\ell}{k}$ be the normalized number of riders requesting a dispatch towards location $\ell$.
Let $q_\ell=\bbP(h_\ell\geq \frac{1}{k})$.
Then
\begin{equation}
\label{eq:conditional_probability_bound}
1-q_\ell \leq \left(1-\frac{p_\ell R_{0,\ell}}{R_0}\right)^{M_0 k}.
\end{equation}
\end{lemma}
\begin{proof}
\mccomment{The proof is immediate from the definition of $\bfh$.  Still TODO: incorporate the randomness in the number of requesting riders
into the probability bounds}.
\end{proof}

Our next Lemma shows that expecations computed with respect to $P$ are close to expectations computed with respect to $Q$:
\begin{lemma}
Let $f:\calH\to\bbR$ be a Lipschitz continuous function with Lipschitz constant $L$ and suppose the values that $f$ takes lie between $0$ and some constant $C>0$.
Then
\begin{equation}
\label{eq:conditional_to_unconditional_expectation}
\left|\bbE\left[f(\bfh)\right] - \bbE\left[f(\bfh)\mid h_\ell\geq \frac{1}{k}\right]\right| \leq C\left(1-\frac{p_\ell R_{0,\ell}}{R_0}\right)^{M_0 k}.
\end{equation}
\end{lemma}
\begin{proof}
Observe the following equations:
$$
\bbE\left[f(\bfh)\right] = \bbE\left[f(\bfh)\mid h_\ell \geq \frac{1}{k}\right] q_\ell + \bbE\left[f(\bfh)\mid h_\ell =0\right](1- q_\ell),
$$
Therefore,
$$
\left|\bbE\left[f(\bfh)\right] - \bbE\left[f(\bfh)\mid h_\ell\geq \frac{1}{k}\right]\right| \leq (1-q_\ell)C.
$$
The claimed bound (\ref{eq:conditional_to_unconditional_expectation}) follows from the inequality (\ref{eq:conditional_to_unconditional_expectation}).
\Xomit{
$$
\bbE\left[f(\bfh)\mid\right] = \bbE\left[f(\bfh)\mid h_\ell \geq \frac{1}{k}\right] q_\ell + \bbE\left[f(\bfh)\mid h_\ell =0\right](1- q_\ell),
$$
\begin{align*}
\bbE\left[f(\bfh)\mid h_\ell\geq \frac{1}{k}\right] &= \sum_{\bfh_0\in\calH} f(\bfh_0)\bbP\left(\bfh=\bfh_0\mid h_\ell \geq \frac{1}{k}\right)\\
&=\sum_{\bfh_0\in\calH} f(\bfh_0)  \frac{P(\bfh_0)}{q_\ell}\delta(\bfh_0).
\end{align*}
}
\end{proof}

\subsubsection{Matching Process Concentration}
\label{subsubsec:matching_concentration}
\input{approx_eqlbm/matching_process_concentration.tex}


==> approx_eqlbm/matching_process_concentration.tex <==
Consider the two-level model with population size $k$ and suppose at time $t$ the market state is $(\omega_t,\bfS_t)$.   
We want to consider the concentration properties for the matching process at a particular location $\ell$.
The matching process can be thought of as a probability distribution parameterized by the number of drivers $M_\ell$,
the number of riders who request a dispatch $R_{(\ell,d)}$ for each destination $d$, and a dispatch-acceptance 
probability $p_{(\ell,d)}$.  Note the disaptch acceptance probability is just a reparameterization of the disutility-acceptance
threshold $x_{(\ell,d)}$:
$$
p_{(\ell,d)} = \bbP\left(X \leq x_{(\ell,d)}\right) = \frac{x_{(\ell,d)}}{C}.
$$
For present purposes, we assume all drivers at $\ell$ use the same acceptance thresholds.

Let's write $\bfh_\ell\sim \mathrm{MP}(M_\ell,\bfR_\ell,\bfx_\ell)$ to mean that $\bfh_\ell$ is a random vector
indexed by actions $a\in\calA_\ell$ such that $(\bfh_\ell)_a$ specifies the number of drivers who take each
action (trip) $a$.
By $\calA_\ell$ I mean the set of all trip types originating from $\ell$, i.e.  $\calA_\ell=\{(\ell,d,\delta) : d\in\calL,\delta\in\{0,1\}\}$.
And when I say $(\bfh_\ell)_a$ specifies the number of drivers, I mean the components of $\bfh$ have not already been divided by the population size $k$.

And really, the end goal is to provide an analysis where $\|\bfh - \bar{\bfh}\|_1$ is small over all locations. This means that, if a particular location
has relatively few drivers or relatively little demand, then we don't have to guarantee concentration for that location because the overall values will be small.
It's important to keep that in mind, but we can just focus on showing that $\|\bfh_\ell - \bar{\bfh}_\ell\|_1$ is smaller than some $\epsilon$,
where $\epsilon$ is a constant (i.e. it doesn't need to depend on the matching-process parameters $M_\ell,\bfR_\ell,\bfx_\ell$.

Another thought worth mentioning is about nuances in the rider counts $R_{(\ell,d)}$. The platform solves the stochastic fluid problem
with respect to $(\omega_t,\bfS_t)$ and sets prices $P_{(\ell,d)}$ for every $(\ell,d)\in\calL^2$.
Then, price inquiry demand comes to the system, meaning there are $D_{(\ell,d)}$ (think of this as an absolute number, 
i.e. not normalized by $k$) riders who consider requesting a trip.
By assumption we know $D_{(\ell,d)}$ is close to its mean $\bar{D}_{(\ell,d)}$. And then we know each of these riders has iid value $V_{(\ell,d)}$,
and they request a ride with probability
$$
q_{(\ell,d)} = \bbP\left(V_{(\ell,d)} \geq P_{(\ell,d)}\right).
$$
So, conditional in dispatch-request demand $D_{(\ell,d)}$, the expected number of riders who request a dispatch is 
$\bar{R}_{(\ell,d)}\mid D_{(\ell,d)}=q_{(\ell,d)} D_{(\ell,d)}$.  And the unconditional expected number of riders who request a dispatch
is
$$
\bar{R}_{(\ell,d)} = \bar{D}_{(\ell,d)}q_{(\ell,d)}.
$$
While this characterization is nice, it poses a difficulty towards characterizing the concentration of $R_{(\ell,d)}$ towards $\bar{R}_{(\ell,d)}$:
we have no way to lower bound the acceptance probability $q_{(\ell,d)}$.
(There are funny examples where prices $P_{(\ell,d)}$ are not monotone in supply.)
So, we can presumably get concentration bounds of $R_{(\ell,d)}$ being close to $\bar{R}_{(\ell,d)}$ in terms of $q_{(\ell,d)}$, but there
is no direct bound on $q_{(\ell,d)}$.

Similarly, there is no way to bound the driver-acceptance probabilities $p_{(\ell,d)}=\frac{x_{(\ell,d)}}{C}$.

\textbf{Important Point 4:} So, we need a concentration bound that holds uniformly for all $x_{(\ell,d)}$ and all prices $P_{(\ell,d)}$.

I think we can get a uniform bound like this via the following argument:  think about the thresholds $x_{(\ell,d)}$ in terms of the 
driver acceptance probabilities $p_{(\ell,d)} = \frac{x_{(\ell,d)}}{C}$ and the prices $P_{(\ell,d)}$ in terms of the rider dispatch probabilities
$q_{(\ell,d)} = \bbP(V_{(\ell,d)} \geq P_{(\ell,d)})$.

Then we identify some thresholds $p^*$ and $q^*$ and make the following claim: If $p_{(\ell,d)} \geq p^*$ then we can claim some good concentration 
properties.  Otherwise, if $p_{(\ell,d)} < p^*$, then driver acceptances towards this destination are negligible. (We would make the same claim about
rider dispatch probabilities $q_{(\ell,d)}$ with respect to $q^*$.

\textbf{Conjecture 1:} It's not immediately clear how to characterize the mean matching vector $\bar{\bfh}$,
or how to analyze its concentration properties, in light of the sampling-without-replacement definition of the matching process.
However, after looking at properties of the multivariate hypergeometric distribution 
(\url{https://en.wikipedia.org/wiki/Hypergeometric_distribution#Multivariate_hypergeometric_distribution}) and seeing
its relationship with the multinomial distribution, I think the following claims are likely to be true:
For each dispatch trip towards $d$, ie for each action $a=(\ell,d,1)$ with $d\in\calL$, 
$$
\bar{h}_{(\ell,d,1)} = M_\ell\frac{p_{(\ell,d)} R_{(\ell,d)}}{\sum_{d'}R_{(\ell,d')}}.
$$
$M_\ell$ is the total number of ``trials'', and $\frac{p_{(\ell,d)} R_{(\ell,d)}}{\sum_{d'}R_{(\ell,d')}}$ is the initial probability
of a trial resulting in a dispatch towards $d$.

And for the relocation trips, first define $B_\ell$ to be the (initial) probability that a trial from location $\ell$ results in a rejected
dispatch:
$$
B_\ell = 1 - \sum_{d\in\calL}\frac{p_{(\ell,d)} R_{(\ell,d)}}{\sum_{d'}R_{(\ell,d')}}.
$$
Also, let $\bfb_\ell$ be the initial population level distribution over relocation destinations, such that
$$
(\bfb_\ell)_d = \frac{\left|\{i\in\calM_{\ell,t} : r_i = d\}\right|}{M_\ell}.
$$

Then I conjecture the expected number of relocation trips for each relocation trip $(\ell,d,0)$, with $d$ ranging over locations $\calL$,
is given by
$$
\bar{\bfh}_{(\ell,d,0)} = M_\ell B_\ell (\bfb_\ell)_d = M_\ell \left(1 - \sum_{d\in\calL}\frac{p_{(\ell,d)} R_{(\ell,d)}}{\sum_{d'}R_{(\ell,d')}}\right)
                                                        \left(\frac{\left|\{i\in\calM_{\ell,t} : r_i = d\}\right|}{M_\ell}\right)
$$

\mccomment{Possibly need some regularity conditions on $x_{(\ell,d)}$ and other parameters for this to be exactly true as stated.}

\textbf{Conjecture 2:}
My second conjecture is that the sampling-without-replacement matching process we've described has sharper concentration than a Multinomial
distribution over actions $\calA_\ell$, with the same number of trials $M_\ell$, and with probabilities specified by $\frac{\bar{\bfh}}{M_\ell}$
where $\bar{\bfh}$ is the mean vector we specified above.


\subsubsection*{Probability Literature to the Rescue}
Consider the matching process operating at a location $\ell$ where there are $M$ drivers, $R_{d}$ dispatch requests towards each destination $d$,
and where the drivers use exactly the same acceptance probabilities $p_{d}$ for each location.
Let $R^{(t)}_d$ be the number of dispatch requests that remain at the beginning of iteration $t$, and let $Q^{(t)}$ be the distribution from which
the dispatch destination on the $t$th iteration is sampled. The distribution $Q^{(t)}$ is specified by
\begin{align*}
\forall d\in\calL \ \ \ \ &Q^{(t)}(d_t=d) = \frac{R^{(t)}_d p_d}{\sum_{d'\in\calL}R^{(t)}_{d'}},\\
& Q^{(t)}(d_t=\emptyset) = 1-\sum_{d\in\calL}Q^{(t)}(d_t=d).
\end{align*}
Let $\mathrm{MP}(M, (R_d), (p_d))$ denote the probability distribution over trip vectors generated by the matching
process, such that the support of $\mathrm{MP}(M,(R_d), (p_d ))$ is vectors $\bfh$ indexed by $\calL\cup\{\emptyset\}$
where each component $(\bfh)_d$ corresponds to the number of trials where the sampled dispatch destination was $d$.

Let $S$ be a set that contains $\sum_{d\in\calL}R_d$ items. For each item $i\in S$ let $d_i\in\calL$ be a destination associated with item $i$,
and suppose there are $R_d$ items associated with each destination $d$. Assume there are weights associated with items, such that
the weigh of an item is equal to the acceptance probability
the drivers used for the associated destination: write $w_i = p_{d_i}$ for each $i\in S$.
Consider the probability distribution where we sample $N$ items from $S$ without replacement, where each item on each trial is
sampled with probability proportional to $w_i$.


\begin{lemma}
Conditional on the number of drivers who accept a dispatch being $N$, sampling dispatch locations from the matching process is
equivalent to sampling $N$ items from $S$ without replacement, where each item on each trial is
sampled with probability proportional to $w_i$.
\end{lemma}
\begin{proof}
We proceed via induction on $M$.  When there is only one driver $M=1$ the result is immediate.

Suppose the result holds for few numbers of drivers $M'<M$
\end{proof}

\url{https://arxiv.org/pdf/math/0609835.pdf} can be used to get concentration bounds on the number of dispatches $N$.

\url{https://arxiv.org/pdf/1603.06556.pdf} and \url{https://projecteuclid.org/journals/annals-of-statistics/volume-2/issue-1/Probability-Inequalities-for-the-Sum-in-Sampling-without-Replacement/10.1214/aos/1176342611.full} 
can be used to get concentration bounds on the sampling-without-replacement


==> approx_eqlbm/proof_outline.tex <==
\subsection{Proof of Theorem \ref{thm:two_level_robustness}}
 The proof of the inductive step 
will take the following steps:
\begin{enumerate}
    \item Show that if $\Pi$ is an $(\epsilon, \delta)$-approximate equilibrium at time $t$, then $1-\epsilon$ fraction
        of the active drivers use a common disutility acceptance threshold $\bfx$. 
    \item Show that the expected welfare under $\Pi$ in the two-level model is almost as large as the optimal fluid welfare
        under the solution $(\bff,\bfg, \bfx)$.
    \item Show that the approximate incentive-compatibility conditions on $\Pi$ imply approximate incentive-compatibility conditions
        on $(\bff,\bfg,\bfx)$.  In other words, show that $(\bff,\bfg,\bfx)$ is an approximate equilibrium for the fluid model.
    \item Show that the welfare of any approximate equilibrium for the fluid model is almost as large as the optimal welfare in the fluid model.
\end{enumerate}

The above steps are sufficient to prove Theorem \ref{thm:two_level_robustness}.  We provide details for each of the steps in the subsubsections below.

\subsubsection*{Notation Summary}
\mccomment{This is a reference subsection that summarizes and records the notation used in the following subsections.}
\begin{itemize}
    \item $\Phi_{\omega_t}(\bfS_t)$ refers to the optimal value of the state-dependent optimization problem, as a function of the market-state
        $(\omega_t,\bfS_t)$.
    \item The state-dependent optimization problem has decision variables $(\bff,\bfg)$, which are vectors indexed by pairs of locations
        $(\ell,d)\in\calL^2$, and with feasibility constraints $\bff,\bfg\geq 0$, $\bff\geq \bfg$, and $\bff^T\bfone_\ell=S_\ell$ for all $\ell$.
    \item The state dependent optimization problem has objective function $\Phi_{\omega_t}(\bff,\bfg)$, where
        \begin{equation}
            \calW_{\omega_t}(\bff,\bfg) =  \calU_{\omega_t}(\bff,\bfg)            + \bbE[\Phi_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff)].
        \end{equation}
        where $\calU_{\omega_t}(\bff,\bfg)$ is the current-period reward, defined by
        \begin{equation}
        \calU_{\omega_t}(\bff,\bfg) = \sum_{(\ell,d)} R_{(\ell,d)}(g_{(\ell,d)}) - c_{(\ell,d)}f_{(\ell,d)} - 
            \sum_\ell \bfg^T\bfone_\ell \bbE\left[X\mid X\leq C\frac{\bfg^T\bfone_\ell}{\bff^T\bfone_\ell}\right].
        \end{equation}
    \item It's possible for a fluid strategy to use a disutility acceptance threshold vector $\bfx$ that is suboptimal for the
        trips specified by $(\bff,\bfg)$.  In this case we define the function
        $\calU_{\omega_t}(\bff,\bfg,\bfx)$ to be
        \begin{equation}
\calU_{\omega_t}(\bff,\bfg,\bfx) = \sum_{(\ell,d)} R_{(\ell,d)}(g_{(\ell,d)}) - c_{(\ell,d)}f_{(\ell,d)} - 
            \sum_\ell \bfg^T\bfone_\ell \bbE\left[X\mid X\leq x_{(\ell,d)}\right].
        \end{equation}
    \item In the above equation, $X$ is a random variable with distribution $\mathrm{Uniform}(0,C)$.  We assume every driver
        has their idiosyncratic disutility sampled independently from $\mathrm{Uniform}(0,C)$ in each time period.
    \item The notation $\bfg^T\bfone_\ell$ means the total mass that $\bfg$ places on destination locations $d$ which originate
        from $\ell$.  Same with $\bff^T\bfone_\ell$.
    \item $R_{(\ell,d)}(g_{(\ell,d)})$ is a function specifying the total rider welfare generated when $g_{(\ell,d)}$ dispatches are
        served along the route $(\ell,d)$.
    \item Let $\calM_{t,\ell}$ be the set of drivers located at $\ell$ at time $t$,
\begin{equation}
    \calM_{t,\ell} = \{i\in\calM_t : \ell_i^t = \ell\}.
\end{equation}

\item For each $t$ there is a set $\calS_t$ of ``good'' market states $(\omega_t,\bfS_t)$.  The probability of being in a good state
    at time $t+1$, conditioned on being in a good state at time $t$ is $1-\epsilon$.

\end{itemize}





==> approx_eqlbm/scratch_text.tex <==

\subsection*{Scratch Section}
\mccomment{This is a temporary section, primarily about concentration properties for random variable in the two level mdoel,
and definitions we can reference which really belong elsewhere in the paper.}
\subsubsection*{Important Properties and Assumptions about Stochastic Two Level Model Dynamics}
We will also need to reference a number of variables which affect the stochastic dynamics of the two level model.
We summarize these variables below.

Let $\calR=(r_i\in\calL : i\in\calM_t)$ be the relocation destinations selected by each of the drivers.
\mccomment{For the remainder of the section I will operate under the assumption that drivers select a single
relocation destination, rather than a distribution of relocation destinations.  This is for simplicity.  This is
out of sync with how the driver strategy model is currently described.}

Let $\bfr = (r_{(\ell,d)} : (\ell,d)\in\calL^2)$ encode the stochastic dispatch request volume on each route $(\ell,d)$.  
We assume each $r_{(\ell,d)}$ is equal to the total number of requests along $(\ell,d)$ divided by the population-size
parameter $k$.
We assume the dispatch request volumes satisfy the concentration property stated in Assumption \ref{assn:request_concentration}.
\begin{assumption}
    \label{assn:request_concentration}
    There exists $\epsilon$ such that $\bfr$ is at most $\epsilon$ away from its mean $\bar{\bfr}$ with probability at least $1-\epsilon$.
    That is,
    \begin{equation}
        \bbP\left(\|\bfr - \bar{\bfr}\|_1 < \epsilon\right) \geq 1-\epsilon.
    \end{equation}
\end{assumption}

Let $\calX = (X_i : i\in\calM_t)$ be the stochastic add-passenger disutilities sampled by each of the drivers.
We assume the empirical distribution of the observed disutility values is close to the true cumulative distribution
for a $\mathrm{Uniform}(0,C)$ distribution. This is stated formally in Lemma \ref{lem:add_passenger_concentration}.
\begin{lemma}
    \label{lem:add_passenger_concentration}
    Suppose we have $M$ iid observations $X_1,\dots,X_M$ from a $\mathrm{Uniform}(0,C)$ distribution,
    and let $F_M(x) = \frac{1}{M}\sum_{i=1}^M \bfone_{\left\{X_i\leq x\right\}}$ be the empirical distribution function
    and let $F(x)=\frac{x}{C}$ be the true distribution function. Then, for every $\epsilon > 0$, the following holds
\begin{equation}
    \bbP\left(\sup_{x\in [0,C]}\left|F_M(x) - F(x)\right| \leq \epsilon\right) \geq 1-2e^{-2n\epsilon^2}.
\end{equation}
\end{lemma}
\begin{proof}
    \url{https://en.wikipedia.org/wiki/Dvoretzky%E2%80%93Kiefer%E2%80%93Wolfowitz_inequality}.
\end{proof}

The realized trips also depend on the matching process used by the platform, and in particular the dispatch
destination allocated to each driver.
Recall $d_i\in\calL\cup\left\{\emptyset\right\}$ indicates the dispatch destination allocated to each
driver $i$.
The matching process that the platform uses to determine the dispatch allocated to each driver depends on a number of factors.
It depends on the realized rider demand $\bfr$, it depends on the realized add-passenger disutilities $\calX$, and it depends
on an external source of randomness used to determine the order in which drivers are prioritized.  Let us parameterize this external
randomness by a random variable $U\sim\mathrm{Uniform}(0,1)$, so that the dispatch allocations $(d_i:i\in\calM_t)$ 
become deterministic conditioned on $(\bfr,\calX, U)$.
Let us write
\begin{equation}
    \calD(\bfr,\calX,U) = (d_i : i\in\calM_t)
\end{equation}
to indicate the dispatch destinations produced by the matching process, as a function of the realization of the random variables $(\bfr,\calX,U)$.

We assume that drivers can be allocated at most one dispatch, meaning that if a driver declines a dispatch they are forced to
take a relocation trip.  One consequence of this assumption is that the matching process effectively partitions the space of drivers
based on the destinations they are allocated.  For each $(\ell,d)$, let $Z_{(\ell,d)}(\bfr,\calX,U)$ be the volume of drivers positioned at
$\ell$ who are allocated a dispatch towards $d$, as a function of dispatch requests $\bfr$, add-passenger disutilities $\calX$, and the
external randomness $U$. Each $Z_{(\ell,d)}(\bfr,\calX,U)$ is defined by
\begin{equation}
    Z_{(\ell,d)}(\bfr,\calX,U) = \frac{1}{k}\left|\left\{i\in\calM_t : \ell_i=\ell, d_i=d\right\}\right|.
\end{equation}
We assume that the dispatches allocated to drivers do not change by a large amount if there is a small change in the dispatch
request volumes $\bfr$.  We formulate this assumption below, in Assumption \ref{assn:lipschitz_matching}.
\begin{assumption}
    \label{assn:lipschitz_matching}
    Let $\calX$ be any add-passenger disutility realization and let $U\in [0,1]$ be any realization of external randomness.
    Then, conditioned on $\calX$ and $U$, the size of each driver partition $Z_{(\ell,d)}$ is Lipschitz continuous when
    viewed as a function of $\bfr$.  That is, there exists a constant $L$ such that for any two request vectors $\bfr, \bfr'$
    we have
    \begin{equation}
        |Z_{(\ell,d)}(\bfr,\calX,U) - Z_{(\ell,d)}(\bfr',\calX,U)| \leq L\|\bfr - \bfr'\|_1.
    \end{equation}
\end{assumption}




\subsubsection*{Concentration Lemma for Two Level Model Trip Vectors}
We are ready to state our main Lemmas to accomplish step two of the proof.
Recall the random vectors $\bff$ and $\bfg$, defined in equations (\ref{eq:two_level_g}) and (\ref{eq:two_level_f}), specify the
realized total volume of total trips and dispatch trips on each route, respectively.
Define $\bar{\bff}$ and $\bar{\bfg}$ to be the expectated values
\begin{equation}
    \bar{\bff} = \bbE[\bff], \ \ \ \bar{\bfg} = \bbE[\bfg].
\end{equation}
Our first lemma is a concentration bound stating that the random variables $\bff$ and $\bfg$ are close to their
expectations with high probability.
\mccomment{Lemma \ref{lem:two_level_action_concentration} is important to relate the expected welfare under $(\bff,\bfg)$
to the welfare of the expected actions $(\bar{\bff}, \bar{\bfg})$.}
\begin{lemma}
    \label{lem:two_level_action_concentration}
    Under Assumptions \mccomment{TODO}, there exist error terms $\epsilon_0$, $\epsilon_1$ such that, with probability at least
    $1-\epsilon_1$, the random vectors $\bff$ and $\bfg$ have distance most $\epsilon_0$ from their mean.  That is,
    \begin{equation}
        \bbP\left(\|\bff - \bar{\bff}\|_1 + \|\bfg - \bar{\bfg}\|_1 \leq \epsilon_0\right) \geq 1-\epsilon_1.
    \end{equation}
\end{lemma}
\begin{proof}
    \mccomment{Establishing this result is more nuanced and complicated than I originally expected.
    The complications are related to working around the randomness inherent to the matching process used by the platform.}
\end{proof}

Let $\bfx$ be the common disutility threshold used by the drivers under $\Pi$, established in Lemma \ref{lem:common_threshold}.
Our next Lemma is to show that $(\bar{\bff}, \bar{\bfg}, \bfx)$ is an approximate equilibrium in the sense of 
Definition \ref{def:approx_eqlbm}.
Let $\bar{\calQ}$ be the Q-values associated with the fluid strategy $(\bar{\bff}, \bar{\bfg}, \bfx)$. Recall the Q-values
specify the expected utility to go values of the different actions drivers take under the specified strategy.  For relocation
trip actions $(\ell,d,0)$ the Q-value is defined by
\begin{equation}
    \bar{\calQ}(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\bfS_{t+1}(\omega_{t+1}, \bar{\bff})\right],
\end{equation}
and for relocation trip actions $(\ell,d,1)$ the Q-value is defined by 
\begin{equation}
    \bar{\calQ}(\ell,d,1, X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}
where $X\in [0,x_{(\ell,d)}]$ is any add-passenger disutility value smaller than the common acceptance threshold $x_{(\ell,d)}$
\mccomment{next steps for me: state concentration assumptions on $\bfS_{t+1}(\omega_{t+1}, \bar{\bff})$, double check that this is the
right way to think about continuation utilities in the context of the expected trip vectors, and state the Lemma asserting that
$(\bar{\bff}, \bar{\bfg}, \bfx)$ is an approximate equilibrium.}

\subsection*{Step 3: Approximate Fluid Equilibria are Approximately Welfare Optimal}
\mccomment{There are two possible approaches for this step.  Approach 1: redo steps of the exact fluid robustness  proof, carrying error
terms through the entire analysis.  Approach 2: use high-level convex analysis arguments to show that an approximate equilibrium
must be close to an exact equilibrium.}

\subsubsection*{Step N: Welfare Bounded by Fluid Solution}
Our next step is to show that the fluid welfare obtained by the strategy $(\bff,\bfg,\bfx)$ is close to the expected welfare
achieved by the approximate equilibrium strategy profile $\Pi$.
\begin{lemma}

\end{lemma}
\begin{proof}
    Observe that the expected welfare under $\Pi$ can be deconstructed as follows.
    \begin{align*}
        \Phi_{\omega_t}(\bfS_t;\Pi) &= \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM}\sum_{\tau=t}^T W_i^\tau \mid (\omega_t,\bfS_t)\right]\\
        &=\frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM_t}W_i^t\right] + \bbE^\Pi\left[\Phi_{\omega_{t+1}}(\bfS_{t+1};\Pi) \mid (\omega_t,\bfS_t)\right]\\
        &\geq \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM_t}W_i^t\right] + 
                \bbE\left[\Phi_{\omega_{t+1}}(\bfS_{t+1})\mid (\omega_t,\bfS_t)\right] - \gamma,
    \end{align*}
    where $\Phi_{\omega_{t+1}}(\bfS_{t+1})$ is the optimal fluid welfare from the state $\bfS_{t+1}$.
\end{proof}

\subsubsection*{Old Additional Lemmas}

We now state a number of useful additional lemmas that are used to prove approximate welfare robustness.

Our next Lemma states that the distribution of time $t+1$ supply location vectors does not have strong dependence on
any one driver's individual actions.
\begin{lemma}
    \label{lem:supply_loc_coupling}
    Fix a time $t$ scenario $\omega_t$ and supply location vector $\bfS_t$ and let $a\in\{(\ell,d,\delta) : d\in\calL, \delta\in\{0,1\}\}$ be any 
    trip that a driver positioned at $\ell$ can take.  Fix any driver $i$ who is positioned at $\ell$. 
    Then there exists a coupling $(\bfS_1,\bfS_2)$ where
    \begin{enumerate}
    \item The marginal distribution of $\bfS_1$ is the same as the distribution of time $t+1$ supply location vectors
        conditioned on driver $i$ taking action $a$, that is $\bfS_1$ has the same distribution as $\bfS_{t+1}\mid a_i=a$.
    \item The marginal distribution of $\bfS_2$ has the same distribution as the time $t+1$ supply location
        vector without any additional information, i.e. $\bfS_2$ has the same distribution as $\bfS_{t+1}$.
    \item On any sample path, $\bfS_1$ and $\bfS_2$ differ by at most $\frac{2}{k}$, that is
        \begin{equation}
        \bbP\left(\|\bfS_1-\bfS_2\|_1 \leq \frac{2}{k}\right) = 1.
        \end{equation}
    \end{enumerate}
\end{lemma}

Our next Lemma states an important concentration property about supply location vectors.
\begin{lemma}
    \label{lem:supply_loc_concentration}
    Fix a scenario $\omega_t$ and a supply location vector $\bfS_t$.  Let 
    $\bar{\bfS}_{t+1} = \bbE[\bfS_{t+1}(\omega_{t+1},\bff)\mid\omega_t,\bfS_t]$ be the expected time $t+1$ supply location vector.
Then there exists error terms $\epsilon_0, \epsilon_1$ such that
    \begin{equation}
        \bbP\left(\|\bfS_{t+1} - \bar{\bfS}_{t+1}\|_1 \leq \epsilon_0\right) \geq 1-\epsilon_1.
    \end{equation}
\end{lemma}
Notice that the expected time $t+1$ supply location vector is a linear function of the expected trip volumes
$\bar{\bff}$:
\begin{equation}
    \bar{\bfS}_{t+1} = \sum_{\omega_{t+1}\in\Omega_{t+1}}\bbP(\omega_{t+1}\mid\omega_t)\bar{\bfS}_{t+1}(\omega_{t+1},\bar{\bff}),
\end{equation}
where $\bar{\bfS}_{t+1}(\omega_{t+1},\bar{\bff})$ is a deterministic function that includes the expected number of new arrivals
at each location, as well as the expected number of drivers arriving at each location as specified by $\bar{\bff}$.




==> approx_eqlbm/step_one_common_thresholds.tex <==

\subsection{Proof of Lemma \ref{lem:common_threshold}}
\label{subsec:common_threshold_proof}
Below is a restatement of Lemma \ref{lem:common_threshold}.
\begin{lemma*}
    Let $\bfx_i=(x_i^d : d\in\calL)$ be the disutility acceptance threshold used by each driver $i$ in time period $t$ under
    the strategy profile $\Pi$. Then for each location $\ell$ there exists a disutility threshold vector 
    $\bfx_\ell = (x_{(\ell,d)} : d\in\calL)$ and an error term $\epsilon$ \mccomment{TODO: fill in $\epsilon_\ell$ details} 
    such that every driver positioned at $\ell$ uses a disutility threshold that is at most $\epsilon$ distance from
    $\bfx_\ell$, i.e.
    \begin{equation}
        \max_{d\in\calL}|x_i^d - x_{(\ell,d)}|_ \leq \epsilon , \ \ \ \ \forall i\in\calM_{t,\ell}.
    \end{equation}
    The error term $\epsilon$ is equal to
    \begin{equation}
    \epsilon = 2\delta + 4\epsilon^{BI} + \frac{CL}{k},
    \end{equation}
    where $\delta$ is the approximation error in the strategy profile $\Pi$, $\epsilon^{BI}$ is the error term from
    the backwards induction assumption Assumption \ref{assn:backwards_induction}\mccomment{$\epsilon^{BI}$ is an error term
    that needs to work for every $\bfS_{t+1}$}, $C$ is a constant, $L$ is the lipschitz
    constant for the state-dependent optimization problem partial derivative, and $k$ is the population-size parameter.
\end{lemma*}
\begin{proof}
    \mccomment{The definition for $\delta$-incentive compatible stated in (\ref{eq:delta_deviation_incentive}) currently states that
    a driver's deviation can depend on the destination $d$ they are allocated, but not their add-passenger disutility $X_i$.
    I think it makes sense to also let the deviation depend on the add-passenger disutility, so that the interpretation would be:
    for each destiation $d$ a driver can be allocated, and any add-passenger disutility $X_i$ they can sample, their incentive
    to deviate is at most $\delta$.  That's how I'll proceed for now.}
    Consider any two drivers $i$ and $j$ positioned at the same location $\ell$, and suppose there is some destination $d$
    for which driver $i$ uses a lower acceptance threshold than driver $j$, i.e. $x^i_d < x^j_d$.
    Let $x\in (x_i^d, x_j^d)$ be a number in between the two thresholds and
    consider the following two distinct events:
    \begin{enumerate}
    \item Driver $i$ is allocated a dispatch towards $d$ and samples $x$ as their add-passenger disutility, i.e. $d_i=d$ and $X_i=x$.
    \item Driver $j$ is allocated a dispatch towards $d$ and samples $x$ as their add-passenger disutility, i.e. $d_j=d$ and $X_j=x$.
    \end{enumerate}
    In event 1, driver $i$ rejects the dispatch towards $d$ and drives empty towards an alternate destination $d'$.
    The utility-to-go that driver $i$ collects conditioned on event 1 is thus equal to
    \begin{equation}
        U^t_i(d_i=d, X_i=x) = -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right].
    \end{equation}
    From the definition of $\Pi$ being an approximate equilibrium, we know that conditioned on event 1 the alternate action
    of accepting the dispatch towards $d$ can only increase driver $i$'s utility to go by at most $\delta$.
    This implies the inequality
    \begin{equation}
        \label{eq:event_1_first_bound}
        -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] + \delta \geq
        P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right].
    \end{equation}
    Let $Z=-c_{(\ell,d')} + \delta - P_{(\ell,d)} + x + c_{(\ell,d)}$ be a temporary variable to track the non-utility to go
    terms from the above expression, so we have
    \begin{equation}
    Z + \bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] \geq \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right].
    \end{equation}
    From the backwards induction assumption, Assumption \ref{assn:backwards_induction}, the above inequality implies
    an inequality in terms of the state-dependent optimization function partial derivatives:
    \begin{align}
        & Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})+ \epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right]\label{eq:start_line}
        \\
        \geq\ \ \ &Z + \bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] \\
        \geq\ \ \  &\bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right]\\
        \geq\ \ \  & \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1})-\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d,1) \right].\label{eq:end_line}
    \end{align}
    In the above, $\bfS_{t+1}$ is the (stochastic) supply-location vector the time $t+1$, and $\epsilon(\omega_{t+1},\bfS_{t+1})$ is the
    error term provided in the backwards induction assumption Assumption \ref{assn:backwards_induction}.

    \mccomment{It might make sense to move the analysis in this paragraph into its own lemma}
    Now, the distribution of $\bfS_{t+1}$ in line (\ref{eq:start_line}) is not exactly the same as the distribution of $\bfS_{t+1}$ in the
    final line (\ref{eq:end_line}), because we are conditioning on driver $i$ taking two different actions.  But the distributions
    are very similar: other than the clear difference that driver $i$ will be in a different location at time $t+1$ if we condition
    on $a_i=(\ell,d',0)$ vs. if we condition on $a_i=(\ell,d,1)$, 
    the only difference between the distributions on line (\ref{eq:start_line}) and (\ref{eq:end_line}) is that in line (\ref{eq:end_line}),
    when driver $i$ accepts the dispatch, there will be one fewer dispatch to go around to the remaining drivers, so it is possible that
    one other driver selects a different action.
    Therefore, we there exists a coupling $(\bfS_1,\bfS_2)$ such that $\bfS_1$ has the same distribution as $\bfS_{t+1}\mid a_i=(\ell,d',0)$,
    $\bfS_2$ has the same distribution as $\bfS_{t+1}\mid a_i=(\ell,d,1)$, and on every sample path the realizations of $\bfS_1$ and $\bfS_2$
    are almost the same: there is always a common $\bfS_0$ such that $\bfS_0$ corresponds to the locations of all but $2$ drivers in each
    of $\bfS_1$ and $\bfS_2$.  Since each driver contributes weight $\frac{1}{k}$ to the supply-location vector, this means
    the maximum difference between $\bfS_1$ and $\bfS_2$ on any sample path is $\frac{4}{k}$.

    \mccomment{I am going to assume that the $\epsilon(\cdot,\cdot)$ error-term function has the same lipschitz
    constant as the partial derivative of the state-dep optimization function. Call this Lipschitz constant $L$}
    Using the coupling $(\bfS_1,\bfS_2)$, the inequality between (\ref{eq:start_line}) and (\ref{eq:end_line}) can be written
    as
    \begin{equation}
        \label{eq:coupling_ineq}
    Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{2})+  \epsilon(\omega_{t+1},\bfS_{1}) + \epsilon(\omega_{t+1},\bfS_{2}) \right] 
        \geq 0.
    \end{equation}
    Let $L$ be the common Lipschitz constant between the partial derivative of the state dependent optimization function, and
    the error-term function $\epsilon(\cdot,\cdot)$.  Then we have
    $$
\bbE\left[-\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{2})+\epsilon(\omega_{t+1},\bfS_{2})\right] \leq
\bbE\left[-\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{1})+\epsilon(\omega_{t+1},\bfS_{1})\right] + \frac{8L}{k},
    $$
    since the distance $\|\bfS_1-\bfS_2\|_1$ is at most $\frac{4}{k}$ on any sample path.
    Therefore equation (\ref{eq:coupling_ineq}) implies the bound
    \begin{equation*}
Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{1})+  2\epsilon(\omega_{t+1},\bfS_{1}) \right] 
        + \frac{8L}{k} \geq 0.
    \end{equation*}
    Recall the marginal distribution of $\bfS_1$ is the same distribution as the time $t+1$ supply-location vector conditioned on
    driver $i$'s action being $a_i=(\ell,d',0)$, so the above bound can be rewritten as:
    \begin{equation}
        \label{eq:event_1_final_bound}
    Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1})+  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right] 
        + \frac{8L}{k} \geq 0.
    \end{equation}

    In event 2, driver $j$ accepts the dispatch and drives a passenger towards $d$.  The utility to go that driver $j$ collects
    conditioned on event 2 is equal to
    \begin{equation}
        U_j^t(d_j=d, X_j=x) = P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_j^{t+1}\mid a_j=(\ell,d,1)\right].
    \end{equation}
    From $\Pi$ being an approximate equilibrium, we know that the utility of accepting the dispatch towards $d$ is at most $\delta$ short of
    the utility from any other action, in particular it is at most $\delta$ short from the utility of taking a relocation
    trip towards driver $i$'s destination $d'$.
    This implies the inequality
    \begin{equation}
P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right]+ \delta \geq 
        -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right].
            \end{equation}
    Following the same steps that took us from equation (\ref{eq:event_1_first_bound}) to (\ref{eq:event_1_final_bound}),
    we deduce the bound
    \begin{equation}
        \label{eq:event_2_bound}
    Z' + \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})  
        +  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_j=(\ell,d,1) \right] 
        + \frac{8L}{k} \geq 0,
    \end{equation}
    where
    $Z' =  -Z + 2\delta.
    $

    \mccomment{I am going to assume there is a coupling between $\bfS_{t+1}\mid a_i=(\ell,d',0)$ and $\bfS_{t+1}\mid a_j=(\ell,d,1)$
    where the sample path difference is at most $\frac{6}{k}$: $\frac{2}{k}$ difference for each of the following: $i$ drives somewhere else,
    $j$ drives somewhere else, and potentially one more driver's trip changes because the number of matches that the platform can allocate
    changes by $1$. I will either eventually expand on the details here, or add a lemma that specifically talks about this coupling argument.}
    Using \mccomment{the above comment, for now} there exists a coupling $(\bfS_1, \bfS_2)$ such that $\bfS_1$ has marginal distribution
    equal to $\bfS_{t+1}$ conditioned on driver $i$ driving empty towards $d'$, $\bfS_2$ has marginal distribution equal
    to the distribution of $\bfS_{t+1}$ conditioned on driver $j$ driving a passenger towards $d$, and the maximum distance
    between $\bfS_1$ and $\bfS_2$ on any sample path is $\frac{6}{k}$.
    Therefore (\ref{eq:event_2_bound}) implies the bound
    \begin{equation}
        \label{eq:event_2_final_bound}
    Z' + \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})  
        +  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right] 
        + \frac{26L}{k} \geq 0,
    \end{equation}
    
    Now, recall the terms $Z$ in equation (\ref{eq:event_1_final_bound}) and $Z'$ in equation (\ref{eq:event_2_final_bound}) include an
    arbitrary disutility threshold $x$ in between $x^d_i$ and $x^d_j$.
    Let us now write $Z(x)$ and $Z'(x)$ to explicitly denote the dependence on $x$.  Next, consider what happens when we add
    the equations (\ref{eq:event_1_final_bound})
    using the threshold $x=x_i^d$ and (\ref{eq:event_2_final_bound}) using the threshold $x=x_j^d$.
    The partial derivative terms cancel, and we are left with
    \begin{equation}
        \label{eq:sum_of_bounds}
        Z(x_i^d) + Z'(x_j^d) + 4\epsilon + \frac{34L}{k} \geq 0.
    \end{equation}
    where we use $\epsilon = \bbE\left[\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0)\right]$.
    Observe that $Z(x_i^d) + Z'(x_j^d) = x_i^d - x_j^d + 2\delta$. Therefore, we have
    \begin{equation}
        \label{eq:similar_thresholds}
    x_j^d - x_i^d \leq 2\delta + 4\epsilon + \frac{34L}{k}.
    \end{equation}

    Therefore, the Lemma holds by taking $\bfx_\ell$ to be the threshold vector $\bfx_i$ used by any driver located at $i$.

    


\end{proof}



==> approx_eqlbm/step_two_approx_eqlbm.tex <==
\subsection*{Step 2: Fluid Solution is an Approximate Equilibrium}
\mccomment{In this section our goal is to show that the fluid solution $(\bff,\bfg,\bfx)$, which we constructed in the previous
section, is an approximate equilibrium for the fluid setting.  The work for this section is the following steps:
\begin{itemize}
    \item Define what we mean by fluid strategy and (approximate) fluid equilibrium.  These definitions are provided in earlier sections, though
        there is not currently a precise definition environment we can refer back to.  My plan for now is to write precise definitions
        for these terms in this section, so they may easily be referred to and so that I can be precise about what I write, and then
        the location of the definitions will move as the layout of the paper is improved.
    \item Formulate the goal ``$(\bff,\bfg,\bfx)$ is an approximate equilibrium'' as a precise mathematical statement.  The part of the definition
        that needs some care is in handling the fact that, as defined, the solution $(\bff,\bfg,\bfx)$ is a random variable which depends
        on stochastic demand.  I plan to take as simple an approach as possible here:  There exists a deterministic fluid strategy
        $(\bar{\bff}, \bar{\bfg}, \bar{\bfx})$ such that $(\bff,\bfg,\bfx)$ is close to $(\bar{\bff}, \bar{\bfg}, \bar{\bfx})$
        with high probability.
    \item Prove the precise mathematical statement formulated in the previous step. This step should be straightforward and depend on
        assumptions about Lipschitz continuity and concentration assumptions.  In the spirit of precision I'll write these assumptions
        in this section as their own Assumption environments.  In future versions of the paper, the location of these assumptions
        within the paper layout will change.
\end{itemize}}

    A feasible fluid strategy $(\bar{\bff},\bar{\bfg},\bfx)$ is a fluid equilibrium if there exists no deviation 
    which increases a driver's expected utility.
    The set of utility to go values that drivers at $\ell$ can achieve under $(\bar{\bff},\bar{\bfg},\bfx)$ is given by:
    \begin{align*}
        \calU(\ell) =& \left\{\bar{\calQ}(\ell,d,0) : d\in\calL, \bar{f}_{(\ell,d)} - \bar{g}_{(\ell,d)} > 0\right\} \\
        & \ \ \cup \left\{\bar{\calQ}(\ell,d,1,X) : d\in\calL, \bar{g}_{(\ell,d)} > 0, 0\leq X \leq x_{(\ell,d)}\right\}.
    \end{align*}
    The set of utility to go values that drivers at $\ell$ can achieve by deviating from $(\bff,\bfg,\bfx)$ is given by:
    \begin{align*}
        \calD(\ell) =& \left\{\bar{\calQ}(\ell,d,0) : d\in\calL\right\} \\
        & \ \ \cup \left\{\bar{\calQ}(\ell,d,1,X) : d\in\calL, \bar{r}_{(\ell,d)} - \bar{g}_{(\ell,d)} > 0\right\}.
    \end{align*}
\begin{definition}
    \label{def:fluid_eqlbm}
    We say $(\bff,\bfg,\bfx)$ is an \emph{exact fluid equilibrium} if the inequality $$\min \calU(\ell) \geq \max \calD(\ell)$$ holds
    for every location $\ell$.
    We say $(\bff,\bfg,\bfx)$ is an \emph{$\epsilon$-approximate fluid equilibrium} if the inequality
$$\min \calU(\ell) \geq \max \calD(\ell)-\epsilon$$
    holds for every location $\ell$.
\end{definition}

Recall the random vectors $\bff$ and $\bfg$, defined in equations (\ref{eq:two_level_g}) and (\ref{eq:two_level_f}), specify the
realized total volume of total trips and dispatch trips on each route, respectively.
Define $\bar{\bff}$ and $\bar{\bfg}$ to be the expectated values
\begin{equation}
    \bar{\bff} = \bbE[\bff], \ \ \ \bar{\bfg} = \bbE[\bfg].
\end{equation}
Let $\bfx$ be the common disutility threshold used by the drivers under $\Pi$, established in Lemma \ref{lem:common_threshold}.
Let $\bar{\calQ}$ be the Q-values associated with the fluid strategy $(\bar{\bff}, \bar{\bfg}, \bfx)$. Recall the Q-values
specify the expected utility to go values of the different actions drivers take under the specified strategy.  For relocation
trip actions $(\ell,d,0)$ the Q-value is defined by
\begin{equation}
    \bar{\calQ}(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\bfS_{t+1}(\omega_{t+1}, \bar{\bff})\right],
\end{equation}
and for relocation trip actions $(\ell,d,1)$ the Q-value is defined by 
\begin{equation}
    \bar{\calQ}(\ell,d,1, X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}
where $X\in [0,x_{(\ell,d)}]$ is any add-passenger disutility value smaller than the common acceptance threshold $x_{(\ell,d)}$

Our next Lemma is to show that $(\bar{\bff}, \bar{\bfg}, \bfx)$ is an approximate equilibrium in the sense of 
Definition \ref{def:fluid_eqlbm}.

\begin{lemma}
    \label{lem:approx_fluid_eqlbm}
    There exists an error term $\epsilon_0$ such that $(\bar{\bff},\bar{\bfg},\bfx)$ is an $\epsilon_0$-approximate fluid equilibrium.
\end{lemma}
\begin{proof}
    We prove Lemma \ref{lem:approx_fluid_eqlbm} by using the incentive compatibility conditions from the definition of what
    it means for $\Pi$ to be an approximate equilibrium, and then by using large-market concentration properties to bound
    the error terms.

    Observe that the
    realization of the dispatch-volume vector $\bfg$ will always be smaller in each coordinate by the realization
    of the request vector $\bfr$.  Therefore, the expected dispatch volume vector $\bar{\bfg}$ will be smaller than the
    expected dispatch request vector $\bar{\bfr}$.  Therefore, $(\bar{\bff}, \bar{\bfg}, \bfx)$ is a feasible strategy
    profile for the fluid model.


    Consider any location $\ell$, consider any driver $i$ positioned at $\ell$, let $\bfx_i$ be the
    dispatch-acceptance threshold used by driver $i$.  Let $d$ be any potential destination, and consider
    the case where the expected dispatch trip volume from $\ell$ to $d$ is less than the expected dispatch request
    volume from $\ell$ to $d$, i.e. the case where  $\bar{g}_{(\ell,d)} < \bar{r}_{(\ell,d)}$.  

    \mccomment{The incentive compatibility conditions hold for each driver conditioned on their realized dispatch destination 
    and add-passenger disutility value.}


    We consider two cases.  For the first case, we consider what happens when driver $i$'s add-passenger disutility $X_i$
    is larger than his acceptance threshold $x_{(\ell,d_i)}$ and he declines the dispatch and takes a relocation trip
    towards some other location $d'$.

\end{proof}


==> approx_eqlbm_preliminaries.tex <==
In this section we summarize how the SSP mechanism operates in the two-level model.
At each time period $t$ the SSP mechanism solves the state-dependent optimization problem,
which is parameterized by the time-scenario $\omega_t$ and a supply-location vector
$\bfS_t$.  In the fluid model,
the supply-location vector $\bfS_t$ is fully determined by the scenario and the trips in the previous time period;
in the two-level model, the number of drivers who enter the market at each location is stochastic, 
and so the supply-location vector is subject to an additional layer of granular randomness.
Let us write
\begin{equation}
\label{eq:expected_supply_vec}
\bar{\bfS}_t = \bbE\left[\bfS_t\right]
\end{equation}
to mean the expected supply-location vector at time $t$, assuming the trips from the previous time period are fixed.

We assume the platform sees how many drivers enter the platform at each location before it sets prices, meaning that
the realized supply-location vector $\bfS_t$ can be observed.
The SSP mechanism then computes an optimal solution $(\bff^*,\bfg^*)$ for the state-dependent optimization
problem with respect to the state $(\omega_t,\bfS_t)$, and sets the price $P_{(o,d)}$ on each route $(o,d)\in\calL^2$
to be
\begin{equation}
\label{eq:sspm_price}
P_{(o,d)} = F_{(o,d,\omega_t)}^{-1}\left(1 - \frac{g^*_{(o,d)}}{\bar{D}_{(o,d)}}\right).
\end{equation}
In the above expression, the value $\bar{D}_{(o,d)}$ appearing in the denominator is the expected number of passengers
who open in the app and check the price for a trip along $(o,d)$.

After the prices are set, each rider who checked the price for a trip decides whether or not to request a dispatch.
In the two-level model each rider's decision is stochastic.  Let $d_{(o,d)}$ be the (stochastic) realized number
of dispatch requests for the route $(o,d)$.  Let $\bfd_t=(d_{(o,d)}:(o,d)\in\calL^2)$ be a vector encoding the realized
number of dispatch requests across all routes, and let
\begin{equation}
\label{eq:expected_demand_vec}
\bar{\bfd}_t=\bbE[\bfd_t]
\end{equation}
be a vector encoding the expected number of dispatch requests across each route.


==> approx_eqlbm_section.tex <==
\input{approx_eqlbm/main_section_text.tex}
\input{approx_eqlbm/establishing_approx_eqlbm.tex}
\input{approx_eqlbm/lemmas.tex}
\input{approx_eqlbm/proof_outline.tex}
\input{approx_eqlbm/step_one_common_thresholds.tex}
\input{approx_eqlbm/step_two_approx_eqlbm.tex}
\input{approx_eqlbm/scratch_text.tex}


==> approx_eqlbm_strategy_vecs.tex <==
\subsection{Strategy Profiles in the Two-Level Model}

To define strategy profiles let us start by describing the strategic decisions facing drivers in a single time period.
Fix a time period $t$ and scenario $\omega_t$.  After new drivers join, let $\calM_t$ be an index set over all active 
drivers in the network, and let $\ell_i$ be the 
location of each driver $i\in\calM_t$.

Recall we use the notation $(\ell,d,0)$ to denote a relocation trip from location $\ell$ to $d$, and $(\ell,d,1)$ denotes a dispatch trip
from $\ell$ to $d$.
Let $d_i$ be the destination location of the dispatch trip that driver $i$ is allocated.
The matching process is mediated by the platform and depends on stochastic demand realizations.
If driver $i$ is not allocated a dispatch
we write $d_i=\emptyset$.

The set of actions available to each driver depends on the driver's location as well as the destination of the dispatched they are matched to,
if any exists. A driver located at $\ell$ who receives a dispatch towards location $d$ has the opportunity to serve the dispatch trip 
specified by $(\ell,d,1)$.  In addition, they also have the option to take a relocation trip towards any possible location $d'$, where
the relocation trip is specified by $(\ell,d',0)$.
The set of actions available to a driver located at $\ell$ who receives a dispatch towards location $d$ can therefore be written
as the following set:
\begin{equation}
    \calA(\ell,d) = \begin{cases}
        \left\{(\ell,d',0) : d'\in\calL\right\} \cup \left\{(\ell,d,1)\right\} & \mbox{if }d \in\calL,\\
        \left\{(\ell,d',0) : d'\in\calL\right\}  & \mbox{if }d =\emptyset.
    \end{cases}
\end{equation}
Let
\begin{equation}
    \calA_i = \calA(\ell_i,d_i)
\end{equation}
be the set of actions available to each driver $i\in\calM_t$.

Before they make a decision about where to drive, each driver gets to observe their add-passenger disutility,
an idiosyncratic quantity that governs the additional cost the driver will incur for adding a passenger to their car,
i.e. for serving a dispatch trip, in the current time period.  Let $X_i$ denote the add-passenger disutility incurred by each driver $i$.

Driver decisions about whether or not to accept a dispatch depend on their realized add-passenger disutility.  A driver with high add-passenger disutility
might choose to reject a dispatch trip, whereas another driver with lower add-passenger disutility who is allocated the same dispatch would choose
to accept the dispatch.

We assume without loss of generality that decisions about whether to accept or reject a dispatch are monotone in the add-passenger disutility: if a driver
accepts a dispatch at a particular disutility value $X_i$, then they would have also accepted the dispatch for all smaller values of $X_i$.
Therefore, each driver's strategy about whether to accept or reject a dispatch can be specified by a disutility threshold they associate
with each potential dispatch destination.

Therefore, driver strategies for the one-shot game we associate with each time period can be specified by the following components:
1) A disutility acceptance threshold associated with each destination, on which the drivers accept/reject decisions are based,
2) A choice of location to drive to if the driver does not serve a dispatch trip.

We encode the strategy used by each driver $i$ with a tuple $(\bfx_i,\bfr_i)$, where $\bfx_i=(x^i_d : d\in\calL)$
is a vector of disutility acceptance thresholds, and $\bfr_i\in\Delta(\calL)$
is a distribution over locations, that driver $i$ uses to select a relocation trip if they don't serve a dispatch trip.
Let us summarize the steps that each driver $i$ uses to obtain their action $a_i\in\calA_i$, given the strategy $(\bfx_i,\bfr_i)$:
\begin{enumerate}
    \item Observe the add-passenger disutility $X_i\geq 0$ and the dispatch destination $d_i$.  If $d_i=\emptyset$ is the empty location,
        i.e. if the matching process does not allocate a dispatch to driver $i$, go to step \ref{item:relocation_choice}.
    \item Compare add-passenger disutility to the acceptance threshold for destination $d_i$.  If add-passenger disutility is smaller than
        the threshold, i.e. if $X_i \leq x^i_{d_i}$, then accept the dispatch.  In this case, the action that driver $i$ takes is specified by
        $a_i=(\ell_i,d_i,1)$.  If add-passenger disutility is larger than the threshold, go to step \ref{item:relocation_choice}.
    \item \label{item:relocation_choice}  Sample a destination $d$ from the distribution $\bfr_i$, independently from all other sources of randomness.
        The action that driver $i$ takes is specified by $a_i=(\ell_i,d,0)$.
\end{enumerate}

We now define what we mean by a strategy profile for the entire multiperiod stochastic game played by the drivers.  Let $\calM$ be an index
set of all drivers who could potentially join the marketplace.  
We define s strategy $\pi_i$ for each driver $i\in\calM$ as a sequence of functions $(\pi_i^1,\pi_i^2,\dots,\pi_i^T)$ where each element $\pi_i^t$
is referred to as the time $t$ strategy and it
selects the acceptance threshold and relocation distribution that driver $i$ uses for the $t$th time period.
(If a driver $i$ hasn't entered the market by time period $t$, then we assume the function $\pi_i^t$ has no bearing on that driver or any
of the market dynamics).

In general, the domain of each function $\pi_i^t$ can depend on the history of observed market states up to the beginning of time $t$.
For simplicity we assume that all drivers use Markovian strategies which only depend on the state at
the beginning of the time period. This assumption is without loss of generality in the context of exact equilibria because we assume that
drivers are expected utility maximizers.   In the current context where we consider approximate equilibria this assumption is almost without loss
of generality. \mccomment{This description about Markovian strategies being WLOG can be clarified / improved.}
The state at the beginning of the time period is specified by a scenario $\omega_t\in\Omega_t$
and a supply-location vector $\bfS_t$. Let $\calS_t$ be the set of all possible time $t$ states,
and let $\calX=\bbR_{\geq 0}^\calL$ be the space of 
feasible disutility-threshold vectors, so that each time $t$ strategy can be specified as function $\pi_i^t:\calS_t\to\calX\times\Delta(\calL)$.

A strategy profile $\Pi=(\pi_i : i\in\calM)$ is a specification of the strategy used by each potential driver over the entire marketplace dynamics.

\subsection{Approximate Equilibria in the Two-Level Model}

Our model is that drivers strategically select their strategies before the marketplace dynamics begin, and then individual drivers
collect utility based on the collective strategy profile the drivers have selected as well as the stochastic market dynamics.
We model strategic driver behaviour by assuming that drivers select strategies which result in an approximate equilibrium strategy profile $\Pi$
In this subsection we will define what it means for a strategy profile $\Pi$ to be an approximate equilibrium.

Fix a strategy profile $\Pi$ and assume that prices and matches are determined using the SSP mechanism.  Once a strategy profile is specified
then the market dynamics become a fully specified stochastic process.
Let $(a_i^t:t\in[T])$ be the sequence of actions taken by each driver $i\in\calM$.  Set $a_i^t=\emptyset$ for any driver $i$ who hasn't entered
the market by time period $t$; otherwise $a_i^t$ is selected based on the output of driver $i$'s strategy $\pi_i^t$ for time period $t$.

Let $R_i^t$ be the reward collected by driver $i$ in time period $t$.  $R_i^t$ is determined from the action $a_i^t$ based on the
following relationship:
\begin{equation}
    R_i^t=\begin{cases}
    P_{(\ell,d)}^t - X_i^t - c_{(\ell,d)} & \mbox{if }a_i^t = (\ell,d,1),\\
        -c_{(\ell,d)} & \mbox{if }a_i^t = (\ell,d,0),\\
        0 & \mbox{if }a_i^t = \emptyset,
    \end{cases}
\end{equation}
where $P_{(\ell,d)}^t$ is the price set by the SSP mechanism for a dispatch from $\ell$ to $d$ in time period $t$, and $X_i^t$
is driver $i$'s add-passenger disutility from time period $t$.

The utility-to-go for each driver at each time period is the expected sum of rewards they collect over all future
time periods, conditioned on the market state at the beginning of the time period.
We let $U_i^t(\Pi)$ denote driver $i$'s utility-to-go in time period $t$.  Note $U_i^t(\Pi)$
depends on the market state $(\omega_t,\bfS_t)$, but we omit this dependence in the notation for simplicity.
The utility-to-go is formally defined as the expected value of the following sum:
\begin{equation}
    U_i^t(\Pi) = \bbE^\Pi\left[\sum_{\tau=t}^TR_i^\tau \mid (\omega_t,\bfS_t)\right],
\end{equation}
where $\bbE^\Pi\left[\cdot\right]$ indicates that the expectation is taken with respect to the stochastic process that arises
from fixing the strategy profile $\Pi$.

It will also be useful to think about a driver's utility-to-go conditional on the destination towards which they are dispatched.
Recall $d_i$ is the (random) destination towards which driver $i$ is dispatched, with $d_i=\emptyset$ meaning that driver $i$
is not allocated a dispatch.  Define $U_i^t(d,\Pi)$ to mean driver $i$'s utility-to-go conditioned on the event that $d_i=d$:
\begin{equation}
    U_i^t(d,\Pi) = \bbE^\Pi\left[\sum_{\tau=t}^TR_i^\tau \mid (\omega_t,\bfS_t), d_i=d\right].
\end{equation}


Informally, a strategy profile $\Pi$ is an approximate equilibrium if (almost) every driver has small incentive to deviate, regardless
of the destination they are dispatched twoards (if any). We use the 
notation $\Pi-\pi_i+\pi_i'$ to represent that driver $i$ deviates from a strategy $\pi_i$ to an alternate strategy $\pi_i'$.
The incentive-to-deviate for a driver, given a particular time period and market state, is defined as the maximum utility 
gain the driver can achieve by switching to an alternate strategy. 
Recall we use the set $\calM_t$ to index the active drivers in the marketplace.
We will use the notation $\calM_t(\delta)$ to mean the set of active drivers whose incentive-to-deviate is at most $\delta$:
\begin{equation}
    \label{eq:delta_deviation_incentive}
    \calM_t(\delta) = \left\{i\in\calM_t : \sup_d\sup_{\pi_i'} U_i^t(d;\Pi-\pi_i+\pi_i') - U_i^t(d;\Pi) \leq \delta\right\}.
\end{equation}
The exact meaning of $\calM_t(\delta)$ implicitly depends on the market state $(\omega_t,\bfS_t)$, but we omit this dependence in the notation
for clarity.
Our formal definition for $\Pi$ to be an approximate equilibrium is stated below.

\begin{definition} \label{def:approx_eqlbm} \begin{enumerate}
    \item Fix a strategy profile $\Pi$, a time period $t$, and let $\epsilon, \delta$ be two error-size parameters.
        We say that $\Pi$ is an $(\epsilon,\delta)$-approximate equilibrium at time $t$ if a proportion of at least $1-\epsilon$ of the drivers
        have at most $\delta$ incentive to deviate, for any time $t$ state.
        That is, $\Pi$ is an $(\epsilon,\delta)$-approximate equilibrium at time $t$ if the inequality 
        \begin{equation}
            \frac{|\calM_t(\delta)|}{|\calM_t|} \geq 1-\epsilon
        \end{equation}
        holds, for any set of active drivers $\calM_t$ and any market state at the beginning of time $t$.
    \item Fix a strategy profile $\Pi$ and two sequences of error terms $(\epsilon_{1:T})$ and $(\delta_{1:T})$.  We say that
        $\Pi$ is an $(\epsilon_{1:T},\delta_{1:T})$-approximate equilibrium to mean, for each time $t$,
        that $\Pi$ is an $(\epsilon_t,\delta_t)$-approximate
        equilibrium for time period $t$.
\end{enumerate}
\end{definition}


\subsection{Welfare-Robustness in the Two-Level Model}

Our main result in this paper concerns the welfare achieved by approximate-equilibrium strategy profiles.
Before stating the result, let us revisit welfare in our model and describe expected welfare as a function of the strategy profile.

Let $W_i^t$ denote the welfare generated in the action driver by $i$ at time $t$.  The welfare $W_i^t$
differs from the driver reward $R_i^t$ when driver $i$ fulfils a dispatch in time $t$; in this case, the rider collects utility
equal to the difference between their value for the trip and the trip price.  Let $V_i^t$ be the value held by the rider whose dispatch
driver $i$ fulfils in time $t$, if any such rider exists.  The welfare term $W_i^t$ is defined as follows:
\begin{equation}
    W_i^t=\begin{cases}
    R_i^t + (V_i^t - P_{(\ell,d)}^t) & \mbox{if }a_i^t=(\ell,d,1),\\
        R_i^t & \mbox{otherwise.}
    \end{cases}
\end{equation}

The total welfare generated by the marketplace is then the sum over welfare terms $W_i^t$ for all drivers $i$ and time periods $t$.
In the context of the two-level model, where the number of riders and drivers scales with the population-size parameter $k$, we
normalize the expected welfare by dividing by $k$, so that expected welfare terms are comparable across different population sizes.

Let $\Phi_{\omega_t}(\bfS_t;\Pi)$ be the expected welfare-to-go given a strategy profile $\Pi$, a population size $k$, as a function
of the market state $(\omega_t,\bfS_t)$:
\begin{equation}
    \Phi_{\omega_t}(\bfS_t;\Pi) = \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM}\sum_{\tau=t}^T W_i^\tau \mid (\omega_t,\bfS_t)\right].
\end{equation}
Notice the expected welfare term $ \Phi_{\omega_t}(\bfS_t;\Pi) $ implicitly depends on the population size parameter $k$, but we
omit this dependence from the notation for convenience.

Recall that $\Phi_{\omega_t}(\bfS_t)$ denotes the optimal value of the state-dependent optimization problem given the state $(\omega_t,\bfS_t)$,
which corresponds to the optimal welfare achievable given the state $(\omega_t,\bfS_t)$ in the stochastic fluid model.
The following Lemma states that the optimal fluid welfare is always an upper bound on the expected welfare in the two-level model.
\begin{lemma}
    Let $\Pi$ be any strategy profile and consider any time $t$ with state $(\omega_t,\bfS_t)$.
    The optimal welfare from the state $(\omega_t,\bfS_t)$ in the fluid model is always larger than the expected welfare generated by $\Pi$ in the
    two-level model, i.e.
    \begin{equation}
        \label{eq:fluid_welfare_ub}
    \Phi_{\omega_t}(\bfS_t) \geq \Phi_{\omega_t}(\bfS_t;\Pi)
    \end{equation}
    always holds.
\end{lemma}

Our main result in this subsection is to show that the bound (\ref{eq:fluid_welfare_ub}) is nearly tight whenever $\Pi$ is an approximate
equilibrium.
\begin{theorem}
    \label{thm:two_level_robustness}
    Let $\Pi$ be an $(\epsilon_{1:T}, \delta_{1:T})$-approximate equilibrium.
    Then for each $t$ there exists an error term $\gamma_t = \dots$ such that
    \begin{equation}
    \Phi_{\omega_t}(\bfS_t;\Pi) \geq \Phi_{\omega_t}(\bfS_t) - \gamma_t
    \end{equation}
    holds for all states $(\omega_t,\bfS_t)$. \mccomment{The statement of this theorem might need to change because there are low-probability
    states $(\omega_t,\bfS_t)$ for which it is hard to provide a bound}
\end{theorem}

\subsection{Proof of Theorem \ref{thm:two_level_robustness}}
Our path to proving Theorem \ref{thm:two_level_robustness} will be to construct and analyze
a feasible solution for the state dependendent optimization problem
based on the actions that drivers take under the strategy profile $\Pi$.
Let us quickly summarize the steps that the analysis will take, before diving in to their details below. 
Let $(\bff,\bfg)$ be the feasible solution we construct based on the realized actions in the current time period.
The solution is defined by the following equations:
\begin{equation}
    \label{eq:two_level_g}
     g_{(\ell,d)} = \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,1)\right\},\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
and
\begin{equation}
    \label{eq:two_level_f}
    f_{(\ell,d)} = g_{(\ell,d)} + \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,0)\right\}.\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
Note that $(\bff,\bfg)$
are random variables that depend on stochastic dispatch demand, stochastic add-passenger disutilities, as well as the randomness inherent
to the matching process.  

We prove Theorem \ref{thm:two_level_robustness} by backwards induction on the time period. Our backwards induction assumption
states that the utility-to-go of drivers at a location $\ell$ is (approximately) equal to the partial derivative of the
state-dependent optimization function, with respect to the volume of drivers at $\ell$. The proof of the inductive step 
will take the following steps:
\begin{enumerate}
    \item Show that if $\Pi$ is an $(\epsilon, \delta)$-approximate equilibrium at time $t$, then $1-\epsilon$ fraction
        of the active drivers use a common disutility acceptance threshold $\bfx$. 
    \item Show that the expected welfare under $\Pi$ in the two-level model is almost as large as the optimal fluid welfare
        under the solution $(\bff,\bfg, \bfx)$.
    \item Show that the approximate incentive-compatibility conditions on $\Pi$ imply approximate incentive-compatibility conditions
        on $(\bff,\bfg,\bfx)$.  In other words, show that $(\bff,\bfg,\bfx)$ is an approximate equilibrium for the fluid model.
    \item Show that the welfare of any approximate equilibrium for the fluid model is almost as large as the optimal welfare in the fluid model.
\end{enumerate}

The above steps are sufficient to prove Theorem \ref{thm:two_level_robustness}.  We provide details for each of the steps in the subsubsections below.

\subsubsection*{Notation Summary}
\mccomment{This is a reference subsection that summarizes and records the notation used in the following subsections.}
\begin{itemize}
    \item $\Phi_{\omega_t}(\bfS_t)$ refers to the optimal value of the state-dependent optimization problem, as a function of the market-state
        $(\omega_t,\bfS_t)$.
    \item The state-dependent optimization problem has decision variables $(\bff,\bfg)$, which are vectors indexed by pairs of locations
        $(\ell,d)\in\calL^2$, and with feasibility constraints $\bff,\bfg\geq 0$, $\bff\geq \bfg$, and $\bff^T\bfone_\ell=S_\ell$ for all $\ell$.
    \item The state dependent optimization problem has objective function $\Phi_{\omega_t}(\bff,\bfg)$, where
        \begin{equation}
            \calW_{\omega_t}(\bff,\bfg) =  \calU_{\omega_t}(\bff,\bfg)            + \bbE[\Phi_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff)].
        \end{equation}
        where $\calU_{\omega_t}(\bff,\bfg)$ is the current-period reward, defined by
        \begin{equation}
        \calU_{\omega_t}(\bff,\bfg) = \sum_{(\ell,d)} R_{(\ell,d)}(g_{(\ell,d)}) - c_{(\ell,d)}f_{(\ell,d)} - 
            \sum_\ell \bfg^T\bfone_\ell \bbE\left[X\mid X\leq C\frac{\bfg^T\bfone_\ell}{\bff^T\bfone_\ell}\right].
        \end{equation}
    \item It's possible for a fluid strategy to use a disutility acceptance threshold vector $\bfx$ that is suboptimal for the
        trips specified by $(\bff,\bfg)$.  In this case we define the function
        $\calU_{\omega_t}(\bff,\bfg,\bfx)$ to be
        \begin{equation}
\calU_{\omega_t}(\bff,\bfg,\bfx) = \sum_{(\ell,d)} R_{(\ell,d)}(g_{(\ell,d)}) - c_{(\ell,d)}f_{(\ell,d)} - 
            \sum_\ell \bfg^T\bfone_\ell \bbE\left[X\mid X\leq x_{(\ell,d)}\right].
        \end{equation}
    \item In the above equation, $X$ is a random variable with distribution $\mathrm{Uniform}(0,C)$.  We assume every driver
        has their idiosyncratic disutility sampled independently from $\mathrm{Uniform}(0,C)$ in each time period.
    \item The notation $\bfg^T\bfone_\ell$ means the total mass that $\bfg$ places on destination locations $d$ which originate
        from $\ell$.  Same with $\bff^T\bfone_\ell$.
    \item $R_{(\ell,d)}(g_{(\ell,d)})$ is a function specifying the total rider welfare generated when $g_{(\ell,d)}$ dispatches are
        served along the route $(\ell,d)$.
    \item Let $\calM_{t,\ell}$ be the set of drivers located at $\ell$ at time $t$,
\begin{equation}
    \calM_{t,\ell} = \{i\in\calM_t : \ell_i^t = \ell\}.
\end{equation}

\item For each $t$ there is a set $\calS_t$ of ``good'' market states $(\omega_t,\bfS_t)$.  The probability of being in a good state
    at time $t+1$, conditioned on being in a good state at time $t$ is $1-\epsilon$.

\end{itemize}



\subsection*{Step 1: Common Disutility Thresholds}
\mccomment{For the purpose of simplicity right now I am going to work under the assumption that \emph{every} driver
has at most $\delta$ incentive to deviate under the strategy profile $\Pi$.  This assumption isn't quite consistent with Definition 
\ref{def:approx_eqlbm}, because it ignores the $\epsilon$ fraction of drivers who might have very high incentive to deviate,
but it does seem to significantly simplify the proof details.  After finishing this draft we can revisit and decide whether to change
the definition or this assumption.}

Our first step is to show that every driver under the strategy profile $\Pi$ uses nearly the same disutility acceptance threshold.
We start by making a backwards induction assumption characterizing the utility-to-go under $\Pi$ in future time periods.

As stated above, our proof of Theorem \ref{thm:two_level_robustness} is a backwards induction argument on the time period $t$.  
Our backwards induction assumption states that, in the future time period $t+1$, the average utility-to-go is close to 
the corresponding partial derivative of the state-dependent optimization problem. 
\begin{assumption}
    \label{assn:backwards_induction}
    In the future time period $t+1$, for any market state $(\omega_{t+1},\bfS_{t+1})$, and for each location $\ell$,
    there exists an error term
    $\epsilon = \epsilon(\omega_{t+1},\bfS_{t+1})$ \mccomment{fill in details of $\epsilon$}
    such that the utility-to-go of each driver $i\in\calM_{t+1,\ell}$ is within $\epsilon$ of the
    partial derivative of the state dependent optimization function for the location $\ell$. That is,
    \begin{equation}
    \left|U_i^{t+1} - \frac{\partial}{\partial S_\ell} \Phi_{\omega_{t+1}}(\bfS_{t+1})\right| \leq \epsilon.
    \end{equation}
\end{assumption}
\mccomment{As stated, this version of Assumption \ref{assn:backwards_induction} is not fully compatible with the definition
\ref{def:approx_eqlbm} because it doesn't account for the $\epsilon$ fraction of drivers who are allowed to have large incentive-to-deviate
under Definition \ref{def:approx_eqlbm}.  I'm keeping the Assumption like this so that the first pass of the proof will be easier to write --
we can then revisit this Assumption and evaluate whether we want to change the definition to be compatible with this assumption,
or change the assumption to be compatible with the definition.}


\begin{lemma}
    \label{lem:common_threshold}
    Let $\bfx_i=(x_i^d : d\in\calL)$ be the disutility acceptance threshold used by each driver $i$ in time period $t$ under
    the strategy profile $\Pi$. Then for each location $\ell$ there exists a disutility threshold vector 
    $\bfx_\ell = (x_{(\ell,d)} : d\in\calL)$ and an error term $\epsilon$ \mccomment{TODO: fill in $\epsilon_\ell$ details} 
    such that every driver positioned at $\ell$ uses a disutility threshold that is at most $\epsilon$ distance from
    $\bfx_\ell$, i.e.
    \begin{equation}
        \max_{d\in\calL}|x_i^d - x_{(\ell,d)}|_ \leq \epsilon , \ \ \ \ \forall i\in\calM_{t,\ell}.
    \end{equation}
    The error term $\epsilon$ is equal to
    \begin{equation}
    \epsilon = 2\delta + 4\epsilon^{BI} + \frac{CL}{k},
    \end{equation}
    where $\delta$ is the approximation error in the strategy profile $\Pi$, $\epsilon^{BI}$ is the error term from
    the backwards induction assumption Assumption \ref{assn:backwards_induction}\mccomment{$\epsilon^{BI}$ is an error term
    that needs to work for every $\bfS_{t+1}$}, $C$ is a constant, $L$ is the lipschitz
    constant for the state-dependent optimization problem partial derivative, and $k$ is the population-size parameter.
\end{lemma}
\begin{proof}
    \mccomment{The definition for $\delta$-incentive compatible stated in (\ref{eq:delta_deviation_incentive}) currently states that
    a driver's deviation can depend on the destination $d$ they are allocated, but not their add-passenger disutility $X_i$.
    I think it makes sense to also let the deviation depend on the add-passenger disutility, so that the interpretation would be:
    for each destiation $d$ a driver can be allocated, and any add-passenger disutility $X_i$ they can sample, their incentive
    to deviate is at most $\delta$.  That's how I'll proceed for now.}
    Consider any two drivers $i$ and $j$ positioned at the same location $\ell$, and suppose there is some destination $d$
    for which driver $i$ uses a lower acceptance threshold than driver $j$, i.e. $x^i_d < x^j_d$.
    Let $x\in (x_i^d, x_j^d)$ be a number in between the two thresholds and
    consider the following two distinct events:
    \begin{enumerate}
    \item Driver $i$ is allocated a dispatch towards $d$ and samples $x$ as their add-passenger disutility, i.e. $d_i=d$ and $X_i=x$.
    \item Driver $j$ is allocated a dispatch towards $d$ and samples $x$ as their add-passenger disutility, i.e. $d_j=d$ and $X_j=x$.
    \end{enumerate}
    In event 1, driver $i$ rejects the dispatch towards $d$ and drives empty towards an alternate destination $d'$.
    The utility-to-go that driver $i$ collects conditioned on event 1 is thus equal to
    \begin{equation}
        U^t_i(d_i=d, X_i=x) = -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right].
    \end{equation}
    From the definition of $\Pi$ being an approximate equilibrium, we know that conditioned on event 1 the alternate action
    of accepting the dispatch towards $d$ can only increase driver $i$'s utility to go by at most $\delta$.
    This implies the inequality
    \begin{equation}
        \label{eq:event_1_first_bound}
        -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] + \delta \geq
        P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right].
    \end{equation}
    Let $Z=-c_{(\ell,d')} + \delta - P_{(\ell,d)} + x + c_{(\ell,d)}$ be a temporary variable to track the non-utility to go
    terms from the above expression, so we have
    \begin{equation}
    Z + \bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] \geq \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right].
    \end{equation}
    From the backwards induction assumption, Assumption \ref{assn:backwards_induction}, the above inequality implies
    an inequality in terms of the state-dependent optimization function partial derivatives:
    \begin{align}
        & Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})+ \epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right]\label{eq:start_line}
        \\
        \geq\ \ \ &Z + \bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right] \\
        \geq\ \ \  &\bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right]\\
        \geq\ \ \  & \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1})-\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d,1) \right].\label{eq:end_line}
    \end{align}
    In the above, $\bfS_{t+1}$ is the (stochastic) supply-location vector the time $t+1$, and $\epsilon(\omega_{t+1},\bfS_{t+1})$ is the
    error term provided in the backwards induction assumption Assumption \ref{assn:backwards_induction}.

    \mccomment{It might make sense to move the analysis in this paragraph into its own lemma}
    Now, the distribution of $\bfS_{t+1}$ in line (\ref{eq:start_line}) is not exactly the same as the distribution of $\bfS_{t+1}$ in the
    final line (\ref{eq:end_line}), because we are conditioning on driver $i$ taking two different actions.  But the distributions
    are very similar: other than the clear difference that driver $i$ will be in a different location at time $t+1$ if we condition
    on $a_i=(\ell,d',0)$ vs. if we condition on $a_i=(\ell,d,1)$, 
    the only difference between the distributions on line (\ref{eq:start_line}) and (\ref{eq:end_line}) is that in line (\ref{eq:end_line}),
    when driver $i$ accepts the dispatch, there will be one fewer dispatch to go around to the remaining drivers, so it is possible that
    one other driver selects a different action.
    Therefore, we there exists a coupling $(\bfS_1,\bfS_2)$ such that $\bfS_1$ has the same distribution as $\bfS_{t+1}\mid a_i=(\ell,d',0)$,
    $\bfS_2$ has the same distribution as $\bfS_{t+1}\mid a_i=(\ell,d,1)$, and on every sample path the realizations of $\bfS_1$ and $\bfS_2$
    are almost the same: there is always a common $\bfS_0$ such that $\bfS_0$ corresponds to the locations of all but $2$ drivers in each
    of $\bfS_1$ and $\bfS_2$.  Since each driver contributes weight $\frac{1}{k}$ to the supply-location vector, this means
    the maximum difference between $\bfS_1$ and $\bfS_2$ on any sample path is $\frac{4}{k}$.

    \mccomment{I am going to assume that the $\epsilon(\cdot,\cdot)$ error-term function has the same lipschitz
    constant as the partial derivative of the state-dep optimization function. Call this Lipschitz constant $L$}
    Using the coupling $(\bfS_1,\bfS_2)$, the inequality between (\ref{eq:start_line}) and (\ref{eq:end_line}) can be written
    as
    \begin{equation}
        \label{eq:coupling_ineq}
    Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{2})+  \epsilon(\omega_{t+1},\bfS_{1}) + \epsilon(\omega_{t+1},\bfS_{2}) \right] 
        \geq 0.
    \end{equation}
    Let $L$ be the common Lipschitz constant between the partial derivative of the state dependent optimization function, and
    the error-term function $\epsilon(\cdot,\cdot)$.  Then we have
    $$
\bbE\left[-\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{2})+\epsilon(\omega_{t+1},\bfS_{2})\right] \leq
\bbE\left[-\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{1})+\epsilon(\omega_{t+1},\bfS_{1})\right] + \frac{8L}{k},
    $$
    since the distance $\|\bfS_1-\bfS_2\|_1$ is at most $\frac{4}{k}$ on any sample path.
    Therefore equation (\ref{eq:coupling_ineq}) implies the bound
    \begin{equation*}
Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{1})+  2\epsilon(\omega_{t+1},\bfS_{1}) \right] 
        + \frac{8L}{k} \geq 0.
    \end{equation*}
    Recall the marginal distribution of $\bfS_1$ is the same distribution as the time $t+1$ supply-location vector conditioned on
    driver $i$'s action being $a_i=(\ell,d',0)$, so the above bound can be rewritten as:
    \begin{equation}
        \label{eq:event_1_final_bound}
    Z + \bbE\left[\frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1})+  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right] 
        + \frac{8L}{k} \geq 0.
    \end{equation}

    In event 2, driver $j$ accepts the dispatch and drives a passenger towards $d$.  The utility to go that driver $j$ collects
    conditioned on event 2 is equal to
    \begin{equation}
        U_j^t(d_j=d, X_j=x) = P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_j^{t+1}\mid a_j=(\ell,d,1)\right].
    \end{equation}
    From $\Pi$ being an approximate equilibrium, we know that the utility of accepting the dispatch towards $d$ is at most $\delta$ short of
    the utility from any other action, in particular it is at most $\delta$ short from the utility of taking a relocation
    trip towards driver $i$'s destination $d'$.
    This implies the inequality
    \begin{equation}
P_{(\ell,d)} - x - c_{(\ell,d)} + \bbE\left[U_i^{t+1}\mid a_i=(\ell,d,1)\right]+ \delta \geq 
        -c_{(\ell,d')} +\bbE\left[U_i^{t+1}|a_i=(\ell,d',0)\right].
            \end{equation}
    Following the same steps that took us from equation (\ref{eq:event_1_first_bound}) to (\ref{eq:event_1_final_bound}),
    we deduce the bound
    \begin{equation}
        \label{eq:event_2_bound}
    Z' + \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})  
        +  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_j=(\ell,d,1) \right] 
        + \frac{8L}{k} \geq 0,
    \end{equation}
    where
    $Z' =  -Z + 2\delta.
    $

    \mccomment{I am going to assume there is a coupling between $\bfS_{t+1}\mid a_i=(\ell,d',0)$ and $\bfS_{t+1}\mid a_j=(\ell,d,1)$
    where the sample path difference is at most $\frac{6}{k}$: $\frac{2}{k}$ difference for each of the following: $i$ drives somewhere else,
    $j$ drives somewhere else, and potentially one more driver's trip changes because the number of matches that the platform can allocate
    changes by $1$. I will either eventually expand on the details here, or add a lemma that specifically talks about this coupling argument.}
    Using \mccomment{the above comment, for now} there exists a coupling $(\bfS_1, \bfS_2)$ such that $\bfS_1$ has marginal distribution
    equal to $\bfS_{t+1}$ conditioned on driver $i$ driving empty towards $d'$, $\bfS_2$ has marginal distribution equal
    to the distribution of $\bfS_{t+1}$ conditioned on driver $j$ driving a passenger towards $d$, and the maximum distance
    between $\bfS_1$ and $\bfS_2$ on any sample path is $\frac{6}{k}$.
    Therefore (\ref{eq:event_2_bound}) implies the bound
    \begin{equation}
        \label{eq:event_2_final_bound}
    Z' + \bbE\left[\frac{\partial}{\partial S_{d}}\Phi_{\omega_{t+1}}(\bfS_{t+1}) - 
        \frac{\partial}{\partial S_{d'}}\Phi_{\omega_{t+1}}(\bfS_{t+1})  
        +  2\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0) \right] 
        + \frac{26L}{k} \geq 0,
    \end{equation}
    
    Now, recall the terms $Z$ in equation (\ref{eq:event_1_final_bound}) and $Z'$ in equation (\ref{eq:event_2_final_bound}) include an
    arbitrary disutility threshold $x$ in between $x^d_i$ and $x^d_j$.
    Let us now write $Z(x)$ and $Z'(x)$ to explicitly denote the dependence on $x$.  Next, consider what happens when we add
    the equations (\ref{eq:event_1_final_bound})
    using the threshold $x=x_i^d$ and (\ref{eq:event_2_final_bound}) using the threshold $x=x_j^d$.
    The partial derivative terms cancel, and we are left with
    \begin{equation}
        \label{eq:sum_of_bounds}
        Z(x_i^d) + Z'(x_j^d) + 4\epsilon + \frac{34L}{k} \geq 0.
    \end{equation}
    where we use $\epsilon = \bbE\left[\epsilon(\omega_{t+1},\bfS_{t+1})\mid a_i=(\ell,d',0)\right]$.
    Observe that $Z(x_i^d) + Z'(x_j^d) = x_i^d - x_j^d + 2\delta$. Therefore, we have
    \begin{equation}
        \label{eq:similar_thresholds}
    x_j^d - x_i^d \leq 2\delta + 4\epsilon + \frac{34L}{k}.
    \end{equation}

    Therefore, the Lemma holds by taking $\bfx_\ell$ to be the threshold vector $\bfx_i$ used by any driver located at $i$.

    


\end{proof}

\subsection*{Step 2: Fluid Solution is an Approximate Equilibrium}
\mccomment{In this section our goal is to show that the fluid solution $(\bff,\bfg,\bfx)$, which we constructed in the previous
section, is an approximate equilibrium for the fluid setting.  The work for this section is the following steps:
\begin{itemize}
    \item Define what we mean by fluid strategy and (approximate) fluid equilibrium.  These definitions are provided in earlier sections, though
        there is not currently a precise definition environment we can refer back to.  My plan for now is to write precise definitions
        for these terms in this section, so they may easily be referred to and so that I can be precise about what I write, and then
        the location of the definitions will move as the layout of the paper is improved.
    \item Formulate the goal ``$(\bff,\bfg,\bfx)$ is an approximate equilibrium'' as a precise mathematical statement.  The part of the definition
        that needs some care is in handling the fact that, as defined, the solution $(\bff,\bfg,\bfx)$ is a random variable which depends
        on stochastic demand.  I plan to take as simple an approach as possible here:  There exists a deterministic fluid strategy
        $(\bar{\bff}, \bar{\bfg}, \bar{\bfx})$ such that $(\bff,\bfg,\bfx)$ is close to $(\bar{\bff}, \bar{\bfg}, \bar{\bfx})$
        with high probability.
    \item Prove the precise mathematical statement formulated in the previous step. This step should be straightforward and depend on
        assumptions about Lipschitz continuity and concentration assumptions.  In the spirit of precision I'll write these assumptions
        in this section as their own Assumption environments.  In future versions of the paper, the location of these assumptions
        within the paper layout will change.
\end{itemize}}

\subsection*{Scratch Section}
\mccomment{This is a temporary section, primarily about concentration properties for random variable in the two level mdoel,
and definitions we can reference which really belong elsewhere in the paper.}
\subsubsection*{Fluid Equilibrium Concepts}

We start by defining fluid strategy profiles and (approximate) fluid equilibria.  Let $\bfS_t$ be the supply-location vector
for the current time period, and let $\bar{\bfr}=(\bar{r}_{(\ell,d)})$ be the expected volume of dispatch requests on each route
$(\ell,d)$ under the SSP prices.

\begin{definition}
Let $\bff=(f_{(\ell,d)} : (\ell,d)\in\calL^2)$ be a vector specifying the total trip volume on each route,
let $\bfg=(g_{(\ell,d)} : (\ell,d)\in\calL^2)$ be a vector specifying the dispatch trip volume on each route,
and let $\bfx = (x_{(\ell,d)} : (\ell,d)\in\calL^2)$ be a vector specifying the disutility acceptance threshold where 
$x_{(\ell,d)}$ specifies the acceptance threshold used by drivers positioned at $\ell$ when dispatched towards destination
$d$. 
    We say the tuple $(\bff,\bfg,\bfx)$ is a \emph{feasible fluid strategy}  if the following properties are satisfied:
    \begin{enumerate}
    \item Each component of $\bff,\bfg,\bfx$ is nonnegative.
    \item Total trip volume is always at least as large as dispatch trip volume, i.e. $f_{(\ell,d)} \geq g_{(\ell,d)}$ for all $d$.
    \item Dispatch trip volume is at most as large as dispatch trip demand for each route, i.e. $\bar{r}_{(\ell,d)} \geq g_{(\ell,d)}$ for all $d$.
    \item Total trip volume originating from each location matches the total volume of supply positioned at the location,
        i.e. the equality $S_\ell=\sum_d f_{(\ell,d)}$ is satisfied for every location $\ell$.
    \item The acceptance thresholds specified by $\bfx$ are compatible with the dispatch trip volumes specified by $\bfg$.
        As discussed in \mccomment{reference section}, compatibility between $\bfx$ and $\bfg$ is achieved when the
            inequality $C\sum_d \frac{g_{(\ell,d)}}{x_{(\ell,d)}} \leq S_\ell$ is satisfied for every location $\ell$    \end{enumerate}
\end{definition}

We define the Q-values associated with a fluid strategy $(\bff,\bfg,\bfx)$ to specify the expected utility that agents collect for
each type of trip. The Q-value for a relocation trip $(\ell,d,0)$ is defined by
\begin{equation}
    \calQ(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\frac{\partial}{\partial S_d}\bar{\bfS}_{t+1}(\bff)\right],
\end{equation}
and the Q-values for a dispatch trip $(\ell,d,1)$, with an add-passenger disutility value $X$, are defined by
\begin{equation}
    \calQ(\ell,d,1,X) = P_{(\ell,d)} - X + \calQ(\ell,d,0).
\end{equation}

\begin{definition}
    \label{def:fluid_eqlbm}
    A feasible fluid strategy $(\bff,\bfg,\bfx)$ is a fluid equilibrium if there exists no deviation which increases a driver's expected utility.
    The set of utility to go values that drivers at $\ell$ can achieve under $(\bff,\bfg,\bfx)$ is given by:
    \begin{align*}
        \calU(\ell) =& \left\{\calQ(\ell,d,0) : d\in\calL, f_{(\ell,d)} - g_{(\ell,d)} > 0\right\} \\
        & \ \ \cup \left\{\calQ(\ell,d,1,X) : d\in\calL, g_{(\ell,d)} > 0, 0\leq X \leq x_{(\ell,d)}\right\}.
    \end{align*}
    The set of utility to go values that drivers at $\ell$ can achieve by deviating from $(\bff,\bfg,\bfx)$ is given by:
    \begin{align*}
        \calD(\ell) =& \left\{\calQ(\ell,d,0) : d\in\calL\right\} \\
        & \ \ \cup \left\{\calQ(\ell,d,1,X) : d\in\calL, \bar{r}_{(\ell,d)} - g_{(\ell,d)} > 0\right\}.
    \end{align*}
    We say $(\bff,\bfg,\bfx)$ is an \emph{exact fluid equilibrium} if the inequality $$\min \calU(\ell) \geq \max \calD(\ell)$$ holds
    for every location $\ell$.
    We say $(\bff,\bfg,\bfx)$ is an \emph{$\epsilon$-approximate fluid equilibrium} if the inequality
$$\min \calU(\ell) \geq \max \calD(\ell)-\epsilon$$
    holds for every location $\ell$.
\end{definition}

\subsubsection*{Important Properties and Assumptions about Stochastic Two Level Model Dynamics}
We will also need to reference a number of variables which affect the stochastic dynamics of the two level model.
We summarize these variables below.

Let $\calR=(r_i\in\calL : i\in\calM_t)$ be the relocation destinations selected by each of the drivers.
\mccomment{For the remainder of the section I will operate under the assumption that drivers select a single
relocation destination, rather than a distribution of relocation destinations.  This is for simplicity.  This is
out of sync with how the driver strategy model is currently described.}

Let $\bfr = (r_{(\ell,d)} : (\ell,d)\in\calL^2)$ encode the stochastic dispatch request volume on each route $(\ell,d)$.  
We assume each $r_{(\ell,d)}$ is equal to the total number of requests along $(\ell,d)$ divided by the population-size
parameter $k$.
We assume the dispatch request volumes satisfy the concentration property stated in Assumption \ref{assn:request_concentration}.
\begin{assumption}
    \label{assn:request_concentration}
    There exists $\epsilon$ such that $\bfr$ is at most $\epsilon$ away from its mean $\bar{\bfr}$ with probability at least $1-\epsilon$.
    That is,
    \begin{equation}
        \bbP\left(\|\bfr - \bar{\bfr}\|_1 < \epsilon\right) \geq 1-\epsilon.
    \end{equation}
\end{assumption}

Let $\calX = (X_i : i\in\calM_t)$ be the stochastic add-passenger disutilities sampled by each of the drivers.
We assume the empirical distribution of the observed disutility values is close to the true cumulative distribution
for a $\mathrm{Uniform}(0,C)$ distribution. This is stated formally in Lemma \ref{lem:add_passenger_concentration}.
\begin{lemma}
    \label{lem:add_passenger_concentration}
    Suppose we have $M$ iid observations $X_1,\dots,X_M$ from a $\mathrm{Uniform}(0,C)$ distribution,
    and let $F_M(x) = \frac{1}{M}\sum_{i=1}^M \bfone_{\left\{X_i\leq x\right\}}$ be the empirical distribution function
    and let $F(x)=\frac{x}{C}$ be the true distribution function. Then, for every $\epsilon > 0$, the following holds
\begin{equation}
    \bbP\left(\sup_{x\in [0,C]}\left|F_M(x) - F(x)\right| \leq \epsilon\right) \geq 1-2e^{-2n\epsilon^2}.
\end{equation}
\end{lemma}
\begin{proof}
    \url{https://en.wikipedia.org/wiki/Dvoretzky%E2%80%93Kiefer%E2%80%93Wolfowitz_inequality}.
\end{proof}

The realized trips also depend on the matching process used by the platform, and in particular the dispatch
destination allocated to each driver.
Recall $d_i\in\calL\cup\left\{\emptyset\right\}$ indicates the dispatch destination allocated to each
driver $i$.
The matching process that the platform uses to determine the dispatch allocated to each driver depends on a number of factors.
It depends on the realized rider demand $\bfr$, it depends on the realized add-passenger disutilities $\calX$, and it depends
on an external source of randomness used to determine the order in which drivers are prioritized.  Let us parameterize this external
randomness by a random variable $U\sim\mathrm{Uniform}(0,1)$, so that the dispatch allocations $(d_i:i\in\calM_t)$ 
become deterministic conditioned on $(\bfr,\calX, U)$.
Let us write
\begin{equation}
    \calD(\bfr,\calX,U) = (d_i : i\in\calM_t)
\end{equation}
to indicate the dispatch destinations produced by the matching process, as a function of the realization of the random variables $(\bfr,\calX,U)$.

We assume that drivers can be allocated at most one dispatch, meaning that if a driver declines a dispatch they are forced to
take a relocation trip.  One consequence of this assumption is that the matching process effectively partitions the space of drivers
based on the destinations they are allocated.  For each $(\ell,d)$, let $Z_{(\ell,d)}(\bfr,\calX,U)$ be the volume of drivers positioned at
$\ell$ who are allocated a dispatch towards $d$, as a function of dispatch requests $\bfr$, add-passenger disutilities $\calX$, and the
external randomness $U$. Each $Z_{(\ell,d)}(\bfr,\calX,U)$ is defined by
\begin{equation}
    Z_{(\ell,d)}(\bfr,\calX,U) = \frac{1}{k}\left|\left\{i\in\calM_t : \ell_i=\ell, d_i=d\right\}\right|.
\end{equation}
We assume that the dispatches allocated to drivers do not change by a large amount if there is a small change in the dispatch
request volumes $\bfr$.  We formulate this assumption below, in Assumption \ref{assn:lipschitz_matching}.
\begin{assumption}
    \label{assn:lipschitz_matching}
    Let $\calX$ be any add-passenger disutility realization and let $U\in [0,1]$ be any realization of external randomness.
    Then, conditioned on $\calX$ and $U$, the size of each driver partition $Z_{(\ell,d)}$ is Lipschitz continuous when
    viewed as a function of $\bfr$.  That is, there exists a constant $L$ such that for any two request vectors $\bfr, \bfr'$
    we have
    \begin{equation}
        |Z_{(\ell,d)}(\bfr,\calX,U) - Z_{(\ell,d)}(\bfr',\calX,U)| \leq L\|\bfr - \bfr'\|_1.
    \end{equation}
\end{assumption}

Our next Lemma states that the distribution of time $t+1$ supply location vectors does not have strong dependence on
any one driver's individual actions.
\begin{lemma}
    \label{lem:supply_loc_coupling}
    Fix a time $t$ scenario $\omega_t$ and supply location vector $\bfS_t$ and let $a\in\{(\ell,d,\delta) : d\in\calL, \delta\in\{0,1\}\}$ be any 
    trip that a driver positioned at $\ell$ can take.  Fix any driver $i$ who is positioned at $\ell$. 
    Then there exists a coupling $(\bfS_1,\bfS_2)$ where
    \begin{enumerate}
    \item The marginal distribution of $\bfS_1$ is the same as the distribution of time $t+1$ supply location vectors
        conditioned on driver $i$ taking action $a$, that is $\bfS_1$ has the same distribution as $\bfS_{t+1}\mid a_i=a$.
    \item The marginal distribution of $\bfS_2$ has the same distribution as the time $t+1$ supply location
        vector without any additional information, i.e. $\bfS_2$ has the same distribution as $\bfS_{t+1}$.
    \item On any sample path, $\bfS_1$ and $\bfS_2$ differ by at most $\frac{2}{k}$, that is
        \begin{equation}
        \bbP\left(\|\bfS_1-\bfS_2\|_1 \leq \frac{2}{k}\right) = 1.
        \end{equation}
    \end{enumerate}
\end{lemma}

Our next Lemma states an important concentration property about supply location vectors.
\begin{lemma}
    \label{lem:supply_loc_concentration}
    Fix a scenario $\omega_t$ and a supply location vector $\bfS_t$.  Let 
    $\bar{\bfS}_{t+1} = \bbE[\bfS_{t+1}(\omega_{t+1},\bff)\mid\omega_t,\bfS_t]$ be the expected time $t+1$ supply location vector.
Then there exists error terms $\epsilon_0, \epsilon_1$ such that
    \begin{equation}
        \bbP\left(\|\bfS_{t+1} - \bar{\bfS}_{t+1}\|_1 \leq \epsilon_0\right) \geq 1-\epsilon_1.
    \end{equation}
\end{lemma}
Notice that the expected time $t+1$ supply location vector is a linear function of the expected trip volumes
$\bar{\bff}$:
\begin{equation}
    \bar{\bfS}_{t+1} = \sum_{\omega_{t+1}\in\Omega_{t+1}}\bbP(\omega_{t+1}\mid\omega_t)\bar{\bfS}_{t+1}(\omega_{t+1},\bar{\bff}),
\end{equation}
where $\bar{\bfS}_{t+1}(\omega_{t+1},\bar{\bff})$ is a deterministic function that includes the expected number of new arrivals
at each location, as well as the expected number of drivers arriving at each location as specified by $\bar{\bff}$.


\subsubsection*{Concentration Lemma for Two Level Model Trip Vectors}
We are ready to state our main Lemmas to accomplish step two of the proof.
Recall the random vectors $\bff$ and $\bfg$, defined in equations (\ref{eq:two_level_g}) and (\ref{eq:two_level_f}), specify the
realized total volume of total trips and dispatch trips on each route, respectively.
Define $\bar{\bff}$ and $\bar{\bfg}$ to be the expectated values
\begin{equation}
    \bar{\bff} = \bbE[\bff], \ \ \ \bar{\bfg} = \bbE[\bfg].
\end{equation}
Our first lemma is a concentration bound stating that the random variables $\bff$ and $\bfg$ are close to their
expectations with high probability.
\mccomment{Lemma \ref{lem:two_level_action_concentration} is important to relate the expected welfare under $(\bff,\bfg)$
to the welfare of the expected actions $(\bar{\bff}, \bar{\bfg})$.}
\begin{lemma}
    \label{lem:two_level_action_concentration}
    Under Assumptions \mccomment{TODO}, there exist error terms $\epsilon_0$, $\epsilon_1$ such that, with probability at least
    $1-\epsilon_1$, the random vectors $\bff$ and $\bfg$ have distance most $\epsilon_0$ from their mean.  That is,
    \begin{equation}
        \bbP\left(\|\bff - \bar{\bff}\|_1 + \|\bfg - \bar{\bfg}\|_1 \leq \epsilon_0\right) \geq 1-\epsilon_1.
    \end{equation}
\end{lemma}
\begin{proof}
    \mccomment{Establishing this result is more nuanced and complicated than I originally expected.
    The complications are related to working around the randomness inherent to the matching process used by the platform.}
\end{proof}

Let $\bfx$ be the common disutility threshold used by the drivers under $\Pi$, established in Lemma \ref{lem:common_threshold}.
Our next Lemma is to show that $(\bar{\bff}, \bar{\bfg}, \bfx)$ is an approximate equilibrium in the sense of 
Definition \ref{def:approx_eqlbm}.
Let $\bar{\calQ}$ be the Q-values associated with the fluid strategy $(\bar{\bff}, \bar{\bfg}, \bfx)$. Recall the Q-values
specify the expected utility to go values of the different actions drivers take under the specified strategy.  For relocation
trip actions $(\ell,d,0)$ the Q-value is defined by
\begin{equation}
    \bar{\calQ}(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\bfS_{t+1}(\omega_{t+1}, \bar{\bff})\right],
\end{equation}
and for relocation trip actions $(\ell,d,1)$ the Q-value is defined by 
\begin{equation}
    \bar{\calQ}(\ell,d,1, X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}
where $X\in [0,x_{(\ell,d)}]$ is any add-passenger disutility value smaller than the common acceptance threshold $x_{(\ell,d)}$
\mccomment{next steps for me: state concentration assumptions on $\bfS_{t+1}(\omega_{t+1}, \bar{\bff})$, double check that this is the
right way to think about continuation utilities in the context of the expected trip vectors, and state the Lemma asserting that
$(\bar{\bff}, \bar{\bfg}, \bfx)$ is an approximate equilibrium.}

\subsection*{Step 3: Approximate Fluid Equilibria are Approximately Welfare Optimal}
\mccomment{There are two possible approaches for this step.  Approach 1: redo steps of the exact fluid robustness  proof, carrying error
terms through the entire analysis.  Approach 2: use high-level convex analysis arguments to show that an approximate equilibrium
must be close to an exact equilibrium.}

\subsubsection*{Step N: Welfare Bounded by Fluid Solution}
Our next step is to show that the fluid welfare obtained by the strategy $(\bff,\bfg,\bfx)$ is close to the expected welfare
achieved by the approximate equilibrium strategy profile $\Pi$.
\begin{lemma}

\end{lemma}
\begin{proof}
    Observe that the expected welfare under $\Pi$ can be deconstructed as follows.
    \begin{align*}
        \Phi_{\omega_t}(\bfS_t;\Pi) &= \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM}\sum_{\tau=t}^T W_i^\tau \mid (\omega_t,\bfS_t)\right]\\
        &=\frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM_t}W_i^t\right] + \bbE^\Pi\left[\Phi_{\omega_{t+1}}(\bfS_{t+1};\Pi) \mid (\omega_t,\bfS_t)\right]\\
        &\geq \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM_t}W_i^t\right] + 
                \bbE\left[\Phi_{\omega_{t+1}}(\bfS_{t+1})\mid (\omega_t,\bfS_t)\right] - \gamma,
    \end{align*}
    where $\Phi_{\omega_{t+1}}(\bfS_{t+1})$ is the optimal fluid welfare from the state $\bfS_{t+1}$.
\end{proof}


==> convex_opt_lem_fixed.tex <==
Consider a two-timeperiod problem with only two routes.  Suppose the objective function
is
$$
\calU(\bff) = \sum_{r\in R} U_r(f_r) + \calW(\bff),
$$
where $\bff=(f_r : r\in R)$ specifies the amount of flow along each route. 
Each route $r\in R$ has a unique origin location $l^-(r)\in L$ and there is $S_l$ supply
positioned at each location, producing the capacity constraint $g_l(\bff)=0$ for
each location $l\in L$, where
$$
g_l(\bff) = \sum_{r\in A^+(l)} f_r - S_l.
$$
We also have a nonnegativity constraint 
$\bff \geq 0$.



Let $\bfalpha=(\alpha_r : r\in R)$ be a dual variable associated with the
nonnegativity constraints $\bff\geq 0$, and let $\bfeta = (\eta_l : l\in L)$
be a dual variable associated with the equality constraints $g_l(\bff) = 0$.
The Lagrangian function for our problem is defined as
$$
L(\bff,\bfeta,\bfalpha) = \calC(\bff) + \sum_l\eta_lg_l(\bff) - \sum_r \alpha_r f_r, 
$$
and the dual function is
$$
\Phi(\eta,\bfalpha) = \inf_{\bff}L(\bff,\eta,\bfalpha).
$$
Weak duality states $$\calC(\bff) \geq \Phi(\eta,\bfalpha)$$ for any feasible
$\bff$ and any dual variables $\eta$, $\bfalpha\geq 0$.

Since the definition of $\Phi(\eta,\bfalpha)$ is in terms of an unconstrained
infimum over $\bff$, the primal solution $\bff$ achieving the infimum
is any solution for which the gradient is zero.
We compute the partial derivatives of $L(\bff,\eta,\bfalpha)$ 
with respect to each component $f_r$ 
as follows:
\begin{equation}
\label{eq:partial}
\frac{\partial}{\partial f_r}L(\bff,\eta,\bfalpha) = 
\frac{\partial}{\partial f_r}\calC(\bff)
+ \eta_{l^-(r)} - \alpha_r=0
\end{equation}

.

.

.

Our optimality conditions state $\bff^*$ is optimal if there exists a dual variable $\bfeta^* = $
such that
$$
\eta^* \geq \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bff^*)
$$
holds for $i=1,2$, and we need the above inequality to be tight when $f_i>0$.

Now suppose we have a candidate solution $\bar{\bff} = (\bar{f}_1,\bar{f}_2)$ and a variable 
$\bar{\eta}$ satisfying the following for $i=1,2$:
$$
\bar{\eta} \geq \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bar{\bff}),
$$
and the above inequality is tight when $\bar{f}_i>0$.
This is almost the optimality condition stated above, except the $\frac{d}{df_i}U_i(f_i^*)$
term still depends the $f_i^*$ component of an optimal solution, 
rather than the $\bar{f}_i$ component of the solution of interest.
Is this sufficient to conclude that $\bar{\bff}$ is an optimal solution?

.

.

.

Computing the partial derivatives of $L(\cdot,\cdot,\cdot)$ gives us an
approach for bounding the suboptimality of an arbitrary feasible solution.
Let $\bff$ be an arbitrary feasible solution, let $\eta,\bfalpha\geq 0$ be
feasible dual variables for which the partial derivatives $\frac{\partial}{\partial f_i}L(\bff,\eta,\bfalpha)$ equal $0$ for $i=1,2$, and let $\bff^*$ be an
optimal primal solution.  Since the partial derivatives are $0$ we have
$\Phi(\eta,\bfalpha)=L(\bff,\eta,\bfalpha)$, so we can bound the suboptimality
of $\bff$ as follows:
\begin{align*}
    \calU(\bff^*) -\calU(\bff) & \leq -\Phi(\eta,\bfalpha) - \calU(\bff) \\
    & = \calU(\bff) - \eta(f_1 + f_2 - S) + \alpha_1f_1 + \alpha_2f_2 - \calU(\bff)\\
    & = \alpha_1f_1 + \alpha_2f_2.
\end{align*}
So, for an arbitrary feasible solution $\bff$, if we can find feasible dual
variables $(\eta,\bfalpha)$ for which the partial derivatives (\ref{eq:partial})
are $0$, then the suboptimality of $\bff$ is bounded by the complementary slackness
violation $\bfalpha^T\bff$.

Now, let's return to our candidate solution $\bar{\bff}$ for which we have
dual values $\bar{\eta}$, $\bar{\bfalpha}\geq 0$ satisfying the following:
$$
\bar{\eta} = \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bar{\bff}) + \bar{\alpha}_i,
$$
in addition to complementary slackness conditions $\bar{\alpha}_i\bar{f}_i=0 $. 
\mccomment{We could try replacing $\bar{\alpha}_i$ with $\bar{\alpha}_i - \frac{d}{df}U_i(f_i^*) -
\frac{d}{df}(U_i(\bar{f}_i))$ but that might violate feasibility of $\bar{\bfalpha}$}


==> driver_strategies.tex <==
After prices filter demand and dispatch requests are realized for each route, the platform
operates a matching process that is responsible for allocating dispatch requests to available drivers.
In this section we describe our assumptions about how drivers interact with the matching process.
We will discuss our detailed assumptions about the matching process in Section \mccomment{ref}

We assume that drivers sample an \emph{add-passenger disutility} in each time period,
which models the idiosyncratic cost that a driver  incurs for fulfilling a dispatch trip (i.e. adding a passenger
to their car) in that time period.  At each time period $t$, let $X_i$ be the add-passenger disutility value
sampled by each active driver $i\in\calM_t$. For simplicity we assume the add-passenger disutilities are sampled
iid from a $\mathrm{Uniform}(0,C)$ distribution, for some constant $C>0$.

\mccomment{continue from here. describe how drivers respond to a dispatch towards location $d$, and define
a driver strategy as a function from $\Omega_t\times\calS$ to $(\bfx_i, r_i)$.}


==> dual_variable_utility_proof.tex <==
\begin{proof}
    \mccomment{Eventually I think this proof belongs in the appendix, but I'll leave it in the main text for now.}
We prove the Lemma by backwards induction on the time period.  We take time $T+1$ as our base case, for which there is nothing to prove.

    For the induction step, consider any location-time-scenario $(\ell,\omega_t)\in\calN$ and suppose the equality $\calV(\ell',\omega'_{t'})=\eta_{(\ell',\omega'_{t'})}$
    holds for all location-time-scenarios $(\ell',\omega'_{t'})$ from future time periods $t'>t$.
    For any destination location $d\in\calL$ define $R_{(\ell,d,\omega_t)}$ to be the average additional utility collected by drivers who
    serve a dispatch along route $(\ell,d,\omega_t)$, above and beyond the utility
    collected by drivers who take a relocation trip along $(\ell,d,\omega_t)$.
    We refer to $R_{(\ell,d,\omega_t)}$ as the dispatch reward for route $(\ell,d,\omega_t)$.  
    The dispatch reward $R_{(\ell,d,\omega_t)}$ can be written as follows:
    \begin{align} 
        R_{(\ell,d,\omega_t)} &= \calQ(\ell,d,\omega_t,1) - \calQ(\ell,d,\omega_t,0)\\
        &= P_{(\ell,d,\omega_t)} - \frac{C}{2}\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\\
        &= F_{(o,d,\omega_t)}^{-1}\left(1-\frac{g_{(o,d,\omega_t)}}{\bar{D}_{(o,d,\omega_t)}}\right)
            - \frac{C}{2}\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}
    \end{align}
    Recall the stationarity condition (\ref{eq:stationarity_g}) relates the difference between the 
    lowest willingness-to-pay rider and the highest add-passenger-disutility driver to the dual variables as follows:
    $$
F_{(o,d,\omega_t)}^{-1}\left(1-\frac{g_{(o,d,\omega_t)}}{\bar{D}_{(o,d,\omega_t)}}\right)
            - C\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}} = \gamma_{(\ell,d,\omega_t)} - \beta_{(\ell,d,\omega_t)}.
    $$
    Here, $\gamma_{(\ell,d,\omega_t)}$ is the dual variable associated with the $g_{(\ell,d,\omega_t)} \leq f_{(\ell,d,\omega_t)}$ constraint,
    and $\beta_{(\ell,d,\omega_t)}$ is the dual variable associated with the nonnegativity constraint $\beta_{(\ell,d,\omega_t)}\geq 0$.
    Therefore, the average add-passenger disutility on route $(\ell,d,\omega_t)$ can be expressed as follows:
    \begin{equation}
        R_{(\ell,d,\omega_t)} = \frac{C}{2}\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}} + \gamma_{(\ell,d,\omega_t)} - \beta_{(\ell,d,\omega_t)}.
    \end{equation}

    We can now express the node-associated utility-to-go values $\calV(\ell,\omega_t)$ in terms of the dispatch-rewards $R_{(\ell,d,\omega_t)}$ as follows:
    \begin{align}
        \calV(\ell,\omega_t) &= \frac{1}{\bff^T\bfone_{(\ell,\omega_t)}}\sum_{d\in\calL}\left[f_{(\ell,d,\omega_t)}\calQ(\ell,d,\omega_t,0) + 
                            g_{(\ell,d,\omega_t)}R_{(\ell,d,\omega_t)}\right]\nonumber\\
                    &= \frac{1}{\bff^T\bfone_{(\ell,\omega_t)}}\sum_{d\in\calL}\left[f_{(\ell,d,\omega_t)}\left(
                    \bbE_{\omega_{t+1}}\left[\calV(d,\omega_{t+1})\mid\omega_t\right] - c_{(\ell,d,\omega_t)}\right) + 
                            g_{(\ell,d,\omega_t)}R_{(\ell,d,\omega_t)}\right]\nonumber\\
                    &=\sum_{d\in\calL}
                    \frac{f_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\left(
                    \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d,\omega_t)}\right) + 
                            \sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}R_{(\ell,d,\omega_t)}.\label{eq:node_utility_expr}
    \end{align}
    where the last line follows from the induction hypothesis.
    The second term in the final expression above,
    $$
\sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}R_{(\ell,d,\omega_t)},
    $$
    is equal to the expected dispatch reward over all drivers positioned at $(\ell,\omega_t)$, including those drivers who do not serve a 
    dispatch trip and collect $0$ dispatch reward.
    We proceed by expanding this average dispatch reward in terms of the optimal dual variables:
    \begin{align}
        \sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}R_{(\ell,d,\omega_t)} &= 
        \sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}
            \left(\frac{C}{2}\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}} 
            + \gamma_{(\ell,d,\omega_t)} - \beta_{(\ell,d,\omega_t)}\right)\nonumber\\
        &= \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)^2 
        + \sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}(\gamma_{(\ell,d,\omega_t)}-\beta_{(\ell,d,\omega_t)})}{\bff^T\bfone_{(\ell,\omega_t)}}\nonumber\\
        &= \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)^2 
        + \sum_{d\in\calL}\frac{f_{(\ell,d,\omega_t)}(\gamma_{(\ell,d,\omega_t)}+\alpha_{(\ell,d,\omega_t)})}{\bff^T\bfone_{(\ell,\omega_t)}}\nonumber\\
        &=\sum_{d\in\calL}\frac{f_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\left(
            \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)^2 +
            \gamma_{(\ell,d,\omega_t)}+\alpha_{(\ell,d,\omega_t)}\right).\label{eq:avg_reward_expr}
    \end{align}
    The second last line above follows from the complementary slackness conditions, which say that 
    $$g_{(\ell,d,\omega_t)}\gamma_{(\ell,d,\omega_t)}=f_{(\ell,d,\omega_t)}\gamma_{(\ell,d,\omega_t)},$$ and 
    $$g_{(\ell,d,\omega_t)}\beta_{(\ell,d,\omega_t)}=0=f_{(\ell,d,\omega_t)}\alpha_{(\ell,d,\omega_t)}.$$
    Plugging (\ref{eq:avg_reward_expr}) back into (\ref{eq:node_utility_expr}), we expand our expression for the node-associated utility-to-go,
    using the optimality conditions (\ref{eq:stationarity_f}):
    \begin{align}
    \calV(\ell,\omega_t) &= 
        \sum_{d\in\calL}
                    \frac{f_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\left(
                    \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d,\omega_t)}\right) + 
                            \sum_{d\in\calL}\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}R_{(\ell,d,\omega_t)}\nonumber\\
        &= \sum_{d\in\calL}\frac{f_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\left(
        \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d,\omega_t)} + \gamma_{(\ell,d,\omega_t)} + \alpha_{(\ell,d,\omega_t)}
        + \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)^2 
        \right)\nonumber\\
        &= \sum_{d\in\calL}\frac{f_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\eta_{(\ell,\omega_t)}\nonumber\\
        &= \eta_{(\ell,\omega_t)}.\label{eq:node_utility_final_expr}
    \end{align}
    The third line follows directly from the second line given the stationarity condition (\ref{eq:stationarity_f}).
    The equality $\calV(\ell,\omega_t)=\eta_{(\ell,\omega_t)}$, established in (\ref{eq:node_utility_final_expr}), concludes the proof of Lemma \ref{lem:dual_variable_utility}.

\end{proof}




==> eqlbm_strategies.tex <==
We assume that drivers play according to an equilibrium of the game induced by the platform pricing policy.
In the stochastic two-level model we use an approximate notion of equilibrium, where the approximation error
vanishes in the large-market where we take the population-size parameter $k$ to infinity.
In the stochastic fluid model, we use an exact notion of equilibrium that corresponds to a mean-field equilibrium of the large-market limit.

For simplicity, and without loss of generality, we restrict our attention to anonymous driver strategies, in which a driver's
trip-allocation and expected utility-to-go depends only on their location.
Further, we avoid explicitly modeling the process through which the platform allocates dispatches to individual drivers;
instead, we view this as part of a trip-allocation process which influences the outcome of an equilibrium driver strategy-profile.

\begin{definition}
A supply-location vector $\bfS=(S_\ell:\ell\in\calL)$ specifies the volume of drivers $S_\ell$ positioned at each location $\ell$.
For a population-size parameter $k$, a supply-location vector $\bfS$ is feasible if and only if every component is a nonnegative integer
multiple of the agent-size $1/k$.  Define 
$$
\calS^k=\left\{\frac{i}{k} : i=0,1,2,\dots\right\}^\calL
$$
to be the set of feasible supply-location vectors under population-size $k$.
For the fluid model, which corresponds to $k=\infty$, define
$$
\calS^\infty = \bbR_+^\calL.
$$
\end{definition}

\begin{definition}
A trip-allocation vector $\bfh=(h_{(r,\delta)} : (r,\delta)\in\calR\times\{0,1\})$ specifies the volume of drivers
$h_{(r,\delta)}$ who take each trip $(r,\delta)$.  
For a population-size $k$, a supply-location vector $\bfS\in\calS^k$, and a dispatch-demand vector 
$\bfd\in\left\{\frac{i}{k}:i=0,1,2,\dots\right\}^\calR$, a trip-allocation vector $\bfh$ is feasible if and only if
every component is a nonnegative integer multiple of $\frac{1}{k}$, the volume of drivers $h_{(r,\delta)}$ serving a dispatch trip on each route $r$
does not exceed the amount of dispatch demand $d_r$ for that route, and the total driver volume on outgoing trips from each location $\ell$ is the
same as the total volume of drivers positioned at $\ell$.
Define
$$
\calH^k(\bfS, \bfd) = \left\{\bfh \mbox{ satisfies (\ref{eq:trip_alloc_supply_constraint}) and (\ref{eq:trip_alloc_dispatch_constraint})} : \bfh\in\left\{\frac{i}{k} : k=0,1,2,\dots\right\}^{\calR\times\{0,1\}}\right\}
$$
\begin{equation}
\label{eq:trip_alloc_supply_constraint}
\forall \ell\  S_\ell = \sum_{r\in A^+(\ell)}\sum_{\delta\in\{0,1\}} h_{(r,\delta)}.
\end{equation}
\begin{equation}
\label{eq:trip_alloc_dispatch_constraint}
\forall r\ h_{(r,1)} \leq d_r.
\end{equation}

For the stochastic fluid model, which corresponds to $k=\infty$, define
$$
\calH^\infty(\bfS, \bfd) = \left\{\bfh \mbox{ satisfies (\ref{eq:trip_alloc_supply_constraint}) and (\ref{eq:trip_alloc_dispatch_constraint})} : \bfh\in\bbR_+^{\calR\times\{0,1\}}\right\}.
$$
\end{definition}

Let's maybe introduce the notation
$$
\bbN_k = \left\{\frac{i}{k}:i=0,1,2,\dots\right\}.
$$

\begin{definition}
A driver strategy-profile is a function which maps the state of the marketplace to an action-profile specifying the actions taken
by each driver in the current time period.  

Formally, for a population-size parameter $k$, 
a strategy-profile is a function $H_k:\bbN_k^\calL\times\bbN_k^\calR\times\Omega_{1:T}\to\bbN_k^{\calR\times\{0,1\}}$ which takes as input
a supply-location vector $\bfS\in\bbN_k^\calL$, a dispatch demand vector $\bfd\in\bbN_k^\calR$, and a time-scenario $\omega_t\in\Omega_{1:T}$,
and produces a trip-allocation vector $\bfh=H_k(\bfS,\bfd,\omega_t)\in\bbN_k^{\calR\times\{0,1\}}$ such that $\bfh$ is a feasible trip-allocation
vector with respect to the market state, i.e. $\bfh\in\calH^k(\bfS,\bfd)$. 
\end{definition}

\pfcomment{Can say something like, ``Note that we only consider pure equilibria.  Our results extend to mixed equilibria because... We choose to focus on pure equilibria to simplify notation.''}

We assume drivers use an anonymous strategy-profile $H$, so the trips specified by the action-profile $\bfh=H(\bfS,\bfd,\omega_t)$
are allocated uniformly across drivers. Specifically, for each location $\ell\in\calL$, each of the $S_\ell$ drivers positioned at
$\ell$ is allocated the trip $(r,\delta)\in A^+(\ell)\times\{0,1\}$ with probability proportional to $h_{(r,\delta)}$.
\Xomit{
\begin{definition}
For an action-profile $\bfh=(h_{(r,\delta)} : (r,\delta)\in\calR\times\{0,1\})$, the notation $\bfh(\ell)$ indicates the distribution
over trips $(r,\delta)\in A^+(\ell)\times\{0,1\}$ allocated to a driver positioned at $\ell$. Let $(\hat{r},\hat{\delta})\sim\bfh(\ell))$
denote a random trip type sampled from the trip-allocation distribution for location $\ell$.  The probability that a realization of this trip type
equals a particular trip type $(r,\delta)\in A^+(\ell)\times\{0,1\}$ is given by
\begin{equation}
\bbP((\hat{r},\hat{\delta})= (r,\delta)) = \frac{h_{(r,\delta)}}{S_\ell}.
\end{equation}
\end{definition}
}

The utility-to-go specifies the expected utility collected by a drivers over all remaining time periods, from their current state.

\begin{definition}
Fix a time period $t$, a scenario $\omega_t$, a pricing
protocol $P$, and a driver strategy-profile $H$.  Let 
$\bfS_t$ be a supply-locatino vector, fix
any location $\ell\in\calL$.  
Let $\calQ_{\omega_t}(r,\delta,\bfh)$ denote the expected utility-to-go associated with a trip-type $(r,\delta)$,
and let $\calV_{(l,\omega_t)}(\bfS)$ denote the expected utility-to-go associated with a location $(\ell,\omega_t)$. 
These depend implicitly on $P$ and $H$, but we suppress this dependence in the notation for simplicity.
The two are defined
recursively as follows:
\begin{equation}
\calQ_{\omega_t}(r,\delta,\bfh)= \begin{cases}
\delta P_r(\bfS) - c_{(r,\omega_t)} & \mbox{if } t=T,\\
\delta P_r(\bfS) - c_{(r,\omega_t)} + \bbE[\calV_{(\ell^+(\hat{r}),\omega_{t+1})}(\bfS_{t+1}(\bfh))] & \mbox{if } t<T.
\end{cases}
\end{equation}
\begin{equation}
\calV_{(\ell,\omega_t)}(\bfS) = \bbE\left[\sum_{(r,\delta)\in A^+(\ell)\times\{0,1\}} \frac{h_{(r,\delta)}}{S_\ell} \calQ_{\omega_t}(r,\delta,\bfh)\right]
\end{equation}
where the expectation is taken over the randomness in the rider demand, which translates into a trip allocation $\bfh$ via $\bfh = H(\bfS)$ and $\bfS$ contains $D$.
\end{definition}
The following definition states what it means for a strategy-profile to be incentive-compatible from a particular market-state $(\omega_t,\bfS_t)$.


\begin{definition} \emph{$(\beta_k,\epsilon_k)$ incentive-compatibility in the two-level model.}
Consider the stochastic two-level model with population-size parameter $k$. Fix a pricing protocol $P$, a driver strategy-profile $\Pi$, 
any time-scenario $\omega_t$, any supply-location vector $\bfS_t$,
and consider any driver located at a location $\ell$.  Let $\hat{\bfh}$ be the (random) action-profile arising in the current time period,
and let $(\hat{r},\hat{\delta})$ be the (random) trip allocated to the driver positioned at $\ell$.
We say  $\Pi$ is $(\beta_k,\epsilon_k)$ incentive-compatible at $\ell$, under the state $\bfS_t$ and $\omega_t$, with respect to the pricing protocol $P$ and 
the strategy-profile $H$ if there exists an upper bound on the Q-factor $Q_\ell^{\max}$ such that the probability of being allocated an action within $\epsilon_k$
of $Q_\ell^{\max}$ is at least $\beta_k$.
We say $\Pi$ is $(\beta_k,\epsilon_k)$ incentive-compatible at $\omega_t,\bfS$ if it is $(\beta_k,\epsilon_k)$ incentive-compatible at every location:
$$
    \forall \ell\  \bbP_k^\ell\left(\calQ_{\omega_t}(\hat{r},\hat{\delta},\hat{\bfh}) \geq \bar{Q}_\ell-\epsilon_k\right) \geq \beta_k,
$$
    where $\bbP_k^\ell$ is the probability measure over $(\hat{r},\hat{\delta},\hat{\bfh})$ from location $\ell$...... is a joint random variable, whose distribution depends on the location $\ell$,
    over the trip-vector $\hat{\bfh}$ and the trip-allocation $\hat{r},\hat{\delta}$
    allocated to an individual driver located at $\ell$.
\end{definition}

\mccomment{mention somewhere that the relevant state for the beginning of strategic considerations is $\omega_t$, $\bfS$.}

\begin{definition} \emph{Incentive-compatibility in the fluid model.}
Consider the stochastic fluid model.  Fix a pricing protocol $P$, a driver strategy-profile $\Pi$, a time-scenario $\omega_t\in\Omega_{1:T}$, 
a supply-location vector $\bfS\in\bbR_+^\calL$.  Let $\bfh=\Pi(\omega_t,\bfS,\bfd)$ be the trip-allocation vector that arises deterministically
under $\Pi$, $P$, conditioned on $\omega_t$ (where $\bfd$ is the dispatch demand vector that arises deterministically under $P$, $S$ and $\omega_t$).
We say $\Pi$ is incentive-compatible at location $\ell$ with respect to $P$, $\bfS$, $\omega_t$, if there exists a constant $Q_\ell$ such that,
for every outgoing trip type $(r,\delta)\in A^+(\ell)\times\{0,1\}$ with $h_{(r,\delta)} > 0$ we have
$$
\calQ_{\omega_t}(r,\delta,\bfh)=Q_\ell,
$$
and 
$$
\calQ_{\omega_t}(r,\delta,\bfh)\leq Q_\ell
$$
holds for all $(r,\delta)\in A^+(\ell)\times\{0,1\}$.

We say $\Pi$ is incentive-compatible with respect to $P$, given the market-state $(\omega_t,\bfS_t)$, if the above incentive-compatibility condition
holds for every location.
\end{definition}

\begin{definition}
\mccomment{do we need a definition about consistency of strategy-profile $\Pi$ as a function of $k$?}
\end{definition}

Note that in both the stochastic two-level model and the stochastic fluid model, 
fixing a pricing protocol $P$ and a strategy-profile $\Pi$ turns the stochastic sequence of market-states $((\omega_t,\bfS_t) : t\in [T])$
into a Markov chain. Fix a sequence of pricing protocols $(P_k : k\in\bbN_+)$ and strategy-profiles $(\Pi_k : k\in\bbN_+)$ for the
two-level model with population-size $k$, which converge to $P$ and $\Pi$ for the fluid model.
Let $\calS_t^k$ be the state-space for the market-state Markov chain induced by $(P_k,\Pi_k)$ at time $t$ in the two-level model with population-size $k$,
and let $\calS_t^\infty$ be the state-space for the market-state Markov chain induced by $(P,\Pi)$ in the fluid model.
Let $\bbP_t^k$ be the distribution over $\calS_t^k$ induced by $(P_k,\Pi_k)$ and let $\bbP_t^\infty$ be the distribution over $\calS_t^\infty$ induced by $(P,\Pi)$.



==> eqlbm_welfare_optimality.tex <==
The purpose of this section is to prove (possibly a slight variant of)
Theorem \ref{thm:general_eqlbm} using the generic convex optimization
lemma Lemma \ref{lem:generic_cvxopt}.  Throughout this section we hold
fixed a time $t$ and scenario $\omega_t$.  Let $H$ be any driver
strategy profile that is an asymptotic equilibrium with respect 
to the SSP pricing policy $P^{SSP}$.  Let $(\bfS_t^k)_{k=1}^\infty$
be a sequence of supply-location vectors, such that the $k$th entry
is in the support of the distribution of supply-location vectors
under population-size $k$, and assume the supply-location vectors
converge: $\lim_{k\to\infty}\bfS_t^k=\bar{\bfS}_t$.

Consider the stochastic
maximum flow optimization problem with respect to the limiting supply-location vector $\bar{\bfS}_t$:
\begin{equation}
\label{eq:single_period_opt_flow}
\calW_{\omega_t}(\bar{\bfS}_t) = \sup_{\bff\geq 0}\left(
\sum_{(r,\omega_t)\in\calA_{\omega_t}^t}U_{(r,\omega_t)}(f_{(r,\omega_t)})
+ \bbE\left[\calW_{\omega_{t+1}}(\bff)\right] : 
\forall (l,\omega_t)\ \bar{S}_{(l,\omega_t)} = 
\sum_{\substack{(r,\omega_t)\in\\ A^+_{\omega_t}(l)}}f_{(r,\omega_t)}
\right).
\end{equation}
The objective function consists of the route-specific utility
functions $U_{(r,\omega_t)}(\cdot)$ and the continuation
welfare $\bbE[\calW_{\omega_{t+1}}(\bff)]$. The expectation is taken
over time $t+1$ scenarios $\omega_{t+1}$, conditional on the time $t$
scenario $\omega_t$.  When we write the continuation utility 
$\calW_{\omega_{t+1}}(\bff)$ as a function of the flow $\bff$, 
we formally mean the continuation utility 
$\calW_{\omega_{t+1}}(\bar{\bfS}_{t+1})$ as a function of the
time $t+1$ supply-location vector $\bar{\bfS}_{t+1}$, where
$\bar{\bfS}_{t+1}$ is a deterministic function of $\bff$
and the scenario $\omega_{t+1}$.
To analyze the above optimization problem in the context
of Lemma \ref{lem:generic_cvxopt}, we take the cost function
in Lemma \ref{lem:generic_cvxopt} to be the negative  objective function
in (\ref{eq:single_period_opt_flow}).  This objective is
continuously differentiable under our uniqueness assumption,
Assumption \mccomment{insert}, as shown by Lemma \ref{lem:marginal_utility}.

Next, we show that trip-allocation vectors arising from an
asymptotically subgame perfect strategy profile $H$ give us random
approximately feasible solutions for the problem
(\ref{eq:single_period_opt_flow}) which satisfy the conditions of
Lemma \ref{lem:generic_cvxopt}.  Let $\bfh_k=H(t,\omega_t,k,\bfS_t^k,\bfd_t)$ be the random trip-allocation
vector produced under $H$ and population-size $k$.  Recall the trip-allocation
vector distinguishes between relocation-trips $h_{(r,\omega_t,0)}$ and
dispatch-trips $h_{(r,\omega_t,1)}$ on each active route $(r,\omega_t)$.
Define the flow associated with $\bfh_k$ to be the vector $\bff_k$ of trip counts that
drops this distinction: the components of $\bff_k$ are indexed by active
routes $(r,\omega_t)\in\calA_{\omega_t}^t$ and each component is given by
$ f^k_{(r,\omega_t)} = h^k_{(r,\omega_t,0)} + h^k_{(r,\omega_t,1)}$.

We will show that the sequence $\bff_1,\bff_2,\dots $ satisfies the conditions
from Lemma \ref{lem:generic_cvxopt}.  First, $\bff_k\geq 0$ almost surely follows
from $\bfh_k\geq 0$ holding almost surely.  Second, the amount by which each $\bff_k$
violates the equality constraints in (\ref{lem:generic_cvxopt}) converges to $0$
because each $\bff_k$ exactly satisfies the equality constraints with respect to 
$\bfS_t^k$, and we assumed the sequence $\bfS_t^k$ converges to $\bar{\bfS}_t$.

The next two conditions we must show the sequence $(\bff_k)$ satisfies are more
involved.  Both of these conditions depend on a sequence of approximate dual 
variables $(\bfeta_k)$, and are stated in terms of the following functions,
indexed by active routes $(r,\omega_t)\in\calA_{\omega_t}^t$:
\begin{align*}
D_{(r,\omega_t)}(\bff,\bfeta) &=\eta_{(l^-(r),\omega_t)}
-\frac{d}{d f}U_{(r,\omega_t)}(f_{(r,\omega_t)})
- \bbE\left[\frac{\partial}{\partial f_{(r,\omega_t)}}\calW_{\omega_{t+1}}(\bff)\right] \\
&= \eta_{(l^-(r),\omega_t)}
-\rho_{(r,\omega_t)}(f_{(r,\omega_t)}) + c_{(r,\omega_t)}
- \bbE\left[\frac{\partial}{\partial f_{(r,\omega_t)}}\calW_{\omega_{t+1}}(\bff)\right] 
\end{align*}
where $\rho_{(r,\omega_t)}(f_{(r,\omega_t)})$ is the welfare-maximizing
price (\ref{eq:max_welfare_price}) if as a function of the flow $f_{(r,\omega_t)}$
traversing the route.
To define the sequence $(\bfeta_k)$, let each $\bfeta_k$ be a vector
indexed by active locations $(l,\omega_t)\in\calN_{\omega_t}^t$,
where the $(l,\omega_t)$ component of the $k$th iterate is equal to
the expected utility-to-go of a driver positioned at $(l,\omega_t)$:
$$
\eta^k_{(l,\omega_t)} = \calV^k_{(l,\omega_t)}(\bfS_t^k;H,P^{SSP}).
$$
We must show that the following limits
$$
f^k_{(r,\omega_t)} D_{(r,\omega_t)}(\bff_k,\bfeta_k)\to 0,\ \ \ 
\mbox{and} \ \ \ 
\min(D_{(r,\omega_t)}(\bff_k,\bfeta_k), 0)\to 0
$$
both converge in probability.


==> fluid_robustness_proof.tex <==
\medskip\noindent\textbf{Preliminaries}
Let $(\bfg^*,\bff^*,\bfx^*)$ be the welfare-optimal equilibrium that the SSP mechanism uses to compute prices,
and let $(\bfg',\bff',\bfx')$ be an arbitrary equilibrium which is induced by the SSP mechanism.
We know the following properties are satisfied:
\begin{itemize}
    \item The volume of dispatches served under the arbitrary equilibrium can be at most the volume of
        dispatch requests that are created under the SSP prices.  Since the SSP mechanisms sets prices so that
        dispatch-supply and dispatch-demand are balanced on each route, the following inequality holds for every
        route $(\ell,d)$:
        \begin{equation}
            \label{eq:dispatch_volume_ub}
        g'_{(\ell,d)} \leq g^*_{(\ell,d)}.
        \end{equation}
    \item A priori, it is possible for an arbitrary equilibrium to serve fewer dispatches than there are dispatch requests
        on any given route, i.e. the inequality (\ref{eq:dispatch_volume_ub}) may be strict.  In these cases, we know that
        the dispatch acceptance threshold the arbitrary equilibrium is using must be strictly smaller than the optimal dispatch
        acceptance threshold:
        \begin{equation}
            \label{eq:threshold_property}
            g'_{(\ell,d)} < g^*_{(\ell,d)} \implies x'_{(\ell,d)} < x^*_{(\ell,d)}.
        \end{equation}
\end{itemize}
Let $\calQ^*$ and $\calQ'$ denote the utility-to-go values for the equilibria $(\bfg^*,\bff^*,\bfx^*)$ and
$(\bfg',\bff',\bfx')$, respectively.  Let $(\bfg,\bff,\bfx)$ denote either of the equilibria under consideration,
and let $\calQ$ denote the corresponding utility-to-go values.  We know the utility-to-go values for
any equilibrium under the SSP prices satisfy the following properties:
\begin{itemize}
    \item On any route $(\ell,d)$ which a nonzero volume of drivers drive without a passenger, the utility-to-go
        is maximized over all non-passenger relocation trips:
        \begin{equation}
            \label{eq:relocation_trip_utility_property}
                f_{(\ell,d)} - g_{(\ell,d)} > 0 \implies \calQ(\ell,d,0) = \max_{d'} \calQ(\ell,d',0).
        \end{equation}
    \item The dispatch acceptance thresholds are the point at which driving towards the most profitable destination without
        a passenger becomes more profitable than accepting a dispatch.
        $$
            \calQ(\ell,d,1,x_{(\ell,d)}) = P_{(\ell,d)} - x_{(\ell,d)} + \calQ(\ell,d,0) = \max_{d'}\calQ(\ell,d',0).
        $$
        This produces the following relationship between the dispatch acceptance thresholds, the SSP prices,
        and the utility-to-go values for any equilibrium:
        \begin{equation}
            \label{eq:dispatch_threshold_utility}
            P_{(\ell,d)} - x_{(\ell,d)} =\max_{d'}\calQ(\ell,d',0) - \calQ(\ell,d,0). 
        \end{equation}
    \item Finally, we invoke a backwards induction argument to obtain the following characterization of the
        relocation utility-to-go values in terms of the expected future welfare-to-go function $\Phi$:
        \begin{equation}
            \label{eq:backwards_induction_assn}
            \calQ(\ell,d,0) = \frac{\partial}{\partial f_{(\ell,d)}} \Phi(\bff).
        \end{equation}
        \mccomment{The definition of $\Phi(\cdot)$ currently doesn't include the $-c_{(\ell,d)}$ cost term, which needs to be included
        in $\calQ(\ell,d,0)$}
\end{itemize}

\medskip\noindent \textbf{Where do the non-dispatched drivers go?}
The first step of our proof is to show that the non-dispatched drivers are incentivized to take welfare-optimal trips,
given any set of dispatch trips.  The next step is to show that all equilibria induced by the SSP prices must serve all available
dispatch demand.  

To show that the non-dispatched drivers are incentivized to take welfare-optimal trips we consider
the optimization problem (\ref{eq:relocation_problem}), which takes as input a nonnegative vector $\bfg$
encoding a fixed set of dispatch trips, and solves for the corresponding welfare-optimal trips $\bff$.
We write $R(\bfg)$ to denote the optimal value of (\ref{eq:relocation_problem}) as a function of the
dispatch trips $\bfg$.
\begin{align}
    \label{eq:relocation_problem}
    R(\bfg)\equiv \ \ \ \ \ \ \ \ \ \ \ \ 
    \sup_{\bff} &\ \ \   \Phi(\bff) & 
\\
    \mbox{subject to} & \nonumber\\ 
    & f_{(\ell,d)} \geq g_{(\ell,d)} \ &\forall (\ell,d)\in\calL^2\label{eq:relocation_inequality_constraint}\\
    &
        \sum_{d\in\calL} f_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL.\label{eq:relocation_equality_constraint}
\end{align}

The first step of our proof is obtained in the following Lemma, which concludes that the relocation trips in any
equilibrium are welfare-optimal, assuming the dispatch trips are held fixed.
\begin{lemma}
    \label{lem:relocation_optimality}
    Let $(\bfg,\bff,\bfx)$ denote any equilibrium, and let $\calQ$ be the associated utility-to-go values.  
    Then $\bff$ is an optimal solution for the relocation
    problem (\ref{eq:relocation_problem}) with respect to the dispatch trips $\bfg$.  Moreover, dual
    variables certifying the optimality of $\bff$ are given by
    \begin{equation}
        \label{eq:relocation_lambda_def}
        \lambda_{(\ell,d)} = \max_{d'}\calQ(\ell,d',0) - \calQ(\ell,d,0),
    \end{equation}
    associated with the inequality constraint (\ref{eq:relocation_inequality_constraint}) for each $(\ell,d)$,
    and
    \begin{equation}
        \label{eq:relocation_eta_def}
        \eta_\ell = \max_{d'}\calQ(\ell,d',0)
    \end{equation}
    associated with the equality constraint (\ref{eq:relocation_equality_constraint}) for each $\ell$.
\end{lemma}
\begin{proof}
    First, observe that the complementary slackness conditions follow immediately from the incentive-compatibility
    properties.  In particular, the property stated in equation (\ref{eq:relocation_trip_utility_property})
    guarantees that $\lambda_{(\ell,d)}$ is $0$ whenever $f_{(\ell,d)}$ is strictly larger than $g_{(\ell,d)}$.


    It remains to check the stationarity conditions. 
    The Lagrangian for (\ref{eq:relocation_problem}) is the following:
    \begin{equation*}
        L(\bff;\bflambda,\bfeta) = -\Phi(\bff) + \bflambda^T(\bfg-\bff) + \sum_\ell \eta_\ell\left(\sum_d f_{(\ell,d)} - S_\ell\right).
    \end{equation*}
    We take the negative objective function in order to convert the problem (\ref{eq:relocation_problem}) into
    a convex minimization problem, for compatibility with standard definitions of the Lagrangian and associated optimality
    conditions.
    The stationarity condition we have to verify is that $0$ is the (sub-)gradient of $L(\bff;\bflambda,\bfeta)$.
    We evaluate the partial derivative of $L(\bff;\bflambda,\bfeta)$ at each coordinate $f_{(\ell,d)}$:
    \begin{align*}
        \frac{\partial}{\partial f_{(\ell,d)}} L(\bff;\bflambda,\bfeta) &= 
        -\frac{\partial}{\partial f_{(\ell,d)}} \Phi(\bff) - \lambda_{(\ell,d)} + \eta_\ell\\
        &= - \calQ(\ell,d,0) - \lambda_{(\ell,d)} + \max_{d'}\calQ(\ell,d,0)\\
        &= 0.
    \end{align*}
    In going from the first line to the second line we use the backwards induction assumption (\ref{eq:backwards_induction_assn}).
    The final line follows from the definitions of $\lambda_{(\ell,d)}$ and $\eta_\ell$.
\end{proof}

\medskip\noindent \textbf{All equilibria serve all available dispatch demand}
We proceed with the second step of our proof, which is to show that all equilibria that arise under the SSP prices must
serve all available dispatch demand.  Consider the optimum solution $(\bfg^*,\bff^*,\bfx^*)$ and an arbitrary equilibrium $(\bfg',\bff',\bfx')$ serves strictly fewer dispatch trips than the corresponding optimum at some route. Recall that $\bfg' \le \bfg^*$ on all routes, and that $g'_{(\ell,d)} < g^*_{(\ell,d)}$ on any route implies that $x'_{(\ell,d)} < x^*_{(\ell,d)}$. Based on our matching process of drivers to passengers, it is no loss  of generality to assume that drivers that in the optimum should have accepted the passenger for a route  $(\ell,d)$ were offered this drive.  To prove Theorem \ref{thm:robust_eqlbm_fluid} we will use Lemma \ref{lem:relocation_optimality} on an auxiliary networks that we construct next. 

For all drivers that serve dispatches in the equilibrium, assume they start in the next period at the destination of their current dispatch. 
For a location $\ell$ where some route $(\ell, d)$ serves strictly fewer dispatch trips in $\bfg'$ then in $\bfg'^*$, if $\ell$ has $k$ routes $(\ell, d)$ that had passengers to dispatch, we create $k$ copies of $\ell$, each associated with one the the routes $(\ell,d)$, denoted by $\ell^d$. We distribute the drivers from the equilibrium who started at location $\ell$ among the copies such that drivers who were offed dispatch $(\ell,d)$ will start at location $\ell^d$, Note if there are unserved 
dispatches at location $\ell$ than all drivers at $\ell$ were offered a dispatch. Each copy $\ell^d$ is connected to the same set of nodes for the next period as $\ell$ with the same cost, but each has one additional 
possible route: $(\ell^d,d')$ going to the same destination as the drive $d$, but with a different cost. Suppose the price offered to the drivers was $p_{\ell,d}$ and cutoff expected by our optimization is $x^*_{(\ell,d)}$, and the cost of the drive is $c_{(\ell,d)}$ then this additional route will have cost $c_{(\ell,d)}-p_{(\ell,d)}-x^*_{(\ell,d)}$. 

First we construct the optimal solution $(\bfg^{**},\bff^{**},\bfx^{**})$ in this network, which is essentially the same as $(\bfg^*,\bff^*,\bfx^*)$ except drivers serving dispatches in the equilibrium start only in the next period at the destination of their dispatch, there are no dispatches available in period 1, so $\bfg_{(\ell,d)}^{**}=0$ for the first period and $f^{**}$ includes all additional dispatches that $\bff^*$ would serve along the routes with the new cost $c_{(\ell,d)}-p_{(\ell,d)}-x^*_{(\ell,d)}$, and $\bfx^{**}$ is only for later periods of the problem. We call this the linearized problem (where the first period values are linear). We first lemma this is an optimal solution to the linearized program, with the same dual variables as the original optimization problem. 
\begin{lemma}\label{lemma:lin-opt}
The flow $(\bfg^{**},\bff^{**},\bfx^{**})$ is an optimal solution to our modified convex program, with optimal value $OPT^{**}$. 
\end{lemma}

Second, for any route $(\ell,d)$ where not all dispatches are served, we can replace $x^*_{(\ell,d)}$ with its equilibrium cutoff $x'_{(\ell,d)}$, this makes the cost lower, and hence the value of the solution $(\bfg'',\bff'',\bfx'')$ is now strictly larger than $OPT''$.

\begin{lemma}\label{lemma:lin-larger-opt}
The optimal solution to our modified convex program, using $x'$ in places of $x^*$ is strictly larger by at least $\sum_{(\ell,d)}(g^*_{(\ell,d)}-g'_{(\ell,d)})(x^*_{(\ell,d)}-x'_{(\ell,d)})$ unless all dispatches are served.
\end{lemma}

Next consider the equilibrium solution $(\bfg',\bff',\bfx')$ on the modified network. To be precise, drivers who accepted dispatches again are starting in the next period at the destination of the dispatch. All other drives either were not offered dispatches or rejected their offer and choose an alternate drive instead. We will call this $(\bfg'',\bff'',\bfx'')$.  The resulting solution is an equilibrium of this network, and actually this is true both with $x^*$ and with $x'$ in our problem. 

\begin{lemma}
The flow $(\bfg',\bff',\bfx')$ is an equilibrium on our modified network 
either with cost $c_{(\ell,d)}-p_{(\ell,d)}-x^*_{(\ell,d)}$ or with costs 
$c_{(\ell,d)}-p_{(\ell,d)}-x'_{(\ell,d)}$ of the drives with modified costs. 
\end{lemma}

Now by Lemma \ref{lem:relocation_optimality} this equilibrium solution is optimal with both version of the problem. Using $x^*$ to define cost we get the the equilibrium solution has value $OPT^{**}$. However, using $x'$ does not change the value of the equilibrium, while the optimum increases by Lemma \ref{lemma:lin-larger-opt} unless all dispatches are served.














\medskip\noindent \textbf{old version starts here}
For the sake of contradiction, assume there exists at least one route $(\ell,d)$
for which the arbitrary equilibrium $(\bfg',\bff',\bfx')$ serves strictly fewer dispatch trips than the corresponding
dispatch demand.
The property stated in equation (\ref{eq:threshold_property}) guarantees that on such routes $(\ell,d)$, the acceptance
threshold $x'_{(\ell,d)}$ used by the arbitrary equilibrium is strictly less than the optimal acceptance threshold
$x^*_{(\ell,d)}$.

The following lemma states a useful relationship between dual variables of the relocation problem (\ref{eq:relocation_problem}),
and gradient of the function $R(\bfg)$.
\begin{lemma}
    \label{lem:relocation_subgradient}
    Recall $R(\bfg)$ gives the optimal value of the relocation problem (\ref{eq:relocation_problem}) as a function of the
    dispatch trips $\bfg$. For any feasible dispatch trip vector $\bfg_0$, let $\bflambda$ be optimal dual variables
    for the inequality constraints (\ref{eq:relocation_inequality_constraint}), for the relocation problem with respect to 
    $\bfg_0$.  Then the following inequality holds for any feasible dispatch trip vector $\bfg$:
    \begin{equation}
        \label{eq:subgradient_ineq}
    -\bflambda^T(\bfg - \bfg_0) \geq R(\bfg) - R(\bfg_0).
    \end{equation}
    That is, $\bflambda$ is a subgradient of $-R(\bfg_0)$.
\end{lemma}
\begin{proof}
    We start by converting the concave maximization problem (\ref{eq:relocation_problem}) into a convex minimization problem
    so that standard tools from convex analysis apply directly.  For consistency with the convex analysis result we plan to invoke,
    we also incorporate the flow conservation equality constraints (\ref{eq:relocation_equality_constraint}) directly into the cost function.
    Define the cost function $\Gamma(\bff)$ by
    \begin{equation}
        \Gamma(\bff) = \begin{cases}
        -\Phi(\bff) & \mbox{if }\sum_d f_{(\ell,d)} = S_\ell \ \forall \ell,\\
        +\infty & \mbox{otherwise.}
        \end{cases}
    \end{equation}
    Fix any choice of $\bfg_0$, and define the cost-to-go function $C(\bfh)$ as the minimum value of the cost function $\Gamma(\bff)$ over all
    feasible $\bff$, where the inequality constraint $\bff\geq\bfg_0$ is perturbed by $-\bfh$:
    \begin{align}
    \label{eq:relocation_problem_minimization}
    C(\bfh)\equiv \ \ \ \ \ \ \ \ \ \ \ \ 
    \inf_{\bff} &\ \ \   \Gamma(\bff) & 
\\
    \mbox{subject to} 
        & -\bff +\bfg_0\leq \bfh. \ &\nonumber
\end{align}
We make the following observations:
    \begin{enumerate}
    \item For any feasible dispatch-trip vector $\bfg$ we have $R(\bfg)=-C(-\bfg+\bfg_0)$.
    \item If $\bflambda_0$ is an optimal dual variable for the optimization problem (\ref{eq:relocation_problem}) with respect to $\bfg_0$, then
        $\bflambda_0$ remains an optimal dual variable for the optimization problem (\ref{eq:relocation_problem_minimization}) with respect to $\bfh=\bfg_0-\bfg_0=0$.
    \end{enumerate}
    We now invoke \mccomment{Problem 9(a) on page 47 of Lewis/Borwein Convex Analysis Book} to conclude that $\bflambda_0\in-\partial C(0)$.
    For any $\bfg$, let $\bfh=\bfg_0-\bfg$.  The subdifferential property of $\bflambda_0$ yields
    $$
    \bflambda_0^T(\bfh) \leq C(\bfh) - C(0)
    $$
    from which we conclude
    $$
    \bflambda_0^T(\bfg_0-\bfg) \leq R(\bfg_0) - R(\bfg).
    $$
    Rearranging, we have
    $$
    R(\bfg) - R(\bfg_0) \leq \bflambda_0^T(\bfg - \bfg_0),
    $$
    which is what we set out to prove.
\end{proof}

We now derive a contradiction under the assumption that the arbitrary equilibrium $(\bfg',\bff',\bfx')$ does not
serve all available dispatch demand on at least one route.
Let $\bflambda'$ and $\bflambda^*$ be the dual variables constructed in equation 
(\ref{eq:relocation_lambda_def}) of Lemma \ref{lem:relocation_optimality} with respect to the arbitrary equilibria
$(\bfg',\bff',\bfx')$ and $(\bfg^*,\bff^*,\bfx^*)$, respectively.
Using the subgradient inequality (\ref{eq:subgradient_ineq}) with respect to $\bflambda'\in \partial(-R)(\bfg')$
we obtain
$$
-\bflambda'^T(\bfg^*-\bfg') \geq R(\bfg^*) - R(\bfg').
$$
Using the subgradient inequality with respect to $\bflambda^*\in\partial (-R)(\bfg^*)$ we obtain
$$
-\bflambda^{*T}(\bfg'-\bfg^*) \geq R(\bfg') - R(\bfg^*).
$$
Combining the above inequalities, the following bound holds:
$$
\bflambda'^T(\bfg^*-\bfg') \leq \bflambda^{*T}(\bfg^*-\bfg'). 
$$
Expanding,
\begin{align*}
    \bflambda'^T(\bfg^*-\bfg') &\leq \bflambda^{*T}(\bfg^*-\bfg')\\
    \sum_{(\ell,d)} \lambda'_{(\ell,d)}(g^*_{(\ell,d)} - g'_{(\ell,d)})  &\leq 
           \sum_{(\ell,d)} \lambda^*_{(\ell,d)}(g^*_{(\ell,d)} - g'_{(\ell,d)})\\
    \sum_{(\ell,d)} \left(P_{(\ell,d)} - x'_{(\ell,d)}\right)  (g^*_{(\ell,d)} - g'_{(\ell,d)})  &\leq 
           \sum_{(\ell,d)}   \left(P_{(\ell,d)} - x^*_{(\ell,d)}\right)  (g^*_{(\ell,d)} - g'_{(\ell,d)}),
\end{align*}
where the last line follows from the definition (\ref{eq:relocation_lambda_def}) of $\lambda'_{(\ell,d)}$ and $\lambda^*_{(\ell,d)}$,
in addition to the property (\ref{eq:dispatch_threshold_utility}).
Now, the price terms cancel out, and the above inequality simplifies to the following:
\begin{equation}
    \label{eq:penultimate_threshold_inequality}
\sum_{(\ell,d)} x^*_{(\ell,d)} (g^*_{(\ell,d)} - g'_{(\ell,d)}) \leq \sum_{(\ell,d)} x'_{(\ell,d)}(g^*_{(\ell,d)} - g'_{(\ell,d)}).
\end{equation}
This inequality is enough to obtain a contradiction: equation (\ref{eq:threshold_property}) states that on any route $(\ell,d)$
where $g^*_{(\ell,d)} - g'_{(\ell,d)}$ is strictly larger than $0$, then the threshold $x'_{(\ell,d)}$ is strictly less
than the optimal threshold $x^*_{(\ell,d)}$.  The difference $g^*_{(\ell,d)} - g'_{(\ell,d)}$ is always nonnegative, 
and by assumption we have at least one route $(\ell,d)$ for which the difference is strictly positive.
Therefore, we have that the following strict inequality holds:
$$
\sum_{(\ell,d)} x'_{(\ell,d)}(g^*_{(\ell,d)} - g'_{(\ell,d)}) < 
\sum_{(\ell,d)} x^*_{(\ell,d)} (g^*_{(\ell,d)} - g'_{(\ell,d)}), 
$$
which is a contradiction to (\ref{eq:penultimate_threshold_inequality}).  

It follows that our assumption that there exists an equilibrium which serves less demand than created by the SSP prices
is false, and therefore every equilibrium serves all available dispatch demand.

\medskip
\noindent \textbf{All equilibria are welfare-maximizing}
\mccomment{old version of section -- notation /text currently out of sync with previous sections}
The SSP mechanism sets the price $P_{(o,d)}$ on each route so that the resulting dispatch demand is exactly equal to
the volume of dispatch supply on that route prescribed under the optimal solution $(\bfg^*,\bff^*)$.  Therefore, the
dispatch-supply variable $g^*_{(o,d)}$ is also equal to the amount of dispatch demand created under the SSP price $P_{(o,d)}$.
Our assumption that the equilibrium $(\bfg,\bff,\bfx)$ serves all dispatch demand we create is equivalent to 
assuming the equality
\begin{equation}
    \label{eq:all_dispatch_served}
    g_{(o,d)}=g^*_{(o,d)}
\end{equation}
holds for all origin-destination pairs $(o,d)\in\calL^2$.
The question that remains is where do the non-dispatched drivers go.
To analyze this question we consider the following optimization problem, which solves for the welfare-optimal
relocation trips assuming that the dispatch trips are fixed.
\begin{align}
    %\label{eq:relocation_problem}
    \mathrm{RelocationProblem}(\bfg)\equiv \ \ \ \ \ \ \ \ \ \ \ \ 
    \sup_{\bfh} &\ \ \   \Phi(\bfh) & 
\\
    \mbox{subject to} & \nonumber\\ 
    & h_{(\ell,d)} \geq g_{(\ell,d)} \ &\forall (\ell,d)\in\calL^2\nonumber\\
    &
        \sum_{d\in\calL} h_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL.\nonumber
\end{align}
The above optimization problem solves for the optimal single-period flow $\bfh$ given the fixed
dispatch trip volumes encoded by $\bfg$. We use the notation $\bfh$ above to distinguish the
total-trip volumes used in our arbitrary equilibrium, $\bff$, from the decision variables $\bfh$.
The function $\Phi(\bfh)$ includes the linear cost of driving on each route in the current period,
as well as the welfare-to-go from the market-state arising at the subsequent time period, under
the trip volumes $\bfh$.
We assume the input dispatch-trip vector $\bfg$ is always nonnegative, hence the lower bound 
$h_{(\ell,d)}\geq g_{(\ell,d)}$ guarantees that the trip-volumes $h_{(\ell,d)}$ are always nonnegative,
in addition to ensuring that the total trip-volume is at least as large as the dispatch trip-volume
on each origin-destination pair.

We will proceed by showing that the equilibrium trip volumes $\bff$ and the optimal trip volumes $\bff^*$
are both optimal solutions to $\mathrm{RelocationProblem}(\bfg^*)$. After establishing that both trip volumes
are optimal for the relocation problem, a duality analysis will show that the equilibrium $(\bfg,\bff,\bfx)$
must also be optimal for the original problem (\ref{eq:dynamic_optimization_recursive}).

Note that our assumption for this case, that the arbitrary equilibrium serves all available dispatch demand,
is equivalent to assuming the equilibrium dispatch-trip vector $\bfg$ is equal to the optimal dispatch-trip
vector $\bfg^*$.  Therefore, both the equilibrium total-trip vector $\bff$ and the optimal total-trip vector $\bff^*$ 
are feasible solutions for $\mathrm{RelocationProblem}(\bfg^*)$.

Let's consider the optimality conditions for $\mathrm{RelocationProblem}(\bfg^*)$. Let $\lambda_{(\ell,d)}\geq 0$ be a dual
variable associated with each constraint $h_{(\ell,d)}\geq g^*_{(\ell,d)}$, and let $\eta_\ell$ be a dual
variable associated with the flow-conservation constraint for each location $\ell$.
Then a trip-vector $\bfh$ is optimal if and only if the complementary slackness condition
\begin{equation}
    \label{eq:relocation_trip_csc}
\lambda_{(\ell,d)}(h_{(\ell,d)} - g^*_{(\ell,d)}) = 0
\end{equation}
holds for all origin-destination pairs $(\ell,d)$, and the following stationarity condition
\begin{equation}
    \label{eq:relocation_trip_stationarity}
\eta_\ell = \partial_{ h_{(\ell,d)}}\Phi(\bfh) + \lambda_{\ell,d}
\end{equation}
holds for all O-D pairs $(\ell,d)$.

Now, following a backwards induction argument, we have that the partial derivative of the welfare-to-go function
with respect to the trip-volume on a particular route
is equal to the utility-to-go of a driver who traverses that route:
$$
\partial_{ h_{(\ell,d)}}\Phi(\bfh) = \bbE_{\omega_{t+1}}\left[\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bfh), d)\right] - c_{(\ell,d)}.
$$
The constant $-c_{(\ell,d)}$ is the fixed cost of driving from $\ell$ to $d$.
We use $\bfS_{\omega_{t+1}}(\bfh)$ to mean the time $t+1$ supply-location vector that occurs when the drivers
move according to the trips $\bfh$, and $\omega_{t+1}$ is the subsequent scenario.  Notice that the scenario
$\omega_{t+1}$ influences the volume of drivers who enter the market at each location.  Therefore
the component of the supply-location vector $\bfS_{\omega_{t+1}}(\bfh)$ corresponding to location $\ell$
counts the total volume of incoming drivers to the location $\ell$ under the trip-vector $\bfh$ plus the
volume of drivers who enter the market at location $\ell$ under the scenario $\omega_{t+1}$.
The notation $\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bfh), d)$ means the expected utility-to-go of a driver
positioned at location $d$ under the scenario $\omega_{t+1}$ and the supply-location vector $\bfS_{\omega_{t+1}}(\bfh)$.
Our backwards induction assumption states that the utility-to-go from location $d$ is the same value for any equilibrium
strategy the drivers use in future periods.

Now, consider the utility of a relocation trip from $\ell$ to $d$ under the arbitrary equilibrium $(\bfg,\bff,\bfx)$.
We write the utility-to-go for a relocation trip from $\ell$ to $d$ as $\calQ(\ell,d,0)$.  
We write $\calQ(\ell,0)$ to mean the maximum utility-to-go of any relocation trip originating from $\ell$:
$$
\calQ(\ell,0) = \max_d \calQ(\ell,d,0).
$$
Because the strategy we are considering is an equilibrium, every route for which a nonzero number of drivers take
a relocation trip has utility-to-go equal to the maximum relocation-trip utility $\calQ(\ell,0)$.  That is,
if a route $(\ell,d)$ has nonzero relocation trips, i.e. $f_{(\ell,d)} - g_{(\ell,d)} > 0$, then the
utility-to-go $\calQ(\ell,d,0)$ is equal to the maximum relocation trip utility $\calQ(\ell,0)$:
$$
f_{(\ell,d)} -g_{(\ell,d)} > 0 \implies \calQ(\ell,d,0) = \calQ(\ell,0).
$$
Now, for every destination $d$, let $\lambda_{(\ell,d)}$ be the difference between the relocation-trip utility towards
destination $d$ and the maximum relocation utility:
$$
\lambda_{(\ell,d)}\coloneqq \calQ(\ell,0) - \calQ(\ell,d,0).
$$
Equality between
$\calQ(\ell,d,0)$ and the partial derivative $\partial_{f_{(\ell,d)}}\Phi(\bff)$ follows immediately from our
backwards induction assumption
$$
\calQ(\ell,d,0) = \bbE_{\omega_{t+1}}\left[\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff), d)\right] - c_{(\ell,d)}
 = \partial_{f_{(\ell,d)}}\Phi(\bff).
$$
Setting $\eta_\ell$ to the maximum relocation utility $\calQ(\ell,0)$, we see that $\bff$ is a feasible primal solution
for $\mathrm{RelocationProblem}(\bfg^*)$, $\eta_\ell$ and $\lambda_{(\ell,d)}$ are feasible dual solutions, and
the stationarity (\ref{eq:relocation_trip_stationarity}) and complementary slackness (\ref{eq:relocation_trip_csc}) 
conditions are satisfied, showing that $\bff$ is an optimal solution for the relocation-trip problem with respect to $\bfg^*$.

Similarly, let $\calQ^*(\ell,d,0)$ be the utility-to-go of a relocation-trip from $\ell$ to $d$ under the optimal
solution $(\bfg^*,\bff^*)$, and let 
$$
\calQ^*(\ell,0)=\max_d\calQ^*(\ell,d,0)
$$
be the maximum relocation utility-to-go from $\ell$ under the optimal solution.
Defining
$$
\lambda_{(\ell,d)}^* = \calQ^*(\ell,0) - \calQ^*(\ell,d,0)
$$
and 
$$
\eta_\ell^*=\calQ^*(\ell,0),
$$
we see that $\bff^*$ is an optimal primal solution to $\mathrm{RelocationTrip}(\bfg^*)$ with optimal dual
variables $\eta_\ell^*$ and $\lambda_{(\ell,d)}^*$.

Now, recall that the optimality conditions for a convex program hold between any pair of optimal primal and dual
variables.  Therefore, $\eta_\ell=\eta_\ell^*$, in other words the relocation utility under the arbitrary equilibrium
is equal to the relocation utility under the optimal solution:
$$
\calQ(\ell,0)=\calQ^*(\ell,0).
$$
This property is enough to conclude welfare-optimality of the arbitrary equilibrium, and conclude the backwards induction
argument, by showing that the thresholds $x_{(\ell,d)}$ used in the arbitrary equilibrium must be equal
to the optimal thresholds $x^*_{(\ell,d)}$.\mccomment{will fill in details here after working out case number 2.}




==> fluid_robustness_proof_old.tex <==
A central tool in our analysis of an arbitrary strategy profile is a modified version of the optimization
problem (\ref{eq:dynamic_optimization_recursive}), in which the reward function is linearized to only reflect the price
collected by drivers, and an additional set of disutility-threshold decision variables are included in the formulation.
First, define a threshold-based add-passenger disutility function $B(g,x)$, which depends on a dispatch-trip variable $g$
and a disutility threshold $x$:
$$
B(g,x) = g\bbE[X\mid X\leq x]=\frac{gx}{2},
$$
where $X\sim\mathrm{Uniform}(0,C)$.
Recall our previous disutility function $A(g,S)$, which took as input a dispatch trip count value $g$ and a total-supply volume $S$:
$$
A(g,S)=g\bbE[X\mid X\leq F^{-1}\left(\frac{g}{S}\right)],
$$
our objective function subtracted the value $A(\bfg^T\bfone_\ell,\bff^T\bfone_\ell)$ for each location $\ell$.
Observe we can recover the function value $A(\bfg^T\bfone_\ell,\bff^T\bfone_\ell)$  in terms of a sum of the threshold-centric
disutility functions $B(g,x)$ as follows.  Define the threshold $x_\ell=F^{-1}\left(\frac{\bfg^T\bfone_\ell}{\bff^T\bfone_\ell}\right)$,
and observe the following equality holds:
$$
\sum_{d\in\calL} B(g_{(\ell,d)},x_\ell) = A(\bfg^T\bfone_\ell,\bff^T\bfone_\ell).
$$
In a sense, the threshold value $x_\ell$ is the optimal threshold to use for each route $(\ell,d)$ originating from $\ell$, 
but for the purpose of our analysis it will be useful to define
an optimization formulation in which the threshold values $x_{(\ell,d)}$ are decision variables.

In this alternate optimization formulation, 
in addition to the flow decision variables $(\bff,\bfg)$, we include new threshold decision variables $x_{(\ell,d)}$ for each origin-destination pair
$(\ell,d)$.  
To ensure feasibility of the new threshold decision variables $x_{(\ell,d)}$ we include nonnegativity constraints $x_{(\ell,d)}\geq 0$
as well as the following constraint for each location $\ell$:
\begin{equation}
    \label{eq:threshold_feasibility}
    \sum_{d\in\calL}\frac{g_{(\ell,d)}}{x_{(\ell,d)}} \leq \frac{S_\ell}{C}.
\end{equation}
The above constraint ensures a ``minimum size'' property on the collection of thresholds $x_{(\ell,d)}$ for all outgoing destination
locations $d\in\calL$, given the dispatch volumes $g_{(\ell,d)}$ at each of these destinations.
Note that the function $(g,x)\mapsto \frac{g}{x}$ is convex over nonzero $(g,x)$, so the new constraint we have added remains convex.

We also linearize the utility part of the objective function, so that only the driver utility component of the original formulation
(\ref{eq:dynamic_optimization_recursive}) is included: instead of having the utility function $U_{(\ell,d)}(g_{(\ell,d)},f_{(\ell,d)})$,
which gives rider and driver utility in the original formulation (\ref{eq:dynamic_optimization_recursive}), we include a linear
function $P_{(\ell,d)}g_{(\ell,d)}$ where $P_{(\ell,d)}$ is the price set by our SSP mechanism, and $g_{(\ell,d)}$ is the volume
of drivers who serve a dispatch trip from $\ell$ to $d$.

The linearized optimization problem is stated below:
\begin{align}
    \sup_{\bff, \bfg} &\ \ \  \sum_{\substack{(\ell,d)\in\\\calL^2}} P_{(\ell,d)}g_{(\ell,d)} - 
        \sum_{(\ell,d)\in\calL^2} B\left(g_{(\ell,d)},x_{(\ell,d)}\right)
         + 
    \Phi(\bff)
 & 
\label{eq:linearized_optimization}\\
    \mbox{subject to} & \nonumber\\ 
    & f_{(o,d)} \geq 0 \ &\forall (o,d)\in\calL^2\nonumber\\
    & g_{(o,d)} \geq 0 \ &\forall (o,d)\in\calL^2\nonumber\\
    & f_{(o,d)} \geq g_{(o,d)} \ &\forall (o,d)\in\calL^2 \nonumber\\
    & g^*_{(o,d)} \geq g_{(o,d)} \ &\forall (o,d)\in\calL^2 \nonumber\\
    & x_{(\ell,d)} \geq 0 & \forall (\ell,d)\in\calL^2\nonumber\\
    & \sum_{d\in\calL}\frac{g_{(\ell,d)}}{x_{(\ell,d)}} \leq \frac{S_\ell}{C} & \forall \ell\in\calL\nonumber\\
    &
        \sum_{d\in\calL} f_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL.\nonumber
\end{align}

We derive optimality conditions for the linearized optimization problem (\ref{eq:linearized_optimization}) below.
We introduce the following dual variables:
\begin{itemize}
    \item $\alpha_{(\ell,d)}\geq 0$ for the $-f_{(\ell,d)}\leq  0$ constraints.
    \item $\beta_{(\ell,d)}\geq 0$ for the $-g_{(\ell,d)}\leq  0$ constraints.
    \item $\gamma_{(\ell,d)}\geq 0$ for the $g_{(\ell,d)} - f_{(\ell,d)}\leq  0$ constraints.
    \item $\theta_{(\ell,d)}\geq 0$ for the $g_{(\ell,d)} - g^*_{(\ell,d)}\leq  0$ constraints.
    \item $\lambda_{(\ell,d)}\geq 0$ for the $-x_{(\ell,d)}\leq 0$ constraints.
    \item $\mu_\ell\geq 0$ for the $\sum_{d\in\calL}\frac{g_{(\ell,d)}}{x_{(\ell,d)}} - \frac{S_\ell}{C}\leq 0$ constraints.
    \item $\eta_\ell$ for the $\sum_{d\in\calL} f_{(\ell,d)}-S_\ell = 0$ constraints.
\end{itemize}
The Lagrangian function $L(\dots)$ takes as input all the primal variables $(\bff,\bfg,\bfx)$, all the dual variables described above,
and it gives the negative welfare function (to convert the problem into a convex minimization problem as opposed to a concave 
maximization problem) plus the product of the left side of all the constraints (as written above) and the corresponding dual variables.

A feasible solution $(\bff,\bfg,\bfx)$ is optimal if and only if there exist feasible dual variables which satisfy the complementary
slackness conditions and the following stationarity conditions:
\begin{align*}
    \partial_{f_{(\ell,d)}} L(\bff,\bfg,\bfx)&=0\\
    \partial_{g_{(\ell,d)}} L(\bff,\bfg,\bfx)&=0,\\
    \partial_{x_{(\ell,d)}} L(\bff,\bfg,\bfx)&=0.
\end{align*}
Expanding the partial derivatives, the stationarity conditions become the following:
\begin{align}
    \label{eq:linearized_stationarity_f}
    -\partial_{f_{(\ell,d)}}\Phi(\bff) - \alpha_{(\ell,d)} - \gamma_{(\ell,d)} + \eta_\ell &= 0, \ \ \ \forall(\ell,d)\in\calL^2,\\
    \label{eq:linearized_stationarity_g}
    -P_{(\ell,d)} + \frac{x_{(\ell,d)}}{2} - \beta_{(\ell,d)} + \gamma_{(\ell,d)} + \theta_{(\ell,d)} + \frac{\mu_\ell}{x_{(\ell,d)}}
    &= 0 , \ \ \ \forall (\ell,d)\in\calL^2,\\
    \frac{g_{(\ell,d)}}{2} - \lambda_{(\ell,d)} - \mu_\ell \frac{g_{(\ell,d)}}{x_{(\ell,d)}^2}
    &= 0 , \ \ \ \forall (\ell,d)\in\calL^2,
    \label{eq:linearized_stationarity_x}
\end{align}

\medskip
\noindent \textbf{Optimality of Arbitrary Equilibrium for Linearized Problem}
In this section we show that an arbitrary equilibrium driver strategy must be an optimal solution to the linearized
optimization problem (\ref{eq:linearized_optimization}).
Let $(\bff,\bfg,\bfx)$ encode an equilibrium driver strategy.  By Lemma \ref{lem:fluid_eqlbm_strategy} we know the thresholds
$\bfx$ satisfy the threshold-size constraint (\ref{eq:threshold_feasibility}), so $(\bff,\bfg,\bfx)$ is a feasible
solution to the linearized optimization problem.
Our next step is to use incentive compatibility conditions to show that $(\bff,\bfg,\bfx)$ satisfies the complementary
slackness conditions, and thus forms an optimal solution for the linearized problem.

\mccomment{Actually, using the incentive compatibility conditions to show optimality of $(\bff,\bfg,\bfx)$ is where I hit a wall.
The following paragraphs explain why.}

Consider the stationarity condition (\ref{eq:linearized_stationarity_x}).
Note the threshold $x_{(\ell,d)}$ is never $0$
for any route $(\ell,d)$ where $g_{(\ell,d)}$ is nonzero; otherwise the ratio $\frac{g_{(\ell,d)}}{x_{(\ell,d)}}$ would be $\infty$
and the feasibility condition would be violated.  Hence, in order for $(\bff,\bfg,\bfx)$ to satisfy complementary slackness, the dual variables
$\lambda_{(\ell,d)}$ associated with the nonnegativity constraint $-x_{(\ell,d)}\leq 0$ for such routes must be $0$.
Therefore, the stationarity condition (\ref{eq:linearized_stationarity_x}) simplifies to the following expression: there exists a dual
variable $\mu_\ell$ for each $\ell$, such that for every location $d$ the following equation holds:
\begin{equation}
    \frac{g_{(\ell,d)}}{2} = \mu_\ell\frac{g_{(\ell,d)}}{x_{(\ell,d)}^2},
\end{equation}
or rearranging,
\begin{equation}
    \mu_\ell=\frac{x_{(\ell,d)}^2}{2}.
\end{equation}
The above property implies the following conditions must be true at any optimal solution for the linearized problem:
\begin{enumerate}
    \item The thresholds $x_{(\ell,d)}$ must all the same value for every destination $d$.
    \item The constraint (\ref{eq:threshold_feasibility}) must be tight at an optimal solution: if the constraint were not tight,
        then nonzero $\mu_\ell$ would violate complementary slackness.
\end{enumerate}

\mccomment{This is where I hit a wall.  How can we show that $(\bff,\bfg,\bfx)$ is an optimal solution without already knowing that 
properties 1 and 2 above already hold? I don't see a simple argument for why incentive compatibility conditions should imply these properties,
and I don't see how to show that $(\bff,\bfg,\bfx)$ is optimal for (\ref{eq:linearized_optimization}) without already having these properties.}


\medskip
\noindent \textbf{Optimality of Original Optimum for Linearized Problem}
We now demonstrate that the linearized optimization problem (\ref{eq:linearized_optimization}) has the same optimal solution
as the original formulation (\ref{eq:dynamic_optimization_recursive}), by showing that an optimal solution $(\bff^*,\bfg^*)$
for the original formulation (\ref{eq:dynamic_optimization_recursive}) remains optimal for the linearized problem
(\ref{eq:linearized_optimization}).

First, we extend the optimal solution $(\bff^*,\bfg^*)$ to a feasible solution to the linearized problem 
(\ref{eq:linearized_optimization}) by defining the thresholds 
$$
x^*_{(\ell,d)} = F^{-1}\left(\frac{\bfg^{*T}\bfone_\ell}{\bff^{*T}\bfone_\ell}\right) = 
C\frac{\bfg^{*T}\bfone_\ell}{\bff^{*T}\bfone_\ell}.
$$
Observe the solution $(\bff^*,\bfg^*,\bfx^*)$ satisfies the feasibility constraint on the threshold values we included
in the linearized problem (\ref{eq:linearized_optimization}):
\begin{equation}
    \label{eq:opt_threshold_constraint}
\sum_{d\in\calL}\frac{g^*_{(\ell,d)}}{x^*_{(\ell,d)}} = 
\sum_{d\in\calL}g^*_{(\ell,d)}\frac{\bff^{*T}\bfone_\ell}{C\bfg^{*T}\bfone_\ell} = 
\frac{\bff^{*T}\bfone_\ell}{C\bfg^{*T}\bfone_\ell}\bfg^{*T}\bfone_\ell
= \frac{\bff^{*T}\bfone_\ell}{C} = \frac{S_\ell}{C}.
\end{equation}

Let $(\alpha_{(\ell,d)},\beta_{(\ell,d)},\gamma_{(\ell,d)},\eta_\ell)$ be dual variables 
certifying the optimality of $(\bff^*,\bfg^*)$ for the original formulation (\ref{eq:linearized_optimization}).
It remains to specify dual variables $\theta_{(\ell,d)}$, $\lambda_{(\ell,d)}$ and $\mu_\ell$.
\begin{itemize}
    \item We set $\lambda_{(\ell,d)} = 0$ for all $(\ell,d)$. Notice the thresholds $x^*_{(\ell,d)}$ are 
        nonzero unless $\ell$ is a location for which no dispatch demand originates towards any destination,
        so $\lambda_{(\ell,d)}$ is necessarily $0$ to satisfy complementary slackness.
    \item Since the constraint evaluated in (\ref{eq:opt_threshold_constraint}) holds with equality, the
        dual variable $\mu_\ell$ can take on any nonzero value and still satisfy complementary slackness.
        Define 
        $$\mu_{\ell}=\frac{x^{*2}_{(\ell,d)}}{2},$$
        which guarantees the stationarity condition (\ref{eq:linearized_stationarity_x}) always holds.
        Note the threshold value $x^*_{(\ell,d)}$ we defined is the same for all locations $d$, so the above
        definition of $\mu_\ell$ is well-defined.
    \item Finally, define the dual value $\theta_{(\ell,d)}$ so that the stationarity condition 
        (\ref{eq:linearized_stationarity_g}) holds:
        $$
        \theta_{(\ell,d)} = P_{(\ell,d)} + \beta_{(\ell,d)} - \gamma_{(\ell,d)}.
        $$
        Note the upper bound $g^*_{(\ell,d)}\leq g^*_{(\ell,d)}$ clearly holds with equality, so
        $\theta_{(\ell,d)}$ can take on any nonnegative value and still satisfy complementary slackness.
        Also note the stationarity conditions for $(\bff^*,\bfg^*)$ guarantee nonnegativity of $\theta_{(\ell,d)}$.
\end{itemize}
\mccomment{
Finally, we can make the remaining stationarity condition (\ref{eq:linearized_stationarity_f}) hold by setting
$$
\alpha_{(\ell,d)} =-\partial_{f_{(\ell,d)}}\Phi(\bff) - \gamma_{(\ell,d)} + \eta_\ell.
$$
The stationarity conditions from Lemma \ref{lem:dynamic_optimality_conditions} guarantee this value of $\alpha_{(\ell,d)}$
is nonnegative.
Therefore, $(\bff^*,\bfg^*,\bfx^*)$ is an optimal solution for the linearized optimization problem 
(\ref{eq:linearized_optimization}).
}

\medskip
\noindent \textbf{Robustness Proof Attempt Number Two: Where do the Non-Dispatched Drivers Go?}
\mccomment{In this section I try to work out the proof details using the ideas discussed in our last meeting
on Thursday 9/2}
Let $(\bfg,\bff,\bfx)$ encode an arbitrary equilibrium which is induced by the SSP prices, where
\begin{itemize}
    \item $\bfg=(g_{(o,d)}:(o,d)\in\calL^2)$ encodes the volume of dispatch trips on each origin-destination
pair, 
\item $\bff=(f_{(o,d)}:(o,d)\in\calL^2)$ encodes the volume of all (relocation and dispatch) trips on each
origin-destination pair,
\item $\bfx=(x_{(o,d)}:(o,d)\in\calL^2)$ encodes the disutility-acceptance threshold used by the drivers on each route.
\end{itemize}

Similarly, let $(\bfg^*,\bff^*)$ denote the optimal flow to the single-period formulation
(\ref{eq:dynamic_optimization_recursive}) that the SSP mechanism uses to set prices in the current time period.
The formulation (\ref{eq:dynamic_optimization_recursive}) assumes that drivers accept dispatches using the welfare-maximizing
acceptance thresholds $x^*_{(\ell,d)}$:
$$
x^*_{(\ell,d)} = C\frac{\bfg^{*T}\bfone_{\ell}}{\bff^{*T}\bfone_{\ell}}.
$$

We analyze the equilibrium $(\bfg,\bff,\bfx)$ by considering the following two cases:
\begin{itemize}
    \item \textbf{Case one:} The equilibrium $(\bfg,\bff,\bfx)$ serves all dispatch demand which occurs under the prices set
        by the SSP mechanism. In this case we will show that the incentive-compatibility conditions imply that the
        equilibrium is welfare-optimal.
    \item \textbf{Case two:} The equilibrium $(\bfg,\bff,\bfx)$ does not serve all dispatch demand which occurs under the prices set
        by the SSP mechanism. In this case we will derive a contradiction: the strategy-profile under consideration will
        have too many drivers driving empty towards over-supplied locations, and these drivers would have a profitable deviation
        to use a higher acceptance threshold on one of the routes with excess dispatch demand.
\end{itemize}

\medskip
\noindent \textbf{Case One: The Arbitrary Equilibrium Serves all Dispatch Demand}
The SSP mechanism sets the price $P_{(o,d)}$ on each route so that the resulting dispatch demand is exactly equal to
the volume of dispatch supply on that route prescribed under the optimal solution $(\bfg^*,\bff^*)$.  Therefore, the
dispatch-supply variable $g^*_{(o,d)}$ is also equal to the amount of dispatch demand created under the SSP price $P_{(o,d)}$.
Our assumption that the equilibrium $(\bfg,\bff,\bfx)$ serves all dispatch demand we create is equivalent to 
assuming the equality
\begin{equation}
    \label{eq:all_dispatch_served}
    g_{(o,d)}=g^*_{(o,d)}
\end{equation}
holds for all origin-destination pairs $(o,d)\in\calL^2$.
The question that remains is where do the non-dispatched drivers go.
To analyze this question we consider the following optimization problem, which solves for the welfare-optimal
relocation trips assuming that the dispatch trips are fixed.
\begin{align}
    \label{eq:relocation_problem}
    \mathrm{RelocationProblem}(\bfg)\equiv \ \ \ \ \ \ \ \ \ \ \ \ 
    \sup_{\bfh} &\ \ \   \Phi(\bfh) & 
\\
    \mbox{subject to} & \nonumber\\ 
    & h_{(\ell,d)} \geq g_{(\ell,d)} \ &\forall (\ell,d)\in\calL^2\nonumber\\
    &
        \sum_{d\in\calL} h_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL.\nonumber
\end{align}
The above optimization problem solves for the optimal single-period flow $\bfh$ given the fixed
dispatch trip volumes encoded by $\bfg$. We use the notation $\bfh$ above to distinguish the
total-trip volumes used in our arbitrary equilibrium, $\bff$, from the decision variables $\bfh$.
The function $\Phi(\bfh)$ includes the linear cost of driving on each route in the current period,
as well as the welfare-to-go from the market-state arising at the subsequent time period, under
the trip volumes $\bfh$.
We assume the input dispatch-trip vector $\bfg$ is always nonnegative, hence the lower bound 
$h_{(\ell,d)}\geq g_{(\ell,d)}$ guarantees that the trip-volumes $h_{(\ell,d)}$ are always nonnegative,
in addition to ensuring that the total trip-volume is at least as large as the dispatch trip-volume
on each origin-destination pair.

We will proceed by showing that the equilibrium trip volumes $\bff$ and the optimal trip volumes $\bff^*$
are both optimal solutions to $\mathrm{RelocationProblem}(\bfg^*)$. After establishing that both trip volumes
are optimal for the relocation problem, a duality analysis will show that the equilibrium $(\bfg,\bff,\bfx)$
must also be optimal for the original problem (\ref{eq:dynamic_optimization_recursive}).

Note that our assumption for this case, that the arbitrary equilibrium serves all available dispatch demand,
is equivalent to assuming the equilibrium dispatch-trip vector $\bfg$ is equal to the optimal dispatch-trip
vector $\bfg^*$.  Therefore, both the equilibrium total-trip vector $\bff$ and the optimal total-trip vector $\bff^*$ 
are feasible solutions for $\mathrm{RelocationProblem}(\bfg^*)$.

Let's consider the optimality conditions for $\mathrm{RelocationProblem}(\bfg^*)$. Let $\lambda_{(\ell,d)}\geq 0$ be a dual
variable associated with each constraint $h_{(\ell,d)}\geq g^*_{(\ell,d)}$, and let $\eta_\ell$ be a dual
variable associated with the flow-conservation constraint for each location $\ell$.
Then a trip-vector $\bfh$ is optimal if and only if the complementary slackness condition
\begin{equation}
    \label{eq:relocation_trip_csc}
\lambda_{(\ell,d)}(h_{(\ell,d)} - g^*_{(\ell,d)}) = 0
\end{equation}
holds for all origin-destination pairs $(\ell,d)$, and the following stationarity condition
\begin{equation}
    \label{eq:relocation_trip_stationarity}
\eta_\ell = \partial_{ h_{(\ell,d)}}\Phi(\bfh) + \lambda_{\ell,d}
\end{equation}
holds for all O-D pairs $(\ell,d)$.

Now, following a backwards induction argument, we have that the partial derivative of the welfare-to-go function
with respect to the trip-volume on a particular route
is equal to the utility-to-go of a driver who traverses that route:
$$
\partial_{ h_{(\ell,d)}}\Phi(\bfh) = \bbE_{\omega_{t+1}}\left[\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bfh), d)\right] - c_{(\ell,d)}.
$$
The constant $-c_{(\ell,d)}$ is the fixed cost of driving from $\ell$ to $d$.
We use $\bfS_{\omega_{t+1}}(\bfh)$ to mean the time $t+1$ supply-location vector that occurs when the drivers
move according to the trips $\bfh$, and $\omega_{t+1}$ is the subsequent scenario.  Notice that the scenario
$\omega_{t+1}$ influences the volume of drivers who enter the market at each location.  Therefore
the component of the supply-location vector $\bfS_{\omega_{t+1}}(\bfh)$ corresponding to location $\ell$
counts the total volume of incoming drivers to the location $\ell$ under the trip-vector $\bfh$ plus the
volume of drivers who enter the market at location $\ell$ under the scenario $\omega_{t+1}$.
The notation $\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bfh), d)$ means the expected utility-to-go of a driver
positioned at location $d$ under the scenario $\omega_{t+1}$ and the supply-location vector $\bfS_{\omega_{t+1}}(\bfh)$.
Our backwards induction assumption states that the utility-to-go from location $d$ is the same value for any equilibrium
strategy the drivers use in future periods.

Now, consider the utility of a relocation trip from $\ell$ to $d$ under the arbitrary equilibrium $(\bfg,\bff,\bfx)$.
We write the utility-to-go for a relocation trip from $\ell$ to $d$ as $\calQ(\ell,d,0)$.  
We write $\calQ(\ell,0)$ to mean the maximum utility-to-go of any relocation trip originating from $\ell$:
$$
\calQ(\ell,0) = \max_d \calQ(\ell,d,0).
$$
Because the strategy we are considering is an equilibrium, every route for which a nonzero number of drivers take
a relocation trip has utility-to-go equal to the maximum relocation-trip utility $\calQ(\ell,0)$.  That is,
if a route $(\ell,d)$ has nonzero relocation trips, i.e. $f_{(\ell,d)} - g_{(\ell,d)} > 0$, then the
utility-to-go $\calQ(\ell,d,0)$ is equal to the maximum relocation trip utility $\calQ(\ell,0)$:
$$
f_{(\ell,d)} -g_{(\ell,d)} > 0 \implies \calQ(\ell,d,0) = \calQ(\ell,0).
$$
Now, for every destination $d$, let $\lambda_{(\ell,d)}$ be the difference between the relocation-trip utility towards
destination $d$ and the maximum relocation utility:
$$
\lambda_{(\ell,d)}\coloneqq \calQ(\ell,0) - \calQ(\ell,d,0).
$$
Equality between
$\calQ(\ell,d,0)$ and the partial derivative $\partial_{f_{(\ell,d)}}\Phi(\bff)$ follows immediately from our
backwards induction assumption
$$
\calQ(\ell,d,0) = \bbE_{\omega_{t+1}}\left[\calV_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff), d)\right] - c_{(\ell,d)}
 = \partial_{f_{(\ell,d)}}\Phi(\bff).
$$
Setting $\eta_\ell$ to the maximum relocation utility $\calQ(\ell,0)$, we see that $\bff$ is a feasible primal solution
for $\mathrm{RelocationProblem}(\bfg^*)$, $\eta_\ell$ and $\lambda_{(\ell,d)}$ are feasible dual solutions, and
the stationarity (\ref{eq:relocation_trip_stationarity}) and complementary slackness (\ref{eq:relocation_trip_csc}) 
conditions are satisfied, showing that $\bff$ is an optimal solution for the relocation-trip problem with respect to $\bfg^*$.

Similarly, let $\calQ^*(\ell,d,0)$ be the utility-to-go of a relocation-trip from $\ell$ to $d$ under the optimal
solution $(\bfg^*,\bff^*)$, and let 
$$
\calQ^*(\ell,0)=\max_d\calQ^*(\ell,d,0)
$$
be the maximum relocation utility-to-go from $\ell$ under the optimal solution.
Defining
$$
\lambda_{(\ell,d)}^* = \calQ^*(\ell,0) - \calQ^*(\ell,d,0)
$$
and 
$$
\eta_\ell^*=\calQ^*(\ell,0),
$$
we see that $\bff^*$ is an optimal primal solution to $\mathrm{RelocationTrip}(\bfg^*)$ with optimal dual
variables $\eta_\ell^*$ and $\lambda_{(\ell,d)}^*$.

Now, recall that the optimality conditions for a convex program hold between any pair of optimal primal and dual
variables.  Therefore, $\eta_\ell=\eta_\ell^*$, in other words the relocation utility under the arbitrary equilibrium
is equal to the relocation utility under the optimal solution:
$$
\calQ(\ell,0)=\calQ^*(\ell,0).
$$
This property is enough to conclude welfare-optimality of the arbitrary equilibrium, and conclude the backwards induction
argument, by showing that the thresholds $x_{(\ell,d)}$ used in the arbitrary equilibrium must be equal
to the optimal thresholds $x^*_{(\ell,d)}$.\mccomment{will fill in details here after working out case number 2.}


\medskip
\noindent \textbf{Case Two: The Arbitrary Equilibrium Does Not Serve all Dispatch Demand}
Let $(\bfg,\bff,\bfx)$ be an arbitrary equilibrium which does not serve all dispatch demand that arises under our prices:
for at least one route $(\ell,d)\in\calL^2$ the strict inequality
\begin{equation}
    \label{eq:excess_demand_condition}
g_{(\ell,d)} < g^*_{(\ell,d)}
\end{equation}
holds. 
We have the following facts:
\begin{enumerate}
    \item On every route $(\ell,d)$ for which the equilibrium is not serving all available demand
        (i.e. the routes $(\ell,d)$ for which the strict inequality (\ref{eq:excess_demand_condition}) holds) 
        the drivers are using an acceptance threshold
        smaller than optimal acceptance threshold: $x_{(\ell,d)} < x^*_{(\ell,d)}$.
    \item Following the logic in the previous section, $\bff$ is a welfare-optimal solution to the relocation problem 
        (\ref{eq:relocation_problem}), assuming the dispatch trips $\bfg$ are held fixed.
    \item For the relocation problem with dispatch trips $\bfg$ held fixed, denoted $\mathrm{RelocationProblem}(\bfg)$,
        we have the optimal dual variable $\lambda_{(\ell,d)}=\calQ(\ell,0) - \calQ(\ell,d,0)$ associated with 
        the inequality constraint $f_{(\ell,d)}\geq g_{(\ell,d)}$ for all routes $(\ell,d)$.
        Here, $\calQ(\ell,0)$ denotes the highest relocation utility under the equilibrium $(\bff,\bfg,\bfx)$
        for a driver positioned at $\ell$, and
        $\calQ(\ell,d,0)$ denotes the relocation utility for driving towards $d$.  
    \item The trips from the original optimum, $\bff^*$, are a welfare-optimal solution to the relocation problem
        (\ref{eq:relocation_problem}), assuming the dispatch trips $\bfg^*$ are held fixed.
    \item For the relocation problem with dispatch trips $\bfg^*$ held fixed, denoted $\mathrm{RelocationProblem}(\bfg^*)$,
        we have the optimal dual variable $\lambda^*_{(\ell,d)}=\calQ^*(\ell,0) - \calQ^*(\ell,d,0)$ associated with 
        the inequality constraint $f_{(\ell,d)}\geq g_{(\ell,d)}$ for all routes $(\ell,d)$.
        Here, $\calQ^*(\ell,0)$ denotes the highest relocation utility under the welfare-optimal solution $(\bff^*,\bfg^*)$
        for a driver positioned at $\ell$, and
        $\calQ^*(\ell,d,0)$ denotes the relocation utility for driving towards $d$.  
\end{enumerate}

We now use properties of Lagrangian duality to compare the optimal solution with respect to dispatch trips $\bfg^*$ 
to the optimal solution with respect to dispatch trips $\bfg$.  For succinctness denote 
$R(g) = -\mathrm{RelocationProblem}(\bfg)$.

We use the fact that if $\bflambda$ is a KKT vector for the optimization problem (\ref{eq:relocation_problem})
then $-\bflambda$ is a subgradient for the function $-R(g)$.
This gives us the following condition
$$
-\bflambda^T(\bfg^*-\bfg)\geq R(\bfg^*) - R(\bfg).
$$
Expanding,
\begin{align*}
    \sum_{d\in\calL} -\lambda_{(\ell,d)}(g^*_{(\ell,d)} - g_{(\ell,d)}) \geq \Phi(\bff^*) - \Phi(\bff).
\end{align*}

Applying the same inequality to $\bflambda^*$,
\begin{align*}
    \sum_{d\in\calL} -\lambda_{(\ell,d)}^*(g_{(\ell,d)} - g^*_{(\ell,d)}) \geq \Phi(\bff) - \Phi(\bff^*).
\end{align*}

.

.

.

We say the routes $(\ell,d)$ for which the strict inequality (\ref{eq:excess_demand_condition}) holds have
excess demand.  Notice that a route only has excess demand if the dispatch-acceptance threshold the drivers
are using is too small:
$$
g_{(\ell,d)} < g^*_{(\ell,d)} \implies x_{(\ell,d)} < x^*_{(\ell,d)}.
$$

Under the dispatch-trips specified by $\bfg$, consider the pool of drivers who aren't allocated a dispatch trip.
At each location $\ell$ the pool of non-dispatched drivers has volume
$$
S_\ell - \sum_{d\in\calL}g_{(\ell,d)}.
$$
These drivers have to make a strategic decision about where to drive empty.
Suppose we gave these drivers an additional option: serve a dispatch on any route with excess demand,
and force them to incur the add-passenger disutility threshold $x^*_{(\ell,d)}$ from the original optimum
for this dispatch.  Because all of the routes with excess demand have an acceptance threshold smaller
than the optimal acceptance threshold, the utility from serving any one of these ``augmented'' dispatch trips
should be less than the utility of a relocation trip, so drivers won't be incentivized to take these dispatch trips.

\begin{align}
    \label{eq:excess_demand_problem}
    \mathrm{RelocProbExcessDemand}(\bfg)\equiv \ \ \ \ \ \ \ \ \ \ \ \ 
    \sup_{\bfh, \bfj} &\ \ \   \sum_{(\ell,d)} j_{(\ell,d)}\left(P_{(\ell,d)} - x^*_{(\ell,d)}\right) + \Phi(\bfh) & 
\\
    \mbox{subject to} & \nonumber\\ 
    & j_{(\ell,d)} \geq g_{(\ell,d)} & \forall (\ell,d)\in\calL^2\nonumber\\
    & j_{(\ell,d)} \leq g^*_{(\ell,d)} & \forall (\ell,d)\in\calL^2\nonumber\\
    & h_{(\ell,d)} \geq j_{(\ell,d)} \ &\forall (\ell,d)\in\calL^2\nonumber\\
    &
        \sum_{d\in\calL} h_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL.\nonumber
\end{align}

Associate the following dual variables with each of the constraints:
\begin{itemize}
    \item $\alpha_{(\ell,d)}$ for the $j_{(\ell,d)} \geq g_{(\ell,d)}$ constraints,
    \item $\beta_{(\ell,d)}$ for the $j_{(\ell,d)} \leq g^*_{(\ell,d)}$ constraints,
    \item $\gamma_{(\ell,d)}$ for the $h_{(\ell,d)} \geq j_{(\ell,d)}$ constraints,
    \item $\eta_\ell$ for the $\sum_{d\in\calL} h_{(\ell,d)} =S_\ell$  constraints.
\end{itemize}

We get the following stationarity conditions:
\begin{equation}
    \eta_\ell = \gamma_{(\ell,d)} + \frac{\partial}{\partial h_{(\ell,d)}}\Phi(h)
\end{equation}
and
\begin{equation}
    \gamma_{(\ell,d)} + \beta_{(\ell,d)} = \alpha_{(\ell,d)} + P_{(\ell,d)} - x^*_{(\ell,d)}.
\end{equation}
We now show that $(\bfg,\bff)$ and $(\bfg^*,\bff^*)$ are both optimal solutions to the relocation problem
with excess demand.

For the $(\bfg,\bff)$ solution, note that $f_{(\ell,d)} = g_{(\ell,d)}$ whenever $(\ell,d)$ has excess demand.
Since the threshold $x_{(\ell,d)}$ is smaller than $x^*_{(\ell,d)}$, the difference $P_{(\ell,d)} - x_{(\ell,d)} > 0$
is strictly positive, so if drivers are turning down dispatches towards $d$ at a profit then they are certaintly not taking
empty relocation trips towards $d$.
Set $$\eta_\ell=\calQ(\ell,0)$$ and set $$\gamma_{(\ell,d)} = \calQ(\ell,0) - \frac{\partial}{\partial f_{(\ell,d)}}\Phi(\bff).$$
Incentive-compatibility of $(\bfg,\bff)$ guarantees the complementary slackness conditions hold.




\subsubsection{Old Contents of Section}
\begin{theorem*} (Welfare-Robustness in the stochastic fluid model)
When the SSP mechanism is used to set prices in the stochastic fluid model, every equilibrium driver strategy achieves
optimal welfare.
\end{theorem*}

\begin{proof}

Consider a scenario $\omega_t$ and a supply-location vector 
    $\bfS=(S_\ell:\ell\in\calL)$.  The SSP mechanism sets prices at time-scenario $\omega_t$ and supply-location
    vector $\bfS$ based on an optimal solution to the following state-dependent optimization problem 
    (\ref{eq:dynamic_optimization_recursive}). \mccomment{insert sentence to describe high-level ideas of proof before
    diving in to details}

    \medskip
    \noindent \textbf{Problem Setup.}
    We start by re-stating the state-dependent stochastic flow problem (\ref{eq:dynamic_optimization_recursive}).
    For simplicity, when referring to the trip type $(o,d,\omega_t)$, which refers to a trip from an 
    origin location $o$ to a destination location $d$ under the time-scenario $\omega_t$, we drop the scenario from the
    notation and just write $(o,d)$.  With this convention, our decision variables become total-trip volumes
    $\bff=(f_{(o,d)}:(o,d)\in\calL^2)$ and dispatch-trip volumes $\bfg=(g_{(o,d)}:(o,d)\in\calL^2)$,
    and the state-dependent optimization problem (\ref{eq:dynamic_optimization_recursive}) can be written
    as follows:
\begin{align}
 \sup_{\bff, \bfg} &\ \ \  \sum_{\substack{(o,d)\in\\\calL^2}} U_{(o,d)}(f_{(o,d)}, g_{(o,d)}) - 
        \sum_{\ell\in\calL} A\left(\bfg^T\bfone_{(\ell)},\bff^T\bfone_{(\ell)}\right)
         + 
    \Phi_{\omega_t}(\bff)
 & 
\label{eq:robust_welf_proof_optimization}\\
    \mbox{subject to} & \nonumber\\ 
    & f_{(o,d)} \geq 0 \ &\forall (o,d)\in\calL^2\nonumber\\
    & g_{(o,d)} \geq 0 \ &\forall (o,d)\in\calL^2\nonumber\\
    & f_{(o,d)} \geq g_{(o,d)} \ &\forall (o,d)\in\calL^2 \nonumber\\
    &
        \sum_{d\in\calL} f_{(\ell,d)} =
        S_\ell 
    \ & \forall \ell\in\calL,\nonumber
\end{align}
    where $\Phi_{\omega_t}(\bff)$ is the optimal continuation welfare from the market state at the subsequent time period,
    each term $A\left(\bfg^T\bfone_{(\ell)},\bff^T\bfone_{(\ell)}\right)$ is equal to the idiosyncratic add-passenger
    disutility incurred by drivers positioned at $\ell$ who serve a dispatch, and $U_{(o,d)}(f_{(o,d)}, g_{(o,d)})$ is
    the sum of the rider utility and driving costs when $f_{(o,d)}$ drivers from $o$ drive towards $d$ and $g_{(o,d)}$
    dispatches are served.

    The SSP mechanism operates by computing an optimal solution $(\bff^*,\bfg^*)$ to (\ref{eq:robust_welf_proof_optimization})
    and setting prices $P_{(o,d)}$ on each route $(o,d)$ to select for rider dispatch requests from the upper quantile of the
    willingness-to-pay distribution, subject to the dispatch capacity $g_{(o,d)}^*$ specified by the optimal solution.
    That is, the price is equal to
    $$
        P_{(o,d)} = F_{(o,d,\omega_t)}^{-1}\left(1-\frac{g_{(o,d)}^*}{\bar{D}_{(o,d,\omega_t)}}\right),
    $$
    where $F_{(o,d,\omega_t)}(\cdot)$ is the CDF of the willingness-to-pay distribution for riders interested in the route 
    $(o,d,\omega_t)$, and $\bar{D}_{(o,d,\omega_t)}$ is the fluid volume of riders interested in the route $(o,d,\omega_t)$.


    \medskip
    \noindent \textbf{Arbitrary Strategy-Profile in the Stochastic Fluid Model}
    The theorem statement concerns arbitrary equilibrium driver strategies under the SSP prices.
    An arbitrary driver strategy is encoded by the single-timeperiod stochastic flow decision variables
    $(\bfa,\bfb)$, such that the components of $\bfb$ specify dispatch-trip volumes and the components of $\bfa$
    specify total (relocation and dispatch) trip volumes. In contrast to the optimization formulation (\ref{eq:robust_welf_proof_optimization}),
    where our decision variables $(\bff,\bfg)$ only specified trip volumes on each origin-destination pair, 
    for an arbitrary equilibrium $(\bfa,\bfb)$ we have to specify the actions drivers take at each distinct level of add-passenger
    disutility $C^{ID}$.  In the context of the optimization formulation (\ref{eq:robust_welf_proof_optimization}) we could avoid this complication
    because we know the optimal centralized solution always allocates dispatch trips to drivers with the lowest possible add-passenger disutility
    values.  However, we can't make this assumption a priori about an arbitrary equilibrium.

    Recall add-passenger disutility values $C^{ID}$ are sampled from a $\mathrm{Uniform}(0,C)$ distribution.
    The components of $\bfa$ are now functions $a_{(o,d)}:[0,C]\to\bbR_+$, mapping add-passenger disutility values $C^{ID}$ to total trip
    volumes $a_{(o,d)}(C^{ID})$ on each origin-destination pair $(o,d)\in\calL^2$. Similarly, the components of $\bfb$ are functions
    $b_{(o,d)}:[0,C]\to\bbR_+$ mapping add-passenger disutility values $C^{ID}$ to dispatch trip volumes $b_{(o,d)}(C^{ID})$.
    \mccomment{Need assumption about measurability of $\bfa$ and $\bfb$}

    In order for the functions $(\bfa,\bfb)$ to specify a feasible strategy profile the following conditions must be satisfied:
    \begin{enumerate}
        \item For each add-passenger disutility value $C^{ID}$ the number of dispatch trips can never exceed the total number of trips: 
            $b_{(o,d)}(C^{ID})\leq a_{(o,d)}(C^{ID})$ for all $C^{ID}$.
        \item The total trip volume allocated to drivers positioned at a location $\ell$, whose add-passenger disutility value is $C^{ID}$,
            must be proportional to the volume of drivers positioned at $\ell$ at the specified add-passenger disutility value.
            This condition depends on the realized supply-location vector $\bfS=(S_\ell:\ell\in\calL)$, where each component $S_\ell$
            specifies the volume of drivers positioned at $\ell$.  Given $S_\ell$ drivers positioned at $\ell$, the volume of drivers at $\ell$
            whose add-passenger disutility is equal to $C^{ID}$ is proportional to $S_\ell\phi(C^{ID})$, where $\phi:[0,C]\to\bbR_+$ is the probability density
            function of the $\mathrm{Uniform}(0,C)$ distribution from which drivers sample their add-passenger disutilities.
            Note that $\phi(C^{ID})=\frac{1}{C}$.  Thus, for each location $\ell$ and each disutility value $C^{ID}\in[0,1]$, the following equality holds:
            \begin{equation}
            \sum_{(o,d)\in\calL^2} a_{(o,d)}(C^{ID}) = S_\ell \phi(C^{ID}) = \frac{S_\ell}{C}.
            \end{equation}
        \item The total volume of dispatch trips that drivers serve on each route over all add-passenger disutility values does not exceed the 
            demand for dispatch trips on that route under the prices set by the SSP mechanism.  The SSP prices are chosen so that the resulting
            demand for dispatch trips on each route is exactly equal to the volume of dispatch trips served by drivers on that route under the welfare-optimal solution.
            That is, if $(\bff^*,\bfg^*)$ is the optimal solution to (\ref{eq:robust_welf_proof_optimization}) used by the SSP mechanism to set prices, then the
            resulting dispatch demand on origin-destination pair is equal to $g^*_{(o,d)}$.  Thus for $(\bfa,\bfb)$ to specify a feasible strategy profile,
            the total dispatch demand on each origin-destination pair cannot exceed $g^*_{(o,d)}$.  This condition can be written in terms of the following
            integral, where $x\in[0,C]$ ranges over all add-passenger disutility values.
            \begin{equation}
            \int_{0}^C b_{(o,d)}(x)\phi(x)dx \leq g^*_{(o,d)}.
            \end{equation}
    \end{enumerate}

    \medskip
    \noindent
    \textbf{What it Means for an Arbitrary Strategy Profile to be an Equilibrium}
    .

    .

    .
    \mccomment{
        \begin{itemize}
        \item what does it mean for $(\bfa,\bfb)$ to be an equilibrium.
        \end{itemize}
    }

    Let $\phi(x)=\frac{1}{C}$, $x\in [0,C]$, be the probability density function for the $\mathrm{Uniform}(0,C)$ distribution.

    $f_{(o,d)}$ specifies the total volume of trips from $o$ to $d$, and $g_{(o,d)}$ specifies
    the total volume of dispatch trips from $o$ to $d$, for each origin-destination pair $(o,d)\in\calL^2$. 
    In order for $(\bff,\bfg)$ to describe a feasible driver strategy, the following properties must be satisfied:
    \begin{enumerate}
        \item $(\bff,\bfg)$ has to be a feasible solution to the state-dependent optimization problem 
            (\ref{eq:robust_welf_proof_optimization}).
        \item The number of dispatch trips $g_{(o,d)}$ for each origin-destination $(o,d)\in\calL^2$ is at most
            the dispatch demand which occurs under the price $P_{(o,d)}$.  The price $P_{(o,d)}$ is chosen to balance
            dispatch demand with dispatch supply under the computed welfare-optimal solution, i.e. under the price 
            $P_{(o,d)}$ the dispatch demand volume is equal to $g^*_{(o,d)}$. Therefore, the number of dispatches under an
            arbitrary equilibrium cannot exceed the dispatch-volume under the computed welfare-optimal solution:
            $$g_{(o,d)} \leq g^*_{(o,d)}.$$
    \end{enumerate}

    When describing an arbitrary driver strategy we also need to specify how the aggregate trip counts are allocated to
    individual drivers once their idiosyncratic add-passenger disutilities have been sampled for the given timeperiod.
    We claim that, for any equilibrium strategy $(\bff,\bfg)$, and for each location $\ell$, 
    dispatch trips are only allocated to drivers whose add-passenger  disutility lies
    in the bottom $\frac{\bfg^{*T}\bfone_\ell}{\bff^{*T}\bfone_\ell}$ quantile of the add-passenger disutility distribution.
    Note that $\frac{\bfg^{*T}\bfone_\ell}{\bff^{*T}\bfone_\ell}$ is the fraction of drivers positioned at $\ell$ who serve
    a dispatch trip under the optimal solution $(\bff^*,\bfg^*)$, whereas $\frac{\bfg^{T}\bfone_\ell}{\bff^{T}\bfone_\ell}$
    is the fraction of drivers positioned at $\ell$ who serve a dispatch under the arbitrary equilibrium $(\bff,\bfg)$.
    The fraction of drivers who serve a dispatch under $(\bff,\bfg)$ can be at most the fraction of drivers who serve
    a dispatch under $(\bff^*,\bfg^*)$, by virtue of the dispatch-demand capacity constraint $g_{(o,d)}\leq g^*_{(o,d)}$.

    The claim that, in any equilibrium driver strategy, dispatch trips are only allocated to drivers whose add-passenger
    disutility falls in the bottom $\frac{\bfg^{*T}\bfone_\ell}{\bff^{*T}\bfone_\ell}$ quantile of the add-passenger
    distribution is a simple property of the optimality conditions (\mccomment{ref}).
    Indeed, if $C^{ID}$ is an idiosyncratic add-passenger disutility value that
    exceeds the appropriate threshold, then $P_{(\ell,d)} - C^{ID}<0$ for any destination $d$, so these drivers always prefer
    to drive empty than to serve a dispatch.

    A driver's action is described by the tuple $(\ell,d,\delta,C^{ID})$, where $\ell$ is the driver's origin location,
    $d$ is the destination location, $\delta\in\{0,1\}$ is an indicator specifying whether or not the trip fulfils a dispatch,
    and $C^{ID}$ is the idiosyncratic add-passenger disutility sampled by the driver.  Let $\calQ(\ell,d,\delta,C^{ID})$ be
    the expected utility-to-go of a driver who takes the action $(\ell,d,\delta,C^{ID})$ under the arbitrary equilibrium
    strategy we are considering.  These Q-values are defined by the recursion:
    \begin{equation}
    \label{eq:Q_val_recursion}
        \calQ(\ell,d,\delta,C^{ID}) = \delta (P_{(\ell,d)}-C^{ID}) - c_{(\ell,d)} +
        \bbE\left[\calV_{(d,\omega_{t+1})}\mid\omega_t\right],
    \end{equation}
    where $\calV_{(d,\omega_{t+1})}$ is the expected utility-to-go of being positioned at location $d$ under the
    expected subsequent time-scenario $\omega_{t+1}$.
    The expected utility-to-go of being positioned at $\ell$ under the time-scenario $\omega_t$ is defined as the
    expectation
    \begin{equation}
    \label{eq:V_def}
        \calV_{(\ell,\omega_t)} = \bbE\left[\calQ(\ell,\hat{d},\hat{\delta},\hat{C^{ID}})\right],
    \end{equation}
    where $(\hat{d},\hat{\delta},\hat{C^{ID}})$ is the joint random variable over a driver's destination trip, dispatch-indicator,
    and idiosyncratic add-passenger disutility.


    \medskip
    \noindent \textbf{Backwards Induction Assumption.}
    We assume, via backwards induction, that every equilibrium driver strategy at future time periods is equal to the dual
    variables associated with the flow-conservation constraints for the locations in those time periods.
    Under the arbitrary equilibrium $(\bff,\bfg)$, the supply-location vector $\bfS_{\omega_{t+1}}(\bff)$ gives the
    spatial distribution of drivers in the subsequent time period under the scenario $\omega_{t+1}$.
    We assume the utility-to-go of being positioned at each location $\ell$ under each subsequent scenario $\omega_{t+1}$
    is equal to the dual variable for the flow-conservation constraint associated with $\ell$ in the state-dependent
    optimization problem at $\omega_{t+1}$ with respect to $\bfS_{\omega_{t+1}}(\bff)$:
    $$
    \calV_{(\ell,\omega_{t+1})} = \eta_{(\ell,\omega_{t+1})}(\bfS_{\omega_{t+1}}(\bff)) 
    = \frac{\partial}{\partial S_\ell} \calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff)),
    $$
    where the second equality follows from the conclusion of Lemma \mccomment{insert}, which shows equality between
    partial derivatives of the state-dependent optimal welfare function $\calW_{\omega_{t+1}}(\cdot)$ and the optimal
    dual variables associated with the flow-conservation constraints.
    This assumption gives us a characterization of the Q-values in terms of the partial derivatives of the continuation
    welfare function $\Phi_{\omega_t}(\bff)$:
    \begin{align}
        \calQ(\ell,d,\delta,C^{ID}) &= 
        \delta (P_{(\ell,d)}-C^{ID}) - c_{(\ell,d)} + \bbE\left[\calV_{(d,\omega_{t+1})}\mid\omega_t\right]\nonumber\\
        &=
        \delta (P_{(\ell,d)}-C^{ID}) - c_{(\ell,d)} + \bbE\left[\frac{\partial}{\partial S_d} 
                \calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))
                \mid\omega_t\right]\nonumber\\
        &=\delta (P_{(\ell,d)}-C^{ID}) - c_{(\ell,d)} + \frac{\partial}{\partial f_{(\ell,d)}} 
                \bbE\left[\calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))
        \mid\omega_t\right]\nonumber\\
&=\delta (P_{(\ell,d)}-C^{ID}) - c_{(\ell,d)} + \frac{\partial}{\partial f_{(\ell,d)}} 
        \Phi_{\omega_t}(\bff).
    \end{align}
    The penultimate line above uses the equality
    $$
\frac{\partial}{\partial S_d}\calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))
=\frac{\partial}{\partial f_{(\ell,d)}}\calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff)),
    $$
    which follows from the chain rule, since the $S_d$ component of $\bfS_{\omega_{t+1}}(\bff)$ is the sum of the $f_{(o,d)}$
    components of $\bff$ over all origin locations $o\in\calL$.
    .

    .

    .

    Let $(\bff^*,\bfg^*)$ be a solution to the state-dependent stochastic
    flow problem (\ref{eq:dynamic_optimization_recursive}) and let $P_{(o,d,\omega_t)} = P_{(o,d,\omega_t)}(g^*_{(o,d,\omega_t)})$
    be the price the SSP mechanism charges on each trip $(o,d,\omega_t)$ under the time-scenario $\omega_t$.

For simplicity of notation, label each of the LT-scenarios $(l,\omega_t)$ with
$i=1,\dots,n$, and assume without loss of generality that
the ODT-scenarios $(r,\omega_t)$ are in one-to-one correspondence with pairs
of locations $(i,j)\in[n]^2$.

Let $x_{ij}$ be a variable which indicates the amount of flow we allocate along
each route $(i,j)$ in the current time period, let $x=(x_{ij}:1\leq i,j\leq n)$
be a vector that encodes the flow in the current time period, and let
$\Phi(x)$ be a function that equals the optimal welfare over future time periods,
given the flow $x$ for the current time period.
The optimization problem (\ref{eq:dynamic_optimization}) can then be
restated as follows:
\begin{equation}
    \label{eq:original_problem}
    \sup_x \left( \sum_{i,j=1}^n U_{ij}(x_{ij}) + \Phi(x) : \mbox{ subject to } 
\forall i\ S_i=\sum_{j=1}^nx_{ij},
\ \forall i,j\ x_{ij}\geq 0
\right).
\end{equation}

The SSP mechanism computes an optimal solution $x^*$ and sets the price along route $ij$
as
$$
\rho_{ij}^* = \frac{d}{dx_{ij}}U_i(x_{ij}^*).
$$
The optimality conditions state there exists a dual variable $\eta_i^*$, associated with the equality constraint for each location $i$, and dual variables $\alpha_{ij}^*\geq 0$, associated with each inequality constraint, satisfying
$$
\eta_i^* = \rho_{ij}^* + \frac{\partial}{\partial x_{ij}}\Phi(x^*) + \alpha_{ij}^*
\ \ 
\forall ij,
$$
as well as the complementary slackness conditions
$$
\alpha_{ij}^*x_{ij}^* = 0.
$$

After we set the prices $\rho^* = (\rho_{ij}^*:1\leq i,j\leq n)$ we find a new feasible solution $x$ which is an equilibrium under $\rho^*$.  This means
there exists a number $V_i$, for each location $i$, for which the following equations holds
\begin{equation}
    \label{eq:V_i_def}V_i = \rho_{ij}^* + \frac{\partial}{\partial x_{ij}}\Phi(x) + \beta_{ij} \ \ 
\forall i,j,
\end{equation}
where $\beta_{ij}$ is defined as
$$
\beta_{ij} = \begin{cases}
0 & \mbox{ if }x_{ij} > 0,\\
V_i - \rho_{ij}^* - \frac{\partial}{\partial x_{ij}}\Phi(x) & \mbox{ else}.
\end{cases}
$$
From $x$ being an equilibrium, it also holds that $\beta_{ij}\geq 0$ is always true.
The above conditions are almost equivalent to the Lagrangian optimality
conditions; the key difference being that the $\rho_{ij}^*$ quantity, appearing
in equation (\ref{eq:V_i_def}), does not depend on the equilibrium $x$, as the price fixed by the SSP mechanism is produced before the drivers choose their trips.

Nonetheless, we will show that the arbitrary equilibrium $x$ achieves optimal welfare for the problem (\ref{eq:original_problem}). 

\medskip
\noindent \textbf{Capacitated Linearized Problem.}
We demonstrate optimality of an arbitrary equilibrium $x$ by
considering a linearized version of the optimization problem
(\ref{eq:original_problem}), in which the total-utility functions
$U_{ij}(x_{ij})$ are replaced by linear functions which reflect
only the utility collected by drivers for taking a passenger.


 For each edge
$ij\in [n]^2$, let $(ij,1)$ indicate the copy of edge $ij$ that
includes a passenger, and let $(ij,0)$ indicate the copy of edge $ij$
that does not include a passenger.
We can represent an optimal solution for the original optimization
problem (\ref{eq:original_problem}) in terms of this 
passenger-distinguishing parameterization as follows.  

Let $x^*=(x_{ij}^*)$ be an optimal solution for
(\ref{eq:original_problem}) using the original parameterization,
let $\rho=(\rho_{ij})$ be the prices set by our mechanism, and let $d_{ij}$ be the
amount of rider demand for each edge $ij$ resulting from our prices.
Note $d_{ij}$ is the number of passenger-trips that occur on edge $ij$
under $x^*$, and $\max(0,x_{ij}^* - d_{ij})$ is the number of relocation-trips that occur on edge $ij$ under $x^*$. Thus we can represent $x^*$ using the passenger-distinguishing parameterization
by defining
$$
x_{(ij,\delta)}^* = \begin{cases}
d_{ij}, & \mbox{if }\delta = 1,\\
\max(0,d_{ij} - x_{ij}^*), & \mbox{if }\delta = 0,
\end{cases}
$$
for each $(ij,\delta)\in [n]^2\times\{0,1\}$.

Consider the following linearized version of the optimization
problem (\ref{eq:original_problem})\footnote{For the purpose of this formulation, we assume the function $\Phi(y)$ includes the linear travel cost terms for each of the routes in the current time period,
i.e. $-c_{ij}(y_{ij,0} + y_{ij,1})$ for each $ij\in[n]^2$.}:
$$
\sup\left(\sum_{i,j=1}^n \rho_{ij} y_{(ij,1)} + \Phi(y) : \forall i\ \sum_{j,\delta} y_{(ij,\delta)} = S_i,\ \forall (ij,\delta) \ y_{(ij,\delta)} \geq 0, \ \forall ij\ y_{(ij,1)}\leq x_{(ij,1)}^* \right).
$$
For a feasible solution $y$ to be 
optimal we get the optimality
conditions
$$
\eta_i = \rho_{ij} + 
\frac{\partial}{\partial y_{(ij,1)}}\Phi(y)
+ \alpha_{(ij,1)} - \gamma_{ij},
$$
and
$$
\eta_i = \frac{\partial}{\partial y_{(ij,0)}}\Phi(y)
+ \alpha_{(ij,0)},
$$
with complementary slackness
conditions:
$$
y_{(ij,1)}\alpha_{(ij,1)} = 0,\ \ 
y_{(ij,0)}\alpha_{(ij,0)} = 0,\ \ 
(x_{(ij,1)}^* - y_{(ij,1)})\gamma_{ij} = 0.
$$
Here, $\alpha_{(ij,\delta)}$ is a dual
variable associated with the $y_{(ij,\delta)}\geq 0$ constraint,
$\eta_i$ is a dual variable associated with
the flow-conservation constraint for location $i$,
$\gamma_{ij}$ is a dual variable associated
with the capacity constraint $y_{(ij,1)} \leq x^*_{(ij,1)}$.
It is also worth noting that the
welfare-to-go function $\Phi$ only
depends on the sum $y_{(ij,0)}+y_{(ij,1)}$ for each
edge $i$, so the partial derivatives $\frac{\partial}{\partial y_{(ij,0)}}\Phi(y)$ and
$\frac{\partial}{\partial y_{(ij,1)}}\Phi(y)$ are equal.
Note that our original optimum $x^*$ satisfies these conditions.

\medskip
\noindent
\textbf{Optimality of Arbitrary Equilibrium for the Capacitated Linearized Problem.}
Let $y=(y_{(ij,\delta)})$ be a 
flow corresponding to an 
equilibrium among the drivers.
This means there is no profitable deviation: no driver can increase
their welfare by taking a relocation trip along any edge, or
a passenger trip along an edge with excess passenger capacity.
We will show that $y$ is optimal by deriving, from the equilibrium condition,
 dual variables for which the optimality conditions are satisfied.

Let $V_{(ij,\delta)}$ be the utility generated on edge $(ij,\delta)$ under
the equilibrium $y$.  The dual variables are obtained as follows:
Let $\eta_i$ be the minimum utility generated on any edge $(ij,\delta)$ where
a nonzero number of drivers go,
let $\gamma_{ij}=max(V_{(ij,1)} - \eta_i, 0)$ for each $ij$, and let
$\alpha_{(ij,\delta)} = \max(\eta_i - V_{(ij,\delta)}, 0)$ for each $(ij,\delta)$.

The stationarity conditions  between $y$ and $(\alpha,\eta,\gamma)$
holds by definition . Complementary slackness follows for the following reasons:
\begin{itemize}
\item The utility $V_{(ij,1)}$ only exceeds $\eta_i$ when it is a passenger-trip edge and when that edge is at capacity, which means $\gamma_{ij}$ is only nonzero when $y_{(ij,1)} = x_{(ij,1)}^*$. Note the utility $V_{(ij,0)}$, for any edge $(ij,0)$ encoding a relocation-trip, will never exceed $\eta_i$, otherwise some drivers would have a profitable deviation to take that edge.
\item The utility $V_{(ij,\delta)}$ is smaller than $\eta_i$ only when no drivers
traverse $(ij,\delta)$, hence $\alpha_{(ij,\delta)}$ is only nonzero when 
$y_{(ij,\delta)}$ is zero.
\end{itemize}
Therefore the dual variables $(\alpha,\eta,\gamma)$ certify the optimality
of $y$ for the capacitated linearized problem.

\medskip
\noindent
\textbf{Optimality of an Arbitrary Equilibrium for the Original Problem.}
Note that complementary slackness holds between any primal optimum and any dual optimum, so we know that $y$ satisfies 
the complementary slackness conditions (for the capacitated linearized problem)
with respect to dual variables $(\alpha^*,\eta^*,\gamma^*)$ associated with the original optimum $x^*$.  We will show this is enough to conclude that $y$ is optimal for the original problem.

First, we claim that all rider-demand 
arising under the prices $\rho$ must receive a dispatch under the equilibrium $y$.
To see this, note the following:
\begin{itemize}
    \item The utility $V_{(ij,\delta)}$,
for any edge $(ij,\delta)$ that drivers actually take under $y$, is equal to the  dual value $\eta_i^*$.
    \item 
    The utility $V_{(ij,1)}$ for any passenger-trip edge $(ij,1)$ with nonzero capacity is equal to $\eta_i^*$, since
    $y$ satisfies complementary slackness
    with respect to $(\alpha^*,\eta^*,\gamma^*)$ and since nonzero capacity on edge $(i,1)$ means
    $\alpha_{ij}^*=0$.
    \item The total capacity for passenger-trip edges is $\sum_{j}x^*_{(ij,1)}\leq S_i$. 
\end{itemize}
Since the utility collected by the driver along each passenger-trip edge $(ij,1)$ with nonzero capacity is $\eta_i^*$, and since we assume drivers are incentivized to drive with a passenger (all else being equal), then the equilibrium $y$ must use all available passenger-trip edge capacity, otherwise some drivers would be incentivized to deviate to one of the available passenger-trip edges.


Let $y'=(y'_i : i=1,\dots,n)$ be a reparameterization of the equilibrium $y$ that drops the passenger-trip vs. relocation-trip distinction, so each
component is defined as $y'_i = y_{(i,0)} + y_{(i,1)}$.  We will show that $y'$ is optimal for the original problem by establishing the optimality conditions hold between $y'$ and $(\alpha^*,\eta^*)$.
To show that the optimality conditions hold for the original problem, we have to establish the following equality for every edge $ij$: 
$$
\eta_i^* = \frac{d}{dy'_{ij}}U_i(y'_{ij}) + \Phi(y') + \alpha_{ij}^*,
$$
and we have to show the complementary slackness conditions $y_{ij}'\alpha_{ij}^*=0$ hold.
From $y$ satisfying optimality conditions for the linearized problem, we already know the the complementary conditions $y_{ij}'\alpha_{ij}^*=0$ hold for each $ij$, and we have the following equality for each $ij$:
$$
\eta_i^* = \rho_{ij} + \Phi(y') + \alpha_{ij}^*.
$$

What's left is to show that $\frac{d}{dy'_{ij}}U_i(y'_{ij}) = \rho_{ij}$ holds for each $ij$.
This equality follows from the fact that all rider demand arising under the prices $\rho$ receives a dispatch under the equilibrium $y$.

For an edge $ij$ with nonzero trip price $\rho_{ij}>0$, note that the equilibrium $y$ will never send a relocation-trip along edge $ij$, because we have already established that all trips under $y$ generate utility $\eta_i^*$ for the driver, and it is impossible for a passenger-trip and a relocation-trip using the same edge to generate the same utility when the price is nonzero.  Thus, the 
flow value $y_{ij}'$ from the equilibrium solution $y_{ij}'$
is the same as the flow value $x_{ij}^*$ from the original optimum $x^*$, so 
$\frac{d}{dy'_{ij}}U_{ij}(y'_{ij}) = \rho_{ij} =\frac{d}{dx^*_{ij}}U_{ij}(x^*_{ij}) $ holds in this case.

For an edge $ij$ where the trip price $\rho_{ij}$ is zero, we know that the volume of dispatches $x^*_{(ij,1)}$ allocated to this edge under the original optimum is equal to the total volume of (price-inquiry) rider demand for this edge.  Since the equilibrium $y$ serves all rider demand arising under our prices we know that the flow value $y_{ij}'$ is at least $x^*_{(ij,1)}$.  We also know the
utility reward function $U_{ij}(\cdot)$ is constant for flow values which exceed the total amount of rider demand.  Thus $\frac{d}{dy'_{ij}}U_{ij}(y'_{ij})=0=\rho_{ij}$ is true in this case as well.

Therefore $y'$ and $(\alpha^*,\eta^*)$ together satisfy the optimality conditions for the original optimization problem, 
establishing that an arbitrary equilibrium under the SSP pricing mechanism achieves optimal welfare.

\end{proof}


==> fluid_strategy_profile_assns.tex <==

In the fluid model we use a 3-tuple $(\bff,\bfg,\bfx)$ to represent the aggregate actions that drivers take in
a single time period.
$\bff=(f_{(\ell,d)} : (\ell,d)\in\calL^2)$ is a vector specifying the total trip volume (dispatch trips plus relocation trips) on each route,
$\bfg=(g_{(\ell,d)} : (\ell,d)\in\calL^2)$ is a vector specifying the dispatch trip volume on each route,
and $\bfx = (x_{(\ell,d)} : (\ell,d)\in\calL^2)$ is a vector specifying the communal acceptance thresholds used by all drivers, where 
 positioned at $\ell$ who receive dispatches towards a destination $d$ only accept this dispatch if their add-passenger disutility does not exceed 
$x_{(\ell,d)}$.

Notice that this definition of a fluid strategy presupposes that all drivers use a common disutility-acceptance threshold $\bfx$,
which is different from our assumption in the two-level model where individual drivers were free to choose different thresholds.
We will show that, for strategy profiles in the two-level model that are approximate equilibria, each driver does use approximately
the same acceptance thresholds as their peers. Therefore, the assumption that drivers all use the same acceptance threshold
in the fluid model will be amenable to the analysis of equilibrium strategy profiles from the two-level model.


Feasibility of a fluid strategy depends on the supply-location vector $\bfS_t=(S_\ell : \ell\in\calL)$, where $S_\ell$ specifies
the volume of drivers positioned at location $\ell$, as well as the dispatch-demand vector $\bar{\bfr}_t=(\bar{r}_{(\ell,d)} : (\ell,d)\in\calL^2)$,
where $\bar{r}_{(\ell,d)}$ represents the dispatch demand volume for each route $(\ell,d)$ under the pricing policy used by the platform.
In order for a tuple $(\bff,\bfg,\bfx)$ to represent a feasible fluid strategy with respect to $\bfS_t$ and $\bar{\bfr}_t$, the following conditions
must be satisfied:
\begin{enumerate}
    \item \label{item:first_feasibility} Each component of $\bff,\bfg,\bfx$ must be nonnegative.
    \item Total trip volume can be at least as large as dispatch trip volume on each route, i.e. $f_{(\ell,d)} \geq g_{(\ell,d)}$ for all $(\ell,d)$.

    \item Dispatch trip volume can be at most as large as dispatch trip demand for each route. That is, if $\bar{r}_{(\ell,d)}$ is the
dispatch request volume on each route $(\ell,d)$, then $\bar{r}_{(\ell,d)} \geq g_{(\ell,d)}$ for all $(\ell,d)$ must be satisfied.

    \item\label{item:trip_volume_feasibility} Total trip volume originating from each location matches the total volume of supply positioned at the location,
        i.e. if $S_\ell$ drivers are positioned at location $\ell$ then the equality $S_\ell=\sum_d f_{(\ell,d)}$ must be satisfied for every location $\ell$.
    \item \label{item:penultimate} The acceptance thresholds specified by $\bfx$ are compatible with the dispatch trip volumes specified by $\bfg$.
        Since we assume the platform can't observe the driver's add-passenger disutilities, the matching process effectively partitions drivers
        based on the destination towards which they are dispatched.  If $g_{(\ell,d)}$ is the volume of drivers who accept a dispatch from $\ell$
        to $d$, then a larger volume $Z_{(\ell,d)}$ of drivers were offered a dispatch from $\ell$ to $d$.  We can recover the volume $Z_{(\ell,d)}$
        from $g_{(\ell,d)}$ and the acceptance threshold $x_{(\ell,d)}$:
        $$
        g_{(\ell,d)} = \bbP(X\leq x_{(\ell,d)}) Z_{(\ell,d)} = \frac{x_{(\ell,d)}}{C}Z_{(\ell,d)}, 
        $$
        therefore $Z_{(\ell,d)} = \frac{Cg_{(\ell,d)}}{x_{(\ell,d)}}$.
        \mccomment{Need to say something for the case where $x_{(\ell,d)} = 0$. Easiest solution would just be to limit attention to strategies that
        never set $x_{(\ell,d)} = 0$ when $\bar{r}_{(\ell,d)} > 0$. Thoughts?}
        We assume that drivers can be allocated at most one dispatch destination.  Therefore, in order for $(\bff,\bfg,\bfx)$ to be feasible, the
        implied size of the partitions $Z_{(\ell,d)}$ cannot exceed the total volume of available drivers.  That is, for each location $\ell$ the following
        condition must be satisfied:
        \begin{equation}
            S_\ell \geq \sum_{d\in\calL} Z_{(\ell,d)} = \sum_{d\in\calL} \frac{Cg_{(\ell,d)}}{x_{(\ell,d)}}.
        \end{equation}
    \item \label{item:last_feasibility}
        We assume the matching process only terminates when all the drivers have been allocated a dispatch, or when all demand has been served.
        Therefore, in order for $(\bff,\bfg,\bfx)$ to represent a feasible fluid strategy, at least one of the following two conditions must be satisfied
        for each location $\ell$:
        \begin{itemize}
        \item All the demand originating from $\ell$ has been served, i.e. $g_{(\ell,d)} = \bar{r}_{(\ell,d)}$ for all destinations $d$.
        \item All drivers have been allocated a dispatch, i.e. 
            \begin{equation}
                S_\ell = \sum_{d\in\calL} Z_{(\ell,d)} = \sum_{d\in\calL}\frac{Cg_{(\ell,d)}}{x_{(\ell,d)}}.
            \end{equation}
        \end{itemize}
\end{enumerate}

A strategy profile in the fluid model is a sequence of functions $\Sigma=(\Sigma_1,\dots,\Sigma_T)$, indexed by the time period $t$,
where $\Sigma_t : \Omega_t \times \calS \to \bbR^{\calL^2}_+\times\bbR^{\calL^2}_+\times\bbR^{\calL^2}_+$
is a function which takes a market state $(\omega_t,\bfS_t)$ as input and produces a feasible trip specification $(\bff,\bfg,\bfx)=\Sigma_t(\omega_t,\bfS_t)$.

In order to define what it means for a fluid strategy profile $\Sigma=(\Sigma_1,\dots,\Sigma_T)$ to be an equilibrium strategy profile,
we associated with $\Sigma$ a value function for each location and a Q-value for each trip type.

The value function induced by $\Sigma$ is a sequence of functions $\bar{\calV}=(\bar{\calV}_1,\dots,\bar{\calV}_T)$,
where $$\bar{\calV}_t : \calL\times\Omega_t\times\calS\to\bbR_+$$ takes as input a location $\ell$ and a market state $(\omega_t,\bfS_t)$
and produces a number $\bar{\calV}_t(\ell,\omega_t,\bfS_t)$ which corresponds to the expected utility-to-go of a driver positioned at $\ell$, under the market
state $(\omega_t,\bfS_t)$, assuming the drivers play according to $\Sigma$.

The Q-values induced by $\Sigma$ is similarly a sequence of functions $\bar{\calQ} = (\bar{\calQ}_1,\dots,\bar{\calQ}_T)$,
where $$\bar{\calQ}_t:\calA\times[0,C]\times\Omega_t\times\calS\to\bbR_+$$ takes as input an action $a\in \calA$, an add-passenger disutility $X\in [0,C]$, and a market state $(\omega_t,\bfS_t)$
and produces a number $\bar{\calQ}_t(a,\omega_t,\bfS_t)$ which corresponds to the expected utility-to-go of a driver who takes the action (trip)
specified by $a$ and has add-passenger disutility equal to $X$, assuming the market state at time $t$ is $(\omega_t,\bfS_t)$ and assuming the drivers play according to $\Sigma$.

We define the value function and the Q-values associated with a strategy profile $\Sigma$ recursively.  For the base case, assume that
$\bar{\calV}_t(\ell,\omega_t,\bfS_t)$ is always $0$ whenever $t$ exceeds the final time period $T$.
Fix a time period $t$ and assume the value function and Q-values have been defined for time periods larger than $t$.

We start by defining the Q-values.  Given an arbitrary trip type $a=(\ell,d,\delta)\in\calA$, and an add-passenger disutility $X\in [0,C]$, define the associated
Q-value as:
\begin{equation}
\bar{\calQ}_t((\ell,d,\delta), X, \omega_t,\bfS_t) =\delta(P_{(\ell,d)} - X) -c_{(\ell,d)} + \bbE\left[\bar{\calV}_{t+1}(d,\omega_{t+1},\bar{\bfS}_{\omega_{t+1}}(\bff))\right].
\end{equation}
In the above, $\delta\in\{0,1\}$ is an indicator specifying whether or not the trip serves a dispatch, $P_{(\ell,d)}$ is the price set by the platform, 
$\bff$ is the aggregate trip vector produced by the strategy profile $\Sigma$ (i.e. $\bff$ is the first component of the tuple $(\bff,\bfg,\bfx) = \Sigma_t(\omega_t,\bfS_t)$),
the expectation is taken over time $t+1$ scenarios $\omega_{t+1}$ given the time $t$ scenario $\omega_t$,
and $\bar{\bfS}_{\omega_{t+1}}(\bff)$ is a deterministic function specifying the time $t+1$ supply-location vector in the event that aggregate driver trips
are specified by $\bff$ and $\omega_{t+1}$ is the time $t+1$ scenario. $\bar{\bfS}_{\omega_{t+1}}(\bff)$ produces a vector indexed by locations, where the component
corresponding to location $\ell$ is defined by
$$
\left(\bar{\bfS}_{\omega_{t+1}}(\bff)\right)_\ell = \bar{M}_{\omega_{t+1},\ell} + \sum_{o\in\calL}f_{(o,\ell)},
$$
where $\bar{M}_{\omega_{t+1},\ell}$ is the volume of drivers who enter the market at location $\ell$ and time $t+1$ if the scenario is $\omega_{t+1}$.

Next, we define the value function.  For each location $\ell$, define the value function as
\begin{equation}
    \bar{\calV}_t(\ell,\omega_t,\bfS_t) = \frac{1}{S_\ell}\sum_{d\in\calL} \left[(f_{(\ell,d)} - g_{(\ell,d)}) \bar{\calQ}_t(\ell,d,0)  + 
                                                        g_{(\ell,d)}\bar{\calQ}_t\left(\ell,d,1, \frac{x_{(\ell,d)}}{2}\right)\right] .
\end{equation}
In the above, we write
$$
\bar{\calQ}_t(\ell,d,0) = \bar{\calQ}_t((\ell,d,0), X, \omega_t,\bfS_t)
$$
to mean the expected utility-to-go of the $f_{(\ell,d)} - g_{(\ell,d)}$ volume of drivers who take a relocation trip from $\ell$ to $d$,
and we write
$$
\bar{\calQ}_t\left(\ell,d,1, \frac{x_{(\ell,d)}}{2}\right) = \bar{\calQ}_t\left((\ell,d,0), \frac{x_{(\ell,d)}}{2}, \omega_t,\bfS_t\right)
$$
to mean the expected utility-to-go of the $g_{(\ell,d)}$ volume of drivers who serve a dispatch from $\ell$ to $d$.  Note that $\frac{x_{(\ell,d)}}{2}$ is the
average pickup disutility incurred by drivers who serve a dispatch from $\ell$ to $d$.
By writing the Q-value in this way, we are exploiting the equality
$$
\bar{\calQ}_t\left(\ell,d,1, \frac{x_{(\ell,d)}}{2}\right) = \frac{1}{x_{(\ell,d)}} \int_0^{x_{(\ell,d)}} \bar{\calQ}_t\left(\ell,d,1, x\right) dx.
$$

In order for a strategy profile $\Sigma$ to be an equilibrium, it has to satisfy two properties:
\begin{enumerate}
    \item The trip specifications it produces $(\bff,\bfg,\bfx)=\Sigma_t(\omega_t,\bfS_t)$ always have to be feasible with respect to the state $(\omega_t,\bfS_t)$.
    \item For any market state $(\omega_t,\bfS_t)$, no driver can have a profitable deviation from the trip specification $(\bff,\bfg,\bfx)=\Sigma_t(\omega_t,\bfS_t)$.
\end{enumerate}

We have already discussed what it means for $(\bff,\bfg,\bfx)$ to be feasible with respect to $(\omega_t,\bfS_t)$ earlier in this section.
The property that no driver can have a profitable deviation can be broken down further into the following subproperties:
\begin{enumerate}
    \item Every driver who takes a relocation trip cannot have the ability to take a relocation trip towards a different destination which yields higher utility:
        \begin{equation}
            f_{(\ell,d)} - g_{(\ell,d)} > 0 \implies \bar{\calQ}_t(\ell,d,0) = \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0).
        \end{equation}
    \item Every driver who accepts a dispatch cannot have the ability to take a relocation trip which yields higher utility:
        \begin{equation}
            g_{(\ell,d)} > 0 \implies \forall X\in [0,x_{(\ell,d)}],\ \  \bar{\calQ}_t(\ell,d,1,X) \geq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0) .
        \end{equation}
    \item Every driver who declines a dispatch cannot have been able to achieve higher utility by accepting the dispatch:
        \begin{equation}
            \bar{r}_{(\ell,d)} > 0, \ x_{(\ell,d)} < C \implies \forall X \in (x_{(\ell,d)}, C],\ \ \bar{\calQ}_t(\ell,d,1,X) \leq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0) .
        \end{equation}
        In the above equation, $\bar{r}_{(\ell,d)}$ refers to the dispatch request volume for trips from $\ell$ to $d$ that are generated by the prices
        set by the platform.
\end{enumerate}

We summarize these properties with the following equations:
\begin{align}
    \label{eq:exact_ic_start}
    f_{(\ell,d)} - g_{(\ell,d)} > 0& \implies \bar{\calQ}_t(\ell,d,0) = \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0)\\
            g_{(\ell,d)} > 0& \implies \forall X\in [0,x_{(\ell,d)}],\ \  \bar{\calQ}_t(\ell,d,1,X) \geq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0) \\
            \bar{r}_{(\ell,d)} > 0, \ x_{(\ell,d)} < C &\implies \forall X \in (x_{(\ell,d)}, C],\ \ \bar{\calQ}_t(\ell,d,1,X) \leq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0) .
    \label{eq:exact_ic_end}
\end{align}

Similarly, we say there is approximately no incentive to deviate, with respect to an approximation error $\epsilon$, if approximate versions of the above
conditions hold:
\begin{align}
    \label{eq:approx_ic_start}
    f_{(\ell,d)} - g_{(\ell,d)} > 0 &\implies \left|\bar{\calQ}_t(\ell,d,0) - \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0)\right|\leq \epsilon\\
    g_{(\ell,d)} > 0 &\implies \forall X\in [0,x_{(\ell,d)}],\ \  \bar{\calQ}_t(\ell,d,1,X) \geq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0)-\epsilon \\
    \bar{r}_{(\ell,d)} > 0, \ x_{(\ell,d)} < C &\implies \forall X \in (x_{(\ell,d)}, C],\ \ \bar{\calQ}_t(\ell,d,1,X) \leq \max_{d'\in\calL}\bar{\calQ}_t(\ell,d',0) +\epsilon.
    \label{eq:approx_ic_end}
\end{align}

\begin{definition}
    We say a fluid strategy profile $\Sigma=(\Sigma_1,\dots,\Sigma_T)$ is an exact equilibrium if it always produces trip specifications which are feasible
    with respect to the observed state, and if it satisfies the incentive compatibility conditions (\ref{eq:exact_ic_start} - \ref{eq:exact_ic_end}).

We say a fluid strategy profile $\Sigma$ is an $\epsilon$-approximate equilibrium if it 
    produces trip specifications which are approximately feasible
    with respect to the observed state, and if it satisfies the approximate incentive compatibility conditions (\ref{eq:approx_ic_start} - \ref{eq:approx_ic_end}).
\end{definition}
\Xomit{
.

.

.

.

$(\bff,\bfg,\bfx)$ to represent an equilibrium in the fluid model, we associate a Q-value with each
trip type, which corresponds to the expected utility-to-go of taking that trip.
We start by defining the utility-to-go for relocation trips $(\ell,d,0)$.  Let $\Phi_{\omega_{t}}(\bfS_t)$ denote the optimal value of
the state-dependent optimization problem \mccomment{ref}.
The Q-value for a relocation trip $(\ell,d,0)$ is defined by
\begin{equation}
    \calQ(\ell,d,0) = -c_{(\ell,d)} + \bbE\left[\frac{\partial}{\partial S_d}\Phi_{\omega_{t+1}}(\bar{\bfS}_{\omega_{t+1}}(\bff))\right],
\end{equation}
where the above expectation is taken over time $t+1$ scenarios $\omega_{t+1}$.
We will formally define $\Phi_{\omega_{t}}(\bfS_t)$ in Section \ref{sec:opt_central}, and we will show via backwards induction that 
the partial derivative $\frac{\partial}{\partial S_d}\Phi_{\omega_{t+1}}(\bar{\bfS}_{\omega_{t+1}}(\bff))$ corresponds to the expected utility-to-go
collected by a driver positioned at $d$ from state with scenario $\omega_{t+1}$ and supply-location vector $\bar{\bfS}_{\omega_{t+1}}(\bff))$.


For dispatch trips $(\ell,d,1)$, the associated Q-value depends on the price $P_{(\ell,d)}$ set by the platform for that route,
and we additionaly parameterize the Q-value by an add-passenger disutility value $X$. The Q-value for a dispatch
trip $(\ell,d,1)$ and disutility value $X\in [0,C]$ is defined as:
\begin{equation}
    \calQ(\ell,d,1,X) = P_{(\ell,d)} - X + \calQ(\ell,d,0),
\end{equation}

We conclude this section by defining two equilibrium concepts for the fluid model.  Definition \ref{def:exact_fluid_eqlbm}
states what it means for $(\bff,\bfg,\bfx)$ to be an exact equilibrium for the fluid model, as well as what it means
to be an approximate equilibrium for the fluid model.

\begin{definition}
    \label{def:exact_fluid_eqlbm}
    A 3-tuple $(\bff,\bfg,\bfx)$ is an $\epsilon$-approximate equilibrium for the fluid model if it is approximately feasible, and if no driver has incentive to deviate. 

    Approximately feasible means that conditions \ref{item:first_feasibility} through
    \ref{item:trip_volume_feasibility} above hold, and conditions \ref{item:penultimate} and \ref{item:last_feasibility} hold approximately.
    The approximate version of condition \ref{item:penultimate} states that
    \begin{equation}
    S_\ell+\epsilon \geq \sum_{d\in\calL} \frac{Cg_{(\ell,d)}}{x_{(\ell,d)}}.
    \end{equation}
    The approximate version of condition \ref{item:last_feasibility} states that, on routes where $g_{(\ell,d)} < \bar{r}_{(\ell,d)}$, the following holds
    \begin{equation}
        S_\ell = \sum_{d\in\calL}\frac{Cg_{(\ell,d)}}{x_{(\ell,d)}} + \epsilon'
    \end{equation}
    where $\epsilon'\in\bbR$ is an error term satisfying $|\epsilon'|\leq \epsilon$.

    A drivers incentive to deviate depends on the destination towards which they are dispatched.  Exactly one of the following cases applies to each 
    route $(\ell,d)$ with nonzero dispatch demand, i.e. with $\bar{r}_{(\ell,d)} > 0$:
    \begin{itemize}
        \item Some drivers accept the dispatch and some drivers reject the dispatch, i.e. $0<x_{(\ell,d)} < C$.
            In order for both the drivers who accept and drivers who reject to have no incentive to deviate, the following equality must hold:
            \begin{equation}
            \calQ(\ell,d,1,x_{(\ell,d)}) = \max_{d'}\calQ(\ell,d',0) + \epsilon',
            \end{equation}
            where $\epsilon'$ is an error term satisfying $|\epsilon'|\leq \epsilon$.
        \item All drivers accept the dispatch, i.e. $x_{(\ell,d)} = C$.  In this case, the inequality must hold:
            \begin{equation}
            \calQ(\ell,d,1,C) \geq \max_{d'}\calQ(\ell,d',0) - \epsilon.
            \end{equation}
        \item All drivers reject the dispatch, i.e. $x_{(\ell,d)} = 0$.
        \mccomment{Need to say something for the case where $x_{(\ell,d)} = 0$.}
        Then we have:
            \begin{equation}
            \calQ(\ell,d,1,0) \leq \max_{d'}\calQ(\ell,d',0) + \epsilon.
            \end{equation}
    \end{itemize}
    In addition, there must be $0$ driver mass on any relocation trip $(\ell,d,0)$ which does
    not maximize $\calQ(\ell,d',0)$ over all $d'$:
    \begin{equation}
    f_{(\ell,d)} - g_{(\ell,d)} > 0 \implies \calQ(\ell,d,0) \geq \max_{d'}\calQ(\ell,d',0) - \epsilon.
    \end{equation}
    We say $(\bff,\bfg,\bfx)$ is an exact equilibrium if is it a $0$-approximate equilibrium.
\end{definition}
}


\Xomit{
\begin{definition}
    \label{def:fluid_eqlbm}
    A feasible fluid strategy $(\bff,\bfg,\bfx)$ is a fluid equilibrium if there exists no deviation which increases a driver's expected utility.
    The set of utility to go values that drivers at $\ell$ can achieve under $(\bff,\bfg,\bfx)$ is given by:
    \begin{align*}
        \calU(\ell) =& \left\{\calQ(\ell,d,0) : d\in\calL, f_{(\ell,d)} - g_{(\ell,d)} > 0\right\} \\
        & \ \ \cup \left\{\calQ(\ell,d,1,X) : d\in\calL, g_{(\ell,d)} > 0, 0\leq X \leq x_{(\ell,d)}\right\}.
    \end{align*}
    The set of utility to go values that drivers at $\ell$ can achieve by deviating from $(\bff,\bfg,\bfx)$ is given by:
    \begin{align*}
        \calD(\ell) =& \left\{\calQ(\ell,d,0) : d\in\calL\right\} \\
        & \ \ \cup \left\{\calQ(\ell,d,1,X) : d\in\calL, \bar{r}_{(\ell,d)} - g_{(\ell,d)} > 0\right\}.
    \end{align*}
    We say $(\bff,\bfg,\bfx)$ is an \emph{exact fluid equilibrium} if the inequality $$\min \calU(\ell) \geq \max \calD(\ell)$$ holds
    for every location $\ell$.
    We say $(\bff,\bfg,\bfx)$ is an \emph{$\epsilon$-approximate fluid equilibrium} if the inequality
$$\min \calU(\ell) \geq \max \calD(\ell)-\epsilon$$
    holds for every location $\ell$.
\end{definition}
}

\Xomit{
\subsubsection*{Original Content}
In this subsection we describe our assumptions for the stochastic fluid model about how 
the platform matches dispatch requests to available
drivers, and what it means for a driver strategy profile to be an equilibrium.

As a preliminary, let's describe the state of the market at the time when the platform
matches dispatches to drivers and when drivers strategically decide which trip to take.
Matching decisions and strategic driver behaviour occurs in each time period $t$.  The state of the market
at the beginning of the time period is described by the stochastic scenario $\omega_t$ and a vector
of supply locations $\bfS$. Each component $S_\ell$ of $\bfS$ specifies the volume of drivers positioned at the location
$\ell$. 
The SSP mechanism computes an optimal solution $(\bfg^*,\bff^*)$ to the state-dependent optimiatization problem 
(\ref{eq:dynamic_optimization_recursive}) and sets the price $P_{\ell,d}$ on each route $(\ell,d,\omega_t)$ so that
the dispatch demand volume occurring on each route is exactly equal to the dispatch trip volume on that route
prescribed by the computed optimal solution.
That is, under the SSP price $P_{\ell,d}$ described in equation (\mccomment{Ref}), the optimal decision variable $g^*_{(\ell,d)}$
describes both the allocated volume of supply for dispatch trips on the route $(\ell,d,\omega_t)$ as well as the volume of rider-side
demand for a dispatch trip on that route.

After the platform sets the trip prices on each route we assume a back-and-forth process occurs between the platform and
the drivers, in which dispatch trips are allocated to drivers, and in which drivers make strategic decisions about whether
or not to accept dispatch trips or drive elsewhere.
We assume the platform randomly selects drivers to whom dispatches are allocated.  When drivers reject their dispatches, we
assume the platform again randomly selects drivers to whom the remaining dispatches are allocated.  We assume that a driver is allocated
at most one dispatch trip, so if they reject a dispatch trip in a particular time period they will necessarily take a relocation-trip
within that time period.

The matching process terminates when either all dispatch demand has been allocated, or all drivers have been allocated one dispatch.
For each origin-destination pair $(\ell,d)$ we use the notation $Z_{(\ell,d)}$ to denote the total volume of drivers who were allocated
a dispatch trip along $(\ell,d)$, and we use $g_{(\ell,d)}$ to denote the total volume of drivers who accepted the dispatch trip.
We use $Y_\ell$ to denote the total volume of drivers positioned at $\ell$ who are not allocated a dispatch trip. $Y_\ell$ is equal to the 
difference between $S_\ell$ and the sum of $Z_{(\ell,d)}$ over all locations $d$:
$$
Y_\ell = S_\ell - \sum_{d}Z_{(\ell,d)}.
$$
At least one of the following two conditions is met when the matching process terminates:  either all drivers have had a chance to
accept a dispatch trip, i.e. $Y = 0$, or all dispatch demand has been satisfied, i.e. $g_{(\ell,d)}=g^*_{(\ell,d)}$ for all locations $d$.
Note that the matching process partitions drivers into one of $|\calL|+1$ types: drivers are partitioned based on the destination $d$ to which
they were allocated a dispatch trip, for each $d\in\calL$, and the remaining drivers reside in a ``no-dispatch'' partition.
The assignment of drivers to each of these partitions depends only on the matching process used by the platform, which we previously
stated allocates dispatches to drivers uniformly at random (in particular, no strategic driver behaviour is behind the assignment of drivers
to these partitions).  Thus, the add-passenger disutility distribution remains $\mathrm{Uniform}(0,C)$ across drivers in each of these partitions.

It remains to describe what an equilibrium strategy profile is among the drivers.  As already mentioned, we use the notation $g_{(\ell,d)}$ to
indicate the volume of drivers who accept a dispatch along the route $(\ell,d)$.  Necessarily, $g_{(\ell,d)}\leq Z_{(\ell,d)}$, because drivers
can only accept a dispatch along $(\ell,d)$ if the platform facilitates the match.  We stick with the notational convention of our optimization
formulation to describe the relocation-trips taken by drivers who don't serve a dispatch: we use $f_{(\ell,d)}$ to denote the total volume of drivers
who traverse the route $(\ell,d)$, so that $f_{(\ell,d)}-g_{(\ell,d)}$ indicates the volume of drivers who drive from $\ell$ to $d$ without a passenger.
The vectors $(\bff,\bfg)$, where $\bff=(f_{(\ell,d)} : (\ell,d)\in\calL^2)$ and $\bfg=(g_{(\ell,d)} : (\ell,d)\in\calL^2)$ are then almost sufficient to
fully describe a driver strategy profile; it remains to describe the add-passenger disutility incurred by the $g_{(\ell,d)}$ drivers who serve a dispatch
on each route $(\ell,d)$. 

Let's avoid the issue of add-passenger disutility of an arbitrary equilibrium for a brief moment, and turn to the driver utility conditions a strategy
profile must satisfy in order for it to be an equilibrium.
Recally we write $\calQ(\ell,d,0)$ for the utility-to-go a driver collects for driving empty from $\ell$ to $d$, and we write
$\calQ(\ell,d,1,x)$ for the utility-to-go a driver with add-passenger disutility $x$ collects for serving a dispatch from $\ell$ to $d$.
Note the relationship
$$
\calQ(\ell,d,1,x) = P_{(\ell,d)}-x + \calQ(\ell,d,0).
$$

Informally, an equilibrium strategy is a strategy such that no one (infinitesimal) driver can increase their utility by choosing a different action.
This implies the following properties:
\begin{enumerate}
\item No driver who takes a relocation-trip can increase their utility by taking a relocation trip to a different destination,
\item No driver who accepts a dispatch request can increase their utility by taking a relocation trip,
\item No driver who declines a dispatch request could have achieved higher utility by accepting the trip.
\end{enumerate}
Property 1 implies that every driver at a location $\ell$ who drives empty (i.e. takes a relocation-trip) achieves the same utility.
Define
$$
\calQ(\ell,0) = \max_d \calQ(\ell,d,0)
$$
to be the utility collected by drivers at $\ell$ for a relocation-trip under an equilibrium strategy.
Property 2 implies that every driver who accepts a dispatch trip towards some location $d$ has an add-passenger disutility value $x$
which cannot be less than this relocation-trip utility:
$$
\calQ(\ell,d,1,x) \geq \calQ(\ell,0).
$$
Property 3 implies that every driver who declines a dispatch trip towards location $d$ has an add-passenger disutility value $x'$
which cannot be more than the relocation-trip utility:
$$
\calQ(\ell,d,1,x') \leq \calQ(\ell,0).
$$
Thus, in an equilibrium strategy, if a driver with add-passenger disutility $x$ is allocated a dispatch towards location $d$,
they accept the dispatch if and only if $\calQ(\ell,d,1,x)$ is at least the relocation-utility $\calQ(\ell,0)$.
In particular, there is a threshold value $x_{(\ell,d)}$,
$$
x_{(\ell,d)} = P_{(\ell,d)} + \calQ(\ell,d,0) - \calQ(\ell,0),
$$
such that a driver with disutility $x$ will accept a dispatch if and only if $x\leq x_{(\ell,d)}$.

Recall our matching process allocates dispatches destined towards $d$ to a collection of drivers of volume $Z_{(\ell,d)}$,
and the add-passenger disutilities amongst this collection of drivers has distribution $\mathrm{Uniform}(0,C)$.  In an equilibrium strategy,
it follows that drivers within this pool only accept the dispatch towards $d$ if their add-passenger disutility $x$ does not exceed the threshold
$x_{(\ell,d)}$.  In particular, for the pool of $g_{(\ell,d)}$ drivers who do accept the dispatch  towards $d$, their add-passenger disutilities have
a $\mathrm{Uniform}(0,x_{(\ell,d)})$ distribution.
Furthermore, the quantities $g_{(\ell,d)}$, $Z_{(\ell,d)}$, and $x_{(\ell,d)}$ are related to each other through the following equality:
$$
g_{(\ell,d)} = \bbP(X\leq x_{(\ell,d)}) Z_{(\ell,d)} = \frac{x_{(\ell,d)}}{C} Z_{(\ell,d)}
$$
where $X\sim\mathrm{Uniform}(0,C)$.
Rearranging, we have
$$
C\frac{g_{(\ell,d)}}{x_{(\ell,d)}} = Z_{(\ell,d)}.
$$
This implies the following upper bound on the thresholds $x_{(\ell,d)}$ and dispatch trip counts $g_{(\ell,d)}$:
$$
\sum_{d\in\calL}\frac{g_{(\ell,d)}}{x_{(\ell,d)}} \leq \frac{1}{C}\sum_dZ_{(\ell,d)}\leq\frac{S_\ell}{C}.
$$
Therefore, we have the following characterization of an equilibrium driver strategy profile:
\begin{lemma}
\label{lem:fluid_eqlbm_strategy}
An equilibrium strategy profile can be described by a vector of dispatch trip volumes $\bfg=(g_{(\ell,d)}:(\ell,d)\in\calL^2)$,
a vector of total trip volumes $\bff=(f_{(\ell,d)}:(\ell,d)\in\calL^2)$, and a vector of thresholds $\bfx = (x_{(\ell,d)} : (\ell,d)\in\calL^2)$.
In order for this characterization to describe a feasible strategy profile, the following inequality must be satisfied for all locations $\ell$:
$$
\sum_{d\in\calL}\frac{g_{(\ell,d)}}{x_{(\ell,d)}} \leq \frac{S_\ell}{C}.
$$
The total add-passenger disutility incurred by this strategy-profile is given by
$$
\sum_{(\ell,d)} g_{(\ell,d)}\bbE[X\mid X\leq x_{(\ell,d)}],
$$
where $X\sim\mathrm{Uniform}(0,C)$.
\end{lemma}
}


==> matching_process_description.tex <==
We now describe the matching process that the platform uses to allocate dispatch requests to drivers.
The matching process refers to our mathematical model for how dispatch requests are allocated to drivers.
Since our ridesharing model assumes that dispatch requests can only be served by drivers already positioned at
the origin location, our matching model operates independently for each location $\ell$.

At each location $\ell$, the matching process depends on the number of drivers at the location, the number of
riders requesting a dispatch towards each destination, and the dispatch-acceptance probabilities used by the drivers.
Let $M$ be the total number of drivers, let $R_d$ be the total number of riders requesting a dispatch towards each location
$d$, and let $p_{i,d}$ be the probability that each driver $i$ will accept a dispatch towards a destination $d$.
Our formal description of how the matching process operates is provided below.

\begin{enumerate}
\item Let $L=|\calL|$ be the number of locations.  Pick any ordering $d_1,d_2,\dots,d_L$. Initialize $j\coloneqq 1$.
\item Let $\calM_\ell = \{1,2,\dots,M\}$ be the set of labels for the drivers positioned at $\ell$.
\item While $j\leq L$ and $\calM_\ell$ is non-empty:
\begin{enumerate}
\item Set the destination location $d=d_j$. 
\item Allocate dispatches towards $d$ until all dispatches towards d have been accepted or until no drivers remain.  
\item While $R_d >0$ and while $\calM_\ell$ is non-empty:
\begin{enumerate}
\item Uniformly sample a driver index $i\sim \calM_\ell$ and remove $i$ from the set of undispatched drivers $\calM_\ell$.
\item Send driver $i$ a dispatch towards location $d$ and observe their accept/reject decision (accept happens with 
probability $p_{i,d}$).  If the dispatch is accepted, decrement $R_d$ by one.
\end{enumerate}
\item Increment the location index $j$ by one.
\end{enumerate}
\end{enumerate}

The important part of our matching process model is that drivers can be allocated at most one dispatch and that the
platform does not preferentially dispatch to certain drivers in an attempt to align incentives.  The details of the 
matching process we described above were chosen for simplicity of analysis, but we believe our results extend to a 
wide range of matching process models.

An important setting for us is where all drivers at the same location use (approximately) the same acceptance probability
for each destination.  This setting arises when drivers at the same location use the same disutility thresholds, which 
is a property we will see holds in equilibrium strategies.
In particular, when analyzing equilibrium strategies we will need to make use of concenetration inequalities for the
outcome of the matching process, which show good error bounds as the population size parameter $k$ grows large.


Consider what happens under the above matching process when all acceptance probabilities $p_{i,d}$ are equal to the
same value $p_d$, for each destination $d$.
Let $M^{(j)}$ be the number of drivers who are allocated a dispatch towards each location $d_j$ and let $Y^{(j)}$ be
the number of drivers who accept a dispatch towards location $d_j$.
We have that the distribution of $M^{(j)}$, conditioned on the values of $M^{(j')}$ for earlier trials $j'\leq j-1$,
 is the minimum of the number of remaining available drivers
and a negative Binomial distribution, which counts the number of trials needed to see $R_{d_j}$ successes 
where each trial has independent probability of success $p_{d_j}$.
Specifically, let $M^{(j')}$ be the number of drivers who were allocated a dispatched in previous iterations $j'\leq j-1$,
and let $Z_j$ be a negative Binomial random variable with parameters $R_{d_j}$ and $p_{d_j}$.
Formally, we have
\begin{equation}
\label{eq:dispatch_size_dist}
M^{(j)}\mid M^{(1)},M^{(2)},\dots,M^{(j-1)} \,{\buildrel d \over =}\, \min\left\{Z_j, M - \sum_{j'=1}^{j-1}M^{(j')}\right\}
\end{equation}
For the number of dispatches that get served, the distribution is quite simple if we know that the above
maximum is not attained. Indeed, we have that all $R_{d_j}$ rides must be served in this case.
\begin{equation}
\bbP\left(Y^{(j)}=R_{d_j}\mid Z_j \leq  M - \sum_{j'=1}^j M_j\right)=1.
\end{equation} of $Y^{(j)}$ is d number of rides that are accepted
If the maximum is attained then we know that we performed $M^{(j)}$ trials and saw fewer than $R_{d_j}$ successes.
The total number of successes is thus given by a conditional Binomial distribution:
\begin{equation}
\left(Y^{(j)}\mid Z_j >   M - \sum_{j'=1}^j M_j\right) \,{\buildrel d \over =}\, \left(B_j\mid B_j < R_{d_j}\right),
\end{equation}
where $B_j$ has a Binomial distribution with parameters $M - \sum_{j'=1}^j M_j$ and $p_{d_j}$.

Deducing the exact expected value of the variables $M^{(j)}$ and $Y^{(j)}$ is complicated, because of the nonlinear
minimum appearing in equation (\ref{eq:dispatch_size_dist}).
However, we will see that as the population-size parameter grows, the expected number of dispatches and dispatch acceptances
converge towards the following simple form.
For each $j=1,2,\dots,L$, define
\begin{equation}
\bar{M}^{(j)} = \min\left\{M - \sum_{j'=1}^{j-1}\bar{M}^{(j')}, \frac{R_{d_j}}{p_{d_j}}\right\},
\end{equation}
and also define
\begin{equation}
\bar{Y}^{(j)} = \bar{M}^{(j)} p_{d_j}.
\end{equation}
We remark that $\bar{M}^{(j)}$ and $\bar{Y}^{(j)}$ are \emph{biased} estimates for the means of $M^{(j)}$ and $Y^{(j)}$,
but we will show that this bias is negligible as $k$ grows large.

\begin{lemma}
\label{lem:matching_concentration}
Suppose that all drivers positioned at $\ell$ use the same acceptance probability $p_d$ for each destination $d$.
Let $k,C\geq 0$ be any constants such that the number of drivers at $\ell$ and the number of riders requesting a dispatch towards
any destination $d$ are all upper bounded by $kC$.  Then there exists an error term $\epsilon(k,C)$ and a probability term $q(k,C)$
such that 
\begin{equation}
    \bbP\left(\frac{1}{k}\sum_{j=1}^L|Y^{(j)} - \bar{Y}^{(j)}|\geq \epsilon(k)\right) \leq q(k).
\end{equation}
    Moreover, the error term $\epsilon(k)$ and the probability term $q(k)$ both go to $0$ as $k$ goes to $\infty$, assuming $C$ is held fixed.
\end{lemma}
The proof of Lemma \ref{lem:matching_concentration} is deferred to Appendix 
\ref{appdx:matching_concentration_proof}.

\subsection{Matching Process in the Fluid Model}
\label{subsec:fluid_matching_process}
We assume strategy profiles in the two-level model are specified by a sequence of functions $\Sigma = (\Sigma_1,\dots,\Sigma_T)$.
For each time period $t$, the function $\Sigma_t$ takes as input the market state $(\omega_t,\bfS_t)$ and produces two vectors: $(\bfx,\bfh) = \Sigma_t(\omega_t,\bfS_t)$.
The vector $\bfx$ has components $x_{(\ell,d)}$ for each pair of locations $(\ell,d)$, and this corresponds to the threshold that drivers at $\ell$ use when
they are allocated a dispatch towards $d$. The vector $\bfh$ also has components $h_{(\ell,d)}$ for each pair of locations $(\ell,d)$, and this corresponds
to the probability that a driver who doesn't serve a dispatch takes a relocation trip from $\ell$ to $d$.

The matching process in the fluid model takes as input the thresholds $\bfx$, the relocation distributions $\bfh$, and produces a trip specification $(\bff,\bfg)$.
The matching process operates separately for each location $\ell$.
The dispatch volumes $\bar{g}_{(\ell,d)}$ are obtained by taking the following steps.
\begin{itemize}
    \item Fix any origin location $\ell$. For $d=1,2,\dots,L$:
        \begin{enumerate}
            \item Let $p_{(\ell,d)} = \frac{x_{(\ell,d)}}{C}$ be the probability of acceptance.
            \item Let $\bar{R}_{(\ell,d)}$ be the volume of riders who request a dispatch from $\ell$ to $d$.
            \item Let $$\bar{M}_{(\ell,d)} = \min\left(\frac{\bar{R}_{(\ell,d)}}{p_{(\ell,d)}}, S_\ell - \sum_{d'=1}^{d-1} \bar{M}_{(\ell,d')}\right)$$
                be the volume of drivers who are allocated a dispatch from $\ell$ towards $d$.
            \item Let \begin{equation} 
                    \label{eq:fluid_dispatch_volume}
                    \bar{g}_{(\ell,d)} = \bar{M}_{(\ell,d)} p_{(\ell,d)}
            \end{equation}
            be the volume of dispatches from $\ell$ to $d$ served in the fluid model.
        \end{enumerate}
    \end{itemize}
After the dispatch counts $\bar{g}_{(\ell,d)}$ have been determined for every destination $d$, the pool of drivers who need to take
        a relocation trip is given by 
        $$ N_\ell = S_\ell - \sum_{d=1}^L \bar{g}_{(\ell,d)}.$$
        The volume of drivers who take a relocation trip from $\ell$ to $d$ is given by $N_\ell h_{(\ell,d)}$.
        Let \begin{equation}
            \label{eq:fluid_total_trip_volume}
        \bar{f}_{(\ell,d)} = \bar{g}_{(\ell,d)} + N_\ell h_{(\ell,d)}
        \end{equation}
        be the volume of trips (dispatch and relocation) from $\ell$ to $d$ served in the fluid model.



==> minor_incentive_welfare_loss.tex <==
In this section our goal is to show that the minor incentive discrepancies which occur
due to rounding and randomness in the stochastic two-level model under the dynamic SSP mechanism
result in only minor loss to total welfare.

\subsection{Driver Strategy Profiles}
The overarching problem we wish to address in this section is that small discrepancies to driver
incentives might incentivize them to take trips that are not explicitly what the SSP mechanism
allocates to them.  However, all of our notation and analysis up to this point has been under
the assumption that drivers always follow their allocated trip-suggestion.  
Let's start this section by introducing a general notion of the strategy-profile 
used by drivers.

\begin{definition}
Fix a time $t$ and scenario $\omega_t$.
An \emph{active trip type} with respect $t$ and $\omega_t$ is any tuple
$(r,\omega_t,\delta)$ where $(r,\omega_t)\in\calA_{\omega_t}^t$ is
any active ODT-scenario and $\delta\in\{0,1\}$ is an indicator specifying
whether the trip fulfils a rider dispatch ($\delta=1$) or not ($\delta=0$).
\end{definition}

\begin{definition}
Consider the stochastic two-level model at a time $t$, scenario $\omega_t$,
with population-size parameter $k$, supply-location vector $\bfS_t$, and 
dispatch-request vector $\bfd_t$.  A \emph{feasible trip-allocation vector} 
is any vector $\bfh$ with components indexed by the active trip types, 
$$
\bfh = (h_{(r,\omega_t,\delta)} : (r,\omega_t)\in\calA_{\omega_t}^t, \delta\in\{0,1\}),
$$
which satisfies the following properties:
\begin{enumerate}
    \item (Discrete Driver Feasibility): each component $h_{(r,\omega_t,\delta)}$ is a nonnegative integer multiple of $1/k$.
    \item (Dispatch Demand Feasibility): each passenger-trip component of $\bfh$ does 
    not exceed the realized amount of dispatch demand for the corresponding route, i.e., 
    $h_{(r,\omega_t,1)} \leq d_{(r,\omega_t)}$ holds for all active routes $(r,\omega_t)$.
    \item (Supply Feasibility): the number of trip-allocations allocated by $\bfh$ to outgoing trips from each active location $(l,\omega_t)$ is exactly equal to the amount of available supply at that location.  i.e. 
    $$
    S_{(l,\omega_t)} = \sum_{(r,\omega_t)\in A^+_{\omega_t}(l)} \sum_{\delta\in\{0,1\}}
    h_{(r,\omega_t,\delta)}
    $$
    holds for all active locations $(l,\omega_t)\in\calN_{\omega_t}^t$.
\end{enumerate}
\end{definition}

\begin{definition}
Consider the stochastic two-level model at a time $t$, scenario $\omega_t$,
with population-size parameter $k$, supply-location vector $\bfS_t$, and 
dispatch-request vector $\bfd_t$.
Let $\bfh$ be a feasible trip-allocation vector with respect to these parameters.
Fix any active location $(l,\omega_t)\in\calN_{\omega_t}^t$.
The \emph{trip-allocation distribution} induced by $\bfh$ at $(l,\omega_t)$
is a discrete probability distribution $\bfh(l,\omega_t)$ supported on
active trip types which originate from $(l,\omega_t)$, defined as follows:
$$
\bfh(l,\omega_t) \equiv \left(\frac{h_{(r,\omega_t,\delta)}}{S_{(l,\omega_t)}} :
                    (r,\omega_t)\in A^+_{\omega_t}(l), \delta\in\{0,1\}\right).
$$
\end{definition}

\begin{definition}
A \emph{driver strategy-profile} is a function $H(\cdot)$ which takes as input
\begin{itemize}
    \item the time $t$,
    \item the scenario $\omega_t$,
    \item the population-size parameter $k$,
    \item the supply-location vector $\bfS_t$,
    \item the dispatch-request demand vector $\bfd_t$,
\end{itemize}
and produces a trip-suggestion vector $\bfh=H(t,\omega_t,k,\bfS_t,\bfd_t)$ that
is feasible with respect to these parameters.
\end{definition}

\begin{definition}
\mccomment{This is my original 'non-degeneracy' assumption to rule out drivers preferring an empty trip which yields the same utility as a passenger trip} A driver strategy-profile $H$ is \emph{non-degenerate} if it only allocates
non-dispatch trips along routes for which it is infeasible to allocate additional
dispatch trips.  That is, for any trip-suggestion vector
$\bfh=H(t,\omega_t,k,\bfS_t,\bfd_t)$, $H$ is non-degenerate if 
$h_{(r,\omega_t,0)} > 0$ implies $h_{(r,\omega_t,1)} = d_{(r,\omega_t)}$.
\end{definition}

\begin{assumption}
\label{assn:no_empty_trips}
When a driver has two or more actions with equal utility-to-go values,
they always have a preference for the action which fulfils a dispatch,
if one exists. \mccomment{drivers can still be indifferent between two relocation trips, so some strong-convexity property will likely still need to be used to address that issue}
\end{assumption}

\begin{definition}
\mccomment{Not sure if we need a definition of expected welfare under
an arbitrary strategy-profile $H$}
The expected welfare under a driver
strategy-profile $H$ is defined as
\begin{equation}
    \calW(H, P) = \bbE\left[\sum_{\substack{(r,\omega_s)\in\calA}} \bbP(\omega_s) U_{(r,\omega_s)}(h_{(r,\omega_s)})\right],
\end{equation}
where the outer expectation is taken over the random trip-counts 
$h_{(r,\omega_s)} = h_{(r,\omega_s,0)} + h_{(r,\omega_s,1)}$.
\end{definition}

\begin{definition}
A \emph{platform pricing protocol} is a function $P(\cdot)$ which takes as input
\begin{itemize}
    \item the time $t$,
    \item the scenario $\omega_t$,
    \item the supply-location vector $\bfS_t$,
    \item the price-inquiry demand vector $\bfD_t$,
\end{itemize}
and produces a price vector $\bfrho=P(t,\omega_t,\bfS_t,\bfD_t)$, where
$\bfrho$ specifies nonnegative trip prices for all active routes:
$$
\bfrho = (\rho_{(r,\omega_t)} : (r,\omega_t) \in\calA_{\omega_t}^t).
$$
\end{definition}

\begin{definition}
Fix a pricing protocol $P$ and a strategy profile $H$.
Consider the stochastic two-level model at a time $t$, scenario $\omega_t$,
with population-size parameter $k$, and supply-location vector $\bfS_t$.
Fix an active location $(l,\omega_t)\in\calN_{\omega_t}^t$.
The \emph{expected utility-to-go} of a driver positioned at $(l,\omega_t)$
with respect to $P$ and $H$ is denoted by $\calV^k_{(l,\omega_t)}(\bfS_t;P,H)$
and defined by the following equation:
$$
\calV^k_{(l,\omega_t)}(\bfS_t;P,H) = \begin{cases}
\bbE^k\left[\delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right] & \mbox{if } t<T,\\
\bbE^k\left[\delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)}\right] & \mbox{if }t=T. 
\end{cases}
$$
The above expectation is taken over multiple sources of randomness:
\begin{itemize}
\item The random price-inquiry demand $\bfD_t = (D_{(r,\omega_t)} : (r,\omega_t)\in\calA_{\omega_t}^t)$ at each active route 
$(r,\omega_t)$.
\item The prices $\bfrho = P(t,\omega_t,\bfS_t,\bfD_t)$ may depend on the random price-inquiry demand.
\item The random dispatch-request demand $\bfd_t = (d_{(r,\omega_t)} : (r,\omega_t)\in\calA_{\omega_t}^t)$ depends on the amount of price-inquiry
demand $\bfD_t$ and the trip-prices $\bfrho$.
\item The trip-allocation vector $\bfh=H(t,\omega_t,k,\bfS_t,\bfd_t)$ depends
on the random dispatch-request demand.
\item The trip type $(r,\omega_t,\delta)$ appearing in the equation is randomly
sampled from the trip-allocation distribution $\bfh(l,\omega_t)$ induced by $\bfh$
at $(l,\omega_t)$.
\item The random time $t+1$ scenario $\omega_{t+1}\sim\bbP(\cdot\mid\omega_t)$.
\item The random time $t+1$ supply-location vector $\bfS_{t+1}$ depends on
    the trip-allocation vector $\bfh$, the scenario $\omega_{t+1}$,
    and the random new-driver counts $M_{(l,\omega_{t+1})}$ at each active time $t+1$ LT-scenario $(l,\omega_{t+1})\in\calN_{\omega_{t+1}}^{t+1}$.
\end{itemize}
\end{definition}

\begin{definition}
Fix a pricing protocol $P$ and a strategy profile $H$.
Consider the stochastic two-level model at a time $t$, scenario $\omega_t$,
with population-size parameter $k$, and supply-location vector $\bfS_t$.
Fix an active location $(l,\omega_t)\in\calN_{\omega_t}^t$.
The \emph{deviation utility-to-go} for a driver positioned at $(l,\omega_t)$
with respect to $P$ and $H$ is denoted by $\tilde{\calV}^k_{(l,\omega_t)}(\bfS_t;P,H)$
and defined by the following equation:
$$
\tilde{\calV}^k_{(l,\omega_t)}(\bfS_t;P,H) = \begin{cases}
/\bbE^k\left[\max_{(r,\omega_t,\delta)} \delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \tilde{\calV}^k_{(l^+(r),\omega_{t+1})}(\tilde{\bfS}_{t+1};P,H)\right] & \mbox{if } t<T,\\
\bbE^k\left[\max_{(r,\omega_t,\delta)} \delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)}\right] & \mbox{if }t=T. 
\end{cases}
$$
The sources of randomness in the above equation are almost all the same as in the previous
definition.  The main difference is that the trip type $(r,\omega_t,\delta)$ is determined
by taking a maximum, instead of being sampled from the trip-allocation distribution
$\bfh(l,\omega_t)$.  This deviation leads to a different supply-location vector at time $t+1$.
We emphasize this difference by using the notation $\tilde{\bfS}_{t+1}$ 
to indicate the supply-location vector that arises after the deviation.  
This definition assumes that only the one driver deviates and all other drivers drive
according to the strategy profile $H$.

For the purpose of deviation utility-to-go we assume that the driver can deviate to
any trip type $(r,\omega_t,\delta)$ originating from their location $(l,\omega_t)$, i.e.
we ignore possible constraints induced by limited demand availability for dispatch trips
and we ignore the logistics of connecting to a rider that was not allocated by 
the platform.  In this sense, the deviation utility-to-go provides an upper bound on the
utility achievable from deviating.
\end{definition}

\begin{definition}
Fix a pricing protocol $P$ and a strategy profile $H$.
Consider the stochastic two-level model at a time $t$, scenario $\omega_t$,
with population-size parameter $k$, supply-location vector $\bfS_t$, and dispatch-request
vector $\bfd_t$.
Let $\bfh=H(t,\omega_t,k,\bfS_t,\bfd_t)$ be the trip-allocation vector produced by
the strategy profile $H$ with respect to these parameters.

Consider a driver who is positioned at
an active location $(l,\omega_t)\in\calN_{\omega_t}^t$. Let $(r,\omega_t,\delta)$ be the
trip type the driver samples from the trip-allocation distribution $\bfh(l,\omega_t)$.
The \emph{incentive gap} with respect to $(r,\omega_t,\delta)$ is the incentive the
driver has to deviate, conditioned on the trip-allocation $(r,\omega_t,\delta)$.
The incentive gap with respect to $(r,\omega_t,\delta)$ is equal to the following expression:
$$
\max_{(\tilde{r},\omega_t,\tilde{\delta})} (\tilde{\delta}\rho_{(\tilde{r},\omega_t)} -
c_{(\tilde{r},\omega_t)}) - (\delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)}) +
\bbE^k\left[\tilde{\calV}^k_{(l^+(r),\omega_{t+1})}(\tilde{\bfS}_{t+1};P,H)
- \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right].
$$
%\mccomment{Maybe in the future will use notation $IG(r,\omega_t,\delta)$ or $IG(r,\omega_t,\delta;P,H,\bfS_t,\bfd_t)$ to denote incentive gap... tbd}
\end{definition}



\begin{definition}
Consider the stochastic two-level model with population-size $k$.  Fix a pricing protocol
$P$ and a strategy profile $H$.  Fix any time $t$, scenario $\omega_t$,
active location $(l,\omega_t)$, and supply-location vector $\bfS_t$.
Let $\epsilon>0$ be an error term, and define $p_k(\epsilon,l,\omega_t,\bfS_t;P,H)$
the be the probability that a driver
located\footnote{In the event there are $0$ drivers located at $\ell$ in time $t$ we
define $p_k(\epsilon,l,\omega_t,\bfS_t;P,H)$ to be $1$.} at $(l,\omega_t)$ receives a trip-allocation for which the incentive gap is
smaller than $\epsilon$, with respect to the market dynamics induced by $P$, $H$ and the size-parameter $k$. 

For each $k\geq 0$ let $\bfS_t^k$ be a sequence of supply-location vectors
in the support of the induced distribution over supply-location vectors
at time $t$, scenario $\omega_t$, and population-size $k$, and assume
the sequence converges $\bfS_t^k\to\bar{\bfS}_t$.

The strategy profile $H$ is an \emph{asymptotic equilibrium} with
respect to the pricing protocol $P$ if, for any $t$, $\omega_t$, $(l,\omega_t)$, and convergent 
sequence of  supply-location vectors $(\bfS_t^k:k=1,2,\dots)$,
there exists a sequence of error terms $\epsilon_k\to 0$ such that $p_k(\epsilon_k,l,\omega_t,\bfS_t^k;P,H)\to 1$.
\end{definition}

\begin{definition}
For a time period $t$, scenario $\omega_t$, and supply-location vector $\bfS_t$,
let $\bff^*(\bfS_t)$ denote the optimal solution for the stochastic maximum
flow problem (\ref{eq:dynamic_optimization}) with respect to the subnetwork
induced by $\omega_t$ and the supply locations $\bfS_t$.

The \emph{stochastic spatiotemporal pricing and matching mechanism} (SSP) is the combination of
a pricing function $P^{SSP}$ and a driver strategy profile $H^{SSP}$.

The pricing
function $P^{SSP}(\cdot)$ produces prices by computing the optimal solution
$\bff^*(\bfS_t)$ and using the optimal flow values $f^*_{(r,\omega_t)}(\bfS_t)$
on each route.  Specifically, the prices
$\bfrho = P^{SSP}(t,\omega_t,\bfS_t)$ are specified by
$$
\rho_{(r,\omega_t)} = F_{(r,\omega_t)}^{-1}\left(1-\frac{f^*_{(r,\omega_t)}}{\bar{D}_{(r,\omega_t)}}\right),
$$
where $F_{(r,\omega_t)}^{-1}$ is the inverse of the rider-value distribution
function, $f^*_{(r,\omega_t)}$and $\bar{D}_{(r,\omega_t)}$ is the mean price-inquiry demand for
the route $(r,\omega_t)$.  Note that the randomness in the SSP prices comes
only from the supply-location vector $\bfS_t$.

The strategy profile $H^{SSP}(\cdot)$ is obtained by producing a trip-allocation
vector which is as close as possible to the actions specified by the optimal
stochastic flow $\bff^*(\bfS_t)$.  The exact details are specified in 
Algorithm \ref{alg:matching_details}.
\end{definition}


Using the framework outlined in the above definitions we can re-state our main
approximate incentive compatibility theorem (Theorem \ref{thm:stochastic_ic}) as
follows:
\begin{theorem*}
Under Assumptions 1-3, the SSP strategy profile
$H^{SSP}$ is an asymptotic equilibrium with respect to the SSP pricing
policy $P^{SSP}$.
\end{theorem*}

The following theorem is a simple property of the trip-allocation vector
produced by the SSP mechanism, which follows from our assumption that
dispatch demand converges in probability to its mean.
\begin{theorem*}
Fix a time $t$, scenario $\omega_t$, and let $\bfS_t^k$ be a sequence of supply-location vectors in the support of the induced distribution over supply-location vectors with respect to the population-size parameter $k$, 
and let $\bar{\bfS}_t$ be the limiting supply-location vector.
Let $\bfd_t$ be the (random) dispatch-request vector, whose distribution
depends on the SSP pricing function $P^{SSP}$, and let 
$\bfh_k^{SSP}=H^{SSP}(t,\omega_t,k,\bfS_t^k,\bfd_t)$ be the resulting random trip-allocation
vector produced by the SSP mechanism. 

Then, under Assumptions 1-3, $\bfh_k^{SSP}$ converges in probability
to the optimal stochastic flow with respect to the limit of the supply location
vectors: 
$$
\lim_{k\to\infty} \bbP^k(\|\bfh_k^{SSP} - \bff^*(\bar{\bfS}_t)\|_1>\epsilon) = 0
$$
for all $\epsilon > 0$.
\end{theorem*}

The following is a conjecture about robustness of equilibria induced by
the SSP prices $P^{SSP}$:
\begin{theorem} \textbf{Conjecture}
\label{thm:general_eqlbm}
Fix a time $t$, scenario $\omega_t$, and let $\bfS_t^k$ be a sequence of supply-location vectors in the support of the induced distribution over supply-location vectors with respect to the population-size parameter $k$, 
and let $\bar{\bfS}_t$ be the limiting supply-location vector.
Let $\bfd_t$ be the (random) dispatch-request vector, whose distribution
depends on the SSP pricing function $P^{SSP}$.

Let $H$ be any non-degenerate strategy profile that is an asymptotic equilibrium with respect to
$P^{SSP}$, and let 
$\bfh_k=H(t,\omega_t,k,\bfS_t^k,\bfd_t)$ be the resulting random trip-allocation
vector produced $H$ under population size $k$. 

Then, under Assumptions 1-3, $\bfh_k$ converges in probability
to the optimal stochastic flow with respect to the limit of the supply location
vectors: 
$$
\lim_{k\to\infty} \bbP^k(\|\bfh_k - \bff^*(\bar{\bfS}_t)\|_1>\epsilon) = 0
$$
for all $\epsilon > 0$.
\end{theorem}

\Xomit{
\subsection{Towards a Proof of (Conjectured) Theorem \ref{thm:general_eqlbm}}
This section is a scratchpad for working out the proof of (the general statement of)
Theorem \ref{thm:general_eqlbm}.
Let us start by stating a number of simple lemmas that will be helpful for our 
analysis.



\begin{lemma}
Fix a time $t$, scenario $\omega_t$, and let $\bfS_t^k$ be a sequence of supply-location vectors in the support of the induced distribution over supply-location vectors with respect to the population-size parameter $k$, 
and let $\bar{\bfS}_t$ be the limiting supply-location vector.
Let $\bfd_t^k$ be the (random) dispatch-request vector, whose distribution
depends on the SSP pricing function $P^{SSP}$ (and, in turn, the output of the
pricing function depends on the supply-location vector $\bfS_t^k$).

Let $\bar{\bfd}_t$ be the dispatch request vector in the fluid limit with respect
to the limiting supply locations $\bar{\bfS}_t$.  The components of $\bar{\bfd}_t$
are specified by
$$
\bar{d}_{(r,\omega_t)} = \min\left(\bar{D}_{(r,\omega_t)}, f^*_{(r,\omega_t)}\right)
$$
for each active route $(r,\omega_t)\in\calA_{\omega_t}^t$, where $\bar{D}_{(r,\omega_t)}$
is the fluid price-inquiry demand for $(r,\omega_t)$ and
$f^*_{(r,\omega_t)}$ is the flow allocated to the route $(r,\omega_t)$ under the
optimal solution with respect to the limiting supply locations,
$\bff^*_{(r,\omega_t)}(\bar{\bfS}_t)$.

Then under the distribution induced by the SSP pricing function $P^{SSP}$,
the random dispatch request vector under population-size parameter $k$
converges in probability to the fluid dispatch request vector $\bar{\bfd}_t$:
$$
\lim_{k\to\infty} \bbP^k\left(\|\bfd_t^k - \bar{\bfd}_t\|_1>\epsilon) = 0
$$
for all $\epsilon > 0$.
\end{lemma}

\mccomment{\textbf{Scratchpad for a formal proof of Theorem \ref{thm:general_eqlbm}}}
\begin{proof}
We proceed via backwards induction and start in the final time period $t=T$.
\begin{itemize}
    \item 
\end{itemize}
\end{proof}}

\subsection{Towards a Proof Using a Generic  Convex Optimization Lemma}
\input{eqlbm_welfare_optimality}

\subsection{A Generic Convex Optimization Lemma}
\input{stochastic_programming_lemma}

\subsection{Example: The Issue with the Current Generic Convex Opt Lemma}

Consider a two-timeperiod problem with only two routes.  Suppose the objective function
is
$$
\calU(\bff) = U_1(f_1) + U_2(f_2) + \calW(\bff),
$$
where $\bff=(f_1,f_2)$ specifies the amount of flow along each route.  We have a constraint 
$\bff \geq 0$ and a capacity constraint $f_1 + f_2=S$.
Our optimality conditions state $\bff^*$ is optimal if there exists a dual variable $\eta^*$
such that
$$
\eta^* \geq \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bff^*)
$$
holds for $i=1,2$, and we need the above inequality to be tight when $f_i>0$.

Now suppose we have a candidate solution $\bar{\bff} = (\bar{f}_1,\bar{f}_2)$ and a variable 
$\bar{\eta}$ satisfying the following for $i=1,2$:
$$
\bar{\eta} \geq \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bar{\bff}),
$$
and the above inequality is tight when $\bar{f}_i>0$.
This is almost the optimality condition stated above, except the $\frac{d}{df_i}U_i(f_i^*)$
term still depends the $f_i^*$ component of an optimal solution, 
rather than the $\bar{f}_i$ component of the solution of interest.
Is this sufficient to conclude that $\bar{\bff}$ is an optimal solution?

Let $\bfalpha=(\alpha_1,\alpha_2)\geq 0$ be a dual variable associated with the
nonnegativity constraints $\bff\geq 0$.
The Lagrangian function for our problem is defined as
$$
L(\bff,\eta,\bfalpha) = -\calU(\bff) + \eta(f_1+f_2-S) - \alpha_1 f_1 - \alpha_2 f_2, 
$$
and the dual function is
$$
\Phi(\eta,\bfalpha) = \inf_{\bff}L(\bff,\eta,\bfalpha).
$$
Weak duality states $$-\calU(\bff) \geq \Phi(\eta,\bfalpha)$$ for any feasible
$\bff$ and any dual variables $\eta$, $\bfalpha\geq 0$.

Since the definition of $\Phi(\eta,\bfalpha)$ is in terms of an unconstrained
infimum over $\bff$, the value of $\bff$ achieving the infimum
can be computed by setting
the gradient to zero.
We compute the partial derivatives of $L(\bff,\eta,\bfalpha)$ 
with respect to $f_1$, $f_2$
as follows. For $i=1,2$:
\begin{equation}
\label{eq:partial}
\frac{\partial}{\partial f_i}L(\bff,\eta,\bfalpha) = 
-\frac{d}{d f_i} U_i(f_i) - \frac{\partial}{\partial f_i}\calW(\bff)
+ \eta - \alpha_i.
\end{equation}

Computing the partial derivatives of $L(\cdot,\cdot,\cdot)$ gives us an
approach for bounding the suboptimality of an arbitrary feasible solution.
Let $\bff$ be an arbitrary feasible solution, let $\eta,\bfalpha\geq 0$ be
feasible dual variables for which the partial derivatives $\frac{\partial}{\partial f_i}L(\bff,\eta,\bfalpha)$ equal $0$ for $i=1,2$, and let $\bff^*$ be an
optimal primal solution.  Since the partial derivatives are $0$ we have
$\Phi(\eta,\bfalpha)=L(\bff,\eta,\bfalpha)$, so we can bound the suboptimality
of $\bff$ as follows:
\begin{align*}
    \calU(\bff^*) -\calU(\bff) & \leq -\Phi(\eta,\bfalpha) - \calU(\bff) \\
    & = \calU(\bff) - \eta(f_1 + f_2 - S) + \alpha_1f_1 + \alpha_2f_2 - \calU(\bff)\\
    & = \alpha_1f_1 + \alpha_2f_2.
\end{align*}
So, for an arbitrary feasible solution $\bff$, if we can find feasible dual
variables $(\eta,\bfalpha)$ for which the partial derivatives (\ref{eq:partial})
are $0$, then the suboptimality of $\bff$ is bounded by the complementary slackness
violation $\bfalpha^T\bff$.

Now, let's return to our candidate solution $\bar{\bff}$ for which we have
dual values $\bar{\eta}$, $\bar{\bfalpha}\geq 0$ satisfying the following:
$$
\bar{\eta} = \frac{d}{df_i}U_i(f_i^*) + \frac{\partial}{\partial f_i}\calW(\bar{\bff}) + \bar{\alpha}_i,
$$
in addition to complementary slackness conditions $\bar{\alpha}_i\bar{f}_i=0 $. 
\mccomment{We could try replacing $\bar{\alpha}_i$ with $\bar{\alpha}_i - \frac{d}{df}U_i(f_i^*) -
\frac{d}{df}(U_i(\bar{f}_i))$ but that might violate feasibility of $\bar{\bfalpha}$}

\section{Generic Convex Opt Lemma: Fixed}
\input{convex_opt_lem_fixed.tex}

\section{Robust Welfare Optimality in the Fluid Model}
\input{robust_fluid_welfare.tex}


\Xomit{
\subsection{Towards a Proof of (Conjectured) Theorem \ref{thm:general_eqlbm} using Approximate Complementary Slackness}

Let us start this section by defining the expected welfare in the stochastic
two-level model under a strategy-profile $H$ and a pricing policy $P$.
In contrast to expected welfare for the stochastic fluid model, where the only
source of randomness was the stochastic scenario tree, the distribution over which
expected welfare in the stochastic two-level model is taken includes all the granular
rider and driver randomness from the second level of the model.


First, we define the expected cumulative rider and driver welfare in a single
time period as a function of the driver trips for that time period.  Consider
a time $t$, scenario $\omega_t$, let $\bfrho_t$ be the trip-price vector produced by
the pricing policy $P$, and let $\bfh_t$ be the trip-allocation vector
produced by the driver strategy profile $H$, specifying the number of dispatch
trips $h_{(r,\omega_t,1)}$, and the number of relocation trips $h_{(r,\omega_t,0)}$,
on each active route $(r,\omega_t)\in\calA_{\omega_t}^t$.

Recall that, in the optimization problem for the stochastic fluid model, we used a
parameterization that did not distinguish between the two types of trips on each
route.  In this setting, for a feasible solution which specified $f=f_{(r,\omega_t)}$
flow along a route $(r,\omega_t)$, the associated reward was defined as:
\begin{equation*}
U_{(r,\omega_s)}(f)= \begin{cases}
    \bar{D}_{(r,\omega_s)}\bar{V}_{(r,\omega_s)}  - fc_{(r,\omega_s)}& \mbox{if }f > \bar{D}_{(r,\omega_s)},\\
    f \bbE\left[V_{(r,\omega_s)}\mid V_{(r,\omega_s)}\geq F_{(r,\omega_s)}^{-1}\left(1-\frac{f}{\bar{D}_{(r,\omega_s)}}\right)\right]
 - fc_{(r,\omega_s)}
    &
    \mbox{if } f \leq \bar{D}_{(r,\omega_s)}.
\end{cases}
\end{equation*}
For now \mccomment{doubt this is good notation} let us use the notation
$\bar{U}_{(r,\omega_s)}(h_0,h_t,\rho)$ to specify the expected utility achieved
in the stochastic two-level model, where we use the shorthand notation 
$h_0=h_{(r,\omega_s,0)}$ to denote the volume of relocation trips,
and $h_1=h_{(r,\omega_s,1)}$ to denote the volume of dispatch trips.
The expected route-specific utility is defined as follows:
\begin{equation}
\bar{U}_{(r,\omega_s)}(h_0,h_1,\rho)= h_1
\bbE\left[V_{(r,\omega_s)}\mid V_{(r,\omega_s)}\geq \rho\right]
- (h_1 + h_0)c_{(r,\omega_s)}.
\end{equation}
This function acounts for driver granularity because it depends on the trip-allocation
counts $h_0$ and $h_1$, but it takes an expectation over the granular rider utilities.

Next, we define expected welfare in the stochastic two-level model.  
Fix a time period $t$ and scenario $\omega_t$.  Let $k$ be the network-size
parameter and let $\bfS_t^k$ be the supply-location vector at the beginning of the
time period, after new supply enters the market.  For now \mccoment{not committing to
this notation at all} let $\bar{\calW}_{\omega_t}^k(\bfS_t^k;H,P)$ denote the expected
welfare-to-go in the stochastic two-level model.  This is defined as follows:
\begin{equation}
    \bar{\calW}^k_{\omega_t}(\bfS_t^k;H,P) = 
    \bbE\left[\sum_{(r,\omega_t)\in\calA_{\omega_t}^t} \bar{U}_{(r,\omega_t)}(h_{(r,\omega_t,0)},
    h_{(r,\omega_t,1)}, \rho_{(r,\omega_t)}) +
    \bbE\left[\calW^k_{\omega_{t+1}}(\bfS_{t+1}^k;H,P)\right]\right].
\end{equation}
The above expectation is taken over the trip-allocations $\bfh$, the 
future scenario $\omega_{t+1}$, and the future supply-location vector $\bfS_{t+1}^k$.

Now, suppose $S_t^k\to\bar{S}_t$ as $k\to\infty$ and note that the stochastic
maximum flow optimization problem in the stochastic fluid model can be
reformulated as the following single-timeperiod problem: \mccomment{this notation will change}
\begin{equation}
\label{eq:single_period_opt_flow}
\calW_{\omega_t}(\bar{\bfS}_t) = \sup_{\bff}\left(
\sum_{(r,\omega_t)\in\calA_{\omega_t}^t}U_{(r,\omega_t)}(f_{(r,\omega_t)})
+ \bbE\left[\calW_{\omega_{t+1}}(\bar{\bfS}_{t+1}^{\omega_{t+1}})\right]\right)
\end{equation}

In the above, the decision variable $\bff$ specifies flow values $f_{(r,\omega_t)}$
for active routes $(r,\omega_t)$, and $\bar{\bfS}_{t+1}^{\omega_{t+1}}$ is the resulting
supply-location vector at the beginning of time $t+1$ resulting from these flow values.
Namely, $\bar{\bfS}_{t+1}^{\omega_{t+1}}$ specifies how many drivers are located
at each time $t+1$ active location $(l,\omega_{t+1})$.

For this formulation we get optimality conditions that look like
$$
 \eta^*_{(l,\omega_t)} \geq \frac{d}{df} U_{(r,\omega_t)}(f^*_{(r,\omega_s)}) + \bbE\left[
 \frac{d}{d S_{(l^+(r),\omega_{t+1})}} \calW_{\omega_{t+1}}(\bar{\bfS}_{t+1}^{\omega_{t+1}}) \right],
$$
indexed over all active routes $(r,\omega_t)$ in the current time period $t$.

To show Theorem \ref{thm:general_eqlbm}, we plan to take the following steps:
\begin{enumerate}
    \item For each $k$, and for any strategy profile $H$, the resulting trip-allocation
    vector $\bfh^k$ is approximately feasible for the fluid optimization problem.  This
    just follows from the definition of a strategy profile.
    \item The utility-to-go values $\calV_{(l,\omega_t)}(\bfS_t^k;H,P)$ are approximately feasible dual variables for the fluid optimization problem.
    \item The approximate incentive-compatibility conditions we assumed on $H$ with respect to $P$ implie approximate complementary slackness holds between $\bfh^k$ and $\calV_{(l,\omega_t)}(\bfS_t^k;H,P)$
    \item The approximation error goes to $0$ as $k$ goes to infinity, so $\bfh^k$ converges to an optimal solution with high probability.
\end{enumerate}

Point (1) regarding approximate feasibility of $\bfh^k$ follows from the
capacity-constraints imposed on $\bfh^k$ and the fact that $\bfS_t^k$ converges
to $\bar{\bfS}_t$ as $k\to\infty$.

Points (2) and (3), regarding approximate feasibility of utility-to-go values
$\calV^k_{(l,\omega_t)}(\bfS_t^k;H,P)$ for the dual problem and approximate
complementary slackness holding between $\bfh^k$ and $\calV^k_{(l,\omega_t)}(\cdot;H,P)$ both
depend on the assumption that $H$ forms an asymptotic equilibrium with respect
to $P$.

Recall our definition of asymptotic equilibrium states the following.  
Fix an active location $(l,\omega_t)$ and let $p_k(\epsilon,l,\omega_t,\bfS_t^k;H,P)$ be the probability under $H$ and $P$
that a driver
positioned at $(l,\omega_t)$ receives a trip-allocation $(r,\omega_t,
delta)$ 
for which the incentive gap (an upper bound on the utility of deviating) 
of $(r,\omega_t,\delta)$ is at most $\epsilon$.
Our definition of $H$ and $P$ being an asymptotic equilibrium
states that for a convergent sequence of supply location vectors 
$\bfS_t^k\to\bar{\bfS}_t$, and for any active location $(l,\omega_t)$,
there exists a sequence of error terms $\epsilon_k\to 0$
for which $p_k(\epsilon_k,l,\omega_t,\bfS_t^k;H,P)\to 1$.

Notice that this definition depends strongly on the distribution of trip-allocations
produced by the strategy profile $H$ for a driver positioned at $(l,\omega_t)$.
Recall, for a trip-allocation vector $\bfh^k$, the induced distribution of trip-allocations
for a driver positioned at $(l,\omega_t)$ is denoted by $\bfh^k(l,\omega_t)$
and each trip type $(r,\omega_t,\delta)$ is allocated to the driver with
probability proportional to $h^k_{(r,\omega_t,\delta)}$.

Now, let $\calD^k\subseteq\calA^t_{\omega_t}\times\{0,1\}$ be the set of trip types
$(r,\omega_t,\delta)$ for which the incentive gap is larger than $\epsilon_k$, i.e.
these are the trip allocations for which there is incentive to deviate.
Recall the utility-to-go value $\calV^k_{(l,\omega_t)}(\bfS_t^k;P,H)$ is defined
as an expectation over trip-allocations $(r,\omega_t,\delta)\sim\bfh^k(l,\omega_t)$.

Let us define a version of utility-to-go that conditions on the allocated trip-allocation
lies in a subset $\calR$ of all feasible trip-allocations:
$$
\calV^k_{(l,\omega_t)}(\bfS_t;P,H\mid\calR) = \begin{cases}
\bbE^k\left[\delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\mid (r,\omega_t,\delta)\in\calR\right] & \mbox{if } t<T,\\
\bbE^k\left[\delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)}\mid (r,\omega_t,\delta)\in\calR\right] & \mbox{if }t=T. 
\end{cases}
$$

With this definition we can decompose utility-to-go as
\begin{align*}
\calV^k_{(l,\omega_t)}(\bfS_t;P,H) = & \  \bbP^k((r,\omega_t,\delta)\in\calD)\calV^k_{(l,\omega_t)}(\bfS_t;P,H\mid\calD) \\
& + \bbP^k((r,\omega_t,\delta)\notin\calD)\calV^k_{(l,\omega_t)}(\bfS_t;P,H\mid\calD^c). 
\end{align*}
As a shorthand let's write
$$
p_k = \bbP^k((r,\omega_t,\delta)\notin\calD) = p_k(\epsilon_k,l,\omega_t,\bfS_t^k;H,P)
$$
for the probability of being allocated a trip for which the incentive
gap is at most $\epsilon_k$. By assumption we have $p_k\to 1$.
Also by assumption, conditioning on the trip-allocation $(r,\omega_t,\delta)$
falling into the at-most-$\epsilon_k$-incentive-to-deviate trips $\calD^c$, the
following inequalities hold:
\begin{align*}
    \calV^k_{(l,\omega_t)}(\bfS_t^k;P,H\mid\calD^c) + \epsilon_k & \geq \max_{(r,\omega_t,\delta)} \delta\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \bbE^k\left[ \tilde{\calV}^k_{(l^+(r),\omega_{t+1})}(\tilde{\bfS}_{t+1};P,H)\right] \\
    & \geq \rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \bbE^k\left[ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right] - \eta_k,
\end{align*}
for all outgoing routes $(r,\omega_t)\in A^+_{\omega_t}(l)$,
where $\tilde{\bfS}_{t+1}$ is the random time $t+1$ supply-location vector which 
accounts for the drivers deviation, and $\eta_k$ is the error term
$$
\eta_k = \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right] - \bbE^k\left[ \tilde{\calV}^k_{(l^+(r),\omega_{t+1})}(\tilde{\bfS}_{t+1};P,H)\right]
$$

Now we use the fact that the utility of being allocated one of the bad trip-allocations
in $\calD$ is smaller than being allocated a trip in $\calD^c$, so we have the
bounds
$$
\calV^k_{(l,\omega_t)}(\bfS_t;P,H\mid\calD^c) \geq \calV^k(\bfS_t;P,H) \geq
p_k\calV^k_{(l,\omega_t)}(\bfS_t;P,H\mid\calD^c).
$$
So, putting it together, we get the approximate optimality conditions:
\begin{equation}
\label{eq:approx_optimality}
\calV^k(\bfS_t;P,H) \geq
p_k\left(\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \bbE^k\left[ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right] - \eta_k \right) +\epsilon_k,
\end{equation}
for all outgoing routes $(r,\omega_t)\in A^+_{\omega_t}(l)$.

For the approximate complementary slackness conditions, consider a trip-allocation
$(r,\omega_t,\delta)\in\calD^c$ for which there is at most $\epsilon_k$ incentive
to deviate.  Then the utility-to-go 
$$
\rho_{(r,\omega_t)} - c_{(r,\omega_t)} + \bbE^k\left[ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right]
$$
is within $\epsilon_k+\eta_k$ of the optimal utility-to-go for deviating. Since this is
true for the utility-to-go of every trip-allocation in $\calD$, we get the following
approximate CS conditions:
\begin{enumerate}
    \item for all routes $(r,\omega_t)$ for which $(r,\omega_t,1)\in\calD$ the
    gap in equation (\ref{eq:approx_optimality}) is approximately tight
    \item If the gap (\ref{eq:approx_optimality}) is not approximately tight, then
    $$h_{(r,\omega_t,1)} + h_{(r,\omega_t,0)} \leq \frac{1-p_k}{S_{t,(l,\omega_t)}^k}$$,
   i.e. the amount of flow allocated on this route goes to $0$ as $k$ goes to $\infinity$.
\end{enumerate}

\Xomit{\subsection{Possible Small-Welfare-Loss Theorem Statements}

\mccomment{
There are a few ways we might want to define welfare loss due to minor incentives:
\begin{itemize}
    \item We could say that the SSP mechanism induces an exact equilibrium for each fixed $k$, and we could show that this exact equilibrium is close to the fluid optimal solution, and that it converges to the fluid optimal solution as $k\to\infty$.  Characterizing the exact equilibrium for general fixed $k$ sounds quite difficult.
    \item We could say that if $\bfh_k$ is a sequence of equilibria (must define what it means for $\bfh_k$ to be an equilibrium first) for different values of $k$, then it must be the case that $\bfh_k\to\bff^*$ is true.
    \item We could say that if $\bfh_k$ is a sequence of equilibria  for different values of $k$, then it must be the case that the welfare under $\bfh_k$ converges to the welfare under $\bff^*$.
    \item A stronger version of the last two claims would only assume that each $\bfh_k$ is an approximate equilibrium.
\end{itemize}}}}


==> model2.tex <==
We now describe our model of a stochastic ridesharing network.

There is a discrete set of locations $\calL$ and a time horizon $T$.
Market interactions occur at discrete time periods $t=1,\dots,T$.
To model high-level uncertainty about the state of the world
a random variable $\toplvlstate{t}$ is sampled at the beginning
of time period $t$.  
We assume that supply and demand levels at each time period $t$ are
influenced by the sequence of state variables $\toplvlstate{1},\dots,\toplvlstate{t}$.
The effect of this state variable sequence will be central throughout the paper.
We use the notation $\toplvlscn{t}=(\toplvlstate{1},\dots,\toplvlstate{t})$ to mean
the sequence of state variables up to and including time $t$.
We refer to a realization of $\toplvlscn{t}$ as the top-level scenario at time $t$.

For example, the set $\calL$ could indicate neighborhoods in a large city
and a two-hour rush period could be modeled by condensing $10$-minute chunks into
one time period and taking $T=12$.
A realization of $\toplvlstate{t}$ might indicate
whether it is raining or whether a sporting event has ended early.
Our assumption that the sequence of state variables $\toplvlscn{t}$ can influence
market dynamics at time $t$ captures important phenomenon. For example,
in the first time period with rain we can expect a large spike in
demand from the beach neighborhood towards residential neighborhoods, but if the rain
persists, the demand spike will abate after three time periods.

For the remainder of this section we discuss our assumptions about the dynamics
within each time period.  Section \ref{sec:two_level} presents these assumptions
in a model where supply and demand are stochastic.  Section \ref{sec:fluid} discusses
a model where supply and demand are deterministic.

\subsection{Stochastic Two-Level Model}
\label{sec:two_level}

\subsection{Stochastic Fluid Model}
\label{sec:fluid}


==> model_dynamics.tex <==


\medskip
\noindent \textbf{Market Dynamics.}
We begin this section by summarizing market dynamics 
for both the stochastic two-level model and the
stochastic fluid model at a high-level.

For simplicity and without loss of generality
we make the following assumptions that all trips take
a single time period to complete, and that drivers never exit the marketplace.
\begin{assumption}
    \label{assn:single_time_period} All trips take a single time period
    to complete.  In addition, a driver who has entered the marketplace
    does not exit the marketplace until the final time period.
\end{assumption}
\begin{assumption}
    \label{assn:driver_exit} A driver who has entered the marketplace
    does not exit the marketplace until the final time period.
\end{assumption}
We emphasize that this assumption is without loss of
generality and that our results readily extend
to settings with arbitrary scenario-dependent 
travel times, as well as settings where driver
can exit the market before the end of the planning
horizon and collect positive utility. We discuss
why this assumption is without loss of generality in  Appendix \mccomment{insert}.

Model dynamics depend on the pricing policy that the platform uses to set trip prices
in each time period. Definition \ref{def:ppp} formalizes what we mean by platform pricing
policy in our model.
\begin{definition}
\label{def:ppp}
A platform pricing policy is a function 
$P:\bbR^\calL\times\bbR^\calR\times\Omega_{1:T}\to\bbR_+^\calR$
which 
takes as input a supply-location vector $\bfS\in\bbR^\calL$, a price-inquiry demand vector $\bfD\in\bbR^\calR$,
and a time-scenario $\omega_t\in\Omega_{1:T}$, and produces a vector
of prices $\bfrho_t=P(\bfS,\bfD,\omega_t)\in\bbR^\calR$ 
to be used in the $t$th time period.
\end{definition}


Market operations proceed at discrete time periods 
$t\in \{1,2,\dots,T\}$. The state of the marketplace at each time
period is described by two variables: the time-scenario
$\omega_t$ and a \emph{supply-location vector}
$\bfS_t(\omega_t)=(S_{\ell}(\omega_t) : \ell\in\calL)$.
Each component $S_{\ell}(\omega_t)$ of the 
supply-location vector specifies the amount of
available drivers at each location $\ell$ under the
time-scenario $\omega_t$.
Before the first time period begins, the 
initial time-scenario is initialized to the empty tuple
$\omega_0 = \emptyset$.

Within each time period the order of events is as
follows:
\begin{enumerate}
\item The time-scenario $\omega_{t}$ is sampled
conditional on the time-scenario $\omega_{t-1}$ and independent of all
other sources of randomness.

\item The supply-location vector 
$\bfS_t(\omega_t)$ 
is obtained from the destination locations of driver
trips in the previous time period, as well as the
locations of new drivers who enter the marketplace.

A variable $M_{\ell}(\omega_t)$ tracks how many 
drivers enter the marketplace at each location $\ell\in\calL$
under the current time-scenario $\omega_t$, and
the vector $\bfM_t(\omega_t) = (M_{\ell}(\omega_t) :
\ell\in\calL)$ tracks driver-entry counts across
all LT-scenarios.
A variable $h_r(\omega_{t-1})$ tracks the amount
of drivers who took a trip along route $r$ under 
the previous time-scenario $\omega_{t-1}$.

Each component $S_{\ell}(\omega_t)$ of $\bfS_t(\omega_t)$ is
then specified by
the following equation:
\begin{equation}
\label{eq:supply_location_update}
    S_\ell(\omega_t) = M_\ell(\omega_t) +
    \sum_{r\in A^-(\ell)} h_r(\omega_{t-1}).
\end{equation}
In the above we use $A^-(\ell)$ to be the set
of routes $r\in\calR$ where $\ell$ is the destination
location.  As stated in Assumption \ref{assn:single_time_period},
all trips take a single time period to complete,
so every driver who traversed a route $r\in A^-(\ell)$
in the previous time period
with $\ell$ as the destination location will be located
at $\ell$ in the current time period.

\begin{enumerate}
\item In the case where $t=1$ is the first time period,
and hence $\omega_{t-1}=\omega_0=\emptyset$ is the
empty tuple, we initialize each driver trip count
variable $h_r(\omega_0)$ to be $0$. In the remaining
time periods, the value of the 
driver trip count variable is specified below
in Step \mccomment{insert}.
\item We assume that driver-entry decisions depend
on the time-scenario $\omega_t$ but are otherwise
exogenous to the state of the marketplace.
As stated in Assumption \ref{assn:driver_exit}, we
assume (without loss of generality) 
that once a driver enters they marketplace, 
they remain in the marketplace for all remaining
time periods.

\end{enumerate}

\item Sound amount of \emph{price-inquiry demand} is
realized for each route.  Each unit of price-inquiry
demand is a rider potentially interested in requesting
a dispatch.  Before making a final decision about 
whether to request a dispatch, each price-inquiring
rider makes an inquiry to the platform about the
price of a dispatch for their route of interest.

For each route $r\in\calR$ the variable 
$D_r(\omega_t)$ specifies how much price-inquiry
demand occurs for route $r$ under the time-scenario
$\omega_t$.  
A vector $\bfD_t(\omega_t)=(D_r(\omega_t) : r\in\calR)$ tracks
price-inquiry demand across all ODT-scenarios.

We assume that price-inquiry demand
depends on the time-scenario $\omega_t$, but is
otherwise exogenous to the state of the marketplace.

    \item The platform sets a price $\rho_r(\omega_t)$ for each route $r\in\calR$.  The variable
    $\bfrho_{t}(\omega_t)=(\rho_r(\omega_t) : r\in\calR)$ tracks
    the price for all routes under the current time-scenario
    $\omega_t$. 
    
    \item Price-inquiring riders react to the prices:
    some riders request a dispatch, and some price-inquiring
    riders leave the system.  We assume that each 
    price-inquiring rider holds a private value for a dispatch,
    and we assume that riders have quasilinear utility for money,
    meaning a rider requests a dispatch if and only if their
    private value is at least as large as the trip price.
    
    The variable $d_r(\omega_t)$ specifies how many dispatch
    requests occur for each route $r\in\calR$, and the
    vector $\bfd_t(\omega_t)=(d_r(\omega_t) : r\in\calR)$ tracks
    the amount of dispatch requests across all ODT-scenarios.
    We assume all dispatch-requests begin as price-inquiry
    requests, so $d_r(\omega_t) \leq D_r(\omega_t)$ always
    holds.
    
    \item A trip-allocation process occurs and every driver
    is allocated a trip for the current time period.
    A driver located at $\ell\in\calL$ can drive towards any destination.
    If $d\in\calL$ is the driver's destination we say they traverse the route
    $(\ell,d)\in\calR$.  We use $A^+(\ell)=\{(\ell,d):d\in\calL\}$ to denote the
    set of routes originating from $\ell$.
    
    When a driver traverses a route we also specify whether or not they
    are fulfilling a dispatch.  To this end we include an indicator variable
    $\delta\in\{0,1\}$ and we specify a driver trip by a tuple $(r,\delta)$,
    where $r\in\calR$ specifies the route traversed and $\delta$ indicates
    whether or not the trip fulfills a dispatch ($\delta=0$ means the trip does
    not fulfill a dispatch; $\delta=1$ means the trip does fulfill a dispatch).
    
    For each trip type $(r,\delta)\in\calR\times\{0,1\}$ the variable
    $g_{(r,\delta)}(\omega_t)$ counts how many drivers take the trip
    $(r,\delta)$ under the time-scenario $\omega_t$.
    
    Sometimes we will want to refer to driver trip counts only in terms of the
    routes that were traversed, i.e. without the distinction of how many drivers
    were or were not fulfilling a dispatch.  We use the variable 
    $h_r(\omega_t)=g_{(r,0)}(\omega_t)+g_{(r,1)}(\omega_t)$ to
    track how many drivers traverse route $r$ under the time-scenario $\omega_t$
    without the dispatch vs. no-dispatch distinction.  
    The variable $h_r(\omega_t)$ was used in equation (\ref{eq:supply_location_update}) 
    to specify how the supply-location counts
    $S_\ell(\omega_t)$ update across time periods.
    
    The details of the trip-allocation process incorporate aspects of 
    strategic driver behaviour and matches facilitated by the platform.  We fill
    in the details of this trip-allocation process below. \mccomment{insert section/
    defn reference if appropriate}
    
\end{enumerate}

The above steps summarize market dynamics in both the stochastic two-level model
and the stochastic fluid model.  The difference between these two models lies in the
assumptions they make about how the demand variables $\bfD_t(\omega_t)$, 
$\bfd_t(\omega_t)$, and
the supply variables $\bfM_{t}(\omega_t)$, are obtained.

\medskip
\noindent \textbf{Stochastic Fluid Model.}
We proceed by describing our assumptions about how the above demand and supply 
variables are obtained in the stochastic fluid model.

In the stochastic fluid model we view riders and drivers as continuous nonatomic agents, and
we assume that the volume of (price-inquiry) demand for each route
and the volume of entering drivers at each location are deterministic quantities
conditioned on a realization of the scenario $\omega_t$.  As such, we assume
the stochastic fluid model is parameterized by a constant 
$\bar{D}_{(r,\omega_t)}$ for each ODT-scenario $(r,\omega_t)\in\calR\times\Omega_{1:T}$,
and $\bar{M}_{(\ell,\omega_t)}$ for each LT-scenario 
$(\ell,\omega_t)\in\calL\times\Omega_{1:T}$, with the understanding that
each constant $\bar{D}_{(r,\omega_t)}$ specifies the price-inquiry demand
volume for route $r$ under time-scenario $\omega_t$, i.e. 
$D_r(\omega_t)=\bar{D}_{(r,\omega_t)}$, and each constant 
$\bar{M}_{(\ell,\omega_t)}$ specifies the driver-entry volume at each location $\ell$
under time-scenario $\omega_t$, i.e. $M_\ell(\omega_t)=\bar{M}_{(\ell,\omega_t)}$.

It remains to describe how much dispatch demand occurs for each route. We assume that,
conditioned on a time-scenario $\omega_t$, the amount of dispatch demand for each
route is a deterministic function of the trip-price produced by the platform for
that route.  The functions mapping trip-price to dispatch demand volume are an additional
set of parameters for the stochastic fluid model.  Namely, for each
ODT-scenario $(r,\omega_t)\in\calR\times\Omega_{1:T}$ we assume the
stochastic fluid model is parameterized by a function 
$\bar{d}_{(r,\omega_t)}:\bbR_+\to[0,1]$, where the value 
$\bar{d}_{(r,\omega_t)}(\rho_r)$ specifies the proportion of price-inquiry demand that
converts to dispatch-request demand on route $r$ under time-scenario $\omega_t$,
as a function of the platform-produced trip-price $\rho_r$.

\begin{assumption} [Driver-entry and Rider-demand in the Stochastic Fluid Model]
    The stochastic fluid model is parameterized by the following quantities:
    \begin{itemize}
        \item A driver-entry constant $\bar{M}_{(\ell,\omega_t)}$ for each
        LT-scenario $(\ell,\omega_t)\in\calL\times\Omega_{1:T}$.
        \item A price-inquiry-demand constant $\bar{D}_{(r,\omega_t)}$ for each 
        ODT-scenario $(r,\omega_t)\in\calR\times\Omega_{1:T}$.
        \item A dispatch-demand function  $\bar{d}_{(r,\omega_t)}:\bbR_+\to [0,1]$
        for each ODT-scenario $(r,\omega_t)\in\calR\times\Omega_{1:T}$.
    \end{itemize}
    These parameters govern the driver-entry and rider-demand variables as follows.
    Under a realized time-scenario $\omega_t$:
    \begin{itemize}
        \item The driver-entry value
        $M_\ell(\omega_t)$ at each location $\ell\in\calL$ is the driver-entry
        constant $\bar{M}_{(\ell,\omega_t)}$.
        \item The price-inquiry demand value $D_r(\omega_t)$ on each route $r\in\calR$
        is the 
        price-inquiry demand constant $\bar{D}_{(r,\omega_t)}$.
        \item The dispatch-demand volume $d_r(\omega_t)$ on each route $r\in\calR$ is
        the product $\bar{D}_{(r,\omega_t)}\bar{d}_{(r,\omega_t)}(\rho_r)$, where
        $\rho_r$ is the trip-price produced by the platform for route $r$.
    \end{itemize}
\end{assumption}

\medskip
\noindent \textbf{The Stochastic Two-Level Model.} 
In the stochastic two-level model, the driver-entry and rider-demand values are
random variables which form an additional level of randomness beneath the
top-level randomness corresponding to the stochastic scenario $\omega_t$.


In the stochastic two-level model we assume that riders and drivers are atomic agents.
Assumption \ref{assn:two_level_model} below states our assumptions about driver-entry and 
rider-demand in the stochastic fluid model.

\begin{assumption}[Driver-entry and Rider-demand in the Stochastic Two-Level Model]
\label{assn:two_level_model}
The stochastic two-level model is parameterized by the following quantities:
\begin{itemize}
    \item An agent-size parameter $1/k$, where $k$ is a positive integer.
    \item A driver-entry distribution $Q_{(\ell,\omega_t)}$ for each LT-scenario
    $(\ell,\omega_t)$.  We assume each of these distributions is supported on 
    nonnegative integer multiples of $1/k$.
    \item A price-inquiry-demand distribution $G_{(r,\omega_t)}$ for each ODT-scenario
    $(r,\omega_t)$. We assume each of these distributions is supported on 
    nonnegative integer multiples of $1/k$.
    \item A rider-value distribution $F_{(r,\omega_t)}$ for each ODT-scenario 
    $(r,\omega_t)$.
\end{itemize}
\end{assumption}

We are interested in a large-market setting where the size of each agent grows small but
the total number of agents grows large. 

We assume the driver-entry values $M_\ell(\omega_t)$ are sampled independently
from a distribution $Q_{(\ell,\omega_t)}$, and the price-inquiry demand values
$D_r(\omega_t)$ are sampled independently from a distribution $G_{(r,\omega_t)}$.

In this setting we take $M_{(\ell,\omega_t)}$ to be a random variable specifying how
many drivers enter the marketplace at the LT-scenario $(\ell,\omega_t)$, we
take $D_{(r,\omega_t)}$ to be a random variable specifying how many riders
submit a price-inquiry request for the ODT-scenario $(r,\omega_t)$, and we take
$d_{(r,\omega_t)}$ to be a random variable specifying how many riders request
a dispatch for the ODT-scenario $(r,\omega_t)$.

We are interested in a large-market setting where the distribution of these random
variables is parameterized by a population-size parameter $k$.  In the large-market
setting with population-size parameter $k$, we assume that the size of each atomic
rider and each atomic driver is equal to $\frac{1}{k}$.  We assume that the mean 
of the random variables $M_{(\ell,\omega_t)}$ and $D_{(r,\omega_t)}$ does not depend
on the parameter $k$.  We also assume that the
random variables $M_{(\ell,\omega_t)}$ and $D_{(r,\omega_t)}$ concentrate around their
mean with high probability as $k$ grows large.  
\mccomment{maybe write a bit more explaining how this is equivalent to assuming:
1) atomic agents always have size $1$, 2) the expected number of riders and drivers grows linearly in $k$, 3) standard deviation grows sublinearly in $k$}

It remains to describe how
the price-inquiring riders respond to the trip-price $\rho_{(r,\omega_t)}$. 
Recall the value $d_{(r,\omega_t)}$ tracks how many of the $D_{(r,\omega_t)}$ 
price-inquiring riders ultimately submit a dispatch request, after observing the price
$\rho_{(r,\omega_t)}$.

The total (unscaled) number of riders who submit a price-inquiry
request is equal to $kD_{(r,\omega_t)}$, since riders have size $1/k$.
Let $i=1,2,\dots,kD_{(r,\omega_t)t}$ index each 
of these riders.
We assume that each of rider $i$ holds a private value $V_i$ for a dispatch, 
and we assume these
values are sampled independently from a rider-value distribution $F_{(r,\omega_t)}$
associated with the ODT-scenario $(r,\omega_t)$.
Furthermore, we assume riders have quasilinear utility for money, meaning that
a rider $i$ requests a trip only if their
value $V_i$ is at least as large as the platform-produced price $\rho_{(r,\omega_t)}$.
Thus, the probability of each rider $i$ requesting a dispatch is given by
$\bbP(V_i\geq \rho_{(r,\omega_t)}) = 1-F_{(r,\omega_t)}(\rho_{(r,\omega_t)})$ 
(we assume the rider-value distribution $F_{(r,\omega_t)}$ is continuous and
nonatomic, so $\bbP(V_i\geq \rho_{(r,\omega_t)})=\bbP(V_i>\rho_{(r,\omega_t)})$).
It follows that the (unscaled) number of riders who request a dispatch
has a Binomial distribution with parameters $kD_{(r,\omega_t)}$ and
$1-F_{(r,\omega_t)}(\rho_{(r,\omega_t)})$.
Adding back in the scaled rider size of $1/k$, the distribution for the
number of riders who request a dispatch on each ODT-scenario 
can be expressed as follows:
\begin{equation}
    \label{eq:d_t_binomial_dist}
    d_{(r,\omega_t)}\sim\frac{1}{k}\mathrm{Binomial}\left(kD_{(r,\omega_t)}, 1-F_{(r,\omega_t)}(\rho_{(r,\omega_t)})\right).
\end{equation}
\mcdelete{
An example would be if each random variable had distribution $\mathrm{Binomial}(k,p)$, such that the parameter $k$ was shared
between all distributions and the parameter $p$ varied for each LT-scenario $(l,\omega_t)$ and each ODT-scenario $(r,\omega_t)$.
In this case, we would have the expected value under each distribution scale linearly in $k$, but the standard deviation would
scale as $\sqrt{k}$.
However, for simplicity of \etedit{notation}, %analysis, 
instead of keeping the size of a driver fixed and having the total volume of drivers grow
linearly in $k$, we assume each discrete driver has size $1/k$ in the large-market setting with size-parameter $k$ while holding
fixed the total volume of drivers, \etedit{so the expectation is fixed while standard deviation decreases with $k$}. 
}

\mcdelete{\medskip
\noindent \textbf{Assumptions on the Distribution for Supply and Demand.}
We use the notation $Q_{(l,\omega_t)}^k$ to denote the distribution from which the new-driver supply random variables $M_{(l,\omega_t)}$
are sampled in the large-market setting with population-size parameter $k$ , and we ues $G_{(r,\omega_t)}^k$ to denote the distribution from which
the price-inquiry demand random variables $D_{(r,\omega_t)}$ are sampled.
We use the notation $\bbP^k(\cdot)$ and $\bbE^k[\cdot]$ to indicate probabilities and expected values under the distributions
arising in the large-market setting with size $k$.
We assume the distributions $Q_{(l,\omega_t)}^k$ and $G_{(r,\omega_t)}^k$ satisfy the properties described in Assumption \ref{assn:large_market}.}

The above modeling assumptions and additional regularity conditions are stated
more formally below.  Assumption \ref{assn:two_level_distns} states basic
properties about the distributions governing $M_{(\ell,\omega_t)}$, 
$D_{(r,\omega_t)}$ and $d_{(r,\omega_t)}$.
Assumption \ref{assn:asymptotic_behaviour} formalizes our assumptions in the stochastic two-level model about driver-entry counts and price-inquiry
rider counts. 
Assumption \ref{assn:asymptotic_behaviour} states our assumptions about the
asymptotic behaviour of these distributions as the population-size parameter
$k$ grows large.
Finally, Assumption \ref{assn:rider_value_dist} states regularity conditions
we require for the rider-value distributions.
\begin{assumption}
    \label{assn:two_level_distns}
    In the stochastic two-level model with population-size parameter $k$, we make the following assumptions:
   \begin{itemize}
        \item The driver-entry count $M_{(\ell,\omega_t)}$ is a random variable with
        distribution $Q_{(\ell,\omega_t)}^k$ for each LT-scenario $(\ell,\omega_t)$.
        \item The price-inquiry rider count $D_{(r,\omega_t)}$ is a random variable
        with distribution $G_{(r,\omega_t)}^k$ for each ODT-scenario $(r,\omega_t)$. 
        \item The distributions 
        $(Q^k_{(\ell,\omega_t)}:(\ell,\omega_t)\in\calL\times\Omega)$ and 
        $(G^k_{(r,\omega_t)} : (r,\omega_t)\in\calR\times\Omega)$ are 
        supported on nonnegative integer
        multiples of $\frac{1}{k}$, modeling that drivers and riders are atomic
        agents of size $\frac{1}{k}$.
       \item The number of riders $d_{(r,\omega_t)}$ 
       who request a dispatch for an ODT-scenario
       $(r,\omega_t)$, conditioned on a number of price-inquiring riders
       $D_{(r,\omega_t)}$, is a Binomial random variable scaled by $1/k$
       with parameters $kD_{(r,\omega_t)}$ and 
       $1-F_{(r,\omega_t)}(\rho_{(r,\omega_t)})$.
   \end{itemize} 
\end{assumption}   

\begin{assumption}
\label{assn:asymptotic_behaviour}
Let $M^k_{(\ell,\omega_t)}$ and $D^k_{(r,\omega_t)}$ denote the supply and demand
random variables arising under the population-size parameter $k$
(i.e. $M^k_{(\ell,\omega_t)}$ has distribution $Q^k_{(\ell,\omega_t)}$ and 
$D^k_{(r,\omega_t)}$ has distribution $G^k_{(r,\omega_t)}$).
In the stochastic two-level model, we make the following assumptions about
asymptotic behaviour as the population-size parameter $k$ grows large:
    \begin{itemize}
    \item The expected value of driver-entry counts and price-inquiry rider counts 
        is the same for all $k$:
        \begin{equation}
        \mbox{For all }k, \ 
        \bbE[D^k_{(r,\omega_t)}] = \bbE[D^1_{(r,\omega_t)}] \  \mbox{ and }\  
        \bbE[M^k_{(\ell,\omega_t)}] = \bbE[{M}^1_{(\ell,\omega_t)}].  
        \end{equation}
    \item  The random variables $M^k_{(\ell,\omega_t)}$ and $D^k_{(r,\omega_t)}$ 
    concentrate around their mean as $k$ grows large.
    There exists a sequence of error terms $(\epsilon_k:k=1,2,\dots)$ which converges to $0$ as $k\to\infty$
            such that the following concentration properties hold:
            \begin{equation}
                    \label{eq:large_market_concentration}
                \bbE\left[|D_{(r,\omega_t)}^k - \bar{D}_{(r,\omega_t)}|\right] \leq \epsilon_k \ \ \ \mbox{and}\ \ \ 
                \bbE\left[|M_{(l,\omega_t)}^k - \bar{M}_{(l,\omega_t)}|\right] \leq \epsilon_k,
            \end{equation}
            and
            \begin{equation}
                        \label{eq:large_market_concentration_whp}
                        \bbP\left(|D_{(r,\omega_t)}^k - \bar{D}_{(r,\omega_t)}|\geq  \epsilon_k\right) \leq \epsilon_k \ \ \mbox{and}\ \ 
                        \bbP\left(|M_{(l,\omega_t)}^k - \bar{M}_{(l,\omega_t)}|\geq \epsilon_k\right) \leq \epsilon_k.
            \end{equation}
            In the above, we use $\bar{D}_{(r,\omega_t)}$ and $\bar{M}_{(r,\omega_t)}$
            to denote the relevant expected value (which, from the above assumption,
            does not depend on $k$).
            \mccomment{this part of the assumption can probably be stated more
            clearly, but I'll leave it as is for now.}
    \end{itemize}
\end{assumption}

\begin{assumption}
    \label{assn:rider_value_dist}
    \mccomment{text here can also be clarified but I'll leave as is for now}Let $F_{(r,\omega_t)}$ denote the distribution function from which rider values are drawn for the route $(r,\omega_t)$.
    We assume the following:
    \begin{enumerate}
        \item There exists an upper bound $V_{max}$ such that every distribution $F_{(r,\omega_t)}$ is supported on $[0,V_{max}]$.
        \item $F_{(r,\omega_t)}:[0,V_{max}]\to [0,1]$ is continuous and invertible.
        \item The inverse function satisfies $F_{(r,\omega_t)}^{-1}(0)=0$.
    \end{enumerate}
\end{assumption}

\begin{assumption}
    \label{assn:add_passenger_disutility}
We assume that drivers experience idiosyncratic disutility for adding a passenger to their car in each time period. 
Specifically, at the beginning of each time period, drivers sample an add-passenger disutility value $C$ from
a $\mathrm{Uniform}(0,C_{\max})$ distribution, for some constant term $C_{\max}>0$. We assume the disutilities are sampled independent
from other drivers and independent across time periods.
\end{assumption}


==> model_proofs.tex <==
\subsection{Proof of Lemma \ref{lem:dispatch_request_concentration}}
    \label{subsec:dispatch_request_concentration}
\begin{lemma*}
    For any route $(r,\omega_t)\in\calA$ fix a trip-price $\rho_{(r,\omega_t)}$ and let $d_{(r,\omega_t)}$ be the random dispatch-request
    volume for $(r,\omega_t)$ under the price $\rho_{(r,\omega_t)}$.
    Note that $d_{(r,\omega_t)}$ has distribution specified by equation (\ref{eq:d_t_binomial_dist}) with expected value
    $$\bar{d}_{(r,\omega_t)} = \bar{D}_{(r,\omega_t)}(1-F_{(r,\omega_t)}(\rho_{(r,\omega_t)})).$$
    There exists a sequence of error terms $\epsilon^k_{(r,\omega_t)}$
    converging to $0$ as $k\to\infty$ such that the following properties hold:
    \begin{equation*}
        \bbE^k\left[|d_{(r,\omega_t)} - \bar{d}_{(r,\omega_t)}|\right] \leq \epsilon^k_{(r,\omega_t)},
    \end{equation*}
    and
    \begin{equation*}
        \bbP^k(|d_{(r,\omega_t)} - \bar{d}_{(r,\omega_t)}|\geq\epsilon^k_{(r,\omega_t)})\leq\epsilon^k_{(r,\omega_t)}.
    \end{equation*}
\end{lemma*}



==> model_utility.tex <==
In this section we describe our assumptions about the pricing and matching decisions made by the platform,
the strategic decisions made by the drivers, and 
the resulting driver utility and total system welfare
generated by these decisions.

\medskip
\noindent 
\textbf{Platform Pricing Protocol.}
We assume that platform pricing decisions are made by the platform
at the beginning of each time period, after observing relevant information about the state of the market.  We assume that prices 
are set on a route-by-route basis, i.e. the platform sets a single
price on each route, and we assume that when a driver serves a 
dispatch along this route the price is a direct transfer from 
rider to driver.  The following definition formalizes a 
platform pricing policy as a function that maps information about
the state of the market at each time period to a price for each
route. 
\begin{definition}
\label{def:ppp}
A platform pricing policy is a function 
$P:\bbR^\calL\times\bbR^\calR\times\Omega_{1:T}\to\bbR_+^\calR$
which 
takes as input a supply-location vector $\bfS\in\bbR^\calL$, a price-inquiry demand vector $\bfD\in\bbR^\calR$,
and a time-scenario $\omega_t\in\Omega_{1:T}$, and produces a vector
of prices $\bfrho_t=P(\bfS,\bfD,\omega_t)\in\bbR^\calR$ 
to be used in the $t$th time period.
\end{definition}
Note that the above definition assumes that platform pricing
decisions 
depend only on the spatial distribution of supply and demand
in the current time period,
as well as the top level scenario $\omega_t$, i.e. we assume
the platform uses a Markovian pricing policy with respect to
the state of the system.  We remark that there is no strictly
technical reason we require the platform to use such a Markovian
policy, but all the pricing policies we will analyze later in this
paper will be Markovian, and so we define the policies this way
for simplicity.
\mccomment{maybe a cleaner way to define the platform pricing function is just let it have
an arbitrary domain?  something like $P:\calI\to\bbR^\calR$.  But then we need to be a bit
formal about the information available to $P$ in terms of the time-scenario $\omega_t$.  
I think people use the phrase ``adapted to the filtration $\omega_t$'' to mean that
a function only uses the available information in this kind of setting?}


\medskip
\noindent
\textbf{Driver Strategy-Profiles.}
Next, we formalize our representation of the actions drivers take in each
time period.  To this end, we associate each active driver in the marketplace with a unique index.
Let $\calD_t$ be the set of 

\medskip
\noindent
\textbf{Driver Strategy-Profiles.}
Next, we formalize our representation of the actions drivers
take in each time period.  Recall that a trip is specified by a tuple
$(r,\delta)$ where $r\in\calR$ is a route and $\delta\in\{0,1\}$ is an 
indicator specifying whether or not the trip fulfills a rider dispatch ($\delta=1$)
or if it is a relocation-trip without a passenger ($\delta=0$).
A \emph{trip-allocation}
vector is any nonnegative vector $\bfg\in\bbR_+^{\calR\times\{0,1\}}$ indexed 
by the augmented set of trips $\calR\times\{0,1\}$.  
Each passenger-trip component $g_{(r,1)}$ specifies
how many drivers traverse route $r$ with a passenger, and each
relocation-trip component $g_{(r,0)}$ specifies how many drivers
traverse route $r$ without a passenger.  

We say that a trip-allocation vector is feasible with respect to a supply-location
vector $\bfS$ and a dispatch demand vector $\bfd$ if it respects the 
natural supply and demand constraints imposed by $\bfS$ and $\bfd$:
\begin{equation}
\label{eq:supply_constraint}
\forall \ell\in\calL: \ 
\sum_{r\in A^+(\ell)}
\sum_{\delta\in\{0,1\}} g_{(r,\delta)} = S_\ell,
\end{equation}
and
\begin{equation}
\label{eq:demand_constraint}
\forall r\in\calR: \ g_{(r,1)} \leq d_r.
\end{equation}
For a trip-allocation vector $\bfg$ to be feasible
in the stochastic two-level model with population-size parameter
$k$, we have an additional condition that
each component $g_{(r,\delta)}$ is an integer multiple of the agent-size $1/k$, i.e. the
allocation of drivers to trips must respect the fact that drivers are atomic agents of size 
$1/k$.

We assume that drivers collectively decide on a feasible trip-allocation vector $\bfg$, and then
an external source of randomness allocates the trips specified by $\bfg$ to individual drivers.
Since drivers can only take trips which originate from their immediate location, this leads to a 
different trip-allocation distribution for each location in the network.  

\mccomment{I'm realizing this ``external source of randomness allocates trips from $\bfg$ to 
drivers'' assumption is closely tied to how we had things set up in the past, i.e. we used
to have the platform explicitly allocate trips to drivers, and this random allocation was
a means of imposing that the platform can't use preferential dispatches to align incentives.
In the new setup, we want a definition of ``driver strategy profile'' that lets drivers take
arbitrary actions, since we are able to prove that every equilibrium under SSP prices
is welfare-optimal.  But it's not clear whether what I've written below
(in Definition \ref{def:strategy_profile}) is the right notion of driver
strategy profile.  Also, the ``trip-allocation vector'' terminology is definitely a relic of
when we modeled explicit matching decisions made by the platform.
}

The next definition formalizes our notion of driver strategy
profile as a function mapping information about the state
of the marketplace to a feasible trip-allocation vector.
\begin{definition}
\label{def:strategy_profile}
In the stochastic fluid model, a driver strategy-profile is a function 
$H$, which takes as input a supply-location vector
$\bfS\in\bbR^\calL$, a dispatch-demand vector $\bfd\in\bbR^\calR$,
a price vector $\bfrho\in\bbR^\calR$, and a time-scenario $\omega_t\in\Omega_{1:T}$, and produces a trip-allocation
vector $\bfg=H(\bfS,\bfd,\bfrho,\omega_t)\in\bbR^{\calR^*}$ that is feasible with respect to
$\bfS$ and $\bfd$.

In the stochastic two-level model, the strategy-profile function 
$H$ additionally takes the population-size parameter $k$ as input, 
and it must produce a trip-allocation vector $\bfg=H(\bfS,\bfd,\bfrho,\omega_t,k)$ that is feasible with
respect to $\bfS$, $\bfd$ and $k$.
\end{definition}

Again, we remark that the above definition assumes the drivers
use a Markovian strategy-profile, in the sense that driver actions
depend only on the spatial distribution of supply, dispatch demand,
prices, and the scenario in the current time period.  We are
adopting this convention for the simplicity of presentation, and
our results easily extend to non-Markovian strategy profiles
\mccomment{Maybe it is better to not mention this stuff at all?  Or have a more general definition of strategy-profile that allows for non-Markovian profiles?  In the end, it doesn't feel like it will matter a whole lot, so I went with this because it seemed simple}.

In addition, we remark that our notion of driver strategy-profile 
corresponds to a \emph{decentralized} method of allocating drivers to
trips, in the sense that we are not explicitly modeling the
platform allocating trips to specific drivers.  \mccomment{elaborate -- the point is this is a more
general assumption than if we had an explicit centralized allocation of trips to drivers}

\medskip
\noindent
\textbf{Driver Utility.}
Once a platform pricing policy $P$ and a driver strategy-profile $H$
have been specified, market dynamics are a stochastic process without
additional strategic considerations.  Indeed, the meaningful strategic
considerations arise from the platform choosing a pricing protocol
and from the drivers choosing a strategy-profile.

We assume that drivers collectively decide on a trip-allocation vector
$\bfg$, and then an external source of randomness allocates the trips
specified by $\bfg$ to individual drivers.  Since drivers can only serve
trips which originate from their immediate location, this leads to 
a different trip-allocation distribution for each location.
In particular, 
when $\bfS$ is the current supply-location vector, and when $\bfg$
is the feasible trip-allocation vector used by the drivers,
the probability that a driver located at $\ell$ is allocated a dispatch $(r,\delta)\in A^+(\ell)\times\{0,1\}$ is equal to $\frac{g_{(r,\delta)}}{S_{\ell}}$.
Let us write $\bfg(\ell)$ to denote the trip-allocation distribution induced
by the trip-vector $\bfg$ for drivers at each location $\ell$, so that
the previous observation can be expressed as:
\begin{equation}
\label{eq:trip_allocn_distn}
\bbP((r,\delta)\sim\bfg(\ell)) = \frac{g_{(r,\delta)}}{S_\ell},
\end{equation}
where $r\in A^+(\ell)$ is any route originating from the location $\ell$, and
$\delta\in\{0,1\}$ indicates whether or not the trip carries a passenger.

The following definition formalizes the expected 
utility-to-go collected by a driver.
\begin{definition}
Fix a time period $t$, a scenario $\omega_t$, a pricing
protocol $P$, and a driver strategy-profile $H$.  Let 
$\bfS_t$ be any supply-location vector corresponding to the
spatial distribution of drivers at time $t$, and fix
any location $\ell\in\calL$.  The expected utility-to-go
of a driver located at $\ell$ at time $t$, as a function
of the spatial driver supply $\bfS_t$, is defined recursively
as follows:
\begin{equation}
\label{eq:utility_to_go}
    \calV_{(\ell,\omega_t)}(\bfS_t;P,H) = 
    \begin{cases}
    \bbE\left[\delta\rho_r - c_{(r,\omega_t)}\right] &
    \mbox{ if } t=T,\\
    \bbE\left[\delta\rho_r - c_{(r,\omega_t)} + 
    \calV_{(\ell^+(r),\omega_{t+1})}(\bfS_{t+1};P,H)\right] &
    \mbox{ if } t < T.
    \end{cases}
\end{equation}
The meaning of the above expectation, and the randomness
over which it is averaging, are summarized as follows:
\begin{itemize}
    \item The variable $r$ indicates the route the
    driver takes and the variable $\delta$ indicates
    whether or not the trip serves a passenger.
    These variables are sampled from the trip-allocation
    distribution $\bfg(\ell)$ as specified in equation
    (\ref{eq:trip_allocn_distn}).
    \item The trip-allocation vector $\bfg$, on which the
    above trip-allocation distribution depends, is obtained
    from the driver-strategy-profile $H$.  The driver 
    strategy-profile decision depends on the spatial 
    distribution of drivers $\bfS_t$, the volume of demand requesting a dispatch in the current time period over all
    routes $\bfd_t$, the scenario $\omega_t$.  In the
    stochastic two-level model, it also depends on the
    population-size parameter $k$.
    \item The dispatch demand for the current time period
    $\bfd_t$ arises from the price vector $\bfrho_t$ set
    by the platform.  The price $\rho_r$ on each route $r$
    filters the demand $D_r$ to some smaller amount of 
    dispatch demand $d_r$, as specified in equation
    (\ref{eq:d_t_binomial_dist}).
    \item The price vector $\bfrho_t$ is obtained from
    the platform pricing policy $P$.  The platform pricing policy depends on the supply-locations $\bfS_t$, the
    price-inquiry demand $\bfD_t$, the scenario $\omega_t$.
    In the stochastic two-level model, it also depends on
    the population-size parameter $k$.
    \item In the case $t<T$, the scenario $\omega_{t+1}$
    is sampled conditioned on the time $t$ scenario $\omega_t$.
    \item The variable $\bfS_{t+1}$ is the supply-location
    vector specifying the spatial distribution of drivers
    in the next time period.  This depends on the current
    supply-locations $\bfS_t$, and the actions they take
    in the current time period, encoded by the trip-allocation
    vector $\bfg$. In the stochastic two-level model,
    $\bfS_{t+1}$ is a random variable because the number
    of new drivers joining the market at each location
    in the next time period is random.  In the fluid
    model, $\bfS_{t+1}$ is deterministic conditioned on $\bfg$. \mccomment{insert equation ref}.
\end{itemize}
\end{definition}

\medskip
\noindent \textbf{Total System Welfare.}
We conclude the model description section by defining the expected total welfare generated by the marketplace, for a fixed pricing protocol and a fixed driver strategy profile.

First, we define the expected total welfare generated
along a single route in a single time period, as a function of how many drivers take a dispatch-trip
along that route, and how many drivers take a relocation trip.
For a time $t$, a scenario $\omega_t$,
and a route $r$, define the function
$U_{(r,\omega_t)}(\rho_r,g_{1},g_{0})$ by
\begin{equation}
\label{eq:expected_utility_route}
    U_{(r,\omega_t)}(\rho_r,g_{1},g_{0}) = g_{1}\bbE\left[V_{(r,\omega_t)} | V_{(r,\omega_t)}\geq \rho_r\right] - (g_{1} + g_{0})c_r.
\end{equation}
In the above, $\rho_r$ denotes the price for the route $r$, $g_1$ denotes the volume of drivers serving a dispatch trip, and $g_0$ denotes the volume of drivers taking a relocation trip along route $r$.  In addition, $V_{(r,\omega_t)}$ is an $F_{(r,\omega_t)}$-distributed random variable, corresponding to the random utility of a rider who requests a dispatch.

\begin{definition}
Fix a time period $t$, a scenario $\omega_t$, and a supply-location vector $\bfS_t$. The expected total welfare-to-go from this state, generated a platform pricing protocol $P$ and a driver strategy profile $H$,
is defined as follows:
\begin{equation}
    \calW_{\omega_t}(\bfS_t;P,H) = \begin{cases}
    \bbE\left[\sum_{r\in\calR}U_{(r,\omega_t)}(\rho_r,g_{(r,1)},g_{(r,0)})\right] & \mbox{ if } t = T,\\
    \bbE\left[\sum_{r\in\calR}U_{(r,\omega_t)}(\rho_r,g_{(r,1)},g_{(r,0)}) + \calW_{\omega_{t+1}}(\bfS_{t+1};P,H)\right] & \mbox{ if } t < T.
    \end{cases}
\end{equation}
\end{definition}
\mccomment{insert a few sentences describing meaning of above equations some more}


==> opt_central_soln.tex <==
In this section we construct an optimization problem  to obtain the 
welfare-optimal movement of drivers for the stochastic fluid model,
ignoring strategic aspects of the problem and assuming that all drivers can be routed
by a centralized planner.

Our optimization problem bears resemblance to a maximum-value flow problem over 
a ``stochastic'' flow network.  This stochastic flow network captures the
spatiotemporal structure in our problem, corresponding to drivers moving across space and
time, as well as the stochastic structure in our problem, corresponding to the
stochastic sequence of scenarios $\omega_1,\omega_2,\dots,\omega_T$.

\begin{figure}
\includegraphics[width=\textwidth]{figures/stochastic_flow_network}
    \caption{The network over which our optimization problem is defined is a stochastic analogue of a
    standard network flow problem.  The stochasticity inherent to the network structure arises from how we
    incorporate the stochastic scenario tree into the problem structure. Nodes in the stochastic flow network
    correspond to (location, time, scenario) tuples, while arcs correspond to (origin, destination, time, scenario)
    tuples. }
\end{figure}

Formally, our stochastic flow network consists of a set of nodes $\calN$ and 
a set of arcs $\calA$.
The set of nodes $\calN$ is the set of all location-time-scenarios,
\begin{equation}
    \calN\equiv \left\{(\ell,\omega_t) : \ell\in\calL,\omega_t\in\Omega_{1:T}
   \right\}, 
\end{equation}  
and the set of arcs $\calA$ is the set of all origin-destination-time-scenarios,
\begin{equation}
    \calA\equiv \left\{(o,d,\omega_t) : o\in\calL,d\in\calL,\omega_t\in\Omega_{1:T}\right\}.
\end{equation}
Each node $(\ell,\omega_t)\in\calN$ corresponds to a location in the network
at a particular time under a particular scenario.  Each arc $(o,d,\omega_t)\in\calA$
corresponds to a trip originating from the location $o$ under the time-scenario $\omega_t$
towards the destination $d$. Alternatively, each arc $(o,d,\omega_t)$ originates from the
node $(o,\omega_t)$.  When a trip along the arc $(o,d,\omega_t)$ begins, the scenario in future
time periods has yet to be sampled, so the destination node for the arc $(o,d,\omega_t)$ can
possibly be any node $(d,\omega_{t+1})$ where $\omega_{t+1}\in\Omega_{t+1}(\omega_t)$ is a time-$t+1$
scenario in the subtree induced by $\omega_t$.  One way to describe the resulting network
structure is that we have a hypergraph, or more specifically, a hypertree, because
our arcs encode a one-to-many relationship amongst nodes instead of a standard one-to-one relationship.

The decision variables in our optimization problem specify the movement of drivers across space and time, for each 
possible realization of the scenario tree.
We have one collection of decision variables $(f_{(o,d,\omega_t)} : (o,d,\omega_t)\in\calA)$ specifying the total
volume of drivers traversing each arc in the network, i.e., the value $f_{(o,d,\omega_t)}$ specifies the volume
of drivers who are positioned at $o$ and drive towards $d$ under the time-scenario $\omega_t$.
We have another collection of decision variables $(g_{(o,d,\omega_t)} : (o,d,\omega_t)\in\calA)$ specifying the volume
of drivers who traverse each arc with a passenger in their car, i.e. $g_{(o,d,\omega_t)}$ specifies the total volume
of rider dispatches that get served.

We have nonnegativity constraints on the trip-volume variables $f_{(o,d,\omega_t)}$ and the dispatch-volume variables
$g_{(o,d,\omega_t)}$, for every arc $(o,d,\omega_t)\in\calA$. We also have a constraint specifying that the total dispatch-volume
on any route cannot exceed the total driver-volume on that route, i.e. $g_{(o,d,\omega_t)}\leq f_{(o,d,\omega_t)}$.

Finally, we have flow-conservation constraints on the trip-volume variables $f_{(o,d,\omega_t)}$, to ensure that our solution
properly accounts for the amount of supply in the network.
Recall that the variable $\bar{M}_{(\ell,\omega_t)}$ specifies how many drivers enter the market at location $\ell$
under time-scenario $\omega_t$ in the stochastic fluid model.
Our flow conservation constraints ensure that the difference between the number of
drivers leaving each node and the number of drivers entering each node is equal to the number of drivers arriving 
at that node:
\begin{equation}
\label{eq:flow_conservation_static}
\begin{rcases}
    \sum_{d\in\calL} f_{(\ell,d,\omega_t)} =
    \bar{M}_{(\ell,\omega_t)} & \mbox{if }t=1\\
    \sum_{d\in\calL} f_{(\ell,d,\omega_t)} 
    - \displaystyle\sum_{o\in\calL} f_{(o,\ell,\omega_{t-1})} =
    \bar{M}_{(\ell,\omega_t)} & \mbox{if }t > 1
\end{rcases}
\ 
\forall (\ell,\omega_t)\in\calN
\end{equation}

Our objective function corresponds to the total social welfare generated by the marketplace under the
plan specified by our decision variables.  To obtain this social welfare we specify two types of reward
functions: an idiosyncratic disutility function and a non-idiosyncratic disutility function.
The non-idiosyncratic disutility function specifies, for each arc, the rider-side welfare generated by serving dispatches
along that arc, and the fixed cost of driving along that arc.
The idiosyncratic disutility function specifies the idiosyncratic disutility for serving dispatches incurred by drivers
who serve dispatches at each node.

We start by describing the non-idiosyncratic utility function.
For each ODT-scenario $(o,d,\omega_t)$, we define $U_{(o,d,\omega_t)}(f,g)$ to be
the total rider welfare generated when $g$ dispatches are served along the route $(o,d,\omega_t)$, in addition to the
loss in utility corresponding to the fixed cost that drivers pay to traverse the route.

To specify the total rider welfare generated as a function of how many dispatches are served,
we first derive the rider-side price which maximizes welfare along that route.
Recall that $\bar{D}_{(o,d,\omega_t)}$ price-inquiring riders arrive at the ODT-scenario $(o,d,\omega_t)$.
For the sake of notational simplicity we don't explicitly include a constraint that the dispatch-volume $g_{(o,d,\omega_t)}$ cannot
exceed rider demand $\bar{D}_{(o,d,\omega_t)}$; instead, we incorporate rider demand volume into the objective function.
If the dispatch-volume is smaller than the price-inquiry rider-volume, then the price should select for the upper
$\frac{g_{(o,d,\omega_t)}}{\bar{D}_{(o,d,\omega_t)}}$ quantile of potential riders to request a dispatch. 
If the dispatch-volume is larger than the price-inquiry rider-volume, then the price should select for all 
potential riders to request a dispatch.
Thus, the welfare-optimal price as a function of the dispatch-volume $g$ can be written as follows:
\begin{equation}
    \rho_{(o,d,\omega_t)}(g) = \begin{cases}
        F_{(o,d,\omega_t)}^{-1}\left(1-\frac{g}{\bar{D}_{(o,d,\omega_t)}}\right) &
        \mbox{if }g\leq \bar{D}_{(o,d,\omega_t)},\\
        0 & \mbox{otherwise},
    \end{cases} 
\end{equation}
where $F_{(o,d,\omega_t)}$ is the distribution from which riders along the ODT-scenario $(o,d,\omega_t)$ sample
their willingness-to-pay values.
We are now ready to specify the non-idiosyncratic-disutility reward function $U_{(o,d,\omega_t)}(f,g)$:
\begin{equation}
    \label{eq:reward_fn_1}
U_{(r,\omega_t)}(f,g)= \begin{cases}
    \bar{D}_{(o,d,\omega_t)}\bbE\left[V_{(o,d,\omega_t)}\right]  - fc_{(o,d,\omega_t)}& \mbox{if }g > \bar{D}_{(o,d,\omega_t)},\\
    g \bbE\left[V_{(o,d,\omega_t)}\mid V_{(o,d,\omega_t)}\geq
    \rho_{(o,d,\omega_t)}\left(g\right)\right]
 - fc_{(o,d,\omega_t)}
    &
    \mbox{if } g \leq \bar{D}_{(o,d,\omega_t)},
\end{cases}
\end{equation}
where $V_{(o,d,\omega_t)}$ is a rider willingness-to-pay random variable with distribution function $F_{(o,d,\omega_t)}$.
The following Lemma characterizes the derivative of each utility function $U_{(o,d,\omega_t)}(\cdot,\cdot)$:
\begin{lemma}
    \label{lem:reward_fn}
    Consider any ODT-scenario $(r,\omega_t)\in\calA$, let $U_{(r,\omega_t)}(f)$ be the reward function defined in equation (\ref{eq:reward_fn_1}),
    and assume the rider-value distribution $F_{(r,\omega_t)}$ satisfies Assumption \ref{assn:rider_value_dist}.  Then $U_{(r,\omega_t)}(f)$
    is concave in $f$, is differentiable at every $f>0$, and the derivative at each $f>0$ satisfies
    the following equation:
    $$
    \frac{d}{df}U_{(r,\omega_t)}(f) = \begin{cases}
    F_{(r,\omega_t)}^{-1}\left(1-\frac{f}{\bar{D}_{(r,\omega_t)}}\right) - c_{(r,\omega_t)} 
        & \mbox{if } f \leq \bar{D}_{(r,\omega_t)},\\
        -c_{(r,\omega_t)} & \mbox{if } f > \bar{D}_{(r,\omega_t)}.
    \end{cases}
    $$
\end{lemma}
We defer the proof to Appendix \ref{appdx:reward_fn_proof}.

Next, we describe the idiosyncratic-disutility reward function, which specifies the utility lost by the drivers for adding
passengers to their vehicle at each timestep.  Recall we assume that drivers sample a random idiosyncratic disutility for adding
a passenger to their vehicle at each timestep, and that this disutility is sampled independent from other drivers and across time periods.
This disutility is only incurred when a driver serves a dispatch, so the minimum total amount of utility lost depends on the total number
of available drivers to serve that dispatch.  In the context of our model, the total amount of available supply corresponds to the total
number of active drivers positioned at any given node in the network, and the corresponding number of dispatches is the volume of dispatch
requests originating from that node that we serve.

Suppose $S$ is the total volume of supply at any given node, and suppose $g$ is the total amount of dispatch demand originating from that node
that we serve.  The minimum amount of disutility we can incur by serving these $g$ dispatches is to select drivers whose add-passenger disutility falls
in the bottom $\frac{g}{S}$ quantile of the disutility distribution.
Let $A(g,S)$ be the total amount of disutility incurred when these drivers serve a dispatch.
Let $\tilde{C}\sim\mathrm{Uniform}(0,C)$ be a random variable with the same distribution as each driver's idiosyncratic disutility for adding a passenger.
Let $E(X) = \bbP(\tilde{C}\leq X)$ be the distribution function for the $\mathrm{Uniform}(0,C)$ distribution.
Note $E^{-1}(p)=Cp$ for $0\leq p\leq 1$.
The idiosyncratic disutility reward function, $A(g,S)$, can then be expressed as follows:
\begin{align}
    A(g,S) &= g\bbE\left[\tilde{C}\mid \tilde{C} \leq E^{-1}\left(\frac{g}{S}\right)\right]\nonumber\\
    &=g\bbE\left[\tilde{C}\mid \tilde{C} \leq C\frac{g}{S}\right]\nonumber\\
    &= \frac{Cg^2}{2S}.
\end{align}
\begin{lemma}
    \label{lem:disutility_cost_fn}
    \mccomment{lemma characterizing derivative of $A(\cdot,\cdot)$ and showing that it is convex in both variables}
\end{lemma}
We defer the proof to Appendix \ref{appdx:disutility_cost_fn_proof}.

In the context of our optimization problem, we incur idiosyncratic disutility for each node in the network.  
Let $\bfg=(g_{o,d,\omega_t}:o,d,\omega_t\in\calA)$ and $\bff=(f_{o,d,\omega_t} : (o,d,\omega_t)\in\calA)$ be our decision variables,
and consider any node $(\ell,\omega_t)\in\calN$.  We will use the expression $\bfg^T\bfone_{(\ell,\omega_t)}$ to mean the total volume
of dispatches served on routes originating from $(\ell,\omega_t)$, i.e. we define
\begin{equation} 
    \bfg^T\bfone_{(\ell,\omega_t)} = \sum_{(\ell,d,\omega_t)\in A^+(\ell,\omega_t)} g_{(\ell,d,\omega_t)}
\end{equation}
and the expression $\bff^T\bfone_{(\ell,\omega_t)}$ to mean the
total volume of active drivers positioned at the node $(\ell,\omega_t)$, i.e.
\begin{equation}
    \bff^T\bfone_{(\ell,\omega_t)} = \sum_{(\ell,d,\omega_t)\in A^+(\ell,\omega_t)} f_{(\ell,d,\omega_t)}.
\end{equation}

The objective function for our optimization formulation takes the sum of the non-idiosyncratic disutilities over all arcs in the
stochastic flow network, and subtracts the idiosyncratic disutilities over all nodes in the stochastic flow network,
and weights each of these values by the probability of the relevant scenario occurring (i.e. we take an expectation with
respect to the stochastic scenario tree):
\begin{equation}
    \label{eq:static_objective}
    W(\bff,\bfg) = \sum_{t=1}^T\sum_{\omega_t\in\Omega_t}\bbP(\omega_t)\left[
        \sum_{(o,d)\in\calL^2} U_{(o,d,\omega_t)}(f_{(o,d,\omega_t)}, g_{(o,d,\omega_t)}) - 
        \sum_{\ell\in\calL} A\left(\bfg^T\bfone_{(\ell,\omega_t)},\bff^T\bfone_{(\ell,\omega_t)}\right)
        \right].
\end{equation}

Our optimization formulation for the welfare-optimal plan in the stochastic fluid model can now be stated as follows:
\begin{align}
    \label{eq:static_opt_formulation}
    \sup_{\bff, \bfg} &\ \ \   W(\bff,\bfg) & \\
    \mbox{subject to} & \nonumber\\ 
    & f_{(o,d,\omega_t)} \geq 0 \ &\forall (o,d,\omega_t)\in\calA\label{eq:f_nonneg_constraint}\\
    & g_{(o,d,\omega_t)} \geq 0 \ &\forall (o,d,\omega_t)\in\calA \label{eq:g_nonneg_constraint}\\
    & f_{(o,d,\omega_t)} \geq g_{(o,d,\omega_t)} \ &\forall (o,d,\omega_t)\in\calA \label{eq:g_lt_f_constraint}\\
    &\begin{rcases}
        \sum_{d\in\calL} f_{(\ell,d,\omega_t)} =
        \bar{M}_{(\ell,\omega_t)} & \mbox{if }t=1\\
        \sum_{d\in\calL} f_{(\ell,d,\omega_t)} 
        - \sum_{o\in\calL} f_{(o,\ell,\omega_{t-1})} =
        \bar{M}_{(\ell,\omega_t)} & \mbox{if }t > 1
    \end{rcases} \ & \forall (\ell,\omega_t)\in\calN\label{eq:flow_constraint}
\end{align}

When characterizing optimal solutions to the above optimization formulation, we consider an equivalent formulation
where both sides of each of the constraints (\ref{eq:f_nonneg_constraint} - \ref{eq:flow_constraint}) are multiplied
by the scenario-probability $\bbP(\omega_t)$, where $\omega_t$ is the scenario component of the arc or node with which
the constraint is associated.  Multiplying both sides of any constraint by a positive constant does not change the optimal primal solution,
so applying this transformation is without loss of generality.  The benefit of applying this transformation is that it changes the scaling
of the optimal dual variables we get for our problem, and we will see in future sections that the resulting dual variables we get with
this scaling have a clean and simple interpretation, related to the utility drivers collect under the optimal solution.

The following Lemma states the Lagrangian optimality conditions we get for the problem (\ref{eq:static_opt_formulation}) when the constraints
are scaled by the corresponding scenario probabilities:
\begin{lemma}
    \label{lem:optimality_conditions}
    Let $(\bff,\bfg)$ be a feasible solution to the optimization problem (\ref{eq:static_opt_formulation}).
    Then $(\bff,\bfg)$ is an optimal solution if and only if there exist dual variables:
    \begin{itemize}
        \item $\alpha_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA$,
        \item $\beta_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA$,
        \item $\gamma_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA$,
        \item $\eta_{(\ell,\omega_t)}$ for all $(\ell,\omega_t)\in\calN$,
    \end{itemize}
    for which the following conditions are satisfied:
    \begin{enumerate}
        \item Complementary Slackness:
            \begin{align}
            f_{(o,d,\omega_t)}\alpha_{(o,d,\omega_t)} = 0 &\quad \forall (o,d,\omega_t)\in\calA,\\
            g_{(o,d,\omega_t)}\beta_{(o,d,\omega_t)} = 0 &\quad \forall (o,d,\omega_t)\in\calA,\\
            (g_{(o,d,\omega_t)}-f_{(o,d,\omega_t)})\gamma_{(o,d,\omega_t)} = 0 &\quad \forall (o,d,\omega_t)\in\calA.
            \end{align}
        \item Stationarity.  For all $(o,d,\omega_t)\in\calA$, the following equations hold:
            \begin{align}
                \rho_{(o,d,\omega_t)}(g_{(o,d,\omega_t)}) -C\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}} &=
                        \gamma_{(o,d,\omega_t)} - \beta_{(o,d,\omega_t)} .\label{eq:stationarity_g}\\
            -c_{(o,d,\omega_t)}  +\frac{C}{2}\left(\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}}\right)^2 &=
                \eta_{(o,\omega_t)} - \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right] - \alpha_{(o,d,\omega_t)} - \gamma_{(o,d,\omega_t)}\label{eq:stationarity_f} .
            \end{align}
    \end{enumerate}
\end{lemma}

We prove Lemma \ref{lem:optimality_conditions} in Appendix \ref{appdx:optimality_conditions_proof}.


==> opt_ic_fluid_model.tex <==
In this section we show that the welfare-optimal plan for the stochastic fluid model is incentive-compatible
under a natural mechanism which derives prices from the computed optimum.
This mechanism, which we refer to as the static pricing mechanism, computes an solution to the welfare-optimal
concave program (\ref{eq:static_opt_formulation}) at the beginning of time, and uses the computed optimum to
set prices at each subsequent time period.

\begin{definition}
    \label{def:static_mechanism}
    Given an instance of the stochastic fluid model, the static pricing mechanism computes
    a solution $(\bff, \bfg)$ to the welfare-optimal concave program (\ref{eq:static_opt_formulation}),
    prior to the beginning of the marketplace dynamics.  At each time period $t=1,2,\dots,T$,
    under any scenario $\omega_t\in\Omega_t$, the static pricing mechanism uses the computed optimum
    to set the price $P_{(o,d,\omega_t)}$ on each route $(o,d,\omega_t)$ as follows:
    \begin{equation}
        \label{eq:static_prices}
        P_{(o,d,\omega_t)} = F_{(o,d,\omega_t)}^{-1}\left(1-\frac{g_{(o,d,\omega_t)}}{\bar{D}_{(o,d,\omega_t)}}\right),
    \end{equation}
    where $F_{(o,d,\omega_t)}(\cdot)$ is the distribution function from which price-inquiring riders for route $(o,d,\omega_t)$
    sample their willingness-to-pay values, and $\bar{D}_{(o,d,\omega_t)}$ is the total volume of price-inquiring riders
    for route $(o,d,\omega_t)$.
\end{definition}

We view the static pricing mechanism as a steppingstone to the ultimate mechanism we propose.  We start by showing a positive
result: the welfare-optimal plan for the stochastic fluid model is incentive-compatible under the static pricing mechanism.
This incentive-compatibility holds even in the presence of the top-level stochastic scenario tree, and the analysis showing incentive-compatibility
will be an important component of our analysis for the ultimate mechanism we propose.  However, we will also show that the
static pricing mechanism is prone to severe problems: the equilibria arising under the static mechanism are not unique, and in fact many
equilibria with bad social welfare will frequently occur; further, when we try to use the static pricing mechanism in the stochastic two-level model,
small discrepancies between expected rider demand and realized rider demand will break incentive-compatibility entirely.

We proceed by showing incentive-compatibility of the welfare-optimal solution under the static prices.  Our first step is to introduce
some notation to describe the utility drivers collect.  Consider a driver who travers some route $(o,d,\omega_t)\in\calA$, 
and let $\delta\in\{0,1\}$ be an indicator variable specifying whether or not this driver is carrying a passenger.  Let $\calQ(o,d,\omega_t,\delta)$
be the expected utility-to-go, associated with this action, that the driver collects over all remaining time periods, assuming the drivers act
according to the welfare-optimal solution, and assuming the static pricing mechanism is used to set prices.
For any location, time-scenario pair $(\ell,\omega_t)\in\calN$, let $\calV(\ell,\omega_t)$ be the expected utility-to-go of a driver
positioned at $\ell$ at time-scenario $\omega_t$, again assuming drivers act according to the welfare-optimal solution, and assuming the static
mechanism is used to set prices.

The arc-associated and the node-associated utility-to-go values are defined by the following recursive equations:
\begin{align}
    \calQ(o,d,\omega_t,1) &= \begin{cases}
        P_{(o,d,\omega_t)} - \frac{C}{2}\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}} 
        - c_{(o,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\calV(d,\omega_{t+1})\mid\omega_t\right] & \mbox{if }t< T,\\
        P_{(o,d,\omega_t)} - \frac{C}{2}\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}} 
        - c_{(o,d,\omega_t)}& \mbox{if }t= T,\\
    \end{cases}\label{eq:Q_def_delta_1}\\
    \calQ(o,d,\omega_t,0) &= \begin{cases}
        - c_{(o,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\calV(d,\omega_{t+1})\mid\omega_t\right] & \mbox{if }t< T,\\
        - c_{(o,d,\omega_t)}& \mbox{if }t< T,
    \end{cases}\label{eq:Q_def_delta_0}\\
    \calV(\ell,\omega_t) & = \sum_{d\in\calL}\left[\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\calQ(\ell,d,\omega_t,1)
                                                                    + \frac{(f_{(\ell,d,\omega_t)} - g_{(\ell,d,\omega_t)})}{\bff^T\bfone_{(\ell,\omega_t)}}
                                                                    \calQ(\ell,d,\omega_t,0)\right].\label{eq:V_def}
\end{align}
In the equation (\ref{eq:Q_def_delta_1}), recall that $\frac{C}{2}\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}}$ is the average 
add-passenger disutility incurred by a driver positioned at $(o,\omega_t)$ who serves a dispatch.
In the equation (\ref{eq:V_def}), note that $\frac{g_{(\ell,d,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}$ is the probability a driver positioned at $(\ell,\omega_t)$
serves a dispatch trip towards destination $d$, and $\frac{(f_{(\ell,d,\omega_t)} - g_{(\ell,d,\omega_t)})}{\bff^T\bfone_{(\ell,\omega_t)}}$ is the probability that
a driver positioned at $(\ell,\omega_t)$ serves an empty relocation trip towards destination $d$; that is, $\calV(\ell,\omega_t)$ is defined as an expected
value of arc-specific utility-to-go values $\calQ(\ell,d,\omega_t,\delta)$, where the expectation is taken with respect to the distribution of trips allocated to
driverse at $(\ell,\omega_t)$ under the welfare-optimal solution.

\mccomment{maybe use the following notation: $$ \bbE[C^{ID}_{(\ell,\omega_t)}] = \frac{C}{2}\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}} $$
or some other similar notation to make referring to "idiosyncratic disutility" easier.}

Next, we state a Lemma showing a correspondence between the location-specific utility-to-go values $\calV(\ell,\omega_t)$, and the dual variables associated with
the flow-conservation constraints at each node.
\begin{lemma}
    \label{lem:dual_variable_utility}
    Let $(\bff,\bfg)$ be an optimal solution for the welfare-optimal concave program (\ref{eq:static_opt_formulation}),
    and let $\alpha_{(o,d,\omega_t)}$, $\beta_{(o,d,\omega_t)}$, $\gamma_{(o,d,\omega_t)}$, for all $(o,d,\omega_t)\in\calA$, 
    and $\eta_{(\ell,\omega_t)}$ for all $(\ell,\omega_t)\in\calN$, be dual variables certifying the optimality of $(\bff,\bfg)$ as
    specified in Lemma \ref{lem:optimality_conditions}.  Let $\calV(\ell,\omega_t)$ be the node-associated utility-to-go values for the
    welfare-optimal solution under the static pricing mechanism.  Then
    \begin{equation}
        \calV(\ell,\omega_t) = \eta_{(\ell,\omega_t)}
    \end{equation}
    holds for all nodes $(\ell,\omega_t)\in\calN$.
\end{lemma}
We prove Lemma \ref{lem:dual_variable_utility} in Section \ref{sec:dual_utility_proof}.

Next, we show that the welfare-optimal solution is incentive-compatible under the static pricing mechanism.
First, let us state what it means for the welfare-optimal solution to be incentive-compatible. 

We will show that, under the static pricing mechanism, the welfare-optimal solution constitutes what we refer to as
a static equilibrium.  Informally, a static equilibrium is a strategy-profile in which drivers have no incentive to
deviate at each time period, assuming that no drivers have deviated in earlier time periods. This notion of equilibrium
is in contrast to a subgame-perfect equilibrium, in which drivers have no incentive to deviate from any state of the marketplace.
We will introduce subgame-perfect equilibria in future sections; for now, our focus is on static equilibria. 

We adopt the convention that a feasible solution $(\bff,\bfg)$ for the welfare-optimal concave program (\ref{eq:static_optimization})
specifies a driver strategy-profile. We assume that trips are allocated uniformly at random to individual drivers.
Note this convention only makes sense that drivers never deviate; if some drivers deviate in earlier time periods, then the spatial distribution
of drivers at later time periods will be incompatible with the flow-conservation constraints at future time periods.  However,
since our notion of static equilibrium in this section requires the assumption that drivers never deviate in early time periods,
this assumption suffices for our present purposes.  \mccomment{Should probably move this discussion of ``static strategy-profile'' up to before
I define $\calQ$ and $\calV$}

Before stating our formal definition of a static equilibrium, we need to introduce one more piece of notation which explicitly includes the idiosyncratic
add-passenger disutility incurred by individual drivers.   The notation $\calQ(o,d,\omega_t,1)$ for the average utility-to-go of a driver who takes a dispatch
trip on the arc $(o,d,\omega_t)$ subtracts off the average idiosyncratic add-passenger disutility.  However, each individual driver collects utility based on their
sampled add-passenger disutility value. Let $C^{ID}$ represent the sampled add-passenger disutility for an individual driver, and let
$\calQ(o,d,\omega_t,\delta,C^{ID})$ denote the utility-to-go of a driver who takes a trip specified by $(o,d,\omega_t,\delta)$ and where $C^{ID}$ is the
add-passenger disutility.  This \emph{idiosyncratic} trip-specific utility-to-go can be specified in terms of the aggregate utility-to-go values as follows:
\begin{align}
    \calQ(o,d,\omega_t,1,C^{ID}) &= \calQ(o,d,\omega_t,1) - (C^{ID} - \bbE\left[\tilde{C}|\delta=1\right]),\label{eq:idiosyncratic_dispatch_utility}\\
    \calQ(o,d,\omega_t,0,C^{ID}) &= \calQ(o,d,\omega_t,0)\label{eq:idiosyncratic_relocation_utility}.
\end{align}
\mccomment{These idiosyncratic dispatch utitility-to-go values are probably what I want to define in the first place -- no need to define the average utility-to-go
values in their place.}
Equation (\ref{eq:idiosyncratic_dispatch_utility}) states the idiosyncratic dispatch utility where we subtract of the difference between the idiosyncratic add-passenger
disutility $C^{ID}$ and the average add-passenger disutility over all drivers who serve a dispatch.  Equation (\ref{eq:idiosyncratic_relocation_utility}) states that 
the idiosyncratic utility for a relocation-trip $(o,d,\omega_t,0)$ does not depend on sampled disutility value $C^{ID}$, since drivers who take a relocation trip
don't add a passenger to their car.

In addition, we use the notation $\calZ(\ell,\omega_t)$ to be the set of trips originating from any node $(\ell,\omega_t)$ to which a driver can
deviate.  The set $\calZ(\ell,\omega_t)$ includes all relocation-trips originating from $(\ell,\omega_t)$, as well as any dispatch trips with excess capacity:
\begin{equation}
    \label{eq:feasible_deviations}
    \calZ(\ell,\omega_t) = \left\{(\ell,d,\omega_t,0) : d\in\calL\right\} \cup \left\{(\ell,d,\omega_t,1) : d\in\calL, g_{(\ell,d,\omega_t)}<\bar{d}_{(\ell,d,\omega_t)}\right\},
\end{equation}
where $g_{(\ell,d,\omega_t)}$ is how many dispatch-trips are served along the route $(\ell,d,\omega_t)$ in the strategy-profile under consideration,
and $\bar{d}_{(\ell,d,\omega_t)}$ is the volume of rider-demand for dispatch trips along the route $(\ell,d,\omega_t)$ for the pricing mechanism under consideration.

Definition \ref{def:static_equilibrium} states our formal definition for a strategy-profile to be a static equilibrium. 
\begin{definition}
    \label{def:static_equilibrium}
    Let $(\bff,\bfg)$ be a static strategy-profile for the stochastic fluid model, and let $\bfP=(P_{(o,d,\omega_t)})$ be any
    static pricing mechanism.  Let $\calQ(o,d,\omega_t,\delta,C^{ID})$ be the 
    idiosyncratic trip-specific utility-to-go values associated with each trip-type, and let $\calV(\ell,\omega_t)$ be the node-specific utility-to-go values
    associated with each location-time-scenario.

    Consider any location $\ell\in\calL$ and any time-scenario $\omega_t$.  Let $\calZ(\ell,\omega_t)$ be the set of trips originating from
    $(\ell,\omega_t)$ to which a driver can deviate. Consider a driver positioned at $\ell$ under the time-scenario $\omega_t$, and assume they
    sample add-passenger disutility $C^{ID}$ and under the strategy-profile $(\bff,\bfg)$ they are allocated a trip-type $(\ell,d,\omega_t,\delta)$.
    We say $(\bff,\bfg)$ is a static equilibrium with respect to $\bfP$ if the following inequality always holds, assuming the drivers have not deviated
    at any earlier time period:
    \begin{equation}
        \label{eq:static_eqlbm_condition}
        \calQ(\ell,d,\omega_t,\delta,C^{ID}) \geq \max_{(\ell,d',\omega_t,\delta')\in\calZ(\ell,\omega_t)}\calQ(\ell,d',\omega_t,\delta',C^{ID}).
    \end{equation}
\end{definition}
Note that this notion of equilibrium
considers deviations of individual drivers, and in the context of the stochastic fluid model, individual drivers are infinitesimal agents.  Thus, when considering the
utility an agent collects for deviating, we assume the spatial distribution of drivers at future time periods is the same as if the driver had not deviated in the
first place.  This lets us (implicitly) use the same node-specific utility-to-go values $\calV(d,\omega_{t+1})$ on both sides of the 
static-equilibrium condition (\ref{eq:static_eqlbm_condition}). That is, we assume a drivers deviation at time-scenario $\omega_t$ affects the utility they collect in the
current time period, and the utility they collect at future time periods changes because their destination location changes, but the deviation of an individual infinitesimal
driver does not change the aggregate utility-to-go values.


Theorem \ref{thm:static_eqlbm} states our main result for this section, which is that the welfare-optimal solution constitutes a static equilibrium
under the static pricing mechanism (\ref{eq:static_prices}).
\begin{theorem}
    \label{thm:static_eqlbm}
    Let $(\bff,\bfg)$ be an optimal solution for the welfare-optimal concave program (\ref{eq:static_optimization}), and let $\bfP$ encode the prices
    used by the static pricing mechanism (\ref{eq:static_prices}).  Then the static equilibrium condition (\ref{eq:static_eqlbm_condition}) always holds,
    i.e. $(\bff,\bfg)$ is a static equilibrium under the static pricing mechanism $\bfP$.
\end{theorem}
Theorem \ref{thm:static_eqlbm} follows from the characterization of the utility-to-go-values $\calV(\ell,\omega_t)$ in terms of the flow-conservation dual variables
$\eta_{(\ell,\omega_t)}$ established in Lemma \ref{lem:dual_variable_utility}, as well as the optimality conditions described in Lemma \ref{lem:optimality_conditions}.
We defer the proof details to Section \ref{sec:static_eqlbm_proof}.




\subsection{Proof of Theorem \ref{thm:static_eqlbm}}
\label{sec:static_eqlbm_proof}
\input{static_eqlbm_proof.tex}

\subsection{Proof of Lemma \ref{lem:dual_variable_utility}}
\label{sec:dual_utility_proof}
\input{dual_variable_utility_proof.tex}

%\subsection{Section Contents Prior to July 29}
%\input{opt_ic_fluid_model_before_july29.tex}


==> opt_ic_fluid_model_before_july29.tex <==
In this section we provide two mechanisms for operating the market in the stochastic fluid model.
Each of these mechanisms sets prices and makes matches by using an optimal solution to one of the optimization problems formulated
in the previous section. Our main results for this section are incentive-compatibility and robustness results for the two
mechanisms we study.

\subsection{Definitions of Static and Dynamic Mechanisms}

The first mechanism, which we refer to as the static mechanism, computes an optimal solution
to the static optimization problem (\ref{eq:static_optimization}) before the market dynamics begin, and it uses this
solution to set prices and make matches throughout all time periods.  The second mechanism, which we refer to as the
dynamic mechanism, re-solves the dynamic optimization problem (\ref{eq:dynamic_optimization}) with respect to
the realized market-state at each time period, and the recomputed optimum is used to set prices and make matches.

Recall a mechanism is specified by a pricing protocol $P$ and a matching function $H$.  The pricing protocol $P$ is called
at the beginning of each time period to produce prices for each route.  The matching function $H$ specifies a vector
of trip-allocations that is used in the trip-allocation process in each time period.  A trip-allocation vector 
$\bfg=(g_r:r\in\calR)$ specifies the number of drivers $g_r$ that the platform wants to allocate to each route $r$.
In order for the trip-allocation vector to be feasible it must satisfy action-allocation constraints with respect
to the realized spatial distribution of drivers.
For a supply-location vector $\bfS=(S_\ell:\ell\in\calL)$ encoding the number of available drivers $S_\ell$ at each
location $\ell$, let $G(\bfS)$ be the set of feasible trip-allocation vectors with respect to $\bfS$.  $G(\bfS)$ is
defined as follows:
\begin{equation}
    G(\bfS) \equiv \left\{\bfg\in\bbR^\calR_+ : \forall \ell \sum_{r\in A^+(\ell)} g_r = S_\ell\right\}.
\end{equation}
\mccomment{elaborate on how the matching part of the mechanism from the platform's perspective
can be stated without the $0/1$ rider-trip distinction. }

We are now ready to define the two mechanisms.


\begin{definition} (Static Mechanism)
    \label{def:fluid_mechanisms_static}  Let $\bff^{*S}=(f^{*S}_{(r,\omega_t)}:(r,\omega_t)\in\calA)$ 
    be an optimal solution for the static optimization problem (\ref{eq:static_optimization}).
    The static mechanism $(P^S, H^S)$ consists of the following components:
    \begin{itemize}
        \item The static pricing policy $P^S:\Omega_{1:T}\to\bbR^\calR_+$ is defined by
    \begin{equation}
        P^S(\omega_t) = (\rho_{(r,\omega_t)}(f^{*S}_{(r,\omega_t)}) : r\in\calR).
    \end{equation}
    \item The static matching policy $H^S:\Omega_{1:T}\times\bbR^\calL_+\to\bbR^{\calR}_+$ is defined by
    \begin{equation}
        H^S(\omega_t, \bfS) = \mathrm{Projection}_{G(\bfS)}(f^{*S}_{(r,\omega_t)}:r\in\calR)
    \end{equation}
    \end{itemize}
   
\end{definition}

\begin{definition} (Dynamic Mechanism)
\label{def:fluid_mechanisms_dynamic}
For any time-scenario $\omega_t$ and any supply-location vector $\bfS$, let 
$\bff^{*D}(\omega_t,\bfS)=\left(f_{(r,\omega_\tau)}^{*D}(\omega_t,\bfS) : (r,\omega_\tau)\in\calA_{\omega_t}^{\geq t}\right)$
be an optimal solution for the dynamic optimization problem (\ref{eq:dynamic_optimization}) with respect
to $\omega_t$ and $\bfS$.
The dynamic mechanism $(P^D, H^D)$ consists of the following components:
\begin{itemize}
    \item The dynamic pricing policy $P^D:\Omega_{1:T}\times\bbR_+^\calL\to\bbR^\calR_+$ is defined by
    \begin{equation}
        P^D(\omega_t,\bfS) = (\rho_{(r,\omega_t)}\left(f^{*D}_{(r,\omega_t)}(\omega_t,\bfS)\right) : r\in\calR).
    \end{equation}
    \item The dynamic matching policy $H^D:\Omega_{1:T}\times\bbR_+^\calL\to\bbR^\calR_+$ is defined by
    \begin{equation}
        H^D(\omega_t,\bfS) = \left(f^{*D}_{(r,\omega_t)}(\omega_t,\bfS): r\in\calR\right).
    \end{equation}
\end{itemize}
\end{definition}

\subsection{Trip-Allocation Process and Notions of Incentive-Compatibility}

Let us now formalize the notions of incentive-compatibility and equilibrium that we will use in the forthcoming results.
Let $(P,H)$ denote an arbitrary pricing and matching mechanism and let $\Pi$ denote an arbitrary driver-strategy profile, encoding
the (strategic) actions taken by the drivers. 
Recall\mccomment{write about this in the model desc. and insert ref} 
we use an abstract trip-allocation process to model the outcome arising from platform matching suggestions and 
strategic driver behaviour. We use $\bfg\sim\tripalloc(\omega_t,\bfS,\Pi,H,P)$ to denote the outcome of the trip-allocation process.
\mccomment{$\tripalloc(\dots)$ should depend on $\bfd$.}

The outcome $\bfg=(g_{(r,\delta)} : (r,\delta)\in\calR\times\{0,1\})$ is a vector indexed by pairs of routes $r$ and 
passenger-indicators $\delta$, such that the component $g_{(r,\delta)}$ indicates the realized number of drivers who
take a trip of type $(r,\delta)$. \mccomment{Note that, for an arbitrary strategy profile $\Pi$, $\bfg$ is a random variable because
we assume an external source of randomness allocates the platform-suggested matches from $H$ to drivers, but under an arbitrary
strategy $\Pi$ not all drivers will make the same accept/reject decisions for their allocated action, potentially leading to 
different aggregate trip-count vectors $\bfg$ based on the initial random allocation of trips to drivers.}

We assume that a driver is always free to reject a trip and switch to another more desirable trip, and this 
reject-and-switch behaviour is encoded by the strategy-profile $\Pi$.
The trip-allocation vector $\bfg\sim\tripalloc(\omega_t,\bfS,\Pi,H,P)$
arising from the trip-allocation process specifies trip counts 
after all the drivers are satisfied with their allocated trip under the strategy $\Pi$.

When a driver considers switching to a more desirable trip, we assume they can
switch to any relocation  trip (i.e. non-dispatch trip) originating from their location, or they can 
switch to any dispatch trip originating from their location which has excess capacity under the realized trip-allocations.
A dispatch trip $(r,1)$ has excess capacity if the amount of dispatch demand arising under the pricing protocol $P$
exceeds the number of drivers serving a dispatch along $r$. For a location $\ell$, a trip-allocation realization $\bfg$,
and a vector $\bfd=(d_r:r\in\calR)$ encoding dispatch demand on each route, the set of trips that a driver can consider deviating
to is defined as follows:
\begin{equation}
    A'(\ell;\bfg,\bfd)\equiv\left\{(r,0) : r\in A^+(\ell)\right\}\cup\left\{(r,1) : r\in A^+(\ell), g_{(r,1)} < d_r\right\}.
\end{equation}

Thus, for a realized trip-allocation vector $\bfg$, the maximum utility a driver located at $\ell$ can obtain by deviating
is the maximum utility over all possible deviations.
\begin{equation}
    D_{(\ell,\omega_t)}(g;\Pi,H,P) \equiv 
    \max_{(r,\delta)\in A'(\ell;\bfg,\bfd)} \delta\rho_{r} - c_{(r,\omega_t)} + \bbE\left[
    \calV_{(\ell^+(r),\omega_{t+1})}(\bfS_{\omega_{t+1}};\Pi,H,P)   
    \right].
\end{equation}
\mccomment{change wording here}
We say that $\Pi$ is incentive-compatible with respect to $H$ and $P$, location $\ell$ if every trip in the support of
$\bfg$ produces utility at least as large as the deviation utility, i.e. if the following inequality holds:
\begin{equation}
\label{eq:ic_condition}
D_{(\ell,\omega_t)}(\bfg;\Pi,H,P) \leq \min_{\substack{(r,\delta)\in A^+(\ell)\times\{0,1\}, \\ g_{(r,\delta)} > 0}}
\delta\rho_r - c_r + 
\bbE\left[\calV_{(\ell^+(r),\omega_{t+1})}(\bfS_{\omega_{t+1}};\Pi,H,P)\right]. 
\end{equation}

The definitions of static equilibrium and subgame-perfect equilibrium are stated below.

\begin{definition}(Static Equilibrium and Subgame-Perfect Equilibrium)
Fix a driver strategy profile $\Pi$ and a mechanism $(P,H)$.  Let $\omega_t$ be any time-scenario
and let $\bfS$ be any supply-location vector.
\begin{itemize}
    \item We say $\Pi$ is a static equilibrium with respect to $(P,H)$ if every possible trip-allocation vector 
    $\bfg$ in the support of $\tripalloc(\omega_t,\bfS,\Pi,H,P)$ is incentive-compatible, assuming $\bfS$ is the 
    supply-location vector arising at time-scenario $\omega_t$ when all drivers followed the trips suggested by $H$ in
    all previous time periods. \mccomment{needs wordsmithing}
    \item  We say $\Pi$ is a static equilibrium with respect to $(P,H)$ if every possible trip-allocation vector 
    $\bfg$ in the support of $\tripalloc(\omega_t,\bfS,\Pi,H,P)$ is incentive-compatible for any supply-location vector $\bfS$.
\end{itemize}
\end{definition}

\subsection{Incentive-Compatibility Results}

Finally, we introduce the following definition of an always-follow driver strategy profile. An always-follow
driver strategy profile is any strategy profile where drivers always follow the initial trip allocated to them
in the trip allocation process.

\begin{definition}
    An always-follow driver strategy profile is any strategy profile $\Pi$ where drivers always accept
    their first allocated trip.  Under the always-follow driver strategy-profile, note that
    the resulting trip-allocation vector will be the same as the trip-allocation vector produced
    by the platforms matching process: $\tripalloc(\omega_t,\Pi,H,\bfd)=H(\omega_t,\bfd)$
\end{definition}

Our first result in this section states that the always-follow strategy profile is incentive-compatible
under both the static mechanism and the dynamic mechanism.


\begin{theorem} (Incentive compatibility in the stochastic fluid model)
    \label{thm:fluid_ic}
    Under Assumption \ref{assn:rider_value_dist} the following statements are true in the stochastic fluid model:
    \begin{enumerate}
        \item The always-follow driver strategy profile is a static equilibrium with respect to the 
            static mechanism.  
        Moreover, assuming drivers have been using the always-follow policy at all previous time periods,
            the utility-to-go of a driver from any LT-scenario is equal to the corresponding optimal dual variable
            from the static formulation: $\calV_{(\ell,\omega_t)}(\bfS_{\omega_t}^S;H^S,P^S)=\eta^S_{(\ell,\omega_t)}$.

        \item The always-follow driver strategy profile is a subgame-perfect equilibrium with respect to the
            dynamic mechanism.
        
        Moreover, the utility-to-go for a driver under the always-follow strategy profile
            is equal to the corresponding optimal dual variable from the
            dynamic optimization formulation, from any market state.
    \end{enumerate}
\end{theorem}

Our next result for this section is the following robustness theorem, which states
that every subgame perfect equilibrium for the dynamic mechanism is welfare-maximizing.
For this result, we make the following assumption that drivers are incentivized to prefer
trips with passengers to trips without passengers, assuming the utility-to-go of the two
trips are otherwise equal.
\begin{assumption}
Drivers are incentivized to prefer trips with passengers than trips without passengers, assuming the
utility-to-go of the two trips are otherwise equal.
\end{assumption}

\begin{theorem} (Welfare-Robustness in the stochastic fluid model)
    \label{thm:robust_fluid_welfare}
    Let $\Pi$ be any driver strategy profile that is a subgame-perfect equilibrium with respect
    to the dynamic mechanism.
    Then $\Pi$ is welfare-maximizing, and the utility-to-go of a driver is equal to the corresponding 
    corresponding dual variable from the dynamic formulation.
\end{theorem}

We defer proofs to Appendix \ref{sec:fluid_ic_proofs}.


\section{Incentive-Compatibility in Fluid Model Section from Workshop Submission}
This section focuses on the stochastic fluid model, which includes stochasticity due to large-scale randomness (weather, events) that correlates behavior of many riders and drivers, but not randomness due to individual idiosyncratic rider and driver behavior.
Using this model, we develop two variants of a natural pricing and matching mechanism based on computing an optimal solution to the stochastic maximum flow problem defined in the previous section.

The first variant, which we refer to as the static mechanism, computes an optimal stochastic flow
at time $0$ and uses the solution of this computation to set prices and make matches throughout all
time periods. While this static mechanism does not adapt to the realized location of drivers, it does
adapt to the top-level state of the world vis-a-vis the stochastic scenario $\omega_t$.

The second variant, which we refer to as the dynamic mechanism, re-computes an optimal stochastic flow
at each time period, solving the stochastic maximum flow problem formulated with respect to the observed
scenario $\omega_t$ and the observed supply-location vector $\bfS_t$.

The first results of this section  then show that, in the stochastic fluid model, both mechanisms are incentive compatible (Theorem~\ref{thm:fluid_ic}) \pfedit{and produce welfare-optimal matches (Theorem~\ref{thm:robust_fluid_welfare})} of drivers to riders and empty relocation for unmatched drivers. \pfdelete{Thus, these mechanisms achieve welfare optimality in the stochastic fluid model.}

\pfedit{In the next section, focusing on the stochastic two-level model (where rider and driver idiosyncratic behavior is also random), we show that welfare-optimality continues to hold asymptotically for {\it all} approximate equilibria under the dynamic mechanism (Theorem \ref{thm:stochastic_ic}).}
\pfedit{This claim, however, does not hold for the static mechanism. Section \ref{sec:example} shows a sequence of approximate equilibria under the static mechanism that result in a large welfare loss.}  

\pfdelete{The difference between the dynamic and static mechanism is that in the dynamic version all equilibria are welfare maximizing in the stochastic fluid model (Theorem \ref{thm:robust_fluid_welfare}) and approximately welfare maximizing in the two-level model (Theorem \ref{thm:stochastic_ic}).}

\pfdelete{We will elaborate on \etedit{the importance of the} difference \etedit{between the two mechanisms via a simple example} in Section \ref{sec:example}.
}

We now proceed, describing how our mechanisms obtain prices and matching decisions from an optimal stochastic flow.
Following our discussion about welfare-maximizing prices along a specific route from the previous section,
to maximize welfare along a route $(r,\omega_t)$ with $f^*_{(r,\omega_t)}$ driver-volume taking the trip,
we must charge a price $\rho_{(r,\omega_t)}$ which selects for the upper $\min\left(\frac{f^*_{(r,\omega_t)}}{\bar{D}_{(r,\omega_t)}}, 1\right)$
quantile of price-inquiry rider demand for that route.  The price which selects for riders from this quantile
is given by the inverse of the rider-value distribution function as follows:
\begin{equation}
    \label{eq:max_welfare_price}
    \rho_{(r,\omega_t)} = F_{(r,\omega_t)}^{-1}\left(\max\left(1-\frac{f^*_{(r,\omega_t)}}{\bar{D}_{(r,\omega_t)}}, 0\right)\right).
\end{equation}
The amount of dispatch-request rider demand which arises under the above price is equal to 
\begin{equation}
    \bar{d}_{(r,\omega_t)} = \bar{D}_{(r,\omega_t)} \min\left(1,\frac{f^*_{(r,\omega_t)}}{\bar{D}_{(r,\omega_t)}}\right).
\end{equation}
Recall that the platforms matching decisions are specified by a matching vector 
$\bfg=(g_{(r,\omega_t,\delta)} : (r,\omega_t)\in\calA_{\omega_t}^t,\delta\in\{0,1\})$, indexed by trip-suggestion types $(r,\omega_t,\delta)$
such that $(r,\omega_t)\in\calA_{\omega_t}^t$ correspond to an active route and $\delta\in\{0,1\}$ is an indicator variable specifying whether
the trip fulfils a dispatch ($\delta=1$) or not ($\delta=0$).
The platform produces a matching vector $\bfg$ from an optimal stochastic flow by first producing dispatch-trip-allocation
counts equal to the amount of dispatch-request demand for the route as specified above, and any remaining flow is included 
in the relocation-trip-allocation count for that route.  In symbols, for each active route $(r,\omega_t)\in\calA_{\omega_t}^t$
the dispatch trip-allocation counts $g_{(r,\omega_t,1)}$ and the relocation trip-allocation counts $g_{(r,\omega_t,0)}$ of the matching vector $\bfg$ 
produced by the platform are defined as follows:
\begin{equation}
    \label{eq:trip_allocation_counts}
    g_{(r,\omega_t,1)} = \bar{d}_{(r,\omega_t)}, \ \ \ \ \ \ \ g_{(r,\omega_t,0)} = f^*_{(r,\omega_t)} - \bar{d}_{(r,\omega_t)}.
\end{equation}

Recall that, for a matching vector $\bfg$ to be well-specified, it must satisfy the action-allocation constraints 
(\ref{eq:action_allocation_constraint}) with respect to the supply-availability $S_{(l,\omega_t)}$ at each active location $(l,\omega_t)$.
For the dynamic mechanism, which recomputes an optimal solution in each time period, incorporating the observed supply-location vector
$\bfS_t$, these action-allocation constraints are satisfied because the corresponding optimal stochastic flow satisfies the flow-conservatino
conditions (\ref{eq:flow_conservation_dynamic}) with respect to $\bfS_t$.
For the static mechanism, which computes an optimal stochastic flow only once at the beginning of time, the trip-allocation counts
defined above may fail to satisfy the action-allocation constraints (\ref{eq:action_allocation_constraint}) if some drivers
deviated from their allocated trip-suggestion at an earlier time period.  In the event that some drivers deviate from their trip-allocations, 
we will leave the matching vector produced by the static mechanism unspecified for all future time periods. Our incentive-compatibility result
for the static mechanism will hold assuming that no drivers have deviated at an earlier time period.

We now formally define our two mechanisms for the stochastic fluid model.
\begin{definition} (Static Mechanism)
    \label{def:fluid_mechanisms_static}  The static mechanism for the stochastic fluid model computes an optimal stochastic flow $\bff^*_0$
    for the time $0$ formulation of the stochastic maximum flow problem (\ref{eq:dynamic_optimization}) and holds this solution fixed across
    all time periods.  At each time $t$ and each scenario $\omega_t$, for each active route $(r,\omega_t)\in\calA_{\omega_t}^t$ the static mechanism 
    produces a trip-price $\rho_{(r,\omega_t)}$ obtained from equation (\ref{eq:max_welfare_price}) computed with respect to $\bff^*_0$.  
    The static mechanism uses equation (\ref{eq:trip_allocation_counts}), computed with respect to $\bff^*$, to produce a matching vector $\bfg$.
    If the matching vector $\bfg$ produced by the static mechanism is infeasible\footnote{The matching 
            vector $\bfg$ is infeasible if it violates the action-allocation 
            constraint (\ref{eq:action_allocation_constraint}) for every active LT-scenario $(l,\omega_t)\in\calN_{\omega_t}^t$.}
            with respect to the spatial distribution of supply at time $t$ then an arbitrary matching vector is used instead.
\end{definition}

\begin{definition} (Dynamic Mechanism)
\label{def:fluid_mechanisms_dynamic}
    The dynamic mechanism for the stochastic fluid model re-computes in each time period $t$ an optimal stochastic flow $\bff^*_t$ 
    for the formulation of the stochastic maximum flow problem (\ref{eq:dynamic_optimization}) which incorporates the time $t$, the scenario $\omega_t$,
    and the supply-location vector $\bfS_t$.  The dynamic mechanism produces prices in time period $t$ using equation (\ref{eq:max_welfare_price})
    with respect to the re-computed flow $\bff^*_t$, and the dynamic mechanism produces a matching vector $\bfg$ using equation (\ref{eq:trip_allocation_counts})
    with respect to the re-computed flow $\bff^*_t$.
\end{definition}

Our main result in this section is the following theorem, which shows that the static mechanism
satisfies a static notion of incentive compatibility, and that the dynamic mechanism satisfies
a dynamic (subgame-perfect) notion of incentive compatibility.

\begin{theorem} (Incentive compatibility in the stochastic fluid model)
    \label{thm:fluid_ic}
   The following statements are true in the stochastic fluid model:
    \begin{enumerate}
        \item When prices and matching decisions are produced by the static mechanism, then no individual driver
            is incentivized to deviate from their trip-allocation, assuming that no drivers have deviated from their
            trip-allocations in previous time periods.
        \item When prices and matching decisions are produced by the dynamic mechanism, then no individual driver
            is incentivized to deviate from their trip-allocation at any time period, regardless of the trips taken in earlier time periods.
        \item The expected utility-to-go of a driver positioned at an LT-scenario $(l,\omega_t)$ is equal to the optimal dual variable $\eta^*_{(l,\omega_t)}$ associated with the LT-scenario.
    \end{enumerate}
\end{theorem}
%\etcomment{Note, I propose to add the last point here to highlight the connection to the dual.}
%\mccomment{write something about how the static i.c. condition above is like collapsing driver-decisions to a single-time-period game?} \etcomment{i don't understand this proposal.}
The last point of the Theorem follows from pricing rule (\ref{eq:max_welfare_price}) and the optimality conditions (\ref{eq:kkt_conditions}). The claimed incentive compatibility then follows by backwards induction on $t$.
%with an LT-scenario $(l,\omega_t)$ is equal to the expected utility-to-go of a driver positioned at that location.
We defer the proof details of Theorem \ref{thm:fluid_ic} to Appendix \ref{sec:fluid_ic_proofs}.

Next we proceed to prove the main theorem of this section, that all equilibria of the dynamic mechanism are welfare-optimal in the fluid model. For this theorem as well as Theorem \ref{thm:stochastic_ic} we will use the following assumption.
\begin{assumption}
\label{assum:driver_pref}
We assume that drivers on the platform are willing to take a passenger instead of driving empty when the two options have the same net utility.
\end{assumption}
\pfedit{A driver might choose to accept passengers when he is otherwise utility-indifferent because of the differential availability of incentive programs to drivers with high acceptance rates \cite{UberPro}.}
\pfedit{Our model allows drivers who are unwilling to accept passengers} to go offline before the start of the period, potentially relocating empty to another location. Going offline is visible to the platform, and hence affects the price it offers.

In future work, we plan an extension in which drivers have an idiosyncratic utility associated with adding a passenger to their vehicle. In this extension, when the net utility of adding a rider is smaller than driving empty, they can reject a dispatch, \pfedit{which} 
% the dispatch 
would then go to another driver. Under this extension, Assumption~\ref{assum:driver_pref} would no longer be needed and dispatches would be allocated to the set of drivers whose disutility for having passengers is small enough that their surplus is positive. Prices would reflect the need for this set to be large enough to fulfill the targeted demand.

\begin{theorem} (Welfare-Robustness in the stochastic fluid model)
    \label{thm:robust_fluid_welfare}
    Let $\Pi$ be any driver strategy profile that is a subgame-perfect equilibrium with respect to the dynamic mechanism, and satisfies Assumption \ref{assum:driver_pref}. 
    Then $\Pi$ is welfare-maximizing, and the utility-to-go of a driver is equal to the  corresponding dual variable from the dynamic formulation.
\end{theorem}


% \begin{remark}
% Note that the preference condition can be implemented by an infinitesimal increase in the price offered. This condition is necessary. To see why, consider a single route when there are too many drivers. The optimal solution suggest to drive all passengers at the lowest possible price. Given the low price an alternate equilibrium solution is to leave all passengers behind. 
% \end{remark}

\begin{proof} We provide a proof sketch here and defer the details to the \ref{subsec:fluid_robustness_proof}. We prove the theorem by induction on the number of periods. Consider the trip-prices offered for each route $r$ for the first period, $\rho_{(r,\omega_1)}$. Recall that the price is set as $\rho_{(r,\omega_1)}=\frac{d}{df} U_{(r,\omega_1)}(f^*_{(r,\omega_1)})$ for the optimal flow $f^*$. Consider the alternate linear reward function on these routes of $\bar U_{(r,\omega_1)}(x)=(\rho_{(r,\omega_1)}-c_{(r,\omega_1)})x$, and note that $f^*$ remains optimal when using these linearized reward functions for the first period, and satisfies complementary slackness with the same dual variables.

Now consider any equilibrium flow $f'$. By the induction hypothesis, the part of the flow after the first period is optimal, conditioned on the driver allocation resulting from the first period. By the equilibrium condition, the flow $f'$ satisfies the complementary slackness conditions with the prices $\rho_{(r,\omega_1)}$ the mechanism uses. This implies that $f'$ is optimal for linearized reward functions $\bar U_{(r,\omega_1)}(x)$. Notice that $\bar U_{(r,\omega_1)}(x) \ge  U_{(r,\omega_1)}(x)$ for all routes and all  $x$, as the reward is concave. To show that $f'$ is optimal for the true reward $U$ also, we have to argue that $\bar U(f')$ is equal to $ U(f^*)$. Consider the routes on which $\bar U_{(r,\omega_t)} \neq U_{(r,\omega_t)}$: first period routes.  For first period routes with passengers, first observe that on such routes $f'_{(r,\omega_1)}\le f^*_{(r,\omega_1)}$ as drivers cannot drive passengers who 
\pfedit{chose not to request a trip because the price was too high.}
%rejected the trip due to too high price. 
To show that the two are equal, note that the total mass of drivers driving passengers in the first period cannot be less in $f'$ \pfedit{than in $f^*$} due to 
\pfedit{Assumption~\ref{assum:driver_pref}}, 
% the assumption of drivers favor driving passengers, 
and \pfedit{the fact that}, at the equilibrium, additional passengers would offer an equal value trip \pfedit{to drivers}. On routes where \pfedit{some} drivers drive empty, the two reward functions are the same.  
\end{proof}
 


==> opt_ic_two_level_model.tex <==
In this section we consider pricing and matching mechanisms in the stochastic two-level model,
where new driver volume and price-inquiry demand form an additional layer of randomness
at each time period.  We use the stochastic fluid model as an approximation to the dynamics
in the stochastic two-level model, and the mechanisms we study in this section are 
the same mechanisms that we developed for the fluid model as in the previous section.
For completeness, we restate these mechanisms below and describe how they work in the context
of the two-level model.

\begin{definition}
The state-independent mechanism computes an optimal solution $\bff^*=(f_{(r,\omega_t)}^* : (r,\omega_t)\in\calA)$ 
for the state-independent optimal stochastic flow problem (\ref{eq:static_optimization}) at the beginning of time, 
and uses the flow values to set prices and make matching decisions in the same method as described by Algorithm \ref{alg:static_fluid}.

The state-dependent mechanism re-solves the state-dependent stochastic flow problem (\ref{eq:dynamic_optimization}) at each time $t$.
The platform observes the time $t$ scenario $\omega_t$, the time $t$ driver-supply vector $\bfS_t$, and the time $t$ price-inquiry
demand vector $\bfD_t$.  The platform computes an optimal solution $\bff_t^*=(f_{(r,\omega_\tau)}^* : (r,\omega_\tau)\in\calA_{\omega_t}^{\geq \tau})$ 
and the flow values $f_{(r,\omega_t)}^*$ for each active route $(r,\omega_t)\in\calA_{\omega_t}^t$ are used to set prices and
matching decisions in the time period $t$.
\end{definition}

In the two-level model, the matching suggestions produced by both the state-dependent and state-independent mechanisms require
some adjusting from the exact flow values from which they are derived, because the realized number of dispatch requests is
no longer a deterministic function of the price.  We assume that the platform makes the resulting empty-trip suggestion counts
as close to the optimal flow values as possible. \mccomment{purposefully left this vague for now -- will come back and fill in
when writing the approx i.c. proof.}


In the two-level model the stochastic flow optimization problems (\ref{eq:static_optimization})
and (\ref{eq:dynamic_optimization}) underlying these mechanisms are only approximations to the underlying welfare optimization problem, 
since these formulations do not account for the second layer of randomness governing new driver volume and price-inquiry demand.
The nature of this approximate solution means that the corresponding incentive guarantees
will also be approximate. We will study this approximation accuracy in a large-market setting where
the network structure is held fixed and the expected volume of new driver supply and price-inquiry demand
grow at the same rate. 

Recall that the family of distributions $(G_{(r,\omega_t)} : (r,\omega_t)\in\calA)$ govern price-inquiry
demand volume and the family of distributions $(Q_{(l,\omega_t)} : (l,\omega_t)\in\calN)$ govern the volume
of new driver supply.  In the large-market setting we include a market-scale parameter $k$ and consider a 
family of distributions $(G_{(r,\omega_t)}^k)$ and $(Q_{(l,\omega_t)}^k)$ for each $k$.
We assume that the expected value of each distribution scales linearly in $k$ and we assume that all distributions
are sub-exponential.  These assumptions are stated formally in Assumption \ref{assn:large_market_dists}
below.
\begin{assumption}
\label{assn:large_market_dists}
\begin{itemize}
\item For each ODT-scenario $(r,\omega_t)\in\calA$ and each market-scale parameter $k\geq 1$ 
let $D_k$ be the random price-inquiry demand volume with distribution $G_{(r,\omega_t)}^k$.  
For every $\epsilon>0$ we assume there exists an error tolerance function $h(\epsilon)$ such that
with probability at least $1-\epsilon$ the following concentration property is satisfied:
$$
|D_k - \bbE[D_k]| \leq h(\epsilon)\bbE[D_k].
$$
\mccomment{placeholder for the real concentration inequality we assume -- will come back to this later. 
If it's not too hard I think we want to assume subexponential  concentration because that applies to Poisson distributions,
but there are some details there to work out that I will think through later}
\item We assume that the expected value grows linearly in $k$: 
$$\bbE[D_k] = k\bbE[D_1].$$
\item We assume both of the above properties also hold for the the new-driver supply random variables $S_k$ with
distribution $Q_{(s,\omega_t)}^k$.
\end{itemize}
\end{assumption}

Next, we define the approximate versions of the static and subgame-perfect incentive compatibility conditions
we studied in the previous section.

\begin{definition}
\mccomment{also placeholder -- need to go into more detail here}
Consider any pricing and matching mechanism for the stochastic two-level model.
\begin{itemize}
\item The mechanism is \emph{statically incentive-compatible with additive gap $\delta$} if the condition (\ref{eq:ic_inequality})
    is violated by at most an additive term $\delta$, assuming that no drivers have deviated from their trip allocations at any of the previous time periods.
\item The mechanism is \emph{subgame-perfect incentive-compatible} if the condition (\ref{eq:ic_inequality})
    is violated by at most an additive term $\delta$, regardless of the actions in previous time periods.
\end{itemize}
\end{definition}

Next, we show that the state-independent mechanism is statically incentive-compatible with additive gap $\delta=\frac{1}{\sqrt{k}}$
under the market scale parameter $k$.

\begin{theorem}
\label{thm:two_level_static_ic}
Consider the state-independent mechanism setting prices and matching decisions for the 
stochastic two-level model with supply and demand distributions corresponding to the market-scale parameter $k$.
Then the mechanism is statically incentive compatible with additive gap $\delta=\frac{1}{\sqrt{k}}$.
\end{theorem}

The proof of Theorem \ref{thm:two_level_static_ic} analyzes the extent to which the driver-state vector at time $t$
can deviate from the driver-state vector that would arise if the optimal stochastic flow was followed exactly.
The factors contributing to the discrepancy between the realized driver-state vector at time $t$ and the driver-state
vecotr that would arise from the optimal stochastic flow are the second level of randomness underlying price-inquiry demand,
request demand, and new-driver supply. The following lemma characterizes the extent of the discrepancy caused by these factors:
\begin{lemma}
\label{lem:state_vector_diff}
\mccomment{placeholder}
\end{lemma}

In the following, we prove Theorem \ref{thm:two_level_static_ic}.
\begin{proof}

\end{proof}

. put proof of theorem \ref{thm:two_level_static_ic} here

. start to discuss dynamic mechanism; introduce concept of partial derivative, then talk about lipschitz conty of partial derivative
and stability of optimal solution
.

.

.

.

.

.

.

.


\mccomment{
\begin{itemize}
\item Introduce the two mechanisms in the previous section so that they do not need to be explicitly redefined here?
    \begin{itemize}
    \item Make sure the static mechanism is well-specified if the state variable is not exactly equal to what it should be
    \item Call the dynamic mechanism the stochastic spatiotemporal pricing and matching (SSP) mechanism in the previous section?
    \end{itemize}
\end{itemize}
}

define static eqlbm here
\mccomment{
\begin{itemize}
\item Define approximate static equilibrium and prove static ic therem here first.  Proof is relatively simple but defer main details to appendix.
\item Next define approximate subgame-perfect ic and prove subgame percet ic next. Try to make proof simple as possible.
\begin{itemize}
\item use relationship 
$$
\eta_{(l,\omega_t)} = \frac{\partial}{\partial S_{(l,\omega_t)}}\calW_{\omega_t}(\bar{\bfS}_t, \bar{\bfD}_t).
$$
\item then use lipschitz continuity of partial derivative together with concentration inequalities.
\end{itemize}
\end{itemize}
}




==> robust_fluid_welfare.tex <==
In this section we define the notion of platform pricing policy and driver strategy profiles
in the stochastic fluid model.  For simplicity in this section let's use a less cumbersome notation
in place of ODT-scenarios and LT-scenarios, and write $r\in\calA_{\omega_t}^t$ to mean the set of
routes that are active at time $t$ under scenario $\omega_t$ and $\ell\in\calN_{\omega_t}^t$
to mean the set of locations that are active at time $t$ under $\omega_t$.

\begin{definition}
In the stochastic fluid model a platform pricing policy is a function $P$ mapping:
\begin{itemize}
    \item the time period $t$,
    \item the scenario $\omega_t$,
    \item the observed supply-location vector $\bar{\bfS}_t$
\end{itemize}
to a price vector $\bfrho = P(t,\omega_t,\bar{\bfS}_t)$ where $\bfrho$ specifies trip prices
for all active routes $\bfrho=(\rho_r : r\in\calA_{\omega_t}^t)$.
\end{definition}

\begin{definition}
A driver strategy-profile is a function $H$ mapping:
\begin{itemize}
    \item the time period $t$ and scenario $\omega_t$,
    \item the price vector $\bfrho$,
    \item the dispatch-request demand vector $\bar{\bfd}$,
\end{itemize}
and produces a trip-allocation vector $\bfh=H(t,\omega_t,\bfrho,\bar{\bfd})$.
\end{definition}

\begin{definition}
In the stochastic fluid model, under a pricing policy $P$ and a strategy profile $H$,
the utility-to-go of a driver positioned at an active location $l\in\calN_{\omega_t}^t$
is defined recursively as:
$$
\bar{\calV}_{(l,\omega_t)}(\bar{\bfS}_t) = \bbE\left[\delta\rho_r - c_r
+ \bar{\calV}_{(l^+(r),\omega_{t+1})}(\bar{\bfS}_{t+1})\right].
$$
In the above, the trip type $(r,\delta)$ is sampled from the trip-allocation distribution
for driver positioned at $l$, i.e. $\bfh(l)$, where $\bfh$ is the trip-allocation vector
produced at time $t$ under $H$.
\end{definition}

\begin{definition}
We say the driver strategy profile $H$ is a subgame-perfect equilibrium with
respect to a pricing policy $P$ if, from
every state $(t,\omega_t,\bar{\bfS}_t)$, and for every trip type
$(r,\delta)$ to which the trip-allocation vector 
$\bfh=H(t,\omega_t,\bar{\bfS_t},\bfrho_t,\bar{\bfd}_t)$ allocates nonzero drivers,
the utility-to-go for that trip, i.e.
$$
\delta\rho_r - c_r + \bbE[\bar{\calV}_{(l^+(r),\omega_{t+1})}(\bar{\bfS}_{t+1})]
$$
is equal to the expected utility-to-go from that location $\bar{\calV}_{(l,\omega_t)}(\bar{\bfS}_t)$, and this is at least as large as the utility for deviating to any relocation-trip, i.e. the above is larger than
$$
\max_{r'\in A^+(l^-(r))_{\omega_t}, \delta\in\{0,1\}} \rho_{r'} -c_{r'} + \bbE[\bar{\calV}_{(l^+(r'),\omega_{t+1})}(\bar{\bfS}_{t+1})]
$$
\end{definition}

\begin{definition}
The expected welfare-to-go from a time $t$, scenario $\omega_t$, and supply-distribution vector $\bar{\bfS}_t$ under a pricing policy $P$ and a 
strategy-profile $H$ is defined recursively as
$$
W_{\omega_t}(\bar{\bfS}_t; P,H) = \sum_{r\in\calA_{\omega_t}^t}\left( U_r(h_{r,1}, \rho_r) - c_r(h_{r,0} + h_{r,1})\right)
+ \bbE\left[W_{\omega_{t+1}}(\bar{\bfS}_{t+1}); P,H)\right],
$$
where $\rho_r$ range over the components of the pricing vector $\bfrho=P(t,\omega_t,\bar{\bfS}_t)$, $h_{(r,\delta)}$ range over the components
of the trip-allocation vector $\bfh=H(t,\omega_t,\bar{\bfS}_t,\rho)$,
and the utility function $U_r(h_{r,1},\rho_r)$ is defined as the total rider-side
utility when $h_{r,1}$ dispatches are served and $\rho_r$ is the price:
$$
U_r(h_{r,1},\rho_r) = h_{r,1}\bbE\left[V_r | V_r \geq \rho_r\right].
$$
The definition of $U_r(\cdot,\cdot)$ assumes that $h_{r,1}$ is feasible with 
respect to the amount of dispatch-request demand for $r$ arising under $\rho_r$,
i.e. the domain of $U_r(\cdot,\cdot)$ imposes the inequality 
$h_{r,1} \leq \bar{D}_r(1-F_r(\rho_r))$.
\end{definition}

\begin{theorem}
\label{thm:fluid_robustness}
Let $H$ be any subgame-perfect driver-strategy profile with respect to the SSP
pricing policy $P^{SSP}$ in the stochastic fluid model.  Then, under 
Assumptions \mccomment{insert}, the expected welfare
under $H$ and $P^{SSP}$ is the optimal expected welfare.
\end{theorem}
\begin{proof}
For completeness we re-state the single time period stochastic flow optimization
problem from which the SSP pricing policy obtains prices:
\begin{equation}
\label{eq:single_period_opt_flow_2}
\calW_{\omega_t}(\bar{\bfS}_t) = \sup_{\bff\geq 0}\left(
\sum_{(r,\omega_t)\in\calA_{\omega_t}^t}U_{(r,\omega_t)}(f_{(r,\omega_t)})
+ \bbE\left[\calW_{\omega_{t+1}}(\bff)\right] : 
\forall (l,\omega_t)\ \bar{S}_{(l,\omega_t)} = 
\sum_{\substack{(r,\omega_t)\in\\ A^+_{\omega_t}(l)}}f_{(r,\omega_t)}
\right).
\end{equation}

We now prove Theorem \ref{thm:fluid_robustness} via backwards induction.  For our
induction hypothesis fix a time period $t$, a scenario $\omega_t$, and assume the 
following hold at future time periods $t$ and future scenarios $\omega_t$:
\begin{itemize}
    \item The welfare
    under $H$ and $P$ is optimal from any supply-location vector, i.e. for any 
    $\bar{\bfS}_{t+1}$ we have the equality 
    $W_{\omega_{t+1}}(\bar{\bfS}_{t+1}) = \calW_{\omega_{t+1}}(\bar{\bfS}_{t+1})$.
    \item For a driver positioned at an LT-scenario $l\in\calN_{\omega_{t+1}}^{t+1}$,
    the utility-to-go for that driver from $l$ is equal to the optimal dual variable
    associated with the $l$ constraint in the convex optimization problem defining
    $\calW_{\omega_{t+1}}(\bar{\bfS}_{t+1})$, i.e. we have the equality
    $\bar{\calV}_{(l,\omega_{t+1})}(\bar{\bfS}_{t+1}) = \eta^*_{l,\omega_{t+1}}(\bar{\bfS}_{t+1})$.
\end{itemize}
\end{proof}

\subsection{A Convex Optimization Lemma for Problems with our Structure}

Consider a convex optimization problem
$$
\inf\left(\calC(\bff) : g_i(\bff) = 0, 1\leq i\leq m, h_j(\bff) \leq 0, 1\leq j \leq n,
\bff \geq 0\right).
$$

.

.

.

Consider a generic convex optimization problem
\begin{equation}
\label{eq:primal}
\inf\left(\calC(\bff) : g_i(\bff) = 0, 1\leq i\leq m, \bff \geq 0 \right),
\end{equation}
for a decision variable $\bff=(f_j:1\leq j\leq n)$, a 
continuously differentiable and convex cost function $\calC(\bff)$ and a continuously differentiable convex equality constraint
functions $g_i(\bff)$.
Let 
$$
L(\bff,\bfeta,\bfalpha) = \calC(\bff) + \sum_i\eta_ig_i(\bff) - \sum_j \alpha_j f_j
$$
be the Lagrangian function for our problem, let
$$
\Phi(\bfeta,\bfalpha) = \inf_{\bff} L(\bff,\bfeta,\bfalpha)
$$
be the Lagrangian dual function, and let
$$
\sup_{\bfeta,\bfalpha}\left(\Phi(\bfeta,\bfalpha) : \bfalpha\geq 0\right)
$$
be the dual optimization problem.  Let $\bff^*$ be
a primal optimal solution and let $(\bfeta^*,
\bfalpha^*)$ be a dual optimal solution.  Weak
duality states $\calC(\bff^*)\geq \Phi(\bfeta^*,
\bfalpha^*)$, and when strong duality holds we have
$\calC(\bff^*) = \Phi(\bfeta^*,\bfalpha^*)$.

When strong duality holds, the following conditions
are sufficient to certify the optimality of $\bff^*$:
\begin{itemize}
\item Stationarity: $$
0 = \nabla\calC(\bff^*) + \sum_i\eta^*_i\nabla g_i(\bff^*)
- \sum_j \alpha^*_j\bfone_j,
$$
where $\bfone_j$ is an $n$-dimensional vector with a $1$ in the $j$th
component and $0$ elsewhere.
\item Complementary slackness:
$$
\alpha^*_j f^*_j = 0
$$
for all $1\leq j\leq n$.
\end{itemize}


==> scrap.tex <==
\subsection{Old Comments and Text from Now-Removed Definition of Total-System-Welfare}
\mccomment{thoughts on calling it ``expected'' welfare?  There are two types 
of expectations I am referring to here.
The first arises when discussing welfare-to-go and just refers to all the randomness in the system
dynamics.  The second expectation is the expected value of the utility collected by a rider conditioned on 
them having paid a certain price.
Hmm.  I guess we will sometimes want to refer to the ``realized total welfare'' at the end of the time
horizon, which depends on actual realizations of rider utility values, rather than the value they receive
in expectation. I'll think a bit more about how we want to define welfare.}

\mccomment{more thoughts on this:  I think we want separate definitions for expected welfare-to-go,
and post-hoc/realized welfare.}

\mccomment{edited up to here on 11/17. Everything below here is old text/notation:}

\color{red}{
Let us now shift our discussion from driver utility to total system welfare.
The total system welfare is the sum of total driver-utility and total rider-utility.
So far in this section we have developed the concept of driver-utility without mention
of rider utility.
On the rider-side, each dispatch-request for a route $(r,\omega_t)$ is made by a rider whose private utility exceeds the
price $\rho_t(r,\omega_t)$.  Thus each rider who requests a dispatch holds the following expected private value
for ther trip:
$$
\bbE\left[V\mid V\geq \rho_t(r,\omega_t)\right],
$$
where the random variable $V$ has distribution $F_{(r,\omega_t)}$.

However, each rider who receives a dispatch must pay the price $\rho_t(r,\omega_t)$,
so this is subtracted off dispatch-requesting rider who receives a dispatch has agreed to pay the price $\rho_T(r,\omega_T)$.
We assume that riders have quasilinear utility for money, meaning that their utility for the dispatch
has the price $\rho_t(r,\omega_t)$ subtracted from their private value.
Thus a rider who receives a dispatch collects the following utility:
$$
R_{(r,\omega_t)} = 
\bbE\left[V\mid V\geq \rho_t(r,\omega_t)\right] - \rho_t(r,\omega_t).
$$

We are now ready to define total system welfare.  Let $W_{\omega_t}(\bfS_t,\bfB_t,\bfE_t)$ denote
total system welfare-to-go at time $t$ under scenario $\omega_t$ 
as a function of the supply vector $\bfS_t$ and the platform trip-suggestion
vectors $\bfB_t$ and $\bfE_t$.  This welfare-to-go is defined as:
$$
W_{\omega_t}(\bfS_t,\bfB_t,\bfE_t) = \sum_{\substack{(r,\omega_t)\in\\ \calA^t(t,\omega_t)}} B_t(r,\omega_t)\left[U_{(r,\omega_t)}^B + R_{(r,\omega_t)}\right] 
    + E_t(r,\omega_t)U_{(r,\omega_t)}^E + \bbE\left[W_{\omega_{t+1}}(\bfS_{t+1},\bfB_{t+1},\bfE_{t+1})\right]
$$
if $t<T$, and 
$$W_{\omega_t}(\bfS_t,\bfB_t,\bfE_t) =
\sum_{(r,\omega_t)\in \calA^t(t,\omega_t)} B_t(r,\omega_t)\left[U_{(r,\omega_t)}^B + R_{(r,\omega_t)}\right] 
+ E_t(r,\omega_t)U_{(r,\omega_t)}^E
$$
if $t=T$.
Finally, let us also use the notation
$$
W_{\emptyset} = \bbE\left[W_{\omega_1}(\bfS_1,\bfB_1,\bfE_1)\right]
$$
to denote the total expected system welfare before the first scenario is sampled in the first time period.
}
\color{black}
Let us use the notation
\begin{align}
    \label{eq:value_fn_def}
    \calW_{\omega_t}(\bfS_t,\bfD_t)\equiv&\mbox{Optimal value of dynamic optimization formulation (\ref{eq:dynamic_optimization})}
\\
    &\mbox{     w.r.t. supply vector $\bfS_t$ and price-inquiry demand vector $\bfD_t$}\nonumber
\end{align}

\begin{lemma}
    \label{lem:stochastic_utility}
Consider any time $t$ and scenario $\omega_t$ and consider a driver
located at an active LT-scenario $(l,\omega_t)\in\calN_{\omega_t}^t$.
Recall $\vtglocation{l,\omega_t}$ denotes the expected utility-to-go collected by a driver
located at $(l,\omega_t)$ assuming that drivers always follow their action suggestions.
.

.

Assume that the derivative of each reward function, i.e. $\frac{d U_{(r,\omega_t)}(f)}{dg}$,
is Lipschitz continuous with constant $\alpha$.

.

Let $\bfeta=(\eta_{(r,\omega_\tau)} : (r,\omega_\tau)\in\calA_{\omega_t}^{\geq t})$ 
be an optimal dual variable for the dynamic optimization formulation (\ref{eq:dynamic_optimization}) with respect
to time period $t$ and scenario $\omega_t$.

.

For each remaining time period $\tau=t,t+1,\dots,T-1,T$, let $D_\tau$ denote the event that the driver we are considering
is allocated an action suggestion which the SSP mechanism produces from rounding the fractional parts of an optimal stochastic 
flow at time $\tau$, i.e. $D_\tau=1$ indicates the event that the driver is allocated a ``rounded'' action suggestion and $D_\tau=0$
indicates otherwise.

Then the expected utility-to-go of our driver under consideration is bounded as follows:
\begin{align}
    \vtglocation{l,\omega_t}\geq\; & \eta_{l,\omega_t} - \sum_{\tau=t}^T\left(1 - \bbP(D_\tau=0)\right)V_{max}\nonumber\\
                      & - \bbE\left[\sum_{\tau=t+1}^T
        \alpha\|\bfD_\tau - \bbE[\bfD_\tau\mid\omega_\tau]\|_1 
        + \alpha(T-\tau+1)\left(\|\bfM^t - \bbE[\bfM_\tau\mid\omega_\tau]\|_1  
        + \|\bfg^\tau-\bfg^{*\tau}\|_1\right) \label{eq:expected_utility_lb}
    \right].
\end{align}
In the above, $\|\bfg^\tau-\bfg^{*\tau}\|_1$ indicates the difference between the SSP action suggestions $\bfg^\tau$
and the fluid optimal solution $\bfg^{*\tau}$. \mccomment{This is how it appears in the earlier writeup.  Not sure if this is
correct or needed.  I'm worried this bound on expected utility won't shrink to $0$ in the large market setting. Oh, the lipschitz constant
$\alpha$ is the thing that goes to $0$ in the large market setting?  Maybe.}
Also,
\begin{equation}
    \label{eq:expected_utility_ub}
\vtglocation{l,\omega_t} \leq \eta^*_{s_\tau} + 
        \bbE\left[\sum_{t=\tau+1}^T
        \alpha\|\bfN^t - \bar{\bfN}^t\|_1 
        + \alpha(T-t+1)\left(\|\bfM^t - \bar{\bfM}^t\|_1  
    + \|\bfg^t-\bfg^{*t}\|_1\right)\right]. 
\end{equation}
For the $\|\bfg^t-\bfg^{*t}\|_1$ terms, we adopt the convention that 
$\bfg^{*t}$ denotes the time $t$ optimal flow vector restricted
to the immediately relevant time $t$ routes $\calR_{\omega_t}^t$.
\end{lemma}

\begin{proof}
We proceed via backwards induction.  If $t=T$ is the final time period then we have:
\begin{align*}
\vtglocation{l,\omega_t} &= \vtglocation{l,\omega_t}(D_t=1) \bbP(D_t=1) + \vtglocation{l,\omega_t}(D_t=0)\bbP(D_t=0)\\
& \geq \vtglocation{l,\omega_t}(D_t=0)\bbP(D_t=0).\\
\end{align*}
In the above, we use $\vtglocation{l,\omega_t}(D_t=0)$ to mean the utility collected if allocated a non-rounded action suggestion,
and $\vtglocation{l,\omega_t}(D_t=1)$ to mean the utility collected if allocated a rounded action suggestion.

For every possible outgoing route $(r,\omega_t)\in N^+(l,\omega_t)$ to which the driver may be allocated a non-rounded action suggestion,
the following equality holds by complementary slackness:
$$
\eta_{(l,\omega_t)} = \frac{d}{df}U_{(r,\omega_t)}(f_{(r,\omega_t)}^*).
$$
By Lemma \ref{lem:reward_fn} we have the characterization
$$
\frac{d}{df}U_{(r,\omega_t)}(f) = \begin{cases}
F_{(r,\omega_t)}^{-1}\left(1-\frac{f}{D_t(r,\omega_t)}\right) - c_{(r,\omega_t)} 
    & \mbox{if } f \leq D_t(r,\omega_t),\\
    -c_{(r,\omega_t)} & \mbox{if } f > D_t(r,\omega_t).
\end{cases}
$$
From the definition of our pricing function $\rho_t(r,\omega_t)$, it follows that the dual variable value $\eta_{(l,\omega_t)}$ is equal to the utility collected along any non-rounded action
suggestion, thus $\vtglocation{l,\omega_t}(D_t=0)=\eta_{(l,\omega_t)}$.
Further, from Lemma \mccomment{insert lemma} we know that for the final time period $t=T$ we have $\eta_{(l,\omega_t)} \leq V_{max}$ we have the following:
\begin{align*}
\vtglocation{l,\omega_t} & \geq \vtglocation{l,\omega_t}(D_t=0)\bbP(D_t=0).\\
& = \eta_{(l,\omega_t)} - (1-\bbP(D_t=0))\eta_{(l,\omega_t)} \\
& \geq \eta_{(l,\omega_t)} - (1-\bbP(D_t=0)) V_{max}.
\end{align*}
This establishes the base case.

For the induction step, assume the result holds for all future time periods $t+1$.
Let $\bff^*=(f^*_{(r,\omega_\tau)}: (r,\omega_\tau)\in\calA_{\omega_t}^{\geq t})$ be an optimal stochastic flow for the dynamic optimization
formulation (\ref{eq:dynamic_optimization}) with respect to the supply vector $\bfS_t$ and the price-inquiry demand vector $\bfD_t$.

Let us introduce the following notation:
\begin{itemize}
\item Let $\bff^*=(f^*_{(r,\omega_\tau)}: (r,\omega_\tau)\in\calA_{\omega_t}^{\geq t})$ be an optimal stochastic flow for the dynamic optimization
formulation (\ref{eq:dynamic_optimization}) with respect to the supply vector $\bfS_t$ and the price-inquiry demand vector $\bfD_t$.
\item Let $\bff=(f_{(r,\omega_\tau)}: (r,\omega_\tau)\in\calA_{\omega_t}^{\geq t})$ be the rounded approximation to $\bff^*$ that the SSP mechanism uses to make
matching decisions in time $t$.
\item Let $\bar{\bfM}_{t+1} = \bbE[\bfM_{t+1}\mid\omega_{t+1}]$ be the expected value of the new-driver location vector at time period $t+1$.
\item Let $\bfE_{t+1}^*$ be the existing driver-location vector at time $t+1$, assuming that drivers are routed according to the fractional optimum $\bff^*$.
\item Let $\bfE_{t+1}'$ be the existing driver-location vector at time $t+1$, assuming that drivers are routed according to the rounded solution $\bff$.
\item Let $$\bfS_{t+1}^*=\bfE_{t+1}^* + \bar{\bfM}_{t+1}$$ be the expected value of the time $t+1$ supply vector assuming that drivers are routed according to the fractional optimum $\bff^*$.
\item Let $$\bfS_{t+1}'=\bfE_{t+1}' + \bfM_{t+1}$$ be the expected value of the time $t+1$ supply vector assuming that drivers are routed according to the fractional optimum $\bff^*$.
\end{itemize}


For each active outgoing route $(r,\omega_t)\in N^+(l,\omega_t)$ for which $f^*_{(r,\omega_t)}$ is nonzero, 
complementary slackness asserts:
\begin{equation*}
\eta_{(l,\omega_t)} = \rho_t(r,\omega_t)-c_{(r,\omega_t)} + \bbE\left[ \eta_{(l^+(r),\omega_t)}  \right].
\end{equation*}
Furthermore, Lemma \mccomment{insert lemma} asserts
$$
\eta_{(l^+(r),\omega_t)} = \frac{\partial}{\partial S_{(l^+(r),\omega_{t+1})}} \calW_{\omega_{t+1}}(\bfS_{t+1}^*).
$$
Thus, 
\begin{equation}
\label{eq:valuefn_optimality_condition}
\eta_{(l,\omega_t)} = \rho_t(r,\omega_t)-c_{(r,\omega_t)} + \bbE\left[ \frac{\partial}{\partial S_{(l^+(r),\omega_{t+1})}} \calW_{\omega_{t+1}}(\bfS_{t+1}^*)  \right].
\end{equation}

\mccomment{
Remaining steps of the proof are as follows:
\begin{enumerate}
\item 
Induction hypothesis states that utility-to-go from the next time period is close to the dual variable $\eta'_{(l^+,\omega_{t+1})}$, 
where $\eta'_{(l^+,\omega_{t+1})}$ is an optimal dual variable for the convex program with respect to $\bfS_{t+1}'$.
\item 
Get a bound showing that expected utility-to-go in this time period $\vtglocation{l,\omega_t}$ is close to
$$
\rho_t(r,\omega_t)-c_{(r,\omega_t)} + \bbE\left[\frac{\partial}{\partial S_{(l^+(r),\omega_{t+1})}} \calW_{\omega_{t+1}}(\bfS_{t+1}')\right]
$$
\item Use assumption about lipschitz continuity of individual reward functions $U_{(r,\omega_t)}(\cdot)$ to assert lipschitz continuity of 
the partial derivative of the value function
\end{enumerate}
}
\end{proof}



\subsection{Asymptotic IC Scrap}

    use the notation $D^k_{(r,\omega_t)}$ to denote the price-inquiry demand random variable under the network-size parameter $k$, which
    is distributed according to $G^k_{(r,\omega_t)}$, and we use the notation $M^k_{(l,\omega_t)}$ to denote the entering driver supply random variable
    under the network-size parameter $k$, which is distributed according to $Q^k_{(l,\omega_t)}$.

    Fix any LT-scenario $(l,\omega_t)$ or ODT-scenario $(r,\omega_t)$ and let $(X_k:k=1,2,\dots)$ be a sequence of 
    random variables distributed according to the sequence of distributions $(Q^k_{(l,\omega_t)}:k=1,2,\dots)$ or $(G^k_{(r,\omega_t)}:k=1,2,\dots)$.  
    We assume that the following properties are satisfied:
    \begin{itemize}
        \item The expected value of $X_k$ grows linearly in $k$, i.e. the following is satisfied for all $k$:
            $$  \bbE[X_k] = k\bbE[X_1].$$
        
        \item $X_k$ concentrates around its mean as $k$ grows large.  Formally, we assume there exists a sequence of $\epsilon_k\geq 0$
            such that $\epsilon_k\to 0$, and a function $h(\epsilon_k)$ satisfying $h(\epsilon_k)/k\to0$ as $k\to\infty$, such that the following
            holds for all $k$:
            \begin{equation}
                \label{eq:concentration}
                \bbP\left(|X_k - \bbE[X_k]|\leq h(\epsilon_k)\bbE[X_k]\right) \geq 1 - \epsilon_k.
            \end{equation}
    \end{itemize}

    Finally, in the large-market setting with network-size parameter $k$, we assume that samples of entering drivers from the distributions $Q_{(l,\omega_t)}^k$
    and samples of price-inquiry demand from the distributions $G_{(r,\omega_t)}$ are scaled inversely by the network-size parameter $k$.
    That is, we use $M^k_{(l,\omega_t)} / k$ as the volume of entering driver supply at an LT-scenario $(l,\omega_t)$, where
    $M^k_{(l,\omega_t)}$ is sampled from the distribution $Q_{(l,\omega_t)}$, and we apply a similar transformation to price-inquiry demand counts.
    Applying this scaling is effectively shrinking the size of a driver for larger values of $k$, namely each driver has size $1/k$ in the large-market
    setting with size parameter $k$.  A consequence of this scaling is that the fluid welfare optimization problem (\ref{eq:dynamic_optimization}) has the 
    same solution for all values of $k$.


    \begin{proof}

    .

    .


    be the upper bound in equation (\ref{eq:immediate_reward_bound}) from Lemma \ref{lem:immediate_reward},
    which is an upper bound on the probability that the SSP mechanism allocates an action-suggestion $(r,\omega_t,\delta)$
    for which $\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t)$ holds, in the large-market setting with size $k$.

    .

    $\frac{\epsilon_k}{S_{(l,\omega_t)}} + \frac{|N^+(l,\omega_t)|}{k S_{(l,\omega_t)}}$
    .

    .

    .

Recall the expected utility-to-go achieved by a driver traversing the route $(r,\omega_t)$ is equal to
$$
\vtgroute{r,\omega_t,\delta} = \delta\rho_t(r,\omega_t) - c_{(r,\omega_t)} + \bbE\left[\vtglocation{l^+(r),\omega_{t+1}}\right],
$$
    where $\delta\in\{0,1\}$ is a parameter indicating whether the trip is a passenger-trip ($\delta=1$) or a relocation-trip ($\delta=0$),
and the expected utility-to-go achieved by a driver located at $(l,\omega_t)$ before actions are allocated for the time period
is equal to
$$
    \vtglocation{l,\omega_t} = \bbE_{(r,\omega_t,\delta)\sim \bfg(l,\omega_t)}
               \left[ \vtgroute{r,\omega_t,\delta} \right],
$$
    where $\bfg(l,\omega_t)$ is the distribution over action-allocations for drivers located at $(l,\omega_t)$ induced by
    the platform matching decision vector $\bfg$.

We proceed via backwards induction and assume that $t=T$ is the final time period.  Let $\bff^*$ be the primal optimal solution
    for the dynamic optimization problem (\ref{eq:dynamic_optimization}), let $\bfeta^*$ be the dual optimal solution, and let 
    $\bfg$ be the matching vector specified by Algorithm \ref{alg:matching_details}.  Since $t=T$ is the final time period, we
    have the utility-to-go for any action-allocation $(r,\omega_t,\delta)$ is equaly to
    $$  \calU_{(r,\omega_t,\delta)} = \delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}.$$
    If the driver is allocated a dispatch trip, i.e. if $\delta=1$, then by complementary slackness and the above expression, we
    see the utility-to-go is equal to the dual variable associated with the driver's location: 
    $$\calU_{(r,\omega_t,1)} = \eta^*_{(l,\omega_t)}.$$
    In addition, if the trip is a relocation-trip, i.e. $\delta=0$, and $\bff^*$ allocates nonzero relocation trips to $(r,\omega_t)$,
    then the utility-to-go is still the dual variable value. In fact, the utility-to-go is equal to the dual variable value whenever
    the corresponding route has nonzero flow allocated to it under $\bff^*$:
    $$ \mbox{If $f^*_{(r,\omega_t,\delta)} > 0$: }\calU_{(r,\omega_t,1)} = \eta^*_{(l,\omega_t)}.$$

    Now we turn to bounding the probability of getting a dispatch $(r,\omega_t,\delta)$ which does not produce $\eta^*_{(l,\omega_t)}$ utility.
    Our above observation shows this probability is bounded by the probability of getting allocated an action $(r,\omega_t,\delta)$ which is 
    not allocated at all under $\bff^*$:
    $$
    \bbP_{(r,\omega_t,\delta)\sim\bfg(l,\omega_t)}\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)}\right) \leq 
    \sum_{(r,\omega_t,\delta) : f^*_{(r,\omega_t,\delta)} = 0} \frac{g_{(r,\omega_t,\delta)}}{S_{(l,\omega_t)}}.
    $$
    The number of dispatches to actions $(r,\omega_t,\delta)$ for which $\bff^*$ allocates $0$ drivers is bounded by the extent to which
    the number of dispatch requests was smaller than the expected number of dispatch requests.  That is, we have:
    $$
    \sum_{\substack{(r,\omega_t,\delta)\in N^+(l,\omega_t) \\ \mbox{s.t. }f^*_{(r,\omega_t,\delta)} = 0}} g_{(r,\omega_t,\delta)} \leq 
    \left|\sum_{\substack{(r,\omega_t)\in\\ N^+(l,\omega_t)}}\bar{d}^k_{(r,\omega_t)}- \frac{1}{k} - d^k_{(r,\omega_t)}\right|,
    $$
    where $\bar{d}^k_{(r,\omega_t)}$ is the expected number of dispatch requests under the SSP mechanism, and $d^k_{(r,\omega_t)}$ is the 
    realized number of dispatch requests.  We pick up an additive term of $\frac{1}{k}$ in each summand because this is the maximum penalty
    due to rounding on each route, since drivers in the large-market setting with parameter $k$ have size $1/k$.

    Thus, by our concentration property (\ref{eq:concentration}) for the large-market setting, we have the following upper bound holds
    with probability $1-\epsilon_k$:
    \begin{equation}
        \label{eq:good_event}
    \left|\sum_{\substack{(r,\omega_t)\in\\ N^+(l,\omega_t)}}\bar{d}^k_{(r,\omega_t)}- \frac{1}{k} - d^k_{(r,\omega_t)}\right|
    \leq \frac{h(\epsilon_k)}{k} \sum_{\substack{(r,\omega_t)\in\\ N^+(l,\omega_t)}}\bar{d}^k_{(r,\omega_t)} + \frac{|N^+(l,\omega_t)|}{k}
    \end{equation}

    Thus,
    \begin{align*}
        \bbP\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)}\right) &\leq (1-\epsilon_k)\bbP\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)} 
        | \mbox{(\ref{eq:good_event}) holds}\right) + \epsilon_k\\
        & \leq \bbP\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)}| \mbox{(\ref{eq:good_event}) holds} \right) + \epsilon_k.
    \end{align*}
    
    Next, in light of the above inequalities, we have the bound:
   \begin{align*} 
       \bbP\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)}| \mbox{(\ref{eq:good_event}) holds} \right) & \leq
\frac{1}{S_{(l,\omega_t)}}\left(\frac{h(\epsilon_k)}{k} \sum_{\substack{(r,\omega_t)\in\\ N^+(l,\omega_t)}}\bar{d}^k_{(r,\omega_t)} + \frac{|N^+(l,\omega_t)|}{k}
\right)\\
       & \leq \frac{h(\epsilon_k)}{k} + \frac{|N^+(l,\omega_t)|}{k S_{(l,\omega_t)}},
   \end{align*}
   where the second line follows because the total volume of expected dispatch demand is always smaller than the total supply available.

   \mccomment{at this final time period, there should be $0$ incentive to deviate from your action suggestion because if there is not
   enough demand we just send you to the route $(r,\omega_t)$ maximizing $-c_{(r,\omega_t)}$}
   Thus,
   $$
\bbP\left(\calU_{(r,\omega_t,\delta)} < \eta^*_{(l,\omega_t)}\right) \leq \frac{h(\epsilon_k)}{k} + \epsilon_k + O(1/k),
   $$
   which $\to 0$ as $k\to\infty$ by our large-market Assumption \ref{assn:large_market}.
   In addition, we obtain the following bound on the utility for being at this location:
   $$
    \eta_{(l,\omega_t)}^*(\bfS_t) \geq \calV_{(l,\omega_t)}(\bfS_t) \geq \eta_{(l,\omega_t)}^*(\bfS_t)\left(1 - \frac{h(\epsilon_k)}{k} + \epsilon_k + O(1/k)\right).
   $$
   Since $\eta_{(l,\omega_t)}^*(\bfS_t)$ is a constant that does not depend on $k$, this shows that the expected utility of being located at $(l,\omega_t)$ approaches
   $\eta^*(\bfS_t)$ as $k\to\infty$ in the final time period.

   For the induction step, assume $t<T$ and assume the result holds in future time periods.
   \mccomment{scratch notes below}
    $$
    \vtgroute{r,\omega_t,\delta}^k = \delta\rho_t(r,\omega_t) - c_{(r,\omega_t)} + \bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1})\right],
    $$
    $$
    \eta^*_{(l,\omega_t)} = \rho_t(r,\omega_t) - c_{(r,\omega_t)} + \bbE\left[\eta^*_{(l^+(r),\omega_{t+1})}(\bfS_{t+1}^*)\right],
    $$

    We have
    $$
\bbP_{(r,\omega_t,\delta)\sim\bfg(l,\omega_t)}\left(\delta\rho_t(r,\omega_t) \neq \rho_t(r,\omega_t)\right) \leq \frac{h(\epsilon_k)}{k} + \epsilon_k + O(1/k).
    $$
    and
    $$
\|\bfS_{t+1} - \bfS_{t+1}^*\| \leq \|\bfg - \bff^*\| + \|\bar{\bfM_{t+1}} - \bfM_{t+1}\|.
    $$

    Use concentration assumptions to show there are $\eta_k\to 0$ and 
    $$
   \bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1})\right] = (1-\eta_k)\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1}) | \mbox{close}\right] 
   + \eta_k \bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1}) | \mbox{not close}\right].
    $$
    Get the bounds
    $$\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1})\right] \geq (1-\eta_k)\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1}) | \mbox{close}\right] $$
    and
    $$\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1})\right] \leq (1-\eta_k)\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1}) | \mbox{close}\right] + \eta_k V_{max}(T-t). $$

    As $k\to\infty$ we have
    $$
(1-\eta_k)\bbE\left[\vtglocation{l^+(r),\omega_{t+1}}^k(\bfS_{t+1}) | \mbox{close}\right] \to \bbE\left[\eta^*_{(l^+(r),\omega_{t+1})}(\bfS_{t+1}^*)\right],
    $$
    and
    $$
\eta_k V_{max}(T-t)\to 0.
    $$


    \end{proof}
\subsection{Optimality and Incentive-Compatibility for the Stochastic Two-Level Model}
\input{opt_ic_two_level_model.tex}

\subsection{scrap from proof of thm 2}
\begin{proof}

    For each $(r,\omega_t)$ define
    $$
        p^k = \bbP^k(\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t))
    $$
    to be the probability that the SSP mechanism allocates an action-suggestion $(r,\omega_t,\delta)$ 
    for which $\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t)$ holds, to a driver positioned at $(l,\omega_t)$,
    in the large-market setting with size $k$.

    
    We will use backwards induction to show show that the following slightly stronger condition holds:
    For any supply-location vector $\bfS$,
    \begin{equation} 
        \label{eq:stronger_condition}
        -p_kc_{max}(T-t) \leq \calV_{(l,\omega_t)}^k(\bfS) - \eta^*_{(l,\omega_t)}(\bfS) \leq p_kV_{max}(T-t).
    \end{equation}
    In the above, $V_{max}$ is a uniform upper bound on the support of rider-value distributions, and $c_{max}$
    is a uniform upper bound on the cost of traversing a route.

    We will use the same analysis to establish the base case as well as the induction step for our backwards
    induction argument asserting that the property (\ref{eq:stronger_condition}) holds.  Fix a time period $t$
    and assume that the property (\ref{eq:stronger_condition}) holds for all larger values of $t$.
    In the base case where $t=T$ is the final time period, let us adopt the convention that $\eta^*_{(l,\omega_{T+1})}(\bfS_{T+1})=0$
    and $\calV_{(l,\omega_{T+1})}^k(\bfS_{T+1}) = 0$, so that our induction assumption trivially holds in the base case.

    Note that the complementary slackness conditions guarantee the following equality holds, for every outgoing
    route $(r,\omega_t)\in N^+(l,\omega_t)$ for which the primal optimal solution allocates nonzero flow, i.e.
    for which $f^*_{(r,\omega_t)} > 0$:
    $$
    \eta^*_{(l,\omega_t)}(\bfS_t) = \rho_t(r,\omega_t) - c_{(r,\omega_t)} + \eta^*_{(l^+(r),\omega_{t+1})}(\bfS^*_{t+1}),
    $$
    where $\bfS^*_{t+1}$ is the supply-location vector which would arise if driver-movement in time period $t$ was
    carried out exactly as according to $\bff^*$, and if the new-driver counts at time $t+1$ were equal to their means.
    The components of $\bfS^*_{t+1}$ are specified in equation (\ref{eq:fluid_supply_loc_vec}).

    In addition, note that the construction of the matching vector $\bfg$, as specified in Algorithm \ref{alg:matching_details},
    guarantees that actions $(r,\omega_t,\delta)$ are only allocated to routes $(r,\omega_t)$ for which the primal optimal
    solution allocates nonzero flow.  That is, for every matching vector $\bfg$ that the platform might produce,
    and for every action $(r,\omega_t,\delta)$ in the support of the action-allocation distribution $\bfg(l,\omega_t)$,
    the primal optimal solution allocations nonzero flow along $(r,\omega_t)$, i.e. $f^*_{(r,\omega_t)} > 0$.
    Since the complementary slackness conditions hold for every route satisfying this condition, we can take
    an expectation over action suggestions for free to conclude that the following holds with equality:
    \begin{equation}
    \eta^*_{(l,\omega_t)}(\bfS_t) = \bbE^k\left[\rho_t(r,\omega_t) - c_{(r,\omega_t)} + \eta^*_{(l^+(r),\omega_{t+1})}(\bfS^*_{t+1})\right],
    \end{equation}
    where the above expectation is with respect to the matching vector $\bfg$ and a random action allocation $(r,\omega_t,\delta)\sim\bfg(l,\omega_t)$.

    Taking the difference between equation (\ref{eq:utility_recursion}) and (\ref{eq:dual_var_recursion}),
    we obtain the following expression:
    $$
        \calV_{(l,\omega_t)}(\bfS_t) - \eta^*_{(l,\omega_t)}(\bfS_t) = \bbE^k\left[\delta\rho_t(r,\omega_t) - \rho_t(r,\omega_t)
                                                            + \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1}) - \eta^*_{(l^+(r),\omega_{t+1})}(\bfS^*_{t+1})\right].
    $$
    Let
    $$
        X_k = \bbE^k\left[\delta\rho_t(r,\omega_t) - \rho_t(r,\omega_t)\right]
    $$
    denote the expected difference in immediate reward collected, and let
    $$
    Z_k = \bbE^k\left[\eta^*_{(l^+(r),\omega_{t+1})}(\bfS_{t+1}) - \eta^*_{(l^+(r),\omega_{t+1})}(\bfS^*_{t+1}) \right]
    $$
    be the difference in optimal dual variable values under $\bfS^*_{t+1}$ and $\bfS_{t+1}$.
    Applying our induction hypothesis, we obtain the bound:
    \begin{align*}
        X_k + Z_k -p_k c_{max}(T-t+1) &\leq \calV_{(l,\omega_{t+1})}(\bfS_t) - \eta_{(l,\omega_{t+1})}^*(\bfS_t)\\
        &\leq X_k + Z_k + p_kV_{max}(T-t+1).
    \end{align*}

    .

    .

    .

    We proceed via backwards induction. In the final timestep $t=T$, the utility-to-go term in the equation (\ref{eq:utility_recursion}) for time $T+1$ is $0$,
    so the expected utility-to-go simplifies to
    $$
    \calV^k_{(l,\omega_t)}(\bfS_t) = \bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}\right].
    $$
    Let 
    $$
    p_k = \bbP^k(\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t))
    $$
    be the probability that the SSP mechanism allocates an action-suggestion $(r,\omega_t,\delta)$
    for which $\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t)$ holds, in the large-market setting with size $k$.
    Let us decompose the expected utility-to-go as follows:
    \begin{align*}
        \calV^k_{(l,\omega_t)}(\bfS_t) = &\bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}|\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t)\right]p_k\\
        &+                            \bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}|\delta\rho_t(r,\omega_t)=\rho_t(r,\omega_t)\right](1-p_k).
    \end{align*}
    Using the upper and lower bounds
    $$
    V_{max} \geq \delta\rho_t(r,\omega_t) - c_{(r,\omega_t)} \geq -c_{max}
    $$
    we obtain the following upper and lower bounds on the expected utility to go:
    \begin{align*}
        p_k V_{max} &\geq \calV^k_{(l,\omega_t)}(\bfS_t) - \bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}|\delta\rho_t(r,\omega_t)=\rho_t(r,\omega_t)\right](1-p_k)\\
        &\geq -p_k c_{max}.
    \end{align*}
    In Lemma \ref{lem:immediate_reward} we showed that $p_k$ is bounded as
    $$p_k\leq\frac{\epsilon_k}{S_{(l,\omega_t)}} + \frac{|N^+(l,\omega_t)|}{k S_{(l,\omega_t)}},$$
    so $p_k\to 0$ as $k\to \infty$.  Thus, it follows that
    $$
        \lim_{k\to\infty}\calV^k_{(l,\omega_t)}(\bfS_t) = \bbE^k\left[\rho_t(r,\omega_t) - c_{(r,\omega_t)}|\delta\rho_t(r,\omega_t)=\rho_t(r,\omega_t)\right].
    $$
    To conclude the base case, observe that routes $(r,\omega_t)$ are only included in the support of the SSP matching vector $\bfg$ if the fluid optimal solution $\bff^*$
    allocates nonzero flow along that route. Thus, complementary slackness states 
    $$\eta^*_{(l,\omega_t)}(\bfS_t) = \rho_t(r,\omega_t) - c_{(r,\omega_t)}$$
    holds for every route in the support of $\bfg$, from which we conclude
    $$
    \lim_{k\to\infty}\calV^k_{(l,\omega_t)}(\bfS_t) = \eta_{(l,\omega_t)}^*(\bfS_t)
    $$
    holds, as desired, in the base case $t=T$.

    For the induction step, assume the equation (\ref{eq:large_market_asymptotic_utility}) holds for larger values of $t$,
    keep the probabilities $p_k$ defined as above, and decompose the expected utility-to-go as follows:
    \begin{align*}
        \calV^k_{(l,\omega_t)}(\bfS_t) = &\bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}+ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1})|\delta\rho_t(r,\omega_t)\neq\rho_t(r,\omega_t)\right]p_k\\
    &+\bbE^k\left[\delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}+ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1})|\delta\rho_t(r,\omega_t)=\rho_t(r,\omega_t)\right](1-p_k).
    \end{align*}
    Using the upper and lower bounds
    $$ V_{max}(T-t) \geq \delta\rho_t(r,\omega_t) - c_{(r,\omega_t)}+ \calV^k_{(l^+(r),\omega_{t+1})}(\bfS_{t+1}) \geq -c_{max}(T-t)$$


\end{proof}


==> sspm_mechanism.tex <==
In this section we present our main contribution: the stochastic spatiotemporal pricing and matching mechanism (SSP).
The SSP mechanism dynamically readjusts its pricing and matching decisions to the realized state of the market
by re-solving the welfare-optimal concave program at each time period.

\mccomment{
Things to describe in this section:
\begin{itemize}
\item How the SSP mechanism computes prices at each timestep
\item What does using the SSP mechanism in the stochastic fluid model mean?
\item What does using the SSP mechanism in the stochastic two-level model mean?
\item What is an arbitrary equilibrium driver strategy in the stochastic fluid model? [maybe this goes in a different section]
\item What is an arbitrary approximate equilibrium driver strategy in the stochastic two-level model? 
[maybe this goes in a different section]
\end{itemize}
}

\mccomment{maybe the name ``SSP'' should change --- really the focus is on pricing, not matching.  Maybe
``SSTP''?  (Hongyao's mechanism is called ''STP'', for Stochastic SpatioTemporal mechanism)}
\begin{definition}[The Stochastic Spatiotemporal Pricing Mechanism]
\label{def:sspm_mechanism}
The stochastic spatiotemporal pricing mechanism (SSP) dynamically computes prices based on the realized market
state in each time period.
Specifically, at any time period $t$, the market state is specified by a scenario $\omega_t$ and
and a supply-location vector $\bfS_t$. 
The SSP computes an optimal solution $(\bff_t^*,\bfg_t^*)$
for the state-dependent optimization problem (\ref{eq:dynamic_optimization_recursive}) with respect to $\omega_t$ and $\bfS_t$.  
Every trip in the current time period
is then priced using the number of dispatches which occur under this optimal solution: for every origin-destination pair
$(o,d)\in\calL^2$ the SSP mechanism sets the price of a dispatch on the route $(o,d,\omega_t)$ to be
\begin{equation}
\label{eq:sspm_prices}
P_{(o,d,\omega_t)} = P_{(o,d,\omega_t)}(g^*_{(o,d,\omega_t)})=F_{(o,d,\omega_t)}^{-1}
\left(1-\frac{g^*_{(o,d,\omega_t)}}{\bar{D}_{(o,d,\omega_t)}}\right),
\end{equation}
where $F_{(o,d,\omega_t)}(\cdot)$ is the cumulative distribution function for the distribution of rider willingness-to-pay
values on the route $(o,d,\omega_t)$, $\bar{D}_{(o,d,\omega_t)}$ is the expected volume of riders who request a price for
the $(o,d,\omega_t)$ trip, and $g^*_{(o,d,\omega_t)}$ is the component of the optimal solution $\bfg_t^*$ specifying how
many dispatches should occur in the welfare-optimal solution along the route $(o,d,\omega_t)$.
\end{definition}

We assume the drivers play according to an equilibrium strategy-profile under the platform's pricing mechanism.
In the stochastic fluid model, we consider an exact equilibrium notion, defined in Definition \mccomment{ref}.
In the stochastic two-level model, we consider an approximate equilibrium notion, where the approximation error
vanishes as the population-size grows, defined in Definition \mccomment{ref}.  Our main theorem is that, under the
dynamic pricing policy provided by the SSP mechanism, every equilibrium strategy achieves optimal welfare.

\begin{theorem}[Welfare-robustness in the stochastic fluid model]
\label{thm:robust_eqlbm_fluid}
When the SSP mechanism is used to set prices in the stochastic fluid model, every equilibrium driver strategy achieves
optimal welfare.
\end{theorem}

\begin{theorem}[Approximate welfare-robustness in the stochastic two-level model]
\label{thm:robust_eqlbm_two_level}
When the SSP mechanism is used to set prices in the stochastic two-level model, every approximate equilibrium
achieves approximately optimal welfare.
\end{theorem}



\subsection{Proof of Theorem \ref{thm:robust_eqlbm_fluid}}
\input{fluid_robustness_proof}

%\subsection{Proof of Theorem \ref{thm:robust_eqlbm_two_level}}




==> sspm_section_copy.tex <==
In this section we describe our main algorithmic contribution, which we refer to as the
stochastic spatiotemporal pricing and matching (SSP) mechanism.
The SSP mechanism re-solves the fluid optimization problem based on the observed market state in each time period
and derives its prices and matching decisions from the computed optimum.

The SSP pricing policy is the same algorithm in both the fluid model and the two level model.  It is formally defined
below, in Definition \ref{def:sspm_pricing}.

\begin{definition}
\label{def:sspm_pricing}
At each time period $t$, the SSP pricing policy observes the market state $(\omega_t,\bfS_t)\in\calS_t$ and computes
the price along each route $(\ell,d)$ to be
$$
P_{(\ell,d)} = P_{(\ell,d,\omega_t)}(g^*_{(\ell,d)}) = F_{(\ell,d,\omega_t)}^{-1}\left(1-\frac{g^*_{(\ell,d)}}{\bar{D}_{(\ell,d,\omega_t)}}\right),
$$
where $(\bff^*,\bfg^*)\in F^*_{\omega_t}(\bfS_t)$ is an optimal solution for the associated fluid optimization problem.
\end{definition}

We defer the exact definition of the SSP matching process to Appendix \ref{appdx:matching_process_defn}. The matching process is defined so that 
two properties are satisfied: 1) we attempt to serve all dispatches, and only fail to do so if too many drivers are declining dispatches, and 2)
the only problem instances where the matching process results in dispatch volume $g_{(\ell,d)}$ strictly smaller than the optimal dispatch volume $g^*_{(\ell,d)}$
are problem instances where the drivers use a threshold $x_{(\ell,d)}$ that is strictly smaller than the acceptance threshold implied by the optimal solution.

\Xomit{
\input{matching_process_scratch.tex}
}

Theorem \ref{thm:robust_eqlbm_fluid}, below, states our welfare-robustness theorem for the SSP mechanism in the stochastic
fluid model.  The proof of Theorem \ref{thm:robust_eqlbm_fluid} is given in Section \ref{subsec:fluid_robustness_proof} and
additional details are given in Appendix \ref{appdx:approx_robustness_fluid_proof}.

\begin{theorem}[Welfare-robustness in the stochastic fluid model]
\label{thm:robust_eqlbm_fluid}
When the SSP mechanism is used to set prices in the stochastic fluid model, every equilibrium strategy profile achieves
optimal welfare, and every $\epsilon$-equilibrium strategy achieves $\epsilon'$-optimal welfare, where $\epsilon'$ goes to $0$ as $\epsilon$ goes to $0$.
\end{theorem}


Our welfare robustness theorem for the two-level model considers approximate equilibria whose approximation error vanishes as the population size
grows large.
We also restrict our attention to a subset of the state space in which the total volume of drivers in the network does not exceed a constant.
Let $\gamma > 0$ be a constant, and for each time period $t\in [T]$ define
$\calS_t(\gamma) = \{(\omega_t,\bfS_t)\in\Omega_t\times\calS : \sum_\ell S_\ell \leq \gamma\}$.
We assume that $\gamma$ is large enough so that the probability of the market state belonging to $\calS_t(\gamma)$ converges to $1$
as the population size grows large, regardless of the strategy profile. This is possible because there are only finitely many
points at which driverse can enter the networ, and all the driver-entry random variables converge to their mean as the population size
grows, and they have means which grow linearly in $k$ (see Assumption \ref{assn:entry_distributions}).  Therefore, we can pick any 
$\gamma$ larger than the maximum fluid driver volume over all scenarios.

Let $\alpha_k\geq 0$ be a sequence of error terms which converge to $0$ as $k\to\infty$, and for each $k\geq 1$
let $\calP^k$ be the set of $\alpha_k$-equilibrium strategy profiles for the two level model with population size $k$,
over the state space $\calS_t(\gamma)$.

For any strategy profile $\Pi$, let $W_{\omega_t}(\bfS_t;\Pi,k)$ denote the normalized expected welfare achieved by $\Pi$ from the
market state $(\omega_t,\bfS_t)$ under the population size parameter $k$.  A formal definition of $W_{\omega_t}(\bfS_t;\Pi,k)$ is
given in Appendix \ref{appdx:two_level_welfare_def}.

Theorem \ref{thm:robust_eqlbm_two_level}, below, states our welfare-robustness theorem for the SSP mechanism in the stochastic
two-level model.  The proof of Theorem \ref{thm:robust_eqlbm_two_level} is summarized in Section \ref{subsec:two_level_robustness_proof},
and additional details are given in Appendix \ref{appdx:approx_robustness_two_level_proof}.

\begin{theorem}[Approximate welfare-robustness in the stochastic two-level model]
\label{thm:robust_eqlbm_two_level}
When the SSP mechanism is used to set prices in the stochastic two-level model, every approximate equilibrium
achieves approximately optimal welfare.

Specifically, there exists a sequence of error terms $\epsilon_k\geq 0$ converging to $0$ as $k\to\infty$ such that the following
is true: for every $k\geq 1$, every $\alpha_k$-approximate equilibrium $\Pi\in\calP^k$, and every market state $(\omega_t,\bfS_t)\in\calS(\gamma)$,
we have
$$
\Phi_{\omega_t}(\bfS_t) - W_{\omega_t}(\bfS_t;\Pi,k) \leq \epsilon_k.
$$
\end{theorem}

We summarize the proof of Theorem \ref{thm:robust_eqlbm_fluid} below in Section \ref{subsec:fluid_robustness_proof},
and the proof of Theorem \ref{thm:robust_eqlbm_two_level} in Section \ref{subsec:two_level_robustness_proof}.
\subsection{Proof of Theorem \ref{thm:robust_eqlbm_fluid}}
\label{subsec:fluid_robustness_proof}
\input{new_fluid_robustness_proof}
%\subsection{Old Fluid Robustness Proof}
%\input{fluid_robustness_proof}

\subsection{Proof of Theorem \ref{thm:robust_eqlbm_two_level}}
\label{subsec:two_level_robustness_proof}
\input{two_level_robustness_proof}




==> state_dep_optimization.tex <==
In this section we describe the state-dependent optimization problem that the SSP mechanism resolves
at each time period to adapt its pricing and matching decisions to the realized state of the market.

There are two components of the market state on which the optimization problem depends: the top-level scenario,
and the spatial distribution of drivers.  The top-level scenario affects the network structure over which the
optimization problem is defined, and the spatial distribution of drivers affects the constants of the flow-conservation
constraints.

First, let's describe how the top-level scenario affects the network structure.  Consider any time period $t\in[T]$
and top-level scenario $\omega_t\in\Omega_t$.  From this point in the market dynamics, the welfare-optimal plan
only needs to specify actions for the remaining time periods $t'=t,t+1,\dots,T$, and the welfare-optimal plan
only needs to consider future scenarios that are compatible with $\omega_t$, i.e. we only need to consider the subtree
of the stochastic scenario tree indexed by the node $\omega_t$.
The resulting stochastic network structure has arcs $\calA_{\omega_t}^{\geq t}$ and $\calN_{\omega_t}^{\geq t}$
which we define below:
\begin{align}
    \calN_{\omega_t}^{\geq t}&= \left\{(\ell,\omega_\tau) :
    \ell\in\calL,\omega_\tau\in\Omega_{t:T}(\omega_t)
   \right\},\\
    \calA_{\omega_t}^{\geq t}&= \left\{(o,d,\omega_\tau) :
    (o,d)\in\calL^2,\omega_\tau\in\Omega_{\tau:T}(\omega_t)\right\}.
\end{align}
Figure \ref{fig:scenario_subnetwork} considers the stochastic network structure shown earlier, when we were first
defining the welfare-optimal stochastic flow problem, in Figure \ref{fig:example_network}.  In Figure \ref{fig:scenario_subnetwork}
we depict the scenario-induced subnetwork corresponding to the second time period under the rain scenario. \mccomment{There's
a mismatch between the time-index I use in text (which starts from $1$) and the time-index I use in the figure (which starts
from $0$).  I will update the figures to use time-indices which start from $1$.}

The optimization problem over the scenario-induced subnetwork $(\calN_{\omega_t}^{\geq t}, \calA_{\omega_t}^{\geq t})$
has the same structure as the optimization problem we defined in Section \ref{sec:opt_central} over the entire
stochastic flow network $(\calN,\calA)$: there are decision variables $f_{(o,d,\omega_t)}$ and $g_{(o,d,\omega_t)}$,
specifying total trip volume and dispatch trip volume, respectively, 
for each arc $(o,d,\omega_t)\in\calA$, there are constraints to ensure nonnegativity of these decision variables, and to
ensure that dispatch trip volume does not exceed total trip volume, and there are flow-conservation constraints for each
node in the subnetwork.

The second component of the market state on which the optimization problem depends is the current spatial distribution
of drivers, which affect the constants in the flow-conservation constraints for the state-dependent problem.
We use a supply-location vector
\begin{equation}
\bfS=(S_\ell : \ell\in\calL)
\end{equation}
to specify the volume of drivers $S_\ell$ positioned at each location $\ell\in\calL$ at the beginning of the time period.
Recall our assumption \mccomment{insert ref to assumption}, made without loss of generality, that all arcs in the network
take a single time period to traverse, so every driver is off-trip and positioned at one of the locations in $\calL$ at
the beginning of each time period.  The observed supply-volume $S_\ell$ is the amount of supply located at each
$(\ell,\omega_t)$ node in the $\omega_t$-induced subnetwork, so the resulting optimization problem incorporates the
value $S_\ell$ in the flow-conservation constraints for these nodes, resulting in the following flow-conservation 
constraints over the entire subnetwork:
\begin{equation}
\label{eq:flow_conservation_dynamic}
\begin{rcases}
    \sum_{d\in\calL} f_{(\ell,d,\omega_\tau)} =
    S_\ell & \mbox{if }\tau=t\\
    \sum_{d\in\calL} f_{(\ell,d,\omega_\tau)} 
    - \displaystyle\sum_{o\in\calL} f_{(o,\ell,\omega_{\tau-1})} =
    \bar{M}_{(\ell,\omega_\tau)} & \mbox{if }\tau > t
\end{rcases}
\ 
\forall (\ell,\omega_\tau)\in\calN_{\omega_t}^{\geq t}.
\end{equation}

The objective function for the state-dependent optimization problem is analogous to the objective function 
(\ref{eq:static_objective}) of the static optimization problem: for feasible decision variables 
$\bff,\bfg\in\bbR_+^{\calA_{\omega_t}^{\geq t}}$ we define $W_{\omega_t}(\bff,\bfg)$ to be the expected welfare
generated by the marketplace over the remaining time periods, with respect to the randomness in the stochastic scenario
(sub-)tree:
 \mccomment{this is the first time I use the phrase ``static
optimization problem'' --- make a decision about whether to use this terminology throughout, or not use it here}
\begin{equation}
    W_{\omega_t}(\bff,\bfg) = \sum_{\substack{\omega_\tau\in\\ \Omega_{t:T}(\omega_t)}}\bbP(\omega_\tau)
    \left[
        \sum_{\substack{(o,d)\in\\\calL^2}} U_{(o,d,\omega_\tau)}(f_{(o,d,\omega_\tau)}, g_{(o,d,\omega_\tau)}) - 
        \sum_{\ell\in\calL} A\left(\bfg^T\bfone_{(\ell,\omega_\tau)},\bff^T\bfone_{(\ell,\omega_\tau)}\right)
        \right].
\end{equation}
We also introduce the notation $\calW_{\omega_t}(\bfS)$ to mean the optimal value of the state-dependent optimization problem
associated with the top-level scenario $\omega_t$, as a function of the observed supply-location vector $\bfS$.
The state-dependent welfare-optimization problem is defined below:
\begin{align}
 \sup_{\bff, \bfg} &\ \ \   W_{\omega_t}(\bff,\bfg) & \label{eq:dynamic_optimization}\\
    \mbox{subject to} & \nonumber\\ 
    & f_{(o,d,\omega_\tau)} \geq 0 \ &\forall (o,d,\omega_\tau)\in\calA_{\omega_t}^{\geq t}\nonumber\\
    & g_{(o,d,\omega_\tau)} \geq 0 \ &\forall (o,d,\omega_\tau)\in\calA_{\omega_t}^{\geq t} \nonumber\\
    & f_{(o,d,\omega_\tau)} \geq g_{(o,d,\omega_t)} \ &\forall (o,d,\omega_t)\in\calA_{\omega_t}^{\geq t} \nonumber\\
    &\begin{rcases}
        \sum_{d\in\calL} f_{(\ell,d,\omega_\tau)} =
        S_\ell & \mbox{if }\tau=t\\
        \sum_{d\in\calL} f_{(\ell,d,\omega_\tau)} 
        - \sum_{o\in\calL} f_{(o,\ell,\omega_{\tau-1})} =
        \bar{M}_{(\ell,\omega_\tau)} & \mbox{if }t > 1
    \end{rcases} \ & \forall (\ell,\omega_\tau)\in\calN_{\omega_t}^{\geq t}\nonumber
\end{align}
The function $\calW_{\omega_t}(\bfS)$, mapping the observed supply-location vector to the value of the state-dependent
optimization problem, is specified below:
\begin{equation}
\calW_{\omega_t}(\bfS) \equiv \mbox{Optimal value of (\ref{eq:dynamic_optimization}) with respect to }\omega_t\mbox{ and }\bfS.
\end{equation}


\begin{figure}[t]
    \centering
\includegraphics[width=\textwidth, height=8cm, keepaspectratio]{figures/scenario_induced_subnetwork}
    \caption{The subnetwork induced at time $1$ under the rain scenario.}
    \label{fig:scenario_subnetwork}
\end{figure}


For the remainder of this section we discuss the structure of the state-dependent optimization problem 
(\ref{eq:dynamic_optimization}). First, we present an equivalent recursive characterization of the optimization problem,
which breaks the problem down into the sum of the welfare from the actions in the current time period and the
optimal welfare of the expected state in the next time period.  To state this recursive characterization, we introduce
notation to characterize the state of the marketplace at the next time period.

Let $\calA_{\omega_t}^t$ be the set of arcs in the $\omega_t$-induced subnetwork which originate in the $t$th time period,
i.e.
$$
\calA_{\omega_t}^t=\left\{(o,d,\omega_t) : (o,d)\in\calL^2\right\}
$$
and let $\bff=(f_{(o,d,\omega_t)}:(o,d,\omega_t)\in\calA_{\omega_t}^t$ be a decision vector which encodes trip volumes
only for arcs which occur under the time-scenario $\omega_t$.
For each scenario $\omega_{t+1}\in\Omega_{t+1}(\omega_t)$ in the subsequent time period and 
in the subtree indexed by $\omega_t$, define $\bfS_{\omega_{t+1}}(\bff)=(S_{(\ell,\omega_{t+1})}(\bff))$ to be the
supply-location vector which arises under the time-scenario $\omega_{t+1}$, assuming the drivers move according to $\bff$
under the time-scenario $\omega_t$.  Each component of $\bfS_{\omega_{t+1}}(\bff)$ is defined as the sum of the 
total incoming supply to each node as well as the expected number of drivers who enter the network positioned at that node:
$$
S_{(\ell,\omega_{t+1})}(\bff) = \bar{M}_{(\ell,\omega_{t+1})} + \sum_{o\in\calL} f_{(o,\ell,\omega_t)},
$$
where $\bar{M}_{(\ell,\omega_{t+1})}$ is the expected volume of drivers who enter the market at the LT-scenario
 $(\ell,\omega_{t+1})$.
We define $\Phi_{\omega_{t}}(\bff)$ to be the optimal welfare achievable over future time periods, given
a choice of trip volumes $\bff\in\bbR_+^{\calA_{\omega_t}^t}$ under the time-scenario $\omega_t$:
\begin{equation}
\label{eq:continuation_welfare}
\Phi_{\omega_{t}}(\bff) = \bbE_{\omega_{t+1}}\left[\calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff)\mid\omega_t\right].
\end{equation}

The objective function for the recursive characterization of the state-dependent optimization problem,
takes as inputs total trip volumes $\bff\in \bbR_+^{\calA_{\omega_t}^t}$ and dispatch trip volumes
$\bfg\in\bbR_+^{\calA_{\omega_t}^t}$, only for arcs which correspond exactly to the scenario $\omega_t$.
The recursive objective function $W^R_{\omega_t}(\bff,\bfg)$ is then equal to the utility collected at time $t$
under $\bff$ and $\bfg$ plus the optimal utility from the expected state at future time periods:
\begin{equation}
    W^R_{\omega_t}(\bff,\bfg) = 
        \sum_{\substack{(o,d)\in\\\calL^2}} U_{(o,d,\omega_t)}(f_{(o,d,\omega_t)}, g_{(o,d,\omega_t)}) - 
        \sum_{\ell\in\calL} A\left(\bfg^T\bfone_{(\ell,\omega_t)},\bff^T\bfone_{(\ell,\omega_t)}\right)
         + 
    \Phi_{\omega_t}(\bff).
\end{equation}
The recursive optimization formulation then maximizes $W^R_{\omega_t}(\bff,\bfg)$ over $\bff,\bfg\in\calA_{\omega_t}^t$
\begin{align}
 \sup_{\bff, \bfg\in\bbR_+^{\calA_{\omega_t}^t}} &\ \ \   W^R_{\omega_t}(\bff,\bfg) & 
\label{eq:dynamic_optimization_recursive}\\
    \mbox{subject to} & \nonumber\\ 
    & f_{(o,d,\omega_t)} \geq 0 \ &\forall (o,d,\omega_t)\in\calA_{\omega_t}^{ t}\nonumber\\
    & g_{(o,d,\omega_t)} \geq 0 \ &\forall (o,d,\omega_t)\in\calA_{\omega_t}^{ t} \nonumber\\
    & f_{(o,d,\omega_t)} \geq g_{(o,d,\omega_t)} \ &\forall (o,d,\omega_t)\in\calA_{\omega_t}^{ t} \nonumber\\
    &
        \sum_{d\in\calL} f_{(\ell,d,\omega_t)} =
        S_\ell 
    \ & \forall (\ell,\omega_t)\in\calN_{\omega_t}^{ t}.\nonumber
\end{align}
The following Lemma states the two formulations (\ref{eq:dynamic_optimization}) and (\ref{eq:dynamic_optimization_recursive})
are equivalent.
\begin{lemma}
For any supply-location vector $\bfS\in\bbR^\calL_+$, the fully expanded optimization problem (\ref{eq:dynamic_optimization})
with respect to $\bfS$ has the same optimal value as the recursive optimization problem (\ref{eq:dynamic_optimization_recursive})
with respect to $\bfS$.
\end{lemma}

The following Lemma states the Lagrangian optimality conditions we get for the state-dependent optimization
problem (\ref{eq:dynamic_optimization}).  These optimality conditions are analogous to the optimality conditions
described in Lemma \ref{lem:optimality_conditions}.

\mccomment{This lemma is very similar to Lemma \ref{lem:optimality_conditions} --- there should be a way to simplify the
discussion of optimality conditions here}
\begin{lemma}
    \label{lem:dynamic_optimality_conditions}
    Let $\bff,\bfg\in\bbR_+^{\calA_{\omega_t}^t}$ be a feasible solution to the recursive formulation of the
    state-dependent welfare-optimization problem (\ref{eq:dynamic_optimization_recursive}).
    Then $(\bff,\bfg)$ is an optimal solution if and only if there exist dual variables:
    \begin{itemize}
        \item $\alpha_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA_{\omega_t}^{ t}$,
        \item $\beta_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA_{\omega_t}^{ t}$,
        \item $\gamma_{(o,d,\omega_t)}\geq 0$ for all $(o,d,\omega_t)\in\calA_{\omega_t}^{ t}$,
        \item $\eta_{(\ell,\omega_t)}$ for all $(\ell,\omega_t)\in\calN_{\omega_t}^{ t}$,
    \end{itemize}
    for which the following conditions are satisfied:
    \begin{enumerate}
        \item Complementary Slackness:
            \begin{align*}
            f_{(o,d,\omega_t)}\alpha_{(o,d,\omega_t)} = 0 &\quad \forall (o,d,\omega_t)\in\calA_{\omega_\tau}^{ t},\\
            g_{(o,d,\omega_t)}\beta_{(o,d,\omega_t)} = 0 &\quad \forall (o,d,\omega_t)\in\calA_{\omega_t}^{ t},\\
            (g_{(o,d,\omega_t)}-f_{(o,d,\omega_t)})\gamma_{(o,d,\omega_t)} = 0 
&\quad \forall (o,d,\omega_t)\in\calA_{\omega_t}^{ t}.
            \end{align*}
        \item Stationarity.  For all $(o,d,\omega_t)\in\calA_{\omega_t}^{ t}$, the following equations hold:
            \begin{align}
                P_{(o,d,\omega_t)}(g_{(o,d,\omega_t)}) -C\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}}
 &=
                        \gamma_{(o,d,\omega_t)} - \beta_{(o,d,\omega_t)} .\label{eq:dynamicopt_stationarity_g}\\
            -c_{(o,d,\omega_t)}  +\frac{C}{2}\left(\frac{\bfg^T\bfone_{(o,\omega_t)}}{\bff^T\bfone_{(o,\omega_t)}}\right)^2 &=
                \eta_{(o,\omega_t)} - \partial f_{(o,d,\omega_t)}\Phi_{\omega_t}(\bff) - \alpha_{(o,d,\omega_t)} - 
            \gamma_{(o,d,\omega_t)}\label{eq:dynamicopt_stationarity_f} .
            \end{align}
where     \end{enumerate}
\end{lemma}
In equation (\ref{eq:dynamicopt_stationarity_f}) above, 
$-\partial f_{(o,d,\omega_t)}\Phi_{\omega_t}(\bff)$ is the subradient of the negative 
optimal welfare continuation value function (\ref{eq:continuation_welfare}).
From the definition fo the continuation welfare function, we have the following equality:
$$
-\partial f_{(o,d,\omega_t)}\Phi_{\omega_t}(\bff) = 
-\bbE_{\omega_{t+1}}\left[\partial f_{(o,d,\omega_t)} \calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))\mid\omega_t\right].
$$
The following Lemma characterizes the subgradient of $-\calW_{\omega_t}(\bfS)$ in terms of dual variables.
\begin{lemma}
\label{lem:unique_dual}
Fix a time-scenario $\omega_t$ and a supply-location vector $\bfS$. Let $\ell\in\calN$ be any location for which there is
nonzero supply volume under $\bfS$, i.e. $S_\ell>0$. Then the value of the optimal dual variable $\eta_{(\ell,\omega_t)}$
for the associated with the flow-conservation constraint at node $(\ell,\omega_t)$, in the state-dependent optimization
problem (\ref{eq:dynamic_optimization_recursive}) is unique.  Moreover, the optimal welfare value function $\calW_{\omega_t}(\bfS)$
is differentiable at $\bfS$ with respect to $S_\ell$, and the partial derivative is equal to the unique dual variable value
for the corresponding flow conservation constraint:
\begin{equation}
\frac{\partial}{\partial S_\ell} \calW_{\omega_t}(\bfS) = \eta_{(\ell,\omega_t)}.
\end{equation}
\end{lemma}

Lemma \ref{lem:unique_dual} provides us a characterization of the continuation welfare function by applying
the chain rule:
\begin{align}
-\partial f_{(o,d,\omega_t)}\Phi_{\omega_t}(\bff) &= 
-\bbE_{\omega_{t+1}}\left[\partial f_{(o,d,\omega_t)} \calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))\mid\omega_t\right]\\
&=
-\bbE_{\omega_{t+1}}\left[\frac{\partial}{\partial S_d} \calW_{\omega_{t+1}}(\bfS_{\omega_{t+1}}(\bff))\mid\omega_t\right]\\
&= 
-\bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right],
\end{align}
where $\eta_{(d,\omega_{t+1})}$ is the optimal dual variable for hte $(d,\omega_{t+1})$ flow-conservation constraint,
for the state-dependent optimizationn problem with respect to $\omega_{t+1}$ and $\bfS_{\omega_{t+1}}(\bff)$.
Note this characterization is analogous to the optimality conditions we had in the static formulation (\ref{eq:stationarity_f}).


Finally, we conclude this section with the following lemma, showing that the state-dependent optimal welfare function
has continuous partial derivatives.
\begin{lemma}
\label{lem:cts_partials}
Fix any time-scenario $\omega_t$ and let $\bfS\in\bbR_+^\calL$ be any supply-location vector. Let $\ell\in\calL$ be
any location and assume there is nonzero supply-volume positioned at $\ell$ under the vector $\bfS$, i.e. assume $S_\ell>0$.
Then $\frac{\partial}{\partial S_\ell}\calW_{\omega_t}(\bfS)$ is continuous at $\bfS$.
\end{lemma}
We defer the proof of Lemma \ref{lem:cts_partials} to Appendix \mccomment{insert}.


We conclude this section with a brief remark about computational tractability of solving the optimization problems 
(\ref{eq:dynamic_optimization}).  Because it is a concave maximization problem we can compute an (approximately) 
optimal solution in time that is polynomial in the size of the problem.  
However, the size of the problem scales with the total number of scenarios in our scenario tree,
 and in most realistic situations the total number of scenarios will depend exponentially on the number of time periods. 
 Despite this exponential dependence, preliminary computational results suggest that problems with thousands of scenarios
 and over ten time periods are computationally tractable.


==> state_dep_partials/approx_ic_results.tex <==
asdf


==> static_eqlbm_proof.tex <==
\begin{proof}
Let $(\bff,\bfg)$ be an optimal solution to the welfare-optimal concave program (\ref{eq:static_optimization}), and consider any time-scenario
$\omega_t\in\Omega_t$.  Assume the drivers have taken trips according to the solution $(\bff,\bfg)$ at all previous time periods.
Consider a driver positioned at location $\ell$, whose sampled idiosyncratic disutility is $C^{ID}$, and who is allocated a trip towards destination
$d\in\calL$, with $\delta\in\{0,1\}$ indicating whether or not their trip includes a passenger.  We will show the static equilibrium
condition (\ref{eq:static_eqlbm_condition}) holds by considering the case where the driver is allocated a dispatch-trip ($\delta=1$) and the
case where the driver is allocated a relocation-trip ($\delta=0$) separately.

We consider first the case  where the driver is allocated a relocation-trip ($\delta=0$).  Recall that $\calZ(\ell,\omega_t)$ is the set of trips
to which a driver positioned at $\ell$ under the time-scenario $\omega_t$ can deviate: $\calZ(\ell,\omega_t)$ includes all relocation-trips, and the subset
of dispatch trips for which there is excess rider demand.  Note that the static pricing mechanism sets prices (\ref{eq:static_prices}) under which
the resulting rider demand is exactly equal to the volume of dispatch trips we serve on each route under the welfare-optimal solution.  Therefore, under
the static pricing mechanism, no trips have excess rider demand, so the set
of trips to which a driver can deviate is simply the set of relocation-trips.

Now, suppose a driver positioned at $\ell$ is allocated a relocation-trip towards location $d\in\calL$, but they are considering deviating from the welfare-optimal
solution and taking a relocation-trip towards some alternative destination $d'\in\calL$.
Using the result from Lemma \ref{lem:dual_variable_utility}, relating the utility-to-go at a node with the dual variable associated with the flow-conservation
constraint for that notde, the utility-to-go for the two actions can be expressed as follows:
\begin{align*}
    \calQ(\ell,d,\omega_t,0) &= -c_{(\ell,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right],\\
    \calQ(\ell,d',\omega_t,0)&= -c_{(\ell,d',\omega_t)} + \bbE_{\omega_{t+1}}\left[\eta_{(d',\omega_{t+1})}\mid\omega_t\right],
\end{align*}
where $\eta_{(d,\omega_{t+1})}$ and $\eta_{(d',\omega_{t+1})}$ are optimal dual variables associated with the flow-conservation constraints at $(d,\omega_{t+1})$
and $(d',\omega_{t+1})$, respectively.
(See Lemma \ref{lem:optimality_conditions}).

Now, since the driver under consideration was allocated a relocation-trip towards destination $d$, we know that the decision variable $f_{(\ell,d,\omega_t)}$, which
specifies the total volume of (relocation- + dispatch-) trips along the route $(\ell,d,\omega_t)$ is greater than $0$, and we also know that it must be strictly
larger than the decision variable $g_{(\ell,d,\omega_t)}$, which species the total volume of dispatch-trips along $(\ell,d,\omega_t)$.
Therefore, the dual variable associated with the constraints $f_{(\ell,d,\omega_t)}\geq 0$ and $g_{(\ell,d,\omega_t)}\leq f_{(\ell,d,\omega-t)}$ are both $0$,
by virtue of the complementary slackness conditions, so the optimality conditions (\ref{eq:stationarity_f}) established in Lemma \ref{lem:optimality_conditions}
assert the following:
$$
\eta_{(\ell,\omega_t)} - \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right) = 
\bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d,\omega_t)}.
$$
Therefore, the utility-to-go of the relocation-trip towards destination $d$ can be expressed in terms of the dual variable associated with
the origin node as follows:
\begin{equation}
    \label{eq:relocation_trip_utility}
\calQ(\ell,d,\omega_t,0) = \eta_{(\ell,\omega_t)} - \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right).
\end{equation}

On the other hand, the dual variables associated with the constraints $f_{(\ell,d',\omega_t)}\geq 0$ and $g_{(\ell,d',\omega_t)}\leq f_{(\ell,d',\omega_t)}$
for the alternative destination $d'$ can be either zero or nonzero, because $d'$ is an arbitrary alternate destination.  Thus, the optimality conditions
(\ref{eq:stationarity_f}) provide the following upper bound on the utility-to-go associated with a relocation-trip towards $d'$:
\begin{align*}
    \eta_{(\ell,\omega_t)} - \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right) &= 
    \bbE_{\omega_{t+1}}\left[\eta_{(d',\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d',\omega_t)} + \alpha_{(\ell,d',\omega_t)} + \gamma_{(\ell,d',\omega_t)} \\
    & \geq \bbE_{\omega_{t+1}}\left[\eta_{(d',\omega_{t+1})}\mid\omega_t\right] - c_{(\ell,d',\omega_t)}\\
    &= \calQ(\ell,d',\omega_t,0).
\end{align*}
Therefore, 
$$
\calQ(\ell,d,\omega_t,0) \leq \calQ(\ell,d',\omega_t,0)
$$
holds, establishing the static equilibrium condition (\ref{eq:static_eqlbm_condition}) in the case of a relocation trip.

For the next and final case, suppose the driver is allocated a dispatch-trip towards destination $d$.  In the previous case we established 
(\ref{eq:relocation_trip_utility}) an upper bound 
$$\eta_{(\ell,\omega_t)} - \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)$$
on the utility-to-go that any relocation-trip originating from $\ell$ at time-scenario $\omega_t$ generates, so it suffices to show
that every driver serving a dispatch trip obtains at least this much utility.

Recall that we assume drivers are preferentially allocated dispatch trips based on their sampled idiosyncratic disutility, which means there
exists a threshold for which idiosyncratic disutilities smaller than the threshold value are allocated a dispatch and disutilities larger than the threshold
are allocated a relocation trip. For drivers positioned at the location-time-scenario $(\ell,\omega_t)$, 
the threshold is the $\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}$-quantile of the add-passenger
disutility distribution. Specifically, a driver positioned at $(\ell,\omega_t)$ with sampled idiosyncratic add-passenger disutility value $C^{ID}$
is allocated a dispatch trip if and only if
$$
C^{ID} \leq C\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}.
$$

Now, invoking Lemma \ref{lem:dual_variable_utility} which connects the utility-to-go of a node with the dual variable associated to that node,
the idiosyncratic utility (\ref{eq:idiosyncratic_dispatch_utility}) the driver collects for serving a dispatch trip towards location $d$
is equal to the following:
$$
\calQ(\ell,d,\omega_t,1,C^{ID}) = P_{(\ell,d,\omega_t)} -C^{ID} - c_{(\ell,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right].
$$
Since we are assuming the dispatch trip towards destination $d$ is allocated under the welfare-optimal solution, we know the  decision variable $g_{(\ell,d,\omega_t)}$,
specifying the volume of dispatch trips towards destination $d$, is nonzero, and hence by the complementary slackness conditions the dual variable associated with
the nonnegativity constraint $g_{(\ell,d,\omega_t)} > 0$ is itself zero. Therefore, the optimality condition (\ref{eq:stationarity_g}) established in Lemma
\ref{lem:optimality_conditions} state the following:
$$
P_{(\ell,d,\omega_t)} - C\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}} = \gamma_{(\ell,d,\omega_t)} \geq 0,
$$
where $\gamma_{(\ell,d,\omega_t)}$ is the dual variable for the $g_{(\ell,d,\omega_t)}\leq f_{(\ell,d,\omega_t)}$ constraint.
That is, the price charged on the route $(\ell,d,\omega_t)$ is at least as large as the maximum add-passenger disutility among any driver who serves a dispatch.

Therefore, since the idiosyncratic add-passenger disutility $C^{ID}$ is at most as large as the threshold disutility, we deduce the following
lower bound on the idiosyncratic dispatch trip utility-to-go:
$$
\calQ(\ell,d,\omega_t,1,C^{ID}) \geq \gamma_{(\ell,d,\omega_t)} - c_{(\ell,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right].
$$
However, since the dual variable for the constraint $f_{(\ell,d,\omega_t)}\geq 0$ must also be zero, the optimality condition (\ref{eq:stationarity_f})
simplifies to the following expression:
$$
\eta_{(\ell,\omega_t)} - \frac{C}{2}\left(\frac{\bfg^T\bfone_{(\ell,\omega_t)}}{\bff^T\bfone_{(\ell,\omega_t)}}\right)
=\gamma_{(\ell,d,\omega_t)} - c_{(\ell,d,\omega_t)} + \bbE_{\omega_{t+1}}\left[\eta_{(d,\omega_{t+1})}\mid\omega_t\right].
$$
Therefore, we conclude the idiosyncratic dispatch utility-to-go $\calQ(\ell,d,\omega_t,1,C^{ID})$ is at least as large on the
relocation-trip utility-to-go (\ref{eq:relocation_trip_utility}), establishing the static equilibrium condition (\ref{eq:static_eqlbm_condition}) in the
case of a dispatch-trip.\end{proof}



==> stochastic_programming_lemma.tex <==

Consider a generic convex optimization problem
\begin{equation}
\label{eq:primal}
\inf\left(\calC(\bff) : g_i(\bff) = 0, 1\leq i\leq m, \bff \geq 0 \right),
\end{equation}
for a decision variable $\bff=(f_j:1\leq j\leq n)$, a 
continuously differentiable and convex cost function $\calC(\bff)$ and a continuously differentiable convex equality constraint
functions $g_i(\bff)$.
Let 
$$
L(\bff,\bfeta,\bfalpha) = \calC(\bff) + \sum_i\eta_ig_i(\bff) - \sum_j \alpha_j f_j
$$
be the Lagrangian function for our problem, let
$$
\Phi(\bfeta,\bfalpha) = \inf_{\bff} L(\bff,\bfeta,\bfalpha)
$$
be the Lagrangian dual function, and let
$$
\sup_{\bfeta,\bfalpha}\left(\Phi(\bfeta,\bfalpha) : \bfalpha\geq 0\right)
$$
be the dual optimization problem.  Let $\bff^*$ be
a primal optimal solution and let $(\bfeta^*,
\bfalpha^*)$ be a dual optimal solution.  Weak
duality states $\calC(\bff^*)\geq \Phi(\bfeta^*,
\bfalpha^*)$, and when strong duality holds we have
$\calC(\bff^*) = \Phi(\bfeta^*,\bfalpha^*)$.

When strong duality holds, the following conditions
are sufficient to certify the optimality of $\bff^*$:
\begin{itemize}
\item Stationarity: $$
0 = \nabla\calC(\bff^*) + \sum_i\eta^*_i\nabla g_i(\bff^*)
- \sum_j \alpha^*_j\bfone_j,
$$
where $\bfone_j$ is an $n$-dimensional vector with a $1$ in the $j$th
component and $0$ elsewhere.
\item Complementary slackness:
$$
\alpha^*_j f^*_j = 0
$$
for all $1\leq j\leq n$.
\end{itemize}
To state the optimality conditions more succinctly, 
for each coordinate $j=1,\dots,n$ define the function 
$$
D_j(\bff,\bfeta) = \frac{\partial}{\partial f_j}\calC(\bff)
+ \sum_{i=1}^m \eta_i \frac{\partial}{\partial f_j}g_i(\bff).
$$
The stationarity and complementary slackness conditions above
are equivalent to the following conditions.  For all $j=1,\dots,n$
we have
$$
D_j(\bff^*,\bfeta^*)\geq 0,
$$
and 
$$
f_j^*D_j(\bff^*,\bfeta^*) = 0.
$$


\begin{lemma}
\label{lem:generic_cvxopt}
Assume strong duality holds for the primal problem (\ref{eq:primal}),
assume the cost function $\calC(\cdot)$ is continuously differentiable,
and assume the equality constraints $g_1(\cdot), \dots, g_m(\cdot)$ are all linear functions with nonnegative coefficients.
Let $(\bfh_k:k=1,2,\dots)$ be a sequence of $n$-dimensional
random variables, let $(\bfeta_k : k=1,2,\dots)$ be a deterministic
sequence of $m$-dimensional vectors, and assume the following
properties hold:
\begin{itemize}
    \item $\bfh_k\geq 0$ holds with probability $1$ for all $k$.
    \item $g_i(\bfh_k)$ converges in probability to $0$ as $k\to\infty$, for all equality constraints $i=1,\dots,m$.
    \item $h_j^kD_j(\bfh_k,\bfeta_k)$ converges in probability to $0$
    as $k\to\infty$,
    where $h_j^k$ is the $j$th component of $\bfh_k$,
    for all $j=1,\dots,n$.
    \item $\min(D_j(\bfh_k,\bfeta_k), 0)$ converges in probability to
    $0$ as $k\to\infty$, for all $j=1,\dots,n$.
    
\end{itemize}
Then the costs $\calC(\bfh_k)$
converge in probability to the optimal cost $\calC(\bff^*)$ as
$k\to\infty$.
\end{lemma}

\begin{proof}
Let $\tilde{\bfh}_k$ be the projection of $\bfh_k$ onto the subset of $\bbR^n$ induced by the equality constraints $g_1(\bfh)=0, \dots,
g_m(\bfh)=0$.
By our assumption that $g_i(\bfh_k)\to 0$ converges in probability, and by the continuity of $\calC(\cdot)$, it follows that the cost difference
$\calC(\bfh_k) - \calC(\tilde{\bfh}_k)\to 0$ converges in probability.
In addition, from our assumption that the cost function $\calC(\cdot)$
is continuously differentiable and the constraint functions
$g_1(\cdot),\dots,g_m(\cdot)$ are linear, it follows that the
function $D_j(\cdot,\cdot)$ is continuous.
Hence, the limits
$$
\tilde{h}_j^kD_j(\tilde{\bfh}_k,\bfeta_k) \to 0,\ \ \ 
\min(D_j(\tilde{\bfh}_k,\bfeta_k), 0)\to 0
$$
both still hold for the projected random variables $\tilde{\bfh}_k$.

Next, for an arbitrary feasible solution $\bfh$, define the set of feasible
dual variables with respect to $\tilde{\bfh}_k$:
$$
\calF(\bfh) = \left\{\bfeta\in\bbR^m : D_1(\bfh,\bfeta)\geq 0,
\dots, D_n(\bfh,\bfeta)\geq 0\right\}.
$$
We claim that $\calF(\bfh)$ is always nonempty under our assumption
that the constraint functions $g_1(\cdot),\dots,g_m(\cdot)$ are
linear functions with nonnegative coefficients.  Under this assumption,
each of the functions $D_j(\bfh,\bfeta)$ is linear in $\bfeta$, i.e.
$$
D_j(\bfh,\bfeta) = \frac{\partial}{\partial h_j}\calC(\bfh) + \bfeta^T\bm{c}_j,
$$
where $\bm{c}_j$ is a nonnegative $m$-dimensional vector consisting of
$\frac{\partial}{\partial h_j}g_i(\cdot)$ in the $i$th component.
Thus, the set $\calF(\bfh)$ is the intersection of $n$ half-spaces
$\bfeta^T\bm{c}_1\geq \frac{\partial}{\partial h_1}\calC(\bfh),
\dots \bfeta^T\bm{c}_n\geq \frac{\partial}{\partial h_n}\calC(\bfh)$.
This intersection is nonempty because all the coefficient vectors
$\bm{c}_j$ are nonnegative.

Next, fix an iterate $k$, condition on a realization of
the projection $\tilde{\bfh}_k$, and let $\tilde{\bfeta}_k$ be
the projection of $\bfeta_k$ onto the set of feasible duals
$\calF(\tilde{\bfh}_k)$.  From the assumption that
$$
\min(D_j(\tilde{\bfh}_k,\bfeta_k), 0)\to 0
$$
converges in probability it follows that the sequence $(\bfeta_k)$
approaches the set of feasible duals, hence the projections 
$\tilde{\bfeta}_k$ approach $\bfeta_k$ as $k\to\infty$.  That is,
$$
\|\tilde{\bfeta}_k - \bfeta_k\|\to 0
$$
converges in probability. By continuity of $D_j(\cdot,\cdot)$,
it follows 
$$
\tilde{h}_j^kD_j(\tilde{\bfh}_k,\tilde{\bfeta}_k) \to 0,
$$
both converge in probability.
Now, for each iterate $k$ define the $n$-dimensional dual
variable $\bfalpha_k$ by setting the $j$th component to be
$$
\alpha_j^k = D_j(\tilde{\bfh}_k, \tilde{\bfeta}_k).
$$
Since $\tilde{\bfeta}_k$ is a feasible dual vector
with respect to $\tilde{\bfh}_k$, it follows that $\bfalpha_k\geq 0$
holds pointwise, so $(\tilde{\bfeta}_k,\bfalpha_k)$ is a feasible
dual solution.
Lagrangian duality now gives us a bound on the suboptimality
of $\tilde{h}_k$ in terms of the duality gap:
$$
\calC(\tilde{h}_k) - \calC(\bff^*) \leq 
\calC(\tilde{h}_k) - \Phi(a\tilde{\bfeta}_k,\bfalpha_k)
\leq \calC(\tilde{\bfh}_k) - L(\tilde{\bfh}_k,\tilde{\bfeta}_k,\bfalpha_k). 
$$
By definition we have
\begin{align*}
    L(\tilde{\bfh}_k,\tilde{\bfeta}_k,\bfalpha_k) & = 
    \calC(\tilde{\bfh}_k) + \sum_i\tilde{\eta}^k_i g_i(\tilde{\bfh}_k)
    - \sum_j \alpha^k_j \tilde{h}^k_j \\
    & = \calC(\tilde{\bfh}_k)- \sum_j \alpha^k_j \tilde{h}^k_j,
\end{align*}
hence
$$
\calC(\tilde{\bfh}_k) - \calC(\bff^*) \leq \sum_j \alpha^k_j \tilde{h}^k_j = \sum_j D_j(\tilde{\bfh}_k,\tilde{\bfeta}_k) \tilde{h}^k_j.
$$
But we have already shown each of the terms $D_j(\tilde{\bfh}_k,\tilde{\bfeta}_k) \tilde{h}^k_j$ converges to $0$,
hence the entire sum converges to $0$, hence $\calC(\tilde{\bfh}_k)$
converges to $\calC(\bff^*)$, concluding the proof.
\end{proof}

\Xomit{
.

.

.

Let $\calR$ be a finite set of routes, let $\calL$ be a finite set of locations, and
let $\Omega$ be a finite collection of scenarios.  Suppose each route $r\in\calR$ has a unique
origin location $\ell^-(r)\in\calL$.  

We consider an optimization problem with decision variables $\bff=(f_r:r\in\calR)$ indexed by the routes $\calR$.
Let $S_\ell$ be the available supply at location $\ell$

Consider the following generic stochastic programming formulation.  
Let $\calR$ be a finite index set over which our decision variable will be defined
(i.e. a collection of routes), let $\calL$ be a partition of our decision variables
such that each index $r\in\calR$ belongs to a unique partition $l^-(r)\in\calL$.
Let $\bff=(f_r:r\in\calR)$ be our decision vector, and let $\bfS=(S_l : l\in\calL)$
be a vector which parameterizes our constraints on $\bff$, namely we optimize over
nonnegative $\bff$ which satisfy the following equality constraint:
\begin{equation}
    \label{eq:constraint}
S_l = \sum_{r\in\calR : l^-(r) = l} f_r.
\end{equation}
Let $\Omega$ be finite collection of scenarios $\omega\in\Omega$ and let $\bbP$ be a 
distribution over $\Omega$.  For each scenario $\omega\in\Omega$ let 
$\calW_{\omega}(\bff)$ be a differentiable reward function, and for each $r\in\calR$
let $U_r(f)$ be a reward function.  Consider the following optimization problem:

$$
\calW(\bfS) = \sup_{\bff} \left(\sum_{r\in\calR} U_r(f_r) + \bbE\left[\calW_{\omega}(\bff)\right] : \bff\in\bbR_+^\calR, \ \bff \mbox{ satisfies 
(\ref{eq:constraint}) wrt }\bfS\right).
$$

The optimality conditions for this problem assert the existence of dual
variables $\eta^*_l$ for each $l\in\calL$ such that the following is satisfied
for each $r\in\calR$:
$$
\eta^*_{l^-(r)} \geq \frac{d}{df_f}U_r(f^*_r) + \bbE\left[\frac{\partial}{\partial f_r} \calW_{\omega}(\bff^*)\right],
$$
and complementary slackness states the inequality is tight for every $r$ with $f_r^*>0$.
Also, we can show that each dual variable is equal to the partial derivative of the
optimal value with respect to the constraint vector:
$$
\eta^*_l = \frac{\partial}{\partial S_l}\calW(\bfS).
$$

The following Lemma is a generic statement about random approximately optimal solutions to the above stochastic programming formulation, from which Theorem \ref{thm:general_eqlbm} follows as a consequence.
\begin{lemma}
For each $k=1,2,\dots$ let $\bfh^k = (h^k_r : r\in\calR)$ be a random vector indexed by $\calR$. Suppose the following conditions are satisfied:
\begin{itemize}
    \item With probability 1, $\bfh^k$ violates the constraints (\ref{eq:constraint}) 
    by an additive factor of at most $\epsilon_k$, for some sequence $\epsilon_k\to 0$.
    \item For every location $l\in\calL$ there exists a number $V(l)$ such that
    the random variable 
    $$
    h_r^k\left|V(l^-(r)) - \frac{d}{dh_r} U(h_r^k) - 
    \bbE\left[\frac{\partial}{\partial h_r}\calW_{\omega}(\bfh^k)\right]\right|
    $$
    converges to $0$ in probability as $k\to\infty$, for every $r\in\calR$.
    \mccomment{Here is a cleaner way to state the above condition, if we assume
    a unique solution:
    \item There exists a subset $\calZ\subseteq\calR$ such that, for every $r\in\calZ$,
    $h^k_r$ converges to $0$ in probability.
    \item There exists a number $V(l)$ associated with each $l\in\calL$ such that
    for every $r\notin \calZ$, 
    $$
    \frac{d}{dh_r} U(h_r^k) - 
    \bbE\left[\frac{\partial}{\partial h_r}\calW_{\omega}(\bfh^k)\right]
    $$
    converges in probability to $V(l^-(r))$.
    }
    \Xomit{
    \mccomment{I think these conditions are only general if we assume there is a unique
    solution to the fluid optimization problem --- 
    if there is no unique solution, then it is possible to have 
    driver strategies that are equilibria but the sequence of $\bfh^k$ do not converge
    to anything (e.g. the subsequence on even $k$ and subsequence on odd $k$ could
    converge to different optimal solutions).  The assumptions I've written above
    wouldn't apply to such equilibria.  But if we assume a unique optimum then these
    assumptions are broad enough.  If we don't want to assume unique optimum then
    the following assumption would probably owrk instead:
     $$
    h_r^k\left|V(l^-(r)) - \frac{d}{dh_r} U(h_r^k) - 
    \bbE\left[\frac{\partial}{\partial h_r}\calW_{\omega}(\bfh^k)\right]\right|
    $$
    converges to $0$ in probability.
    }}
\end{itemize}
Suppose $\calW(\bfS)$ is differentiable in $\bfS$, and each $\calW_{\omega}(\bff)$
is differentiable in $\bff$. satisfy \mccomment{insert necessary smoothness conditions}.

Then the values $V(l)$ are equal to the optimal dual variables $\eta^*_l$, and the
utility under $\bfh^k$, i.e.
$$
\sum_{r\in\calR} U_r(h^k_r) + \bbE\left[\calW_{\omega}(\bfh^k)\right]
$$
converges in probability to the optimal utility $\calW(\bfS)$.
\end{lemma}

\begin{proof}
For each $k$ let $\tilde{\bfh}^k$ be the projection of $\bfh^k$ onto the set of
solutions which satisfy the constraints (\ref{eq:constraint}) exactly.  From our assumption
that $\bfh^k$ violates the constraints by a vanishing additive error $\epsilon_k$, and from
the continuity of the objective function
$$
\calU(\bff) = \sum_{r\in\calR} U_r(f_r) + \bbE\left[\calW_{\omega}(\bff)\right],
$$
we have that the difference in the utility under $\bfh^k$ and $\tilde{\bfh}^k$ converges to $0$:
$$
\lim_{k\to\infty}\calU(\bfh^k) - \calU(\tilde{\bfh}^k) = 0.
$$
\end{proof}
}


==> strategies_and_equilibria.tex <==
\subsection{Equilibrium Strategies in the Stochastic Fluid Model}
\input{fluid_strategy_profile_assns.tex}


\subsection{Strategy Profiles in the Two-Level Model}

To define strategy profiles let us start by describing the strategic decisions facing drivers in a single time period.
Fix a time period $t$ and scenario $\omega_t$.  After new drivers join, let $\calM_t$ be an index set over all active 
drivers in the network, and let $\ell_i$ be the 
location of each driver $i\in\calM_t$.

Recall we use the notation $(\ell,d,0)$ to denote a relocation trip from location $\ell$ to $d$, and $(\ell,d,1)$ denotes a dispatch trip
from $\ell$ to $d$.
Let $d_i$ be the destination location of the dispatch trip that driver $i$ is allocated.
The matching process is mediated by the platform and depends on stochastic demand realizations.
If driver $i$ is not allocated a dispatch
we write $d_i=\emptyset$.

The set of actions available to each driver depends on the driver's location as well as the destination of the dispatched they are matched to,
if any exists. A driver located at $\ell$ who receives a dispatch towards location $d$ has the opportunity to serve the dispatch trip 
specified by $(\ell,d,1)$.  In addition, they also have the option to take a relocation trip towards any possible location $d'$, where
the relocation trip is specified by $(\ell,d',0)$.
The set of actions available to a driver located at $\ell$ who receives a dispatch towards location $d$ can therefore be written
as the following set:
\begin{equation}
    \calA(\ell,d) = \begin{cases}
        \left\{(\ell,d',0) : d'\in\calL\right\} \cup \left\{(\ell,d,1)\right\} & \mbox{if }d \in\calL,\\
        \left\{(\ell,d',0) : d'\in\calL\right\}  & \mbox{if }d =\emptyset.
    \end{cases}
\end{equation}
Let
\begin{equation}
    \calA_i = \calA(\ell_i,d_i)
\end{equation}
be the set of actions available to each driver $i\in\calM_t$.

Before they make a decision about where to drive, each driver gets to observe their add-passenger disutility,
an idiosyncratic quantity that governs the additional cost the driver will incur for adding a passenger to their car,
i.e. for serving a dispatch trip, in the current time period.  Let $X_i$ denote the add-passenger disutility incurred by each driver $i$.

Driver decisions about whether or not to accept a dispatch depend on their realized add-passenger disutility.  A driver with high add-passenger disutility
might choose to reject a dispatch trip, whereas another driver with lower add-passenger disutility who is allocated the same dispatch would choose
to accept the dispatch.

We assume without loss of generality that decisions about whether to accept or reject a dispatch are monotone in the add-passenger disutility: if a driver
accepts a dispatch at a particular disutility value $X_i$, then they would have also accepted the dispatch for all smaller values of $X_i$.
Therefore, each driver's strategy about whether to accept or reject a dispatch can be specified by a disutility threshold they associate
with each potential dispatch destination.

Therefore, driver strategies for the one-shot game we associate with each time period can be specified by the following components:
1) A disutility acceptance threshold associated with each destination, on which the drivers accept/reject decisions are based,
2) A choice of location to drive to if the driver does not serve a dispatch trip.

We encode the strategy used by each driver $i$ with a tuple $(\bfx_i,\bfr_i)$, where $\bfx_i=(x^i_d : d\in\calL)$
is a vector of disutility acceptance thresholds, and $\bfr_i\in\Delta(\calL)$
is a distribution over locations, that driver $i$ uses to select a relocation trip if they don't serve a dispatch trip.
Let us summarize the steps that each driver $i$ uses to obtain their action $a_i\in\calA_i$, given the strategy $(\bfx_i,\bfr_i)$:
\begin{enumerate}
    \item Observe the add-passenger disutility $X_i\geq 0$ and the dispatch destination $d_i$.  If $d_i=\emptyset$ is the empty location,
        i.e. if the matching process does not allocate a dispatch to driver $i$, go to step \ref{item:relocation_choice}.
    \item Compare add-passenger disutility to the acceptance threshold for destination $d_i$.  If add-passenger disutility is smaller than
        the threshold, i.e. if $X_i \leq x^i_{d_i}$, then accept the dispatch.  In this case, the action that driver $i$ takes is specified by
        $a_i=(\ell_i,d_i,1)$.  If add-passenger disutility is larger than the threshold, go to step \ref{item:relocation_choice}.
    \item \label{item:relocation_choice}  Sample a destination $d$ from the distribution $\bfr_i$, independently from all other sources of randomness.
        The action that driver $i$ takes is specified by $a_i=(\ell_i,d,0)$.
\end{enumerate}

We now define what we mean by a strategy profile for the entire multiperiod stochastic game played by the drivers.  Let $\calM$ be an index
set of all drivers who could potentially join the marketplace.  
We define s strategy $\pi_i$ for each driver $i\in\calM$ as a sequence of functions $(\pi_i^1,\pi_i^2,\dots,\pi_i^T)$ where each element $\pi_i^t$
is referred to as the time $t$ strategy and it
selects the acceptance threshold and relocation distribution that driver $i$ uses for the $t$th time period.
(If a driver $i$ hasn't entered the market by time period $t$, then we assume the function $\pi_i^t$ has no bearing on that driver or any
of the market dynamics).

In general, the domain of each function $\pi_i^t$ can depend on the history of observed market states up to the beginning of time $t$.
For simplicity we assume that all drivers use Markovian strategies which only depend on the state at
the beginning of the time period. This assumption is without loss of generality in the context of exact equilibria because we assume that
drivers are expected utility maximizers.   In the current context where we consider approximate equilibria this assumption is almost without loss
of generality. \mccomment{This description about Markovian strategies being WLOG can be clarified / improved.}
The state at the beginning of the time period is specified by a scenario $\omega_t\in\Omega_t$
and a supply-location vector $\bfS_t$. Let $\calS_t$ be the set of all possible time $t$ states,
and let $\calX=\bbR_{\geq 0}^\calL$ be the space of 
feasible disutility-threshold vectors, so that each time $t$ strategy can be specified as function $\pi_i^t:\calS_t\to\calX\times\Delta(\calL)$.

A strategy profile $\Pi=(\pi_i : i\in\calM)$ is a specification of the strategy used by each potential driver over the entire marketplace dynamics.


\subsection{Matching Process in the Two-Level Model}
\input{matching_process/matching_process_description.tex}

%\subsection*{Old Matching Process}
%\input{approx_eqlbm/matching_process.tex}

\subsection{Approximate Equilibria in the Two-Level Model}

Our model is that drivers strategically select their strategies before the marketplace dynamics begin, and then individual drivers
collect utility based on the collective strategy profile the drivers have selected as well as the stochastic market dynamics.
We model strategic driver behaviour by assuming that drivers select strategies which result in an approximate equilibrium strategy profile $\Pi$
In this subsection we will define what it means for a strategy profile $\Pi$ to be an approximate equilibrium.

Fix a strategy profile $\Pi$ and assume that prices and matches are determined using the SSP mechanism.  Once a strategy profile is specified
then the market dynamics become a fully specified stochastic process.
Let $(a_i^t:t\in[T])$ be the sequence of actions taken by each driver $i\in\calM$.  Set $a_i^t=\emptyset$ for any driver $i$ who hasn't entered
the market by time period $t$; otherwise $a_i^t$ is selected based on the output of driver $i$'s strategy $\pi_i^t$ for time period $t$.

Let $R_i^t$ be the reward collected by driver $i$ in time period $t$.  $R_i^t$ is determined from the action $a_i^t$ based on the
following relationship:
\begin{equation}
    R_i^t=\begin{cases}
    P_{(\ell,d)}^t - X_i^t - c_{(\ell,d)} & \mbox{if }a_i^t = (\ell,d,1),\\
        -c_{(\ell,d)} & \mbox{if }a_i^t = (\ell,d,0),\\
        0 & \mbox{if }a_i^t = \emptyset,
    \end{cases}
\end{equation}
where $P_{(\ell,d)}^t$ is the price set by the SSP mechanism for a dispatch from $\ell$ to $d$ in time period $t$, and $X_i^t$
is driver $i$'s add-passenger disutility from time period $t$.

The utility-to-go for each driver at each time period is the expected sum of rewards they collect over all future
time periods, conditioned on the market state at the beginning of the time period.
We let $U_i^t(\Pi)$ denote driver $i$'s utility-to-go in time period $t$.  Note $U_i^t(\Pi)$
depends on the market state $(\omega_t,\bfS_t)$, but we omit this dependence in the notation for simplicity.
The utility-to-go is formally defined as the expected value of the following sum:
\begin{equation}
    U_i^t(\Pi) = \bbE^\Pi\left[\sum_{\tau=t}^TR_i^\tau \mid (\omega_t,\bfS_t)\right],
\end{equation}
where $\bbE^\Pi\left[\cdot\right]$ indicates that the expectation is taken with respect to the stochastic process that arises
from fixing the strategy profile $\Pi$.

It will also be useful to think about a driver's utility-to-go conditional on the destination towards which they are dispatched.
Recall $d_i$ is the (random) destination towards which driver $i$ is dispatched, with $d_i=\emptyset$ meaning that driver $i$
is not allocated a dispatch.  Define $U_i^t(d, X,\Pi)$ to mean driver $i$'s utility-to-go conditioned on the event that $d_i=d$ and $X_i=X$:
\begin{equation}
    U_i^t(d,X,\Pi) = \bbE^\Pi\left[\sum_{\tau=t}^TR_i^\tau \mid (\omega_t,\bfS_t), d_i=d, X_i=X\right].
\end{equation}


Informally, a strategy profile $\Pi$ is an approximate equilibrium if (almost) every driver has small incentive to deviate, regardless
of the destination they are dispatched twoards (if any). We use the 
notation $\Pi-\pi_i+\pi_i'$ to represent that driver $i$ deviates from a strategy $\pi_i$ to an alternate strategy $\pi_i'$.
The incentive-to-deviate for a driver, given a particular time period and market state, is defined as the maximum utility 
gain the driver can achieve by switching to an alternate strategy. 
Recall we use the set $\calM_t$ to index the active drivers in the marketplace.
We will use the notation $\calM_t(\epsilon)$ to mean the set of active drivers whose conditional incentive-to-deviate is at most $\epsilon$:
\begin{equation}
    \label{eq:delta_deviation_incentive}
    \calM_t(\epsilon) = \left\{i\in\calM_t : \sup_{d\in\calL}\sup_{X\in[0,C]}\sup_{\pi_i'} U_i^t(d,X;\Pi-\pi_i+\pi_i') - U_i^t(d,X;\Pi) \leq \epsilon\right\}.
\end{equation}
The exact meaning of $\calM_t(\delta)$ implicitly depends on the market state $(\omega_t,\bfS_t)$, but we omit this dependence in the notation
for clarity.
Our formal definition for $\Pi$ to be a high-probability approximate equilibrium is stated below.

\begin{definition} \label{def:approx_eqlbm} 
Let $\Pi=(\pi_i : i\in\calM)$ be a strategy-profile for the two-level model, let $p_1,\dots,p_T$ be a sequence of probability terms,
and let $\epsilon_1,\dots,\epsilon_T$ be a sequence of error terms.  We define $\Pi$ to be a $(p_t,\epsilon_t)$-approximate equilibrium
at time period $t$ if the following conditions hold:
\begin{enumerate}
    \item There is a subset of the state space $\calS_t$ such that, under $\Pi$, the probability the time $t$ market state lies in $\calS_t$
            is at least $p_t$:
\begin{equation}
\bbP^\Pi\left((\omega_t,\bfS_t)\in\calS_t\right)\geq p_t.
\end{equation}
    \item In the event that the time $t$ market state does lie in the set $\calS_t$, the incentive-to-deviate from $\Pi$ is at most $\epsilon_t$
for every driver in the marketplace:
\begin{equation}
(\omega_t,\bfS_t)\in\calS_t \implies \calM_t(\epsilon_t) = \calM_t.
\end{equation}
\end{enumerate}
We define $\Pi$ to be a $(p_{1:T},\epsilon_{1:T})$-approximate equilibrium if it is a $(p_t,\epsilon_t)$-approximate equilibrium for each time period $t$.
\end{definition}





==> two_level_robustness_proof.tex <==
In this section we summarize the key steps we take to prove Theorem \ref{thm:robust_eqlbm_two_level}.
We prove Theorem \ref{thm:robust_eqlbm_two_level} by backwards induction on the time period.
Fix a time period $t\in [T]$.  For each $k\geq 1$ assume there exists an error term $\epsilon_{t+1}(k)$, 
converging to $0$ as $k\to\infty$, such that the the following properties hold:
\begin{itemize}
\item For every market state $(\omega_{t+1},\bfS_{t+1})\in\calS_{t+1}(\gamma)$, and any approximate equilibrium $\Pi\in\calP^k$,
$$
\Phi_{\omega_{t+1}}(\bfS_{t+1}) - W_{\omega_{t+1}}(\bfS_{t+1};\Pi,k) \leq \epsilon_{t+1}(k).
$$
\item For any approximate equilibrium $\Pi\in\calP^k$, at time $t+1$, every driver has expected utility-to-go that is close to the partial derivative of the fluid optimization function.
        Specifically, for any market state $(\omega_{t+1},\bfS_{t+1})$ and any driver $i\in\calM_{t+1}$
        whose location is $\ell_i^{t+1}=\ell$,
        the following bound holds:
        $$
        \left| \bbE^{\Pi}[U_i^{t+1} \mid \ell_i^{t+1}=\ell, (\omega_{t+1},\bfS_{t+1})] - \frac{\partial}{\partial S_\ell}\Phi_{\omega_{t+1}}(\bfS_{t+1})\right| \leq \epsilon_{t+1}(k).
        $$
\end{itemize}


Our proof technique is to convert the stochastic actions taken by a strategy profile $\Pi$ to an approximate equilibrium fluid strategy.
We proceed via a series of lemmas.  The first Lemma shows that in an approximate equilibrium, drivers at the same location use approximately the same disutility
acceptance thresholds.
We provide the proof of Lemma \ref{lem:common_threshold} in Appendix \ref{appdx:common_threshold_proof_}

\begin{lemma}
    \label{lem:common_threshold}
    There exists an error function $\delta(k)\geq 0$, converging to $0$ as $k\to\infty$, such that the following is true:
    For any $k\geq 1$, any approximate equilibrium $\Pi\in\calP^k$, and any market state $(\omega_t,\bfS_t)\in\calS_t(\gamma)$,
    let $\bfx_i=(x_i^d : d\in\calL)$ be the disutility acceptance threshold used by each active driver $i\in\calM_t$.
    Then for each location $\ell$ there exists a disutility threshold vector 
    $\bfx_\ell = (x_{(\ell,d)} : d\in\calL)$ 
    such that the disutility threshold vector used by every driver positioned at $\ell$ is at most $\delta(k)$ away from 
    $\bfx_\ell$, i.e.
    \begin{equation}
        \max_{d\in\calL}|x_i^d - x_{(\ell,d)}| \leq \delta(k) , \ \ \ \ \forall i\in\calM_{t,\ell}.
    \end{equation}
\end{lemma}

Our next Lemma shows that the stochastic actions taken under equilibrium strategy profile $\Pi$ concentrate
towards the fluid actions which arise under the common disutility threshold established by Lemma \ref{lem:common_threshold}.

For any $k\geq 1$, $\Pi\in\calP^k$ and $(\omega_t,\bfS_t)\in\calS_t(\gamma)$, 
let $(\bff,\bfg)$ encode the stochastic trip volumes that occur on each route. 
Recall that $a_i^t$ is a random variable which corresponds to the action that each active driver $i\in\calM_t$ takes
in time period $t$.
Define $g_{(\ell,d)}$ by 
\begin{equation}
    \label{eq:two_level_g}
     g_{(\ell,d)} = \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,1)\right\},\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
and $f_{(\ell,d)}$ by
\begin{equation}
    \label{eq:two_level_f}
    f_{(\ell,d)} = g_{(\ell,d)} + \frac{1}{k} \sum_{i\in\calM_t} \bfone\left\{a_i^t = (\ell,d,0)\right\}.\ \ \ \ \forall (\ell,d)\in\calL^2
\end{equation}
Note that $(\bff,\bfg)$
are random variables that depend on stochastic dispatch demand, stochastic add-passenger disutilities, as well as the randomness inherent
to the matching process.  

We want to compare $(\bff,\bfg)$ to trips that arise in a fluid version of the strategy $\Pi$.
Define a fluid strategy profile that produces a disutility threshold vector $\bfx$, where $\bfx$ is the common
disutility threshold vector whose existence is established by Lemma \ref{lem:common_threshold}, and define the relocation
distribution $\bfe$ using the relocation destinations selected by all drivers in the population:
For each destination $d$ define
$$e_{(\ell,d)} = 1/|\calM_{t,\ell}| \sum_{i\in\calM_{t,\ell}}\bfone\{r_i = d\}$$
where $r_i$ is the relocation destination selected by each driver $i$.
Let $\bar{\bff},\bar{\bfg}$ be the fluid trip volumes that occur under the market state $(\omega_t,\bfS_t)$ and
the fluid strategy $(\bfx,\bfe)$.

Recall that $\bfS_{\omega_{t+1}}(\bff)$ is the stochastic time $t+1$ supply location vector, given the
time $t$ trips $\bff$ and a time $t+1$ scenario $\omega_{t+1}$, and $\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})$
is the deterministic time $t+1$ supply location vector arising in the fluid model.  The following Lemma
states that $\bfS_{\omega_{t+1}}(\bff)$ is close to $\bar{\bfS}_{\omega_{t+1}}(\bar{\bff})$ with high probability
for large $k$. We provide the proof of Lemma \ref{lem:supply_vec_concentration} in Appendix \ref{appdx:supply_vec_concentration_proof}.

\begin{lemma}
    \label{lem:supply_vec_concentration}
    There exists an error function $\kappa(k)\geq 0$, and another function $q(k)\geq 0$, both 
    converging to $0$ as $k\to\infty$, such that the following is true:
    For any $k\geq 1$, any approximate equilibrium $\Pi\in\calP^k$, and any market state $(\omega_t,\bfS_t)\in\calS_t(\gamma)$,
    let $(\bff,\bfg)$ be the stochastic trip volumes and $(\bar{\bff},\bar{\bfg})$ be the fluid trip volumes
    as defined above.
    Then following inequalities holds:
    \begin{align*}
        \bbP\left(\|\bfg - \bar{\bfg}\|_1 \geq \kappa(k)\right) &\leq q(k),\\
        \bbP\left(\|\bff - \bar{\bff}\|_1 \geq \kappa(k)\right) &\leq q(k),\\
        \bbP\left(\|\bfS_{\omega_{t+1}}(\bff) - \bar{\bfS}_{\omega_{t+1}}(\bar{\bff})\|_1 \geq \kappa(k)\right) &\leq q(k).
    \end{align*}
\end{lemma}

Our final lemma shows that $(\bar{\bff},\bar{\bfg},\bfx)$ corresponds to an approximate equilibrium in the fluid model.
We defer the proof of Lemma \ref{lem:fluid_eqlbm_from_two_level_eqlbm} to Appendix \ref{appdx:fluid_eqlbm_from_two_level_eqlbm}.

\begin{lemma}
    \label{lem:fluid_eqlbm_from_two_level_eqlbm}
    There exists an error function $\iota(k)\geq 0$, converging to $0$ as $k\to\infty$, such that the following is true:
    For any $k\geq 1$, any approximate equilibrium $\Pi\in\calP^k$, and any market state $(\omega_t,\bfS_t)\in\calS_t(\gamma)$,
    let  $(\bar{\bff},\bar{\bfg})$ be the fluid trip volumes associated with $\Pi$ under the market state $(\omega_t,\bfS_t)$,
    and let $\bfx$ be the common disutility threshold that drivers use under $\Pi$, established in Lemma \ref{lem:common_threshold}.
    Then $(\bar{\bff},\bar{\bfg},\bfx)$ corresponds to an $\iota(k)$-approximate equilibrium for the fluid model.
\end{lemma}

Lemma \ref{lem:supply_vec_concentration} and \ref{lem:fluid_eqlbm_from_two_level_eqlbm} are sufficient to
conclude the proof of Theorem \ref{thm:robust_eqlbm_two_level}.

From the second part of Theorem \ref{thm:robust_eqlbm_fluid} we know that there is an error function $\epsilon(k)\geq 0$ which
converges to $0$ as $k\to\infty$, such that the welfare achieved by $(\bar{\bff},\bar{\bfg},\bfx)$ in the fluid model
is at most $\epsilon(k)$ off from the optimal welfare.

Next, observe a consequence of Lemma \ref{lem:supply_vec_concentration} is the expected welfare under $\Pi$ converges
to the welfare of the associated fluid strategy, and the expected utility of drivers at $\ell$ under $\Pi$
converges to the expected utility of drivers at $\ell$ in the associated fluid strategy.  That is, there exists
an error function $\theta(k)\geq 0$ converging to $0$ as $k\to\infty$ such that
$$
|W_{\omega_t}(\bfS_t;\Pi,k) - \calW_{\omega_t}(\bar{\bff},\bar{\bfg},\bfx)| \leq \theta(k),
$$
and
$$
\left| \bbE^{\Pi}[U_i^{t} \mid \ell_i^{t}=\ell, (\omega_{t},\bfS_{t})] - \frac{\partial}{\partial S_\ell}\Phi_{\omega_{t}}(\bfS_{t})\right| \leq \theta(k)
$$
holds for every $k\geq 1$, $\Pi\in\calP^k$, $(\omega_t,\bfS_t)\in\calS_t(\gamma)$.

The above inequality establishes the second part of our backwards induction assumption.  
The first part our backwards induction assumption also follows:
$$
W_{\omega_t}(\bfS_t;\Pi,k) \geq \calW_{\omega_t}(\bar{\bff},\bar{\bfg},\bfx) - \theta(k) \geq \Phi_{\omega_t}(\bfS_t) - \epsilon(k) - \theta(k).
$$





==> vcg_connection.tex <==
\bigskip

\mccomment{04/27: need to revise the following to use recent notation changes}
\begin{remark} The pricing used in Theorem \ref{thm:fluid_ic} are effectively VCG prices as explained below. It is interesting to see that VCG-like prices work OK in a stochastic model of ride-sharing. 
\end{remark}
\begin{proof} To see the connection recall that prices offered in the (discrete) VCG mechanism for a driver at an LT-scenario $(l,\omega_t)$ would be the marginal value of a driver at the location for the overall system. The fluid limit analog of this is the marginal value of a driver positioned at location $l$ at time $t$ in the scenario $\omega_t$ , which is the following limit:
$$
\lim_{\epsilon\to 0^+}\frac{\calW_{\omega_t}(\bfS_t) - \calW_{\omega_t}(\bfS_t - \bfone_{(l,\omega_t)}\epsilon)}{\epsilon},
$$
\etcomment{Massey: can you fix the notation!} \mccomment{went through and made a few small changes}
The dual variable $\eta^*_{(l,\omega_t)}(\bfS_t)$ is associated with the flow conservation constraint at time $t$ in scenario $w_t$ at location $l$. Using the definition of a dual, decreasing the driver volume at $(l, \omega_t)$ by $\epsilon$ must decrease the overall objective by at least $\epsilon \eta^*_{(l,\omega_t)}(\bfS_t)$, as the dual solution has this value with the decreased supplies:
$$
\calW_{\omega_t}(\bfS_t - \bfone_{(l,\omega_t)}\epsilon)\le \calW_{\omega_t}(\bfS_t)-\epsilon \eta^*_{(l,\omega_t)}(\bfS_t)
$$ 
This shows that the limit is at least $\eta^*_{(l,\omega_t)}$. 

Now consider the optimal flow $\bff$ realizing the value $\calW_{\omega_t}(\bfS_t)$. To show the other direction, we need to establish a flow for supply location vector $\bfS_t - \bfone_{(l,\omega_t)}$ with value $\calW_{\omega_t}(\bfS_t)-\epsilon \eta^*_{(l,\omega_t)}(\bfS_t)$. We establish this by backwards induction on $t$. For the last step $t=T$, there is nothing to prove. When $t<T$, consider the equation (\ref{eq:utility_recursion}) for the utility to go at the LT-scenario  $(l,\omega_t)$ for an arc $r$ leaving this LT-scenario that is used by some drivers, and recall that the optimal dual variable $\eta^*_{(l,\omega_t)}$ associated
with an LT-scenario $(l,\omega_t)$ is equal to the expected utility-to-go of a driver positioned at LT scenario $(l,\omega_t)$. \etcomment{this fact was stated after Theorem 1, but is only proven in the Appendix. Given how late things are, I would tempted to accept this for now, as this whole part is just a remark anyhow.}
By decreasing the flow amount by $\epsilon$ on this arc, we create flow conservation at $(l,\omega_t)$ with the supply location vector $\bfS_t - \bfone_{(l,\omega_t)}$, but have $\epsilon$ less flow arrive at $l^+(r)$. By the induction hypotheses $\eta^*_{(l^+(r),\omega_{t+1})}(\bfS_{t+1})$ is the marginal value of a diver at $(l^+(r),\omega_{t+1})$ for all possible scenarios $\omega_{t+1}$ that can follow $\omega_t$. Adding the lost utility on arc $r$ results in a flow for  supply location vector $\bfS_t - \bfone_{(l,\omega_t)}$ of the value of $\calW_{\omega_t}(\bfS_t)-\epsilon \eta^*_{(l,\omega_t)}(\bfS_t)$, as claimed.  
\end{proof}
\Xomit{
\bigskip

OLD TEXT STARTS HERE!!!!!!!!!!!!!!!!

The proof of Theorem \ref{thm:fluid_ic} and Theorem \ref{thm:stochastic_ic} both rely
on establishing a connection between the expected utility-to-go under the SSP mechanism
for a driver at a particular location with the optimal dual value associated with that
location.

In the stochastic fluid model at time $t$ under scenario $\omega_t$ and for a supply-location
vector $\bfS_t$ this equality can be written as $\calV_{(l,\omega_t)}(\bfS_t) = \eta^*_{(l,\omega_t)}(\bfS_t)$.

Now, let's consider what is the marginal value of a driver located at an LT-scenario $(l,\omega_t)$.
Using the notation $\calW_{\omega_t}(\bfS_t)$ to denote the optimal value of the stochastic maximum flow
problem (\ref{eq:dynamic_optimization}) formulated with respect to $t$, $\omega_t$ and $\bfS_t$, the 
marginal value of a driver positioned at $(l,\omega_t)$ is the following limit:
$$
\lim_{\epsilon\to 0^+}\frac{\calW_{\omega_t}(\bfS_t) - \calW_{\omega_t}(\bfS_t - \bfone_{(l,\omega_t)}\epsilon)}{\epsilon},
$$
where $\bfone_{(l,\omega_t)}$ is an indicator vector with a $1$ in the $(l,\omega_t)$ component and $0$ elsewhere.

Next, Lemma \ref{lem:stability} establishes that the function mapping a supply-location vector $\bfS_t$ to
the optimal stochastic flow $\bff^*(\bfS_t)$ with respect to that supply-location vector is continuous.
 
\subsection{Contents of Note: VCG Lemma Improved}
Consider the stochastic flow optimization problem maximizing utility defined as ${\mathcal U}_{\omega_t}(m_{\ge t},N)$ 
for the fluid limit of the optimization problem starting with scenario $w_t$ at time $t$ and the $m_{\ge t}$ is the vector of driver supply at each location $s$ and times $\tau \ge t$, and $N$ is the vector of demand at each $(\tau,r)$, time and route pairs. 

We assume for simplicity of notation, and without loss of generality, that each ride is taking a single unit of time. This is no loss of generality as we didn't assume that the costs $c_r$ satisfy the triangle inequality, so we can add extra nodes subdividing each route into routes of length 1, and add $c_r$ for any route emanating from the newly added nodes (including exiting the market from these nodes) as extremely high (infinite) to make sure that the socially optimal action for drivers at these nodes is to continue the route. 

As established before ${\mathcal U}_{\omega_t}(m_{\ge t},N)$ is differentiable, where $m_{\ge t}$ is the expected drive in each scenario starting at time $t$ with $\omega_t$. First we compute the marginal value of additional drivers at time $t$ and location $s$ as
$$v_{\omega_t}(s,m_{\ge t})=\frac{\partial}{\partial m_{s_t}}{\mathcal U}_{\omega_t}(m_{\ge t},N)$$
This is the marginal value of additional driver at time time $t$ location $s$, and we want this to be the expected net value of all drivers at that location.


To accomplish this we set prices at a route $r$ from $s$ to $h(r)$ at time $t$, to satisfy the following equation. 
\begin{equation}\label{eq:cont-value}
    v_{\omega_t}(s,m)=p_{r_t}-c_r+\bbE[v_{\omega_{t+1}}(h(r),m_{\ge t+1})] 
\end{equation}

The following two facts will establish our claimed results about the incentive compatibility of our mechanism in the fluid limit. 
\begin{enumerate}
    \item the prices set by our stochastic optimization problem satisfy equation (\ref{eq:cont-value}).
    \item using these prices, following the advice from the stochastic optimization problem is incentive compatible, and a driver's expected value at time $t$ in location $s$ in scenario $\omega_t$ is $v_{\omega_t}(s)$.
\end{enumerate}
The claim (1) is proven in \etcomment{Section 7.1 of the old write-up}. The equation (\ref{eq:cont-value}) holds with equation on all routes that some drivers are recommended to follow. We can set a high enough price $p_{r_t}$ for route $r$ at time $t$ that no-one is recommended to follow to make the same equation also hold for these routes as well. 

Now we prove claim (2) by backwards induction on the time horizon. When $t=T$ (no more rides will be offered), there is nothing to prove: $v_{\omega_t}(s)=0$ for all $s$, and there is nothing else the drivers can do. 

Consider an earlier time step $t$, and assume the incentive compatibility is true for any time $t+1$ and any scenario $w_{t+1}$ and starting driver mass $m_{t+1}$. Assuming all drivers follow the given advice, the expected value for a driver recommended to follow route $r$ at time $t$ is
$$p_{r_t}-c_r+\bbE[v_{\omega_{t+1}}(h(r),m_{\ge t+1})]$$

Following an alternate route $r'$ (without passengers at this time) the driver gets

$$-c_{r'}+\bbE[v_{\omega_{t+1}}(h(r'),m_{\ge t+1})]$$

By (1) we know that route $r'$ also satisfies equation (\ref{eq:cont-value}) and that $p_{r'_t}\ge c_{r'}\ge 0$, so the value of taking route $r'$ is less. 

\paragraph{Alternate argument for incentive compatibility}
\etcomment{It seems that the next argument is not needed, i.e., it already follows from the dual variables and complementary slackness and all that. But that is what is giving me intuition.}

The derivative is the limit of changed value with a small change $\delta>0$ as $\delta \rightarrow 0$. So the value following the advice is (using the fact that the value at $h(r)$ is the marginal value for the last driver at that point): 

$$
p_{r_t}-c_r+\bbE[\frac{\partial}{\partial w_{h(r)_{t+1}}}{\mathcal{U}}_{w_{t+1}}(m_{t+1},N)]
=p_{r_t}-c_r+\lim_{\delta \rightarrow 0} \frac{{\mathcal{U}}_{w_{t+1}}(m_{t+1},N)-{\mathcal{U}}_{w_{t+1}}(m_{t+1}-\delta 1_{h(r)_{t+1}},N)}{\delta}
$$

Following an alternate route $r'$ with a $\delta\rightarrow 0$ mass of driver, they get value: 

$$=-c_{r'}+\lim_{\delta \rightarrow 0} \frac{{\mathcal{U}}_{w_{t+1}}(m_{t+1}+\delta( 1_{h(r')_t}-1_{h(r)_t}),N)-{\mathcal{U}}_{w_{t+1}}(m_{t+1}-\delta 1_{h(r)_{t+1}},N)}{\delta}
$$
Where the first utility term reflect that a $\delta$ mass of drivers choose to follow $r'$ instead of $r$. 

Consider the difference between these expressions with a fixed $\delta$, and to simplify the expression multiply the difference by $\delta$. Note that the last terms are exactly the same in both expressions. What we get is

$$
\delta(p_{r_t}-c_r+c_{r'})+
\bbE[{\mathcal{U}}_{\omega_{t+1}}(m_{\ge 0},N)-
{\mathcal{U}}_{\omega_{t+1}}(m_{\ge t+1}+\delta(1_{h(r')_{t+1}}-h(r)_{t+1}),N)]
$$
Note that $p_{r_t}$ is also used to moderate demand, so it is exactly the lowest value of a riders served along route $r$ at time $t$. This gives that the difference above is the change in expected value of the solution by taking $\delta$ amount of drivers from route $r$ and recommending them to follow route $r'$ with no passengers. Given that the recommended solution is socially optimal, this change in social value is necessarily non-negative.

}


==> welfare_robustness_appdx.tex <==
\subsection{Expected Welfare of a Strategy Profile in the Two Level Model}
\label{subsec:two_level_welfare_def}
Let $W_i^t$ denote the welfare generated in the action driver by $i$ at time $t$.  The welfare $W_i^t$
differs from the driver reward $R_i^t$ when driver $i$ fulfils a dispatch in time $t$; in this case, the rider collects utility
equal to the difference between their value for the trip and the trip price.  Let $V_i^t$ be the value held by the rider whose dispatch
driver $i$ fulfils in time $t$, if any such rider exists.  The welfare term $W_i^t$ is defined as follows:
\begin{equation}
    W_i^t=\begin{cases}
    R_i^t + (V_i^t - P_{(\ell,d)}^t) & \mbox{if }a_i^t=(\ell,d,1),\\
        R_i^t & \mbox{otherwise.}
    \end{cases}
\end{equation}

The total welfare generated by the marketplace is then the sum over welfare terms $W_i^t$ for all drivers $i$ and time periods $t$.
In the context of the two-level model, where the number of riders and drivers scales with the population-size parameter $k$, we
normalize the expected welfare by dividing by $k$, so that expected welfare terms are comparable across different population sizes.

Let $W_{\omega_t}(\bfS_t;\Pi)$ be the expected welfare-to-go given a strategy profile $\Pi$, a population size $k$, as a function
of the market state $(\omega_t,\bfS_t)$:
\begin{equation}
    W_{\omega_t}(\bfS_t;\Pi) = \frac{1}{k}\bbE^\Pi\left[\sum_{i\in\calM}\sum_{\tau=t}^T W_i^\tau \mid (\omega_t,\bfS_t)\right].
\end{equation}
Notice the expected welfare term $ \Phi_{\omega_t}(\bfS_t;\Pi) $ implicitly depends on the population size parameter $k$, but we
omit this dependence from the notation for convenience.

Recall that $\Phi_{\omega_t}(\bfS_t)$ denotes the optimal value of the state-dependent optimization problem given the state $(\omega_t,\bfS_t)$,
which corresponds to the optimal welfare achievable given the state $(\omega_t,\bfS_t)$ in the stochastic fluid model.
The following Lemma states that the optimal fluid welfare is always an upper bound on the expected welfare in the two-level model.
\begin{lemma}
    Let $\Pi$ be any strategy profile and consider any time $t$ with state $(\omega_t,\bfS_t)$.
    The optimal welfare from the state $(\omega_t,\bfS_t)$ in the fluid model is always larger than the expected welfare generated by $\Pi$ in the
    two-level model, i.e.
    \begin{equation}
        \label{eq:fluid_welfare_ub}
    \Phi_{\omega_t}(\bfS_t) \geq W_{\omega_t}(\bfS_t;\Pi)
    \end{equation}
    always holds.
\end{lemma}



